Sharp adaptive and pathwise stable similarity testing for scalar ergodic diffusions

Within the nonparametric diffusion model, we develop a multiple test to infer about similarity of an unknown drift $b$ to some reference drift $b_0$: At prescribed significance, we simultaneously identify those regions where violation from similiarity occurs, without a priori knowledge of their number, size and location. This test is shown to be minimax-optimal and adaptive. At the same time, the procedure is robust under small deviation from Brownian motion as the driving noise process. A detailed investigation for fractional driving noise, which is neither a semimartingale nor a Markov process, is provided for Hurst indices close to the Brownian motion case.

==> Sections/Composite_Hypothesis.tex <==
\section{Testing of composite hypotheses}


\subsection{One-sided alternative}

We fix, $A,\gamma,\sigma>0$, $C\geq 1$ and set 
\[\mathcal{H}_{\leq 0} := \{ f\in \Sigma(C,A,\gamma,\sigma)\mid f\leq 0\textrm{ on } [-A,A]\}. \]
We will assume under the alternative, that $b$ belongs to some Hölder class $\mathcal{H}(1,L)$, $L>0$ and of couse admits ergodic properties, i.e. $b\in\Sigma(1,L,0)$.We measure the distance to $\mathcal{H}_{\leq 0}$ by
\[ \Delta(b) := \inf_{b_0\in\mathcal{H}_{\leq 0}} \| 1_{[-A,A]}(b_0 - b)\rho_b^\frac13\|_\infty \]
and it is easily seen that for $b\notin\mathcal{H}_{\leq 0}$ we have
\[ \Delta(b) = \sup_{x\in [-A,A]} \left( b(x) \rho_b(x)^\frac13\right).\]

We set
\[ \mathcal{T} := (0,1]\times [-A+h, A-h] \]
and considert the test statistic
\[ T_b(X)  = \sup_{(y,h)\in\mathcal{T}} \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)\]
where
\[ \tilde{\Psi}_{y,h}^b(X) = \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} + \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
This is the same statistic as $\Psi_{y,h}(X)$ in section $3$ when we choose $b_0=0$ on the interval $[-A,A]$. To built our test, we want to identify a worst case within the set $\mathcal{H}_{\leq 0}$ in order to have a non-degenerate random variable that delivers the quantiles for our test. \\
In a first step we want to show that an asymptotically worst case within this set of hypothesis is $f=0$ which is the reasonable expectation as it is the hypothesis closest to the alternative of functions being larger than zero anywhere within $[-A,A]$.

Clearly, the second summand is always negative for $b\in\mathcal{H}_{\leq 0}$ and vanishes for $b=0$, where the latter is understood as restricted to $[-A,A]$. Outside of this interval the drift clearly needs to deviate from zero in order to ensure ergodic properties of the solution or put differently, to ensure $b\in\Sigma(C,A,\gamma,\sigma)$. In this latter case we know that the invariant density $\rho_0=c$ is constant on $[-A, A]$ and hence the weak limit of the test statistic is given by
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C( \|cK_{y,h}\|_{L^2}^2)\right),\]
where
\[ Z(y,h) = \frac{\int_{-A}^A K_{y,h}(z) dW_z}{\|K_{y,h}\|_{L^2}}.\]
But it is not directly clear that $b_0=0$ is the worst case from these considerations, as the first summand contains the process $X$ which depends on the choice of drift and it is not clear that this term is also stochastically dominated by the choice $b_0=0$. But nevertheless, the assertion turns out to be true asymptotically: for negative choices of $b_0$ the first term may be larger, but this is compensated by the second term which in turn is negative. This is spelt out in detail in the next result and its proof in Appendix D.

\begin{proposition}\label{worst_case_one-sided}
For each $b\in\mathcal{H}_{\leq 0}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_b(X) > r\right) \leq \Pr\left( S>r\right),\]
where
\[ S := \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left(\|K_{y,h}\|_{L^2}^2\right) + C\left( (1\vee (L^*\wedge (2h)^{-1})^{-1}\right)\right).\]
\end{proposition}

As an application of Theorem \ref{Multiscale_Lemma} is immediate for $S$, we know that the critical value
\[ \kappa_{\leq 0, \alpha} := \min \{ r\in\R:\ \Pr(S\leq r)\geq 1-\alpha\}\]
is well defined and we reject the null hypothesis $\mathcal{H}_{\leq 0}$ at level $\alpha$ if $T_b(X)> \kappa_{\leq 0, \alpha}$. This turns again turns out to be optimal with the best possible constant. Note that the optimal recovery kernel $K_\beta$ in the case of $\beta=1$ is given by the triangular kernel $K(x) = 1_{\{|x|\leq 1\}}(1-|x|)$ with $\|K\|_{L^2}^2 = \frac23$. In this case the optimal constant of section $3$ is given by $c_* = L^\frac13$.

\begin{thm}\label{theorem_one-sided}
Let $(\epsilon_T)_{T\geq 0}$ be given such that $\lim_{T\to\infty} \epsilon_T =0$ and $\lim_{T\to\infty} \epsilon_T\sqrt{\log T} =\infty$, let $T_b$ be given with the choice of the rectangular kernel $K$ and 
\[ \rho_T := \left( \frac{\log T}{T}\right)^\frac13.\]
\begin{enumerate}
\item[(a)] For any test $\phi_T$ with $\E_0[\phi_T]\leq \alpha$ we have
\[ \limsup_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,0): \Delta(b)\geq (1-\epsilon_T) L^\frac13 \delta_T}} \E_b [ \phi_T(X)] \leq \alpha.\]
\item[(b)] Our test satisfies
\[ \lim_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,0): \Delta(b)\geq (1+\epsilon_T) L^\frac13 \delta_T}} \Pr_b\left( T_b(X)\geq \kappa_{\leq 0, \alpha}\right) =1.\]
\end{enumerate}
\end{thm}





\subsection{$\delta$-environment}
Now we turn to test for a $\delta$-environment. Pick a drift function $b_0\in\Sigma(C,A,\gamma,\sigma)$ and $\delta>0$ and define 
\[ \mathcal{H}_\delta(b_0) := \left\{ b\in \Sigma(C,A,\gamma,\sigma)\mid \| 1_{[-A,A]} (b-b_0)\|_\infty \leq \delta\right\}.\]
As an alternative we again choose some Hölder class $\mathcal{1,L}$, $L>0$ with ergodic properties of the solution. The distances is given in this case for $b\notin\mathcal{H}_\delta(b_0)$ as
\[ \Delta(b) = \sup_{x\in [-A,A]} \left( (|b(x)-b_0(x)| - \delta) \rho_b(x)^\frac13\right).\]
With the definition of $\Psi_{y,h}(X)$ from section $3$ we define a test statistic
\[ T_\delta(X) := \sup_{(y,h)\in\mathcal{T}} \left(\left| \Psi_{y,h}(X)\right| - C(\sigma_{y,h}^2) - \Psi_\delta\right),\]
where
\[ \Psi_\delta := \frac{\frac{\delta}{\sqrt{T}} \int_0^T K_{y,h}(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
As a worst case we expect the function $b_0\pm\delta$: on the one hand because this choice eliminates the term $\Psi_\delta$, on the other hand intuitively, as it is the boundery case to the alternative and therefore a predestinated candidate. But as in the case of a one-sided alternative it is not exactly clear, as the distribution of $X$ depends on the drift. But we may again show that we are on the right track.

\begin{proposition}\label{worst_case_delta}
For each $b\in\mathcal{H}_{\delta}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_\delta(X) > r\right) \leq \Pr\left( S_1\vee S_2>r\right),\]
where
\begin{align*}
S_1 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0+\delta}(z)} dW_z}{\|K_{y,h}\sqrt{\rho_{b_0+\delta}}\|_{L^2}}\right| - C\left(\|K_{y,h}\sqrt{\rho_{b_0+\delta}}\|_{L^2}^2\right)\right),\\
S_2 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0-\delta}(z)} dW_z}{\|K_{y,h}\sqrt{\rho_{b_0-\delta}}\|_{L^2}}\right| - C\left(\|K_{y,h}\sqrt{\rho_{b_0-\delta}}\|_{L^2}^2\right)\right).
\end{align*} 
\end{proposition}

We may apply Theorem \ref{Multiscale_Lemma} to both $S_1$ and $S_2$ to get a well defined critical value
\[ \kappa_{\delta,\alpha} := \min\{ r\in\R:\ \Pr(S_1\vee S_2 \leq r) \geq 1-\alpha\}.\]
Then our test rejects the null hypothesis $\mathcal{H}_\delta$ at level $\alpha$ if $T_\delta(X) >\kappa_{\delta,\alpha}$.


\begin{thm}\label{theorem_delta}
Let $(\epsilon_T)_{T\geq 0}$ be given such that $\lim_{T\to\infty} \epsilon_T =0$ and $\lim_{T\to\infty} \epsilon_T\sqrt{\log T} =\infty$, let $T_\delta$ be given with the choice of the rectangular kernel $K$ and 
\[ \rho_T := \left( \frac{\log T}{T}\right)^\frac13.\]
\begin{enumerate}
\item[(a)] For any test $\phi_T$ with $\E_0[\phi_T]\leq \alpha$ we have
\[ \limsup_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,b_0\pm\delta): \Delta(b)\geq (1-\epsilon_T) L^\frac13 \delta_T}} \E_b [ \phi_T(X)] \leq \alpha.\]
\item[(b)] Our test $T_\delta$ satisfies
\[ \lim_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,b_0\pm\delta): \Delta(b)\geq (1+\epsilon_T) L^\frac13 \delta_T}} \Pr_b\left( T_\delta(X)\geq \kappa_{\delta, \alpha}\right) =1.\]
\end{enumerate}
\end{thm}




==> Sections/Implementation.tex <==
\section{Computability and numerical example}\label{Sec_Implementation}
In this section we first discuss how the test statistic $T_T^\eta(X)$ given in \eqref{eq: T_eta} can be computed for a given observation $X=(X_t)_{t\in [0,T]}$. In a second part, an extended simulation study is given.


\subsection{Computability of the test statistic $T_T^\eta$}
When implementing the test statistic $T_T^\eta(X)$ for an observed path $X$ one has to evaluate several Lebesgue integrals and the stochastic It\^{o} integral $\int_0^T K_{y,h}(X_s) dX_s$. Given a continuously differentiable kernel $K$ we have seen in Section \ref{Sec_Stability} that by It\^{o}'s formula
\[ \int_0^T K_{y,h}(X_s) dX_s = \int_{X_0}^{X_T} K_{y,h}(z) dz - \frac{\sigma^2}{2} \int_0^T (K_{y,h})'(X_s) ds \]
and based on this we established a version $\tilde\Psi_{T,y,h}^{b_0}(X)$ of $\Psi_{T,y,h}^{b_0}(X)$, given in \eqref{eq: tilde_psi}, that is defined pathwise. Working with this version directly yields a way to compute the local statistics for any given path $X$ and we have seen in Theorem \ref{Upper_bound} that for a rate optimal procedure, we can indeed choose a kernel that is continuously differentiable. 
%Moreover, the proof of Theorem \ref{thm_continuity} established continuity of the mapping
%\begin{align*}
%\mathcal{T}\ &\rightarrow\ \ \ \R,\\
%(y,h) &\mapsto\  \tilde\Psi_{T,y,h}^{b_0}(X).
%\end{align*}
%In consequence, the test statistic $T_T^\eta$ is measurable as it reduces to a supremum over a countable set.


%\begin{remark}[The case $\beta\leq 1$]
%For $\beta\leq 1$ we defined $T_T^\eta$ with the optimal recovery kernel $K_\beta$ that is not differentiable. However, as it has compact support, we can approximate $K=K_\beta$ uniformly by $K^n$ that are continuously differentiable by the Stone-Weierstraß theorem. By dominated convergence for stochastic integrals we than have
%\[ \int_0^T K_{y,h}^n(X_s) dX_s \rightarrow \int_0^T K_{y,h}(X_s) dX_s\]
%in probability and the left-hand side may be rewritten as
%\[ \int_{X_0}^{X_T} K_{y,h}^n(z) dz - \frac{\sigma^2}{2h}\int_0^T (K_{y,h}^n)'(X_s) ds.\]
%This representation is again a continuous in $(y,h)$ version of $\int_0^T K_{y,h}^n(X_s) dX_s$. In Lemma \ref{lemma_approx_K_beta} we show that for a certain choice of $K^n$ its convergence is uniform in $(y,h)\in\mathcal{T}$ for any path $X$ fullfilling $c_1 q_b \leq \frac{1}{\sigma^2 T} L_T^\cdot(X)\leq c_2  q_b$ for some constants $0<c_1\leq c_2$ and hence the limit is also continuous in $(y,h)$, in particular, it is measurable.
%\end{remark}




\begin{remark}[Grid of bandwidths]\label{remark_bandwidth}
In practice, one has to restrict to a finite subset $\mathcal{T}'\subset\mathcal{T}$ when computing the statistic $T_T^\eta$. The proof of Theorem \ref{Upper_bound} reveals that the minimal bandwidth used for detection is of order $(\log T/T)^{1/(2\beta+1)}$. Hence, it suffices to choose $h$ from the finite set
\[ \mathcal{H}_T := \left\{ k T^{-1} \mid k=1,2,\dots, \lfloor AT\rfloor \right\}. \]
The same distance of points should be applied to define a grid for $y$, i.e. we choose this parameter from
\[ \mathcal{Y}_T := \left\{ -A + kT^{-1} \mid k=1,2,\dots \lfloor 2AT\rfloor \right\} \]
and the finite set $\mathcal{T}'$ of location and bandwidth parameters for implementation may be chosen as $\mathcal{T}' = (\mathcal{Y}_T\times \mathcal{H}_T)\cap\mathcal{T}$, assuming $T\in\Q$.
\end{remark}



\begin{remark}[Quantiles for the simple null]
%Remember the test $\phi_T^{b_0}$ given in \eqref{eq: phi_0} for the simple null. % Here we definded the test statistic $T_T^{b_0}(X)$ in \eqref{eq: T_simple} and the corresponding quantiles in \eqref{eq: quantile_simple}. 
From a practical point of view it is much more convenient to replace the quantile $\kappa_{T,\alpha}^{\neq b_0}$ in the test $\phi_T^{b_0}$ given in \eqref{eq: phi_0} by the quantile
\[ \kappa_\alpha^{b_0} := \min\left\{ r\in\R \mid \Pr\left( S_{b_0}\leq r\right)\geq 1-\alpha\right\} \]
of the limiting statistic $S_{b_0}$ from Theorem \ref{weak_conv} which can be easily simulated by Monte Carlo methods as the explicit form of the invariant density $q_{b_0}$ is known.
\end{remark}











\subsection{Numerical example}

In this section we will give a numerical illustration of the testing procedure of Section~\ref{Sec_similarity} for the parameter specification $b_0(x) =-x$ together with $A=\sigma^2=1$.\\
%To compute the test $\phi_T^\eta(X)$ given in \eqref{eq: phi_eta} for simulated data, we first need to specify the quantiles $\kappa_{\eta,\alpha}$ given in \eqref{eq: kappa_eta_alpha}. 
The quantiles $\kappa_{\eta,\alpha}$ given in \eqref{eq: kappa_eta_alpha} are estimated by the empirical quantiles of $N=10000$ independent samples of $U_1\vee U_2+4\sqrt{A\eta/\sigma^2}$. Results for different $\eta$ and $\alpha$ are given in Table~\ref{Table_quant}. It can be seen that the influence of $\eta$ on the quantiles is mostly due to the additive correction term $4\sqrt{A\eta/\sigma^2}$. An algorithm for their derivation is provided in Section~\ref{App_implementation}. Note that $q_{b_0\pm\eta}$ is given explicitly for the specification $b_0(x)=-x$ by the stationary density of an Ornstein-Uhlenbeck process which is known to be Gaussian. 


\begin{center}
\begin{table}[h]
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.3781$ & $1.6775$ & $2.2468$ \\
$0.05$ & $1.4222$ & $1.7311$ &  $2.3178$ \\
$0.1$ & $1.4473$ & $1.7391$ & $2.3726$ \\
$0.2$ & $1.4503$ & $1.7497$ & $2.3047$ \\
$0.3$ & $1.4646$ & $1.7458$ & $2.3403$ \\
$0.4$ & $1.4642$ & $1.7692$ & $2.3748$ \\
$0.5$ & $1.5021$ & $1.7670$ & $2.3114$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.3781$ & $1.6775$ & $2.2468$ \\
$0.05$ & $2.3166$ & $2.6256$ &  $3.2122$ \\
$0.1$ & $2.7122$ & $3.0040$ & $3.6375$ \\
$0.2$ & $3.2391$ & $3.5386$ & $4.0935$ \\
$0.3$ & $3.6555$ & $3.9367$ & $4.5312$ \\
$0.4$ & $3.9900$ & $4.2990$ & $4.9046$ \\
$0.5$ & $4.3305$ & $4.5954$ & $5.1398$ \\
\end{tabular}
\medskip
\caption{\small{Quantiles of $U_1\vee U_2$ (left) and $U_1\vee U_2+4\sqrt{A\eta/\sigma^2}$ (right) for different $\eta$ and $\alpha$. The simulated quantiles are taken from a sample of $N=10000$, the parameters of the algorithm in Section~\ref{App_implementation} are chosen as $n_1 =100$ and $n_2=100$.}}\label{Table_quant}
\end{table}
\end{center}





To demonstrate the detection power of our test, we simulate data that follows the SDE in \eqref{eq: SDE} with
\[ b_{alt}(x) := -x  - 0.8 K\left(\frac{x+0.6}{0.15}\right) + 0.15 K\left(\frac{x}{0.2}\right) + 0.5 K\left(\frac{x-0.5}{0.1}\right),\]
where
\begin{align}\label{eq: K_alt}
K(x) := \frac{15}{16} \left( 1-x^2\right)^2 \1_{\{|x|\leq 1\}}.
\end{align} 
By Remark~\ref{remark_fixed_point}, our results hold true in the case of a fixed starting point of the diffusion and we assume $X_0=0$ for simplicity in implementation. A display of $b_{alt}$ is included in Figure~\ref{Figure_2}. The simulation is done with a time horizon $T=10000$ on an equidistant grid with width $0.001$, i.e. we simulate $10^7$ values of the diffusion according to the Euler-Maruyama scheme (cf. Section~$9.1$ and $10.2$ in \cite{Kloeden}). In Figure~\ref{Figure_2} the minimal intervals of $D_{\alpha}^\eta$ given in Remark~\ref{remark_D_alpha} are depicted for $\alpha=0.05$ and the two values $\eta_1=0.05$ and $\eta_2=0.2$. Here, an interval $I\in D_\alpha^\eta$ is called minimal, if for any interval $I\neq J\in D_\alpha^\eta$ we have $J\nsubseteq I$. The test statistic is computed with the kernel given in \eqref{eq: K_alt}.  




%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot01}
%\end{minipage}
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot03}
%\end{minipage}%
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot02}
%\end{minipage}
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot04}
%\end{minipage}


\begin{center}
\begin{figure}
%\begin{table}[h]
\begin{tabular}{cc}
\includegraphics[scale=0.3]{Plot01} & \includegraphics[scale=0.3]{Plot03}\\
\includegraphics[scale=0.3]{Rplot_new3} & \includegraphics[scale=0.3]{Rplot_new2}
\end{tabular}
\caption{\small{Both upper pictures show the drift $b_{alt}$ together with its $\eta$-environment for $\eta_1=0.05$ (left) and $\eta_2=0.2$ (right). In the bottom the minimal intervals are depicted for both cases according to the parameter specification given in the text and $\alpha=0.05$.}}\label{Figure_2}
%\end{table}
\end{figure}
\end{center}







In the following table the proportion of detections is given for various values of $\eta$ and $\alpha$ for $N=400$ simulated paths. It also contains this proportion 'locally' to show which of the three possible violations from $H_0(b_0,\eta)$ is detected (it depends on $\eta$ if $b_{alt}$ lies outside an $\eta$-environment of $b_0$ or not).


\begin{center}
\begin{table}[h]
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $1.00$ & $1.00$ \\
$0.1$ & $1.00$ & $1.00$ & $1.00$ \\
$0.2$ & $1.00$ & $1.00$ & $1.00$ \\
$0.3$ & $0.98$ & $0.97$ & $0.91$ \\
$0.4$ & $0.47$ & $0.36$ & $0.19$ \\
$0.5$ & $0.14$ & $0.11$ & $0.07$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $1.00$ & $1.00$ \\
$0.1$ & $1.00$ & $1.00$ & $1.00$ \\
$0.2$ & $1.00$ & $1.00$ & $1.00$ \\
$0.3$ & $0.98$ & $0.96$ & $0.88$ \\
$0.4$ & $0.42$ & $0.32$ & $0.17$ \\
$0.5$ & $0.12$ & $0.09$ & $0.06$ \\ 
\end{tabular}
\hfill
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{} \\
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $0.99$ & $0.98$ & $0.94$ \\
$0.05$ & $0.75$ & $0.64$ & $0.46$ \\
$0.1$ & $0.49$ & $0.40$ & $0.23$ \\
$0.2$ & $0.14$ & $0.11$ & $0.06$ \\
$0.3$ & $0.04$ & $0.03$ & $0.02$ \\
$0.4$ & $0.01$ & $0.01$ & $0.00$ \\
$0.5$ & $0.00$ & $0.00$ & $0.00$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{} \\
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $0.99$ & $0.96$ \\
$0.1$ & $0.92$ & $0.85$ & $0.60$ \\
$0.2$ & $0.33$ & $0.28$ & $0.19$ \\
$0.3$ & $0.16$ & $0.12$ & $0.08$ \\
$0.4$ & $0.06$ & $0.05$ & $0.03$ \\
$0.5$ & $0.02$ & $0.02$ & $0.01$ \\
\end{tabular}
\medskip
\caption{\small{Proportions of rejection of the null for different $\eta$ and $\alpha$ and $N=400$ simulated paths. We count, if there is any detected interval (upper left), a minimal interval intersecting with $[-0.75,-0.45]$ (upper right), $[-0.2,0.2]$ (bottom left) or $[0.4,0.6]$ (bottom right).}}\label{Table_prop_rejection}
\end{table}
\end{center}






==> Sections/Trials.tex <==
\section{Trials}



\begin{lemma}
Suppose that $c_1\leq \frac1T L_T^x(X)\leq c_2$. Then we have for all $u,\delta>0$
\[N\left( (u\delta)^\frac12, \{ (y,h)\in\mathcal{T}: \sigma((y,h))^2\leq\delta\}, \rho\right) \leq ....u^{-2}\delta^{-1},\]
where
\[ \sigma((y,h))^2 := \frac1T\int_0^T K_{y,h}(X_s)^2 ds\]
and
\[ \rho( (y,h), (y',h')) :=\frac1T \int_0^T \left( K_{y,h}(X_s) - K_{y',h'}(X_s)\right)^2 ds.\]
\end{lemma}
\begin{proof}
We split the interval $[a,b]$ into a partition $(M_k)_{1\leq k\leq N}$ such that $\lambda(M_k)=\frac{u\delta}{2c_2\|K\|_{TV}}$ for $1\leq k\leq N-1$ and $\lambda(M_N)\leq \frac{u\delta}{2c_2\|K\|_{TV}}$. Then we have
\[ \lambda([a,b]) = \sum_{k=1}^N \lambda(M_k)\geq (N-1)\frac{u\delta}{2c_2\|K\|_{TV}}, \]
or equivalently
\[ N\leq 1+ \frac{2(b-a)c_2\|K\|_{TV}}{u\delta}.\]
Take $(y,h)\in\mathcal{T}$ such that $\sigma(y,h)^2\leq\delta$, i.e.
\[ \frac1T\int_0^T K_{y,h}(X_s)^2 ds = \int_\R K_{y,h}(z)^2 \frac1T L_T^z(X) dz \leq \delta.\]
Now using the lower bound for the averaged local time we get
\[ \delta\geq c_1\int_\R K_{y,h}(z)^2 dz = c_1\int_{y-h}^{y+h} K\left(\frac{z-y}{h}\right)^2 dz = c_1h\int_{-1}^1 K(z)^2 dz = hc_1\| K\|_{L^2}^2,\]
which implies $h\leq \delta c_1^{-1}\|K\|_{L^2}^{-2}$. Now suppose $y-h\in M_i$ and $y+h\in M_j$. As we know the length of the intervals $M_k$ we conclude
\[ (i-j-1)\frac{u\delta}{2c_2\|K\|_{TV}} \leq \frac{2\delta}{c_1\|K\|_{L^2}^2}\quad\Leftrightarrow\quad i-j\leq 1+\frac{4c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2} u^{-1}.\]
Furthermore, we know that there are at most 
\begin{align*}
&\left( 1+\frac{4c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2} u^{-1}\right)\left( 1+2(b-a)c_2\|K\|_{TV}(u\delta)^{-1}\right)\\
&\hspace{1.5cm}\leq  8c_2\|K\|_{TV} \max\left\{ b-a, \frac{2}{c_1\|K\|_{L^2}^2}, \frac{4(b-a)c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2}\right\} u^{-2}\delta^{-1}
\end{align*} 
such pairs. Thus the proof is finished if we could show that there is at most one such point $(y,h)$ in a maximal subset $\mathcal{T}'$ of $\{ (y,h)\in\mathcal{T}: \sigma(y,h)^2\leq \delta\}$ with $\rho((y,h),(y',h'))^2>u\delta$ for arbitrary $(y,h),(y',h')\in\mathcal{T}'$. We pick $(y,h), (y',h')\in\mathcal{T}$ such that $y-h, y'-h'\in M_i$ and $y+h, y'+h'\in M_j$ and are done if we can show that for those $\rho((y,h),(y',h'))^2\leq u\delta$.\\
As $K$ is of bounded variation, there exists a probability measure $\mu$ on $[-1,1]$ and a measurable function $g$ with $|g|\leq \|K\|_{TV}$ such that for almost all $x\in [-1,1]$ we have
\[ K(x) = \int_{-1}^x g d\mu.\]
Since $K$ is bounded by one, we have
\begin{align*}
&\frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds\\
&\hspace{1.5cm} \leq \frac1T\int_0^T \left| K_{y,h}(X_s)-K_{y',h'}(X_s)\right| ds\\
&\hspace{1.5cm} = \int_\R\left| K\left(\frac{z-y}{h}\right) - K\left(\frac{z-y'}{h'}\right)\right| \frac1T L_T^z(X) dz\\
&\hspace{1.5cm} \leq c_2 \int_\R \left| \int_{-1}^{\frac{z-y}{h}} g(u) d\mu(u)- \int_{-1}^{\frac{z-y'}{h'}} g(u) d\mu(u)\right| dz\\
&\hspace{1.5cm} \leq c_2\int_\R \left|\int_{\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}}^{\max\left\{1, \frac{z-y}{h}, \frac{z-y'}{h'}\right\}} g(u) d\mu(u)\right| dz\\
&\hspace{1.5cm} \leq c_2\int_\R \int_{\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}}^{\max\left\{ 1,\frac{z-y}{h}, \frac{z-y'}{h'}\right\}} |g(u)| d\mu(u) dz\\
&\hspace{1.5cm} \leq c_2\|K\|_{TV} \int_\R\int_{-1}^1 1_{B_z((y,h),(y',h'))} (u) d\mu(u) dz\\
&\hspace{1.5cm} = c_2 \|K\|_{TV} \int_{-1}^1 \int_\R 1_{B_z((y,h),(y',h'))} (u) dz d\mu(u),
\end{align*}
with
\[B_z((y,h),(y',h')) = \left[\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}, \max\left\{1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}\right]\]
and an application of Fubini's theorem in the last step. Now $u\in B_z((y,h),(y',h'))$ if and only if
\[ -1\leq \frac{z-y}{h}\leq u\leq \frac{z-y'}{h'}\leq 1\quad \textrm{ or }\quad -1\leq\frac{z-y'}{h'}\leq u\leq \frac{z-y}{h}\leq 1.\]
The first condition is equivalent to $uh'+y'\leq z\leq uh+y$, the second one to $uh+y\leq z\leq uh'+y'$. Thus, the inner integral equals $|y' + uh' - y - uh|$ and we get
\begin{align*}
\frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds&\leq c_2 \|K\|_{TV}\int_{-1}^1 |y'+uh'-y-uh| d\mu(u)\\
&\leq c_2 \|K\|_{TV}\max_{u=\pm 1} |y-y' +u( h-h')|\\
&\leq c_2\|K\|_{TV} \lambda([y-h,y+h]\bigtriangleup [y'-h',y'+h']),
\end{align*}
where the second inequality follows from the fact, that $|y-y' + u(h-h')|$ is maximized for $u=\textrm{sign}(y-y')\textrm{sign}(h-h')$.\\
As we chose $(y,h),(y',h')\in\mathcal{T}$ to fullfill $y-h,y'-h'\in M_i$ and $y+h,y'+h'\in M_j$ we know that
$\lambda([y-h,y+h]\bigtriangleup [y'-h',y'+h']) \leq 2\frac{u\delta}{2c_2\|K\|_{TV}}$. Hence,
\[ \frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds\leq 2c_2\|K\|_{TV}\frac{u\delta}{2c_2\|K\|_{TV}} = u\delta\]
and the proof is complete.
\end{proof}








\subsection{Alternative Proof of the upper bound}

First of all, we introduce the most important function spaces needed for the proof \textbf{(later put them in front part of the paper)}.
\begin{enumerate}
\item[(1)] For positive numbers $\beta, L$ we define the Hölder class $\mathcal{H}(\beta, L)$ as the set of $l=\lfloor \beta\rfloor$ times differentiable functions $f:S \rightarrow\R$, $S\subset\R$ whose derivative $f^{(l)}$ satisfies
\[ \left| f^{(l)}(x) - f^{(l)}(y)\right| \leq L|x-y|^{\beta -l}\quad \textrm{ for all } x,y\in S.\]
\item[(2)] For constants $M,\gamma, \sigma >0$ and $C\geq 1$ we set
\[ \Sigma(C,A,\gamma, \sigma) :=\left\{ b\in \textrm{Lip}_{loc}(\R):\ |b(x)|\leq C(1+|x|)\ \forall x\in\R\textrm{ and } \frac{b(x)}{\sigma^2}\textrm{sgn}(x)\leq -\gamma\ \forall |x|\geq A\right\}.\]
For all this functions $b\in\Sigma(C,A,\gamma, \sigma)$ there exists a unique strong solution of the SDE $dX_t = b(X_t) dt +\sigma dW_t$ with ergodic properties and invariant density
\[ \rho_b(x) := \frac{1}{C_{b,\sigma} \sigma^2} \exp\left( \int_0^x \frac{2b(y)}{\sigma^2} dy\right) \quad\textrm{ for all } x\in\R,\]
with the normalising constant $C_{b,\sigma}:= \int_\R \frac{1}{\sigma^2}\exp\left(\int_0^u \frac{2b(y)}{\sigma^2} dy\right)du$. We will denote the corresponding invariant measure by $\mu_b$.
%Moreover, we can deduce from this assumption some regularity properties of the invariant density $\phi_b$. In particular, there exists a constant $\mathcal{L}=\mathcal{L}(C,A,\gamma,\sigma)$ such that
%\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \max\left\{ \|\phi_b\|_\infty, \|\phi_b'\|_\infty\right\} <\mathcal{L}, \]
%and for any $\theta>0$ we have
%\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)}\sup_{x\in\R} |x|^\theta\phi_b(x) <\infty.\]

%\item[(3)] Last but not least we set for $\beta, L>0$
%\[ \Sigma(\beta, L) := \Sigma(\beta, L, C,A,\gamma) := \left\{ b\in\Sigma(C,A,\gamma,1): \phi_b\in\mathcal{H}(\beta+1, L)\right\}.\]

\item[(3)] Last but not least set for $\beta, L>9$
\begin{align*}
\Sigma(\beta, L) := \Sigma(\beta, L, C,A,\gamma,b_0)  := \left\{ b_1\in \Sigma(C,A,\gamma,1) : (b_1-b_0) \in\mathcal{H}(\beta,L)\right\}.
\end{align*}
\end{enumerate}








\subsubsection{Regularity of drift and invariant density}

\begin{lemma}
For $f\in\mathcal{H}(\beta +1, L)$, we have $f'\in\mathcal{H}(\beta,L)$.
\end{lemma}
\begin{proof}
As $1+\beta>1$ we know from the definition of the Hölder class that $f$ is at least one time differentiable and $f'$ exists. Furthermore, as $\lfloor\beta+1\rfloor = 1+\lfloor \beta\rfloor$, $f'$ is $l=\lfloor\beta\rfloor$ times differentiable and
\begin{align*}
\left| (f')^{(\lfloor\beta\rfloor)}(x) - (f')^{(\lfloor\beta\rfloor)}(y)\right| &= \left| f^{(1+\lfloor\beta\rfloor)}(x) - f^{(\lfloor\beta\rfloor)}(y)\right|\\
& \leq L|x-y|^{\beta+1 - (1+\lfloor\beta\rfloor)} = L|x-y|^{\beta-\lfloor\beta\rfloor}.
\end{align*}
\end{proof}




\begin{lemma}\label{bound_invariant_density}
There exists a constant $L = L(C,A,\gamma,\sigma)$ such that
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \max\left\{ \|\rho_b\|_\infty, \| \rho_b'\|_\infty\right\} \leq L.\]
\end{lemma}
\begin{proof}[Proof]
Let $b\in\Sigma(C,A,\gamma,\sigma)$. First we look for an upper bound of the normalizing factor $C_{b,\sigma}^{-1}\sigma^{-2}$ which equivalent to looking for a lower bound of $C_{b,\sigma}$. By the at most linear growth condition we get
\[ \left| \int_0^x 2\sigma^{-2} b(y) dy\right| \leq 2\sigma^{-2} \int_0^{|x|} |b(y)|dy \leq 2\sigma^{-2} \int_0^{|x|} C(1+|y|)dy \leq 2C\sigma^{-2}(1+|x|)|x|.\]
Hence on the interval $[-a,a]$ with $a\leq 1$ we have
\[ \exp\left( \int_0^x \frac{b(y)}{\sigma^2} dy \right) \geq \exp\left( - 2C\sigma^{-2} (1+a)a\right) \geq \exp\left( - 2C\sigma^{-2}\right).\]
Setting $a=\frac{1}{C}$ we get by non-negativity of $\exp$ that
\[ C_{b,\sigma} \geq \int_{-C^{-1}}^{C^{-1}} \sigma^{-2} \exp\left(\int_0^u 2\sigma^{-2} b(y) dy\right) du \geq \frac{2}{C\sigma^2} \exp\left( -2C\sigma^{-2}\right).\]
Thus,
\[ \frac{1}{C_{b,\sigma}\sigma^2} \leq \frac{C\sigma^2}{2} e^{2C\sigma^{-2}},\]
so the normalizing constant of the invariant density $\rho_b$ is bounded by some constant depending only on $C$ and $\sigma$.\\
We now turn to $\exp\left(\int_0^x 2\sigma^{-2} b(y) dy\right)$ and see that it suffices to bound the exponent by some constant. For $x>0$ we may upper-bound via
\begin{align*}
\int_0^x 2\sigma^{-2} b(y) dy &\leq \int_0^{A\wedge x} 2\sigma^{-2}b(y) dy + \int_{A\wedge x}^x 2\sigma^{-2}b(y) dy \\
&\leq 2\sigma^{-2} C(1+A) A + 2\int_{A\wedge x}^x -\gamma dy\\
&= 2\sigma^{-2} C(1+A) A -2\gamma(x-A\wedge x)\\
&\leq 2\sigma^{-2} C(1+A) A + 2A\gamma.
\end{align*} 
Similarly, we ge for $x<0$
\begin{align*}
\int_0^x 2\sigma^{-2} b(y) dy &= -\int_0^{-x} 2\sigma^{-2} b(y) dy\\
&= - \int_0^{A\wedge(-x)} 2\sigma^{-2}b(y) dy - \int_{A\wedge (-x)}^{-x}2\sigma^{-2}b(y) dy\\
&\leq 2\sigma^{-2} C(1+A)A - 2\int_{A\wedge (-x)}^{-x} \gamma dy\\
&= 2\sigma^{-2} C(1+A)A - 2\gamma (-x - A\wedge (-x))\\
&\leq 2\sigma^{-2} C(1+A)A +2A\gamma.
\end{align*}
So finally, we have the bound
\[ \rho_b(x) \leq \frac{C\sigma^2}{2} e^{2C\sigma^{-2}} e^{2\sigma^{-2}C(1+A)A + 2A\gamma}.\]
Now we consider $\|\rho_b'\|_\infty$ and use $\rho_b' = 2b\rho_b$. Unfortunately, $b$ is not bounded by some constant so we are not done immediately. 
But we have shown above that
\[ \exp\left( \int_0^x 2\sigma^{-2} b(y) dy\right) \leq \exp\left( 2\sigma^{-2}C(1+A)A + 2A\gamma - 2\gamma |x|\right).\]
This gives
\begin{align*}
|\rho_b'(x)| \leq |2b(x) \rho_b(x)| &\leq C\sigma^{-2} e^{2C\sigma^{-2}} (1+|x|)e^{\tilde{c} - 2\gamma |x|}\\
&\leq C\sigma^{-2} e^{2C\sigma^{-2}}  \left( e^{\tilde{c}} + |x|e^{\tilde{c} - 2\gamma |x|}\right)
\end{align*} 
with  $\tilde{c} = 2\sigma^{-2}C(1+A)A + 2A\gamma$. Now the function $|x| e^{\tilde{c} - 2\gamma|x|}$ is bounded and maximized for $|x| = \frac{1}{2\gamma}$. Thus,
\[ |\rho_b'(x)| \leq C\sigma^{-2} e^{2C\sigma^{-2}}  \left( e^{\tilde{c}} + \frac{1}{2\gamma}e^{\tilde{c}-1}\right)\]
and the proof is finished by taking $L$ as the maximum of both the upper bounds.
\end{proof}


\begin{lemma}\label{local_time-Invariant}
Let $h_T = c\left(\frac{\log T}{T}\right)^\alpha$, $\alpha>0$. Furthermore, let $b\in\Sigma(C,A,\gamma,\sigma)$. Then for every $z\in [y-h_T, y+h_T]$
\[ \frac1T L_T^z(X) - \rho_b(y) = o_{\Pr}\left( (\log T)^{-1}\right).\]
\end{lemma}
\begin{proof}[Proof]
We first split in the obious way
\[ \frac1T L_T^z(X) - \rho_b(y) = \left( \frac1T L_T^z(X) -\rho(z)\right) + \left( \rho_b(z)-\rho_b(y)\right).\]
As $\rho_b$ is differentiable with bounded derivative it is Lipschitz continuous, more precisely we get with Lemma \ref{bound_invariant_density}
\[ \left|\rho_b(z)-\rho_b(y)\right| \leq L(C,A,\gamma,\sigma) |y-z| \leq 2L(C,A,\gamma,\sigma) h_T.\]
Using the definition of $h_T$ it follows $ (\rho_b(y)-\rho_b(z))1_{[y-h_T, y+h_T]}(z)\in o_T\left((\log T)^{-1}\right)$.\\
For the other term we use the fact that
\[ \sqrt{T} \left(\frac1T L_T^z(X) - \rho_b(z)\right) \] 
converges in distribution to a centered Gaussian random map according to Lemma $56$ in \textbf{Diss Willems/Strauch...look for the paper}. Hence, $\sqrt{T}\left(\frac1T L_T^z(X) - \rho_b(z)\right)\in \mathcal{O}_{\Pr}(1)$ and consequently
$\log T\left(\frac1T L_T^z(X) - \rho_b(z)\right)\in o_{\Pr}(1)$ and the claim follows.
\end{proof}








\subsubsection{The choice of the kernel}

Let $K= K(\cdot,\beta)$ be the unique solution of the following optimization problem:
\[ \textrm{Minimize } \|K\|_{L^2} \textrm{ over all } K\in\mathcal{H}(\beta,1) \textrm{ with } K(0)\geq 1.\]

In the case $0<\beta\leq 1$ it is not difficult to see that
\[ K(x) = 1_{|x|\leq 1} \left(1-|x|^\beta\right),\]
as we even have $K(x) \leq f(x)$ for all $x\in [-1,1]$ and $f\in\mathcal{H}(\beta,1)$ in this case. For $\beta =2$ an explicit solution is known (see Leonov...). Furthermore, for all $\beta>0$ $K$ is compactly supported, an even function and satisfies $K(0)=1>|K(x)|$ for $x\neq 0$. We will denote this compact support by $[-R,R]$.\\

For any scale parameter $h>0$ and location parameter $y\in\R$ we denote
\[ K_{y,h}(x) = K\left(\frac{x-y}{h}\right) \]
and this function is clearly supported in $[y-Rh, y+Rh]$.

\begin{lemma}\label{Lemma_rescaling}
For any $\delta>0$ the function $\tilde{K}:= \pm\delta K_{y,h}$ belongs to $\mathcal{H}(\beta, \delta h^{-\beta})$ and minimizes $\|\tilde{K}\|_{L^2}$ over this class under the additional constraint $\pm \tilde{K}(y)\geq \delta$.
\end{lemma}
\begin{proof}[Proof]
Clearly, as it holds for $K$, $\tilde{K}$ is $\lfloor \beta\rfloor$-times differentiable and we have
\begin{align*}
\left| \tilde{K}^{\lfloor\beta\rfloor}(x) - \tilde{K}^{\lfloor\beta\rfloor}(x')\right| &= \delta h^{-\lfloor\beta\rfloor} \left| K^{\lfloor\beta\rfloor}\left(\frac{x-y}{h}\right) - K^{\lfloor\beta\rfloor}\left(\frac{x'-y}{h}\right) \right| \\
&\leq \delta h^{-\lfloor\beta\rfloor}\left|\frac{x-y}{h} - \frac{x'-y}{h}\right|^{\beta-\lfloor\beta\rfloor} \\
&= \delta h^{-\beta} |x-x'|^{\beta-\lfloor\beta\rfloor},
\end{align*}
which establishes $\tilde{K}\in\mathcal{H}(\beta, \delta h^{-\beta})$.\\
For every $K$ with $K(0)\geq 1$, we have $\pm\tilde{K}(y) = \delta K(0)\geq\delta$ and for $L^2$-norm we have
\[ \|\tilde{K}\|_{L^2} = \left(\int_\R \delta^2 K\left(\frac{x-y}{h}\right)^2 dx\right)^\frac12 = \delta h^{-\frac12} \left(\int_\R K(x)^2 dx\right)^\frac12 = \delta h^{-\frac12} \|K\|_{L^2},\]
so this norm is minimized, if $\|K\|_{L^2}$ is minimized and we are done.
\end{proof}










\begin{proof}[Alternative Proof of Theorem \ref{Upper_bound}]
Denote $K_{y,h}(X_s) = K\left(\frac{X_s-y}{h}\right)$. For every $y$, the probability $\Pr(T(X)>\kappa_\alpha)$ of rejecting the null hypothesis is bounded from below by
\begin{align*}
&\Pr_{b_1}\left( \left| \Psi_T(y,h_T)\right| > C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right) + \kappa_\alpha\right) \\
&\hspace{0.5cm} =\Pr_{b_1}\left(\frac{\left| \frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s  + \frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left( b_1(X_s) - b_0(X_s)\right) ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right.\\
&\hspace{4cm}\left. > C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right)+\kappa_\alpha\right)\\
&\hspace{0.5cm} \geq \Pr_{b_1}\left( -\textrm{sign}\left(\int_0^T K_{y,h_T}(X_s)\left( b_1(X_s) - b_0(X_s)\right) ds\right) \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right. \\
&\hspace{2cm} \left. < \frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right)+\kappa_\alpha\right).
\end{align*}
The idea of the proof is to proceed as follows: First, we show that the left side of the inequality forms a tight sequence and hence the claim is established once we show that the right side diverges to infinity in a second step.\\
As $z$ is taken from a compact set $A$, we find constants $c_1, c_2>0$ such that $c_1\leq \phi_b\leq c_2$. Now define the set
\[\mathcal{C}_T :=\left\{ \sup_{z\in A} \left| \frac1T \L_T^z(X) - \phi_b(z)\right| <\frac{c_1}{2}\right\}.\] 
By the result of van Zanten \textbf{tex this somewhere)} we have $\Pr_{b_1}(\mathcal{C}_T) \rightarrow 1$ for $T\to\infty$ and on $\mathcal{C}_T$ it holds that
\[ \frac12 \phi_b(z)\leq \frac1T \L_T^z(X)\leq \frac32 \phi_b(z).\]
Now let $\epsilon>0$ and take $T\geq T_0$ large enough such that $\Pr_{b_1}(\mathcal{C}_T)>1-\frac{\epsilon}{2}$. For $K>0$ we can write
\begin{align*}
&\Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K\right)\\
&\hspace{0.5cm} = \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T\right) + \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T^c\right)
\end{align*}
The second term is bounded by $\Pr(\mathcal{C}_T^c)<\frac{\epsilon}{2}$. For the first own we use the occupation times formula to get
\[ \frac1T \int_0^T K_{y,h_T}(X_s)^2 ds = \int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz\]
and on $\mathcal{C}_T$ we can upper- and lower-bound the averaged local time to get
\[ \frac12 \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz \leq \frac1T\int_0^T K_{y,h_T}(X_s)^2 ds \leq \frac32 \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz.\]
Now we apply Proposition \ref{Exp_ineq} with $\theta = \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz$ and $S=\sqrt{3}$ to get
\[ \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T\right) \leq 4K\sqrt{e} (1+\log(\sqrt{3}))\exp\left(-\frac{K^2}{2}\right).\]
Clearly, we can choose $K$ large enough to bound this term again by $\frac{\epsilon}{2}$ and the proof of the thightness is finished.\\

Now we want to show that
\[ \left( 1+\epsilon_T\right)\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds\right)\rightarrow \infty\]
for all $b_1-b_0\in\Sigma(\beta, L)$ such that $\|(b_1-b_0)\rho_{b_1}^\frac{\beta}{2\beta+1}\|_\infty \geq \delta_T$. Let $b_1$ be such a function with $\left|(b_1(y)-b_0(y)\rho_{b_1}(y)^\frac{\beta}{2\beta+1}\right|>\delta_T$, or equivalently
\[ |b_1(y) - b_0(y) | > c_*\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^{\frac{\beta}{2\beta+1}} =:\tilde{\delta}_T.\]
We define 
\[ h_T := \left(\frac{c_*}{L}\right)^{\frac{1}{\beta}}\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^{\frac{1}{2\beta+1}}.\]
Then from Lemma \ref{Lemma_rescaling} we know that $\tilde{\delta}_T K_{y,h_T}\in\mathcal{H}(\beta, \tilde{\delta}_T h_T^{-\beta}) = \mathcal{H}(\beta, L)$ and minimizes the $L^2$-norm over his class for all functions $f$ satisfying $f(y)\geq\delta$. In particular, this implies
\[ \left| \int_\R \tilde{\delta}_T K_{y,h_T}(z) (b_1(z)-b_0(z)) dz \right| \geq \tilde{\delta}_T^2 \int_\R K_{y,h_T}(z)^2 dz.\]
By the occupation times formula and Lemma \ref{local_time-Invariant} we may write
\begin{align*}
&\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} = \frac{\sqrt{T}\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) \frac1T L_T^z(X)dz\right|}{\sqrt{\int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz}}\\
&\hspace{1cm}=\frac{\sqrt{T}\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) \left( \rho_{b_1}(y) + \frac1T L_T^z(X) - \rho_{b_1}(y)\right)dz\right|}{\sqrt{\int_\R K_{y,h_T}(z)^2\left(\rho_{b_1}(y) + \frac1T L_T^z(X) - \rho_{b_1}(y)\right) dz}}\\
&\hspace{1cm} = \frac{\sqrt{T} \left(\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})\right)\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) dz\right|}{\sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})}\sqrt{\int_\R K_{y,h_T}(z)^2dz}}\\
&\hspace{1cm} = \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T}\frac{\tilde{\delta}_T^{-1} \left|\int_\R \tilde{\delta}_T K_{y,h_T}(z) ( b_1(z)-b_0(z)) dz \right|}{\sqrt{\int_\R K_{y,h_T}(z)^2dz}}\\
&\hspace{1cm}\geq \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T} \frac{\tilde{\delta}_T \int_\R K_{y,h_T}(z)^2 dz}{\sqrt{\int_\R K_{y,h_T}(z)^2 ds}}\\
&\hspace{1cm} = \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T h_T} \tilde{\delta}_T \| K\|_{L^2}
\end{align*}
where the last step follows by substitution of $\tilde{x}=\frac{x-y}{h_T}$ in the integral. Now be definition of $h_T$ and $\tilde{\delta}_T$ we have
\begin{align*}
\sqrt{Th_T}\tilde{\delta}_T &= T^\frac12 \left(\frac{c_*}{L}\right)^{\frac{1}{2\beta}} \left( \frac{\log T}{T\rho_{b_1}(y)}\right)^\frac{1}{2(2\beta+1)} c_*\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^\frac{\beta}{2\beta+1}\\
&= c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \rho_{b_1}(y)^{-\frac{1}{2(2\beta+1)} - \frac{\beta}{2\beta+1}} T^{\frac12 - \frac{1}{2(2\beta+1)} - \frac{\beta}{2\beta+1}} (\log T)^{\frac{1}{2(2\beta+1)} + \frac{\beta}{2\beta+1}}\\
&= c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \rho_{b_1}(y)^{-\frac12} (\log T)^{\frac12},
\end{align*}
as $\frac{1}{2(2\beta+1)} + \frac{\beta}{2\beta+1} = \frac{1+2\beta}{2(2\beta+1)} = \frac12$. So we arrive at
\begin{align*}
\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} &\geq \sqrt{1+o_{\Pr}((\log T)^{-1})} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2}\sqrt{\log T}\\
&= \sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2}.
\end{align*}


Next, we treat the compensating term $C(\cdot)$ in a similar way. We have
\begin{align*}
C\left(\frac1T \int_0^T K_{y,h_T}(X_s)^2 ds\right) &= C\left( \int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz\right) \\
&= C\left( (\rho_{b_1}(y)+o_{\Pr}(1)) \int_\R K_{y,h_T}(z)^2 dz\right) \\
&= C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right).
\end{align*}
With the definition of $C$ we proceed the following way:
\begin{align*}
&C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right) = \left( 2\log\left(\frac{1}{(\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T}\right)\right)^\frac12\\
&\hspace{1cm} = \left( -2 \log\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right)\right)^\frac12\\
&\hspace{1cm} = \left( - 2\log(h_T) - 2\log((\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 )\right)^\frac12\\
&\hspace{1cm}= \left( -2\log(h_T) +\mathcal{O}_{\Pr}(1)\right)^\frac12.
\end{align*}
Now with our definition of $h_T$ we have
\[ \log(h_T) = \frac{1}{\beta} \log\left( \frac{c_*}{L}\right) + \frac{1}{2\beta+1}\left( \log\log T - \log T - \log(\rho_{b_1}(y)) \right)\]
and consequently,
\[ C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right) = \left( \frac{2}{2\beta+1} \log T - \frac{2}{2\beta+1}\log\log T  + \mathcal{O}_{\Pr}(1)\right)^\frac12.\]
Now we can put everything together and evaluate the whole expression. With an application of Lemma \ref{log-terms} in the second step this yields
\begin{align*}
&\left( 1+\epsilon_T\right)\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds\right)\\
&\hspace{0.5cm} \geq (1+\epsilon_T)\sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2} - \left( \frac{2}{2\beta+1} \log T - \frac{2}{2\beta+1}\log\log T  + \mathcal{O}_{\Pr}(1)\right)^\frac12\\
&\hspace{0.5cm} = (1+\epsilon_T)\sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2} - \sqrt{\frac{2}{2\beta+1} \log T} + o_{\Pr}(1)\\
& \textbf{here we need the def of $c_*$ which will be in the theorem...} c_* = \left( \frac{2L^{\frac1\beta}}{(2\beta+1)\|K\|_{L^2}^2}\right)^{\frac{\beta}{2\beta+1}}\\
&\hspace{0.5cm} = \sqrt{\frac{2}{2\beta+1}} \left( \sqrt{\log T + o_{\Pr}(1)}- \sqrt{\log T} + \epsilon_T\sqrt{\log T + o_{\Pr}(1)}\right) + o_{\Pr}(1)\\
&= \sqrt{\frac{2}{2\beta +1}} \left( o_{\Pr}(1) + \epsilon_T\sqrt{\log T + o_{\Pr}(1)}\right) + o_{\Pr}(1) \rightarrow \infty.
\end{align*}
In the last step we have used that $\epsilon_T\sqrt{T}\rightarrow \infty$ and hence $\epsilon_T\sqrt{\log T + o_T(1)}\rightarrow\infty$ next to
\begin{align*}
\sqrt{\log T + o_{\Pr}(1)}- \sqrt{\log T} &= \frac{\log T + o_{\Pr}(1) - \log T}{\sqrt{\log T + o_{\Pr}(1)} + \sqrt{\log T}}\\
&= \frac{o_{\Pr}(1)}{\sqrt{\log T+o_{\Pr}(1)} + \sqrt{\log T}} =o_{\Pr}(1).
\end{align*} 
\end{proof}













\subsubsection{Sharp lower bound}

Like in any other proof of lower bounds we will reduce the problem to some challenging hypothesis - in our case some small deviations of the drift that will not be detected. In order to construct those, we choose a kernel function $K:\R\rightarrow\R$ with $K\in\mathcal{C}_c^\infty(\R)$, $\textrm{supp}(K) = [-1,1]$, $|K(x)|\leq 1$, $K(0)=1$ and $K\in\mathcal{H}(\beta, 1)$. We set
\[ h_T^w := \left(\frac{c_*}{L}\right)^\frac{1}{\beta} \left( \frac{\log T}{T w}\right)^\frac{1}{2\beta+1}.\]
Then we pick some drift $b_0\in\Sigma\left( \frac{C}{2},A, \gamma, 1\right)$ for the zero hypothesis and define the alternatives
\[ b_j^w(x) := b_0(x) + L(h_T^w)^\beta K\left(\frac{x-y_j^w}{h_T^w}\right),\]
where $y_j^w$ is some location depending continuously on $w$. To be valid hypotheses we need three conditions on $b_j^w$: 
\begin{itemize}
\item The SDE with drift $b_j^w$ should be ergodic, more precisely, we need $b_j^w\in \Sigma(C,A,\gamma, \sigma)$,
\item we need $b_0 - b_j^w\in\mathcal{H}(\beta, L)$,
\item the support of the $b_j-b_0$ should be disjoint which corresponds to a good choise of $y_hj^w$, and
\item we want 
\[\left|(b_j^w(y_j^w) - b_0(y_j^w))\rho_{b_j^w}(y_j^w)^\frac{\beta}{2\beta+1}\right| = L(h_T^w)^\beta K(0)\left|\rho_{b_j^w}(y_j^w)\right|^\frac{\beta}{2\beta+1} = c_*\left(\frac{\log T}{T}\right)^\frac{\beta}{2\beta+1}.\]
Using our definition of $h_T^w$ this is equivalent to
\[ w = \rho_{b_j^w}(y_j^w).\]
\end{itemize} 
As we are dealing with asymptotics, it is in fact enough to verify those conditions for $T\geq T_0$. The first two are standard and will be established in Lemmata \ref{lemma_cond_2} and \ref{lemma_cond_1}. The third condition will be dealt with in the proof of the main theorem by constructing the alternatives inductively. The last one could in fact be relaxed to $\geq$ instead of equality, but is self-evident to expect the hardest detectable alternative in the case of equality which is what we assume above. It also has the nice feature that is gives rise to a fixed-point problem: We associate to any $w$ in some suitable chosen interval a drift function $b_j^w$ which again is associated to a drift function $\rho_{b_j^w}$ which is known in the ergodic case. This drift can be evaluated at $y_j^w$ and we ask if it possible to chose $w$ in such a way that the outcome of the concatenation of these mapings is again $w$.




\begin{lemma}\label{lemma_cond_2}
For the drift functions $b_0$ and $b_j^w$ defined above we have $b_0-b_j^w\in\mathcal{H}(\beta, L)$
\end{lemma}
\begin{proof}
As $b_0 - b_j^w = L (h_T^w)^\beta K\left( \frac{\cdot - y_j^w}{h_T^w}\right)$ we know that this difference is $\lfloor\beta\rfloor$-times differentiable as this holds for $K$. Furthermore, 
\begin{align*}
&\left| (b_0-b_j^w)^{(\lfloor\beta\rfloor)}(x) - (b_0-b_j^w)^{(\lfloor\beta\rfloor)}(x')\right| \\
&\hspace{1cm}= L(h_T^w)^{\beta-\lfloor\beta\rfloor}\left| K^{(\lfloor\beta\rfloor)}\left( \frac{x-y_j^w}{h_T^w}\right) - K^{(\lfloor\beta\rfloor)}\left(\frac{x'-y_j^w}{h_T^w}\right)\right|\\
&\hspace{1cm}\leq L(h_T^w)^{\beta-\lfloor\beta\rfloor}\left| \frac{x-y_j^w}{h_T^w} - \frac{x'-y_j^w}{h_T^w}\right|^{\beta- \lfloor\beta\rfloor}\\
&\hspace{1cm}= L|x-x'|^{\beta-\lfloor\beta\rfloor},
\end{align*}
where we used in the second step that $K\in\mathcal{H}(\beta, 1)$.
\end{proof}




\begin{lemma}\label{lemma_cond_1}
For the drift $b_j^w$ defined above we have $b_j^w\in \Sigma(C,A,\gamma, \sigma)$ for all $T$ large enough to ensure $L(h_T^w)^\beta\leq \frac{C}{2}$.
\end{lemma}
\begin{proof}
We have $b_j^w(x) = b_0(x)$ for $|x|\geq A$ and hence $\frac{b_j^w(x)}{\sigma^2}\textrm{sgn}(x) \leq -\gamma$ for those $x$ as the condition is fullfilled for $b_0$. Furthermore, as $b_0$ and $K$ are locally Lipschitz, the same holds true for $b_j^w$. Last but not least, 
\[ |b_j^w(x)| \leq |b_0(x)| + L(h_T^w)^\beta \left| K\left(\frac{x-y_j^w}{h_T^w}\right)\right| \leq \frac{C}{2}(1+|x|) + L(h_T^w)^\beta \leq C(1+|x|).\]
\end{proof}



\begin{lemma}\label{lemma_fixed_point}
Choose $y\in\R$ and set $y_j^w = y+h_T^w$. Then for $T\geq T_0$ large enougt, there exists $\tilde{w}>0$ such that $\rho_{b_j^{\tilde{w}}}(y_j^{\tilde{w}}) = \tilde{w}$.
\end{lemma}
\begin{proof}
Denote by $f$ the concatenation of the following maps
\begin{equation*}
\begin{matrix}
& \R_{>0} & \longrightarrow & (\mathcal{C}^0, \|\cdot\|_\infty)\times \R &\longrightarrow & (\mathcal{C}^0, \|\cdot\|_\infty)\times \R &\longrightarrow &\R_{\geq 0}, \\
& w & \mapsto & \begin{pmatrix}b_j^{w}\\ y_j^w\end{pmatrix} &\mapsto & \begin{pmatrix}\rho_{b_j^w}\\ y_j^w\end{pmatrix} &\mapsto  & \rho_{b_j^w}(y_j^w).
\end{matrix}
\end{equation*}
Our proof will establish
\begin{itemize}
\item[(1)] continuity of $f:\R_{> 0}\rightarrow\R_{\geq 0}$, 
\item[(2)] existance of a compact interval $I\subset\R_{>0}$ such that $f(I)\subset I$. 
\end{itemize}
Then it follows that there exists a fixed point $\tilde{w}$ within the interval $I$ and the proof is complete.\\
We begin with statement $(1)$. The map $f$ consists of three parts and we will show continuity for each arrow seperately, each time $j$ and $T$. In each case the preimage of the map is the image of the previous mapping understood as a subspace of the given space in the diagram above. 
\begin{itemize}
\item[(a)] The first map $w\mapsto b_j^w$ can be split into $w\mapsto h_T^w \mapsto b_j^w$ as $y_j^w$ is also a function of $h_T^w$. In this composition continuity of the first part is obvious. For the second one we consider $w, w'>0$ and estimate with the fact that $K\in\mathcal{C}_c^\infty$
\begin{align*}
&\left| b_j^w(x) - b_j^{w'}(x)\right|\leq L\left| (h_T^w)^\beta K\left(\frac{x-y_j^w}{h_T^w}\right) - (h_T^{w'})^\beta K\left(\frac{x-y_j^{w'}}{h_T^{w'}}\right)\right|\\
&\hspace{0.5cm}\leq L\left| (h_T^w - h_T^{w'}) K\left(\frac{x-y_j^w}{h_T^w}\right) + h_T^{w'}\left( K\left(\frac{x-y_j^{w'}}{h_T^{w'}}\right) - K\left(\frac{x-y_j^w}{h_T^w}\right)\right)\right|\\
&\hspace{0.5cm} \leq \|K\|_\infty |h_T^w - h_T^{w'}| + h_T^{w'} \|K'\|_\infty\left| \frac{x-y_j^{w'}}{h_T	^{w'}} - \frac{x-y_j^w}{h_T^w}\right|\\
&\hspace{0.5cm} = \|K\|_\infty |h_T^w - h_T^{w'}| + h_T^{w'} \|K'\|_\infty\left| \frac{h_T^w ( x-y_j^{w'}) - h_T	^{w'} (x-y_j^w)}{h_T^{w'}h_T^w}\right|
\end{align*}
For the  numerator of the last term we have
\begin{align*}
h_T^w ( x-y_j^{w'}) - h_T	^{w'} (x-y_j^w) &= (h_T^w - h_T^{w'})x - h_T^w y_j^{w'} + h_T^{w'}y_j^w\\
&=  (h_T^w - h_T^{w'})x  - h_T^w ( y_j^{w'} - y_j^w) + y_j^w (h_T^{w'} - h_T^w) \\
&= (h_T^w - h_T^{w'})\left( x  + h_T^w - y_j^w\right)
\end{align*}
which yields 
\[ \left| b_j^w(x) - b_j^{w'}(x)\right|\leq \left( \|K\|_\infty + \frac{|y-x|}{h_T^w}\right) \left|h_T^w - h_T^{w'}\right|.\]
As the difference $b_j^w- b_j^{w'}$ vanishes outside $[-A,A]$ the factor is bounded in $x$ and we get continuity in supremum norm.\\
Continuity in the second parameter is again obvious as $y_j^w = 2j h_T^w$ is again a continuous function in $w$.

\item[(b)] Nothing happens in the second component, so we only have to work for the first one. Our hypotheses are of the form $b_j^w = b_0 + g_j^w$, so $\|b_j^w - b_j^{w'}\|_\infty = \|g_j^w - g_j^{w'}\|_\infty$ and the $g_j^w$ are supported within $[-A,A]$, i.e. the supremum norm of the difference vanishes outside this interval. The invariant density is of the form
\[ \rho_{b_{j^w}}(x) = \frac{1}{C_{b_j^w,\sigma}\sigma^2}\exp\left( \int_0^x \frac{2b_j^w}{\sigma^2} dy\right),\]
and we show continuity of $b_j^w\mapsto C_{b_j^w,\sigma}$ and $b_j^w\mapsto \exp\left(\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy \right)$ where the latter is understood as a continuous function in $(\mathcal{C}^0, \|\cdot\|_\infty)$.\\
Let $\epsilon>0$, then there exists $\delta>0$ such that 
\[ \left\| \exp\left(\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy \right)-\exp\left(\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy \right)\right\| <\epsilon\]
if 
\[ \left\|\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy-\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy\right\|_\infty<\delta.\]
But the last expression can be bound in terms of $\|b_j^w - b_j^{w'}\|_\infty$ as
\begin{align*}
&\left|\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy-\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy\right| \leq 2\sigma^{-2} \left| \int_0^x b_j^w(y) - b_j^{w'}(y) dy\right|\\
&\hspace{1cm} \leq 2\sigma^{-2} \int_0^{|x|} \left| g_j^w(y) - g_j^{w'}(y)\right| dy \leq 2\sigma^{-2} \int_{-A}^A\left| g_j^w(y) - g_j^{w'}(y)\right| dy \\
&\hspace{1cm} \leq 4A\sigma^{-2} \|g_j^w - g_j^{w'}\|_\infty = 4A\sigma^{-2} \|b_j^w - b_j^{w'}\|_\infty.
\end{align*}
We move on to $b_j^w\mapsto C_{b_j^w,\sigma}$. By the triangle inequality we directly get
\begin{align*}
&\left| C_{b_j^w, \sigma} - C_{b_j^{w'}, \sigma}\right| \leq \sigma^{-2} \int_\R\left|\exp\left( \int_0^y 2\sigma^{-2} b_j^w(u) du \right) - \exp\left(\int_0^y 2\sigma^{-2} b_j^{w'}(u) du \right)\right| dy \\
& \hspace{0.5cm}= \sigma^{-2} \int_\R \exp\left(\int_0^y 2\sigma^{-2} b_0(u) du \right) \left|\exp\left( \int_0^y 2\sigma^{-2} g_j^w(u) du \right) - \exp\left(\int_0^y 2\sigma^{-2} g_j^{w'}(u) du \right)\right| dy\\
&\hspace{0.5cm} \leq C_{b_0,\sigma} \left\|\exp\left( \int_0^\cdot 2\sigma^{-2} g_j^w(u) du \right) - \exp\left(\int_0^\cdot 2\sigma^{-2} g_j^{w'}(u) du \right)\right\|_\infty
\end{align*}
So $|C_{b_j^w, \sigma} - C_{b_j^{w'}, \sigma}|<\epsilon$ if the last supremum norm ist $<\frac{\epsilon}{C_{b_0,\sigma}}$ which can be archived for $\|g_j^w - g_j^{w'}\|_\infty = \|b_j^w - b_j^{w'}\|_\infty$ small enough according to the first part of (b).

\item[(c)] We add zero and get
\[ \left| \rho_{b_j^w}(y_j^w) - \rho_{b_j^{w'}}(y_j^{w'}\right| \leq \left| \rho_{b_j^w}(y_j^w) - \rho_{b_j^w}(y_j^{w'})\right| + \left| \rho_{b_j^w}(y_j^{w'}) - \rho_{b_j^{w'}}(y_j^{w'})\right|.\]
For arbitrary $\epsilon>0$ and $|y_j^w - y_j^{w'}|<\delta$, $\delta>0$ appropriate, the first summand can be chosen $\leq\epsilon$ as evaluation of a continuous function is a continuous mapping. The same holds trivially true for the second summand for $\| \rho_{b_j^w}-\rho_{b_j^{w'}}\|_\infty< \epsilon$.
\end{itemize}

We now turn to the statement $(2)$. From Lemma \ref{bound_invariant_density} we know that there exists a constant $L^*=L^*(C,A,\gamma,\sigma)$ such that for every drift function $b\in\Sigma(C,A,\gamma,\sigma)$ we have $\|\rho_b\|_\infty\leq L^*$. Set
\[ I := \left[\frac14 \min_{-A\leq x\leq A}\rho_{b_0}(x) , L^*\right] =: [L_*, L^*]. \]
Now we want to show that for large enough $T$ this interval fulfills $f(I)\subset I$. Choose $w\in [L_*,L^*]$. If $T$ is large enough to ensure
\[ L (h_T^w)^\beta = c_* \left(\frac{\log T}{Tw}\right)^\frac{\beta}{2\beta+1} \leq  c_* \left(\frac{\log T}{TL_*}\right)^\frac{\beta}{2\beta+1}  \leq \frac{C}{2}\]
we know by Lemma \ref{lemma_cond_1} that $b_j^w\in\Sigma(C,A,\gamma,\sigma)$ and hence 
\[ \rho_{b_j^w}(y_j^w) \leq \| \rho_{b_j^w}\|_\infty \leq L^*.\]
For the lower bound first note that due to $\|K\|_\infty\leq 1$
\[ \left| \int_0^x g_j^w(y) dy\right| \leq \int_0^{|x|} g_j^w(y) dy \leq \int_{-A}^A g_j^w(y) dy \leq 2A L(h_T^w)^\beta \leq 2AL (h_T^{L_*})^\beta.\]
So we may choose $T\geq T_0$ large enough such that $2AL(h_T^{L_*})^\beta\leq \min\left\{ \frac{\sigma^2\log 2}{2}, \log 2\right\}$. Then we have for the constant 
\begin{align*}
C_{b_j^w,\sigma} &= \sigma^{-2}\int_\R \exp\left( \int_0^y 2\sigma^{-2}b_0(u) du \right)\exp\left( \int_0^y 2\sigma^{-2} g_j^w(u) du \right) dy\\
&\leq  \exp\left(4\sigma^{-2} AL(h_T^{L_*})^\beta\right) \int_\R \sigma^{-2}\exp\left( \int_0^y 2\sigma^{-2} b_0(u) du \right) dy\\
&\leq 2 C_{b_0,\sigma}
\end{align*}
or equivalently, $(\sigma^2 C_{b_j^w, \sigma})^{-1} \geq \frac12 (\sigma^2 C_{b_0,\sigma})^{-1}$. By the same argument and the same choice of $T\geq T_0$ we get
\begin{align*}
\exp\left( \int_0^{y_j^w} b_j^w(y) dy\right) &= \exp\left( \int_0^{y_j^w} b_0(x) dx\right)\exp\left( \int_0^{y_j^w} g_j^w(y) dy\right)\\
& \geq \exp\left( \int_0^{y_j^w} b_0(x) dx\right) \exp\left(-\log 2\right).
\end{align*} 
Combining this, we get
\begin{align*}
\rho_{b_j^w}(y_j^w) &= \frac{1}{C_{b_j^w, \sigma}\sigma^2} \exp\left( \int_0^{y_j^w} 2\sigma^{-2} b_j^w(u) du \right)\\
&\hspace{1cm}\geq \frac12 \frac{1}{C_{b_0,\sigma}} \exp\left( \int_0^{y_j^w} b_0(x) dx\right)\frac12= \frac14 \rho_{b_0}(y_j^w) \geq L_*.
\end{align*}  
\end{proof}





\begin{lemma}\label{lemma_E_absvalue}
Let $Z_1,\dots, Z_m$ be stricly positive, uncorrelated random variables with $\E[Z_i]=1$ for all $1\leq i\leq m$. Then for all $\epsilon>0$ and $0<\gamma\leq 1$ we have
\begin{align*}
\E\left[\left| \frac1m \sum_{i=1}^m Z_i - 1\right|\right] &\leq \sqrt{\epsilon} + \left( 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{i=1}^m \E[ Z_i^{1+\gamma}] \right)^\frac12 + 2\epsilon^{-\gamma}m^{-(1+\gamma)}\sum_{i=1}^m \E[ Z_i^{1+\gamma}].
\end{align*} 
\end{lemma}
\begin{proof}
First of all, we note that from $\E[Z_i]=0$ and the uncorrelatedness we get $\E[Z_i Z_j] =1$ for $i\neq j$.\\
With $1=\E[Z_i] = \E[ Z_i 1_{\{Z_i\leq \epsilon m\}} + Z_i 1_{\{Z_i > \epsilon m\}}] = \E[Z_i 1_{\{Z_i \leq \epsilon m\}}] + \E[Z_i 1_{\{Z_i > \epsilon m\}}]$ and the fact that $Z_i\geq 0$ we get
\begin{align*}
&\E\left[\left| \frac1m \sum_{i=1}^m Z_i -1\right|\right] \\
&\hspace{0.5cm}= \E\left[ \left| \frac1m\sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right) + \frac1m\sum_{i=1}^m \left( Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right) \right|\right] \\
&\hspace{0.5cm}\leq \frac1m\E\left[ \left| \sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right)\right|\right] + \frac1m\E\left[\left|\sum_{i=1}^m \left( Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right) \right|\right]\\
&\hspace{0.5cm}\leq \frac1m\E\left[ \left| \sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right)\right|^2\right]^\frac12 +\frac1m \E\left[\sum_{i=1}^m \left| Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right| \right]\\
&\hspace{0.5cm}\leq \frac1m \textrm{Var}\left( \sum_{i=1}^m  Z_i1_{\{Z_i \leq \epsilon m\}}\right)^\frac12 + \frac1m \E\left[ \sum_{i=1}^m \left| Z_i 1_{\{ Z_i>\epsilon m\}} \right| +  \left|\E[Z_i 1_{\{Z_i > \epsilon m\}}] \right| \right]\\
&\hspace{0.5cm}\leq \frac1m \textrm{Var}\left( \sum_{i=1}^m  Z_i1_{\{Z_i \leq \epsilon m\}}\right)^\frac12 + \frac2m \sum_{i=1}^m \E\left[ Z_i 1_{\{ Z_i>\epsilon m\}}\right]\\
&\hspace{0.5cm}= \frac1m \left( \sum_{i=1}^m \textrm{Var}\left( Z_i 1_{\{ Z_i\leq \epsilon m\}}\right) + \sum_{i,j=1}^m \textrm{Cov}\left(  Z_i 1_{\{ Z_i\leq \epsilon m\}},  Z_j 1_{\{ Z_j\leq \epsilon m\}}\right)\right)^\frac12 + \frac2m \sum_{i=1}^m \E\left[ Z_i 1_{\{ Z_i>\epsilon m\}}\right]\\
&\hspace{0.5cm} =: \frac1m\left( A_1 + A_2\right)^\frac12 + A_3.
\end{align*}
Now we treat eacht term $A_i$ seperately. As a variance the term $A_1+A_2$ is positive and it suffices to find an upper bound for it without taking the absolute value. In particular we may drop negative summands without double-checking that they are in absolute value smaller than the remaining positive ones. For the first one a bound is straightforward as
\[ A_1 \leq \sum_{i=1}^m \E\left[ Z_i^2 1_{\{ Z_i\leq \epsilon m\}}\right] \leq \epsilon m \sum_{i=1}^m \E\left[ Z_i1_{\{ Z_i\leq \epsilon m\}}\right] \leq \epsilon m\sum_{i=1}^m \E[Z_i] = \epsilon m^2.\]
For the second term we first note that 
\[1_{\{ Z_i\leq \epsilon m\}} = 1-1_{\{ Z_i> \epsilon m\}}\]
and similarly
\begin{align*}
1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}} &= 1- 1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j > \epsilon m\}} - 1_{\{ Z_i> \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}}-1_{\{ Z_i> \epsilon m\}}1_{\{ Z_j> \epsilon m\}}\\
&=: 1- A_{ij}.
\end{align*} 
Now we can start with
\begin{align*}
A_2 &= \sum_{i,j=1}^m \E\left[ Z_iZ_j 1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}}\right]  - \E\left[Z_i1_{\{ Z_i\leq \epsilon m\}}\right]\E\left[Z_j1_{\{ Z_j\leq \epsilon m\}}\right] \\
&= \sum_{i,j=1}^m \E\left[ Z_iZ_j ( 1- A_{ij})\right] - \E\left[ Z_i (1-1_{\{ Z_i>\epsilon m\}})\right]\E\left[ Z_j (1-1_{\{ Z_j> \epsilon m\}})\right]\\
&= -\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] + \sum_{i,j=1}^m \E[Z_iZ_j] - \left( \E[Z_i] - \E[Z_i1_{\{ Z_i>\epsilon m\}}]\right)\left(\E[Z_j] - \E[Z_j1_{\{ Z_j> \epsilon m\}}]\right)\\
&=-\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] + \sum_{i,j=1}^m 1- \left( 1 - \E[Z_i1_{\{ Z_i>\epsilon m\}}]\right)\left(1- \E[Z_j1_{\{ Z_j> \epsilon m\}}]\right)\\
&= -\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right]\\
&\hspace{1cm} + \sum_{i,j=1}^m  1- \left( 1- \E[Z_i1_{\{ Z_i>\epsilon m\}}]-\E[Z_j1_{\{ Z_j>\epsilon m\}}] + \E[Z_i1_{\{ Z_i>\epsilon m\}}]\E[Z_j1_{\{ Z_j>\epsilon m\}}]\right)\\
&= - \sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] +\E[Z_i1_{\{ Z_i>\epsilon m\}}]\E[Z_j1_{\{ Z_j>\epsilon m\}}] + \sum_{i,j=1}^m  \E[Z_i1_{\{ Z_i>\epsilon m\}}]+\E[Z_j1_{\{ Z_j>\epsilon m\}}] 
\end{align*}
As $Z_i\geq 0$ and $A_{i,j}\geq 0$ the first of the summands is negative and we get
\[ A_2 \leq \sum_{i,j=1}^m  \E[Z_i1_{\{ Z_i>\epsilon m\}}]+\E[Z_j1_{\{ Z_j>\epsilon m\}}] = 2m\sum_{i=1}^m \E[Z_i1_{\{ Z_i>\epsilon m\}}]. \]
Now we use the indicator in the last remaining expectation to estimate for $0<\gamma\leq 1$
\[ \E[Z_i1_{\{ Z_i>\epsilon m\}}]j \leq (\epsilon m)^{-\gamma} \E\left[Z_i^{1+\gamma}1_{\{ Z_i>\epsilon m\}}\right]\leq  (\epsilon m)^{-\gamma} \E\left[Z_i^{1+\gamma}\right]. \]
Altogether we arrive at 
\[ A_2 \leq 2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right].\]
Using $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for $a,b\geq 0$ we finally get
\begin{align*}
\frac1m(A_1 + A_2)^\frac12 &\leq \frac1m\left( \epsilon m^2 + 2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12\\
&\leq \frac1m\left( \sqrt{\epsilon} m + \left(2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12 \right)\\
&= \sqrt{\epsilon} + \left( 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12
\end{align*}
which are exactly the first to summands in the assertion of the lemma. We close the proof by the estimation of $A_3$. But here we simply use the same trick with $0<\gamma\leq 1$ and directly get
\[ A_3 \leq 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{k=1}^m \E\left[Z_i^{1+\gamma}\right].\]
\end{proof}





Within the proof of the sharp lower bound, we will make use of the following:

\begin{proposition}\label{moments_local-invariant}
Let $X$ be a diffusion with $b\in\Sigma(C,A,\gamma,\sigma)$. Then there exist constants $c_1, c_2>0$m such that, for any $p, T\geq 1$, 
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \left(\E_{b}\left[ \left\| \frac1T L_T(X) - \rho_b\right\|_\infty^p\right]\right)^\frac1p \leq c_1\left( \frac{p}{T} + \frac{1}{\sqrt{T}}\left( 1+ \sqrt{p} + \sqrt{\log T}\right) + Te^{-c_2T}\right).\]
\end{proposition}
\begin{proof}
See Willems/Strauch, Lemma 43 in Dissertation....check for the paper!!!
\end{proof}




\begin{proof}[Proof of the sharp lower bound]
We first begin building our hypothesis. $b_0$ and $h_T^w$ are chosen as above and we proceed inductively:
\begin{itemize}
\item In the first step we set $y_1^w := -A + h_T^w$. Then by Lemma \ref{lemma_fixed_point} there exists $w_1>0$ such that $\rho_{b_j^{w_1}}(y_j^{w_1}) = w_1$ and we set $b_1 := b_1^{w_1}$, $y_1:=y_1^{w_1}$. Clearly, the support of $b_1-b_0$ is given by $[-A, -A + 2h_T^{w_1}] = [y_j-h_T^{w_1}, y_j+h_T^{w_1}]$.
\item If $b_j$ is constructed with $y_j$ we put $y_{j+1}^w := y_j + h_T^{w_j}+ h_T^w$. Again Lemma \ref{lemma_fixed_point} ensures existance of $w_{j+1}>0$ with $\rho_{b_{j+1}^{w_{j+1}}}(y_{j+1}^{w_{j+1}}) = w_{j+1}$ and we set $b_{j+1} := b_{j+1}^{w_{j+1}}, y_{j+1}:= y_{j+1}^{w_{j+1}}$. The support of $b_{j+1}-b_0$ is given by $[y_j + h_T^{w_j}, y_j + h_T^{w_j}+2h_T^{w_{j+1}}] = [y_{j+1}- h_T^{w_{j+1}}, y_{j+1}+h_T^{w_{j+1}}]$ and hence is disjoint of all $b_j-b_0$ constructed before.
\item The construction ends when for the first time the right endpoint of the newly constructed interval $[y_N - h_T^{w_N}, y_N+h_T^{w_N}]$ is greater than $A$.
\end{itemize}
From Lemma \ref{bound_invariant_density} we get a constant $L^* =L^*(C,A.\gamma,\sigma)$ such that every drift $b\in\Sigma(C,A,\gamma,\sigma)$ admits an invariant density $\rho_b$ with $\|\rho_b\|_\infty\leq L^*$. In particular, we have $w_j\leq L^*$ for all $j=1,\dots, N$. Next, we specify $N$. From the construction of the hypothesis we have $2A \geq \sum_{j=1}^N 2h_T^{w_j}$. Hence, 
\begin{align*}
A \geq \sum_{j=1}^N h_T^{w_j} &= \sum_{j=1}^N \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{Tw_j}\right)^{\frac{1}{2\beta +1}} \\
&= \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{T}\right)^{\frac{1}{2\beta +1}} \sum_{j=1}^N \left(\frac{1}{w_j}\right)^{\frac{1}{2\beta +1}}\\
&\geq \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{T}\right)^{\frac{1}{2\beta +1}} N \left(\frac{1}{L^*}\right)^{\frac{1}{2\beta+1}}.
\end{align*}
This can be transformed into an inequality of the form $N\leq\dots$ and from our construction algorithm we know that $N$ is the largest integer fullfilling this inequality, thus
\[ N =N_T = \left\lfloor \frac{A}{(L^*)^{\frac{1}{2\beta+1}}} \left(\frac{L}{c^*}\right)^\frac{1}{\beta}\left(\frac{T}{\log T}\right)^{\frac{1}{2\beta +1}} \right\rfloor.\]
Before we proceed, we fix the notation 
\[ A_{T,j} := (1-\epsilon_T) L\left( h_T^{w_j}\right)^\beta\quad \textrm{ and }\quad K_j(\cdot) := K_{y_j, h_T^{w_j}}(\cdot)\]
so we can write $b_j = b_0 + A_{T,j} K_j$.\\


Now, let $\phi$ be test with $\E_{b_0}[\phi]\leq\alpha$. Then we have
\begin{align*}
\inf_{b\in\Sigma(\beta, L): \|(b-b_0)\phi_b^{\beta/(2\beta+1)}\|_\infty\geq (1-\epsilon_T)c_* \delta_T} \E_b[\phi] - \alpha &\leq \min_{1\leq k\leq N} \E_{b_k}[\phi] - \E_{b_0}[\phi]\\
&\leq \E_{b_0}\left[ \left(\frac1N \sum_{k=1}^N \frac{d\Pr_{b_k}}{d\Pr_{b_0}}(X) - 1\right) \phi\right]\\
&\leq  \E_{b_0}\left[ \left| \frac1N \sum_{k=1}^N \frac{d\Pr_{b_k}}{d\Pr_{b_0}}(X) - 1\right|\right].
\end{align*}
For ease of notation we introduce
\[ Z_k := \frac{d\Pr_{b_k}}{d\Pr_{b_0}} (X) \]
and note that $\E_{b_0}[Z_k] = 1$ for each $1\leq k\leq N$. Furthermore, the $Z_k$ are pairwise uncorrelated. To see this, we calculate $\E_{b_0}[Z_iZ_j]$ for $i\neq j$. In this case we have $K_i(X_s) K_j(X_s) =0$ as the supports of $K_i$ and $K_j$ are disjoint which will be used in the third step:
\begin{align*}
\E_{b_0}[Z_i Z_j] &= \E_{b_0}\left[ \exp\left( \int_0^T A_{T,i} K^i(X_s) dW_s - \frac12\int_0^T A_{T,i}^2 K_i^2(X_s)^2 ds\right) \right.\\
&\hspace{1.5cm} \cdot\left. \exp\left( \int_0^T A_{T,j}K_j(X_s) dW_s - \frac12\int_0^T A_{T,j}^2 K_j(X_s)^2 ds\right)\right]\\
&= \E_{b_0}\left[ \exp\left( \int_0^T \left(A_{T_i}K_i(X_s) + A_{T_j}K_j(X_s)\right) dW_s \right.\right.\\
&\hspace{2.5cm}  \left.\left. - \frac12\int_0^T \left( A_{T,i}^2 K_i(X_s)^2 + A_{T,j}^2 K_j(X_s)^2 \right) ds\right)\right]\\
&= \E_{b_0}\left[ \exp\left( \int_0^T \left(A_{T_i}K_i(X_s) + A_{T_j}K_j(X_s)\right) dW_s \right.\right.\\
&\hspace{2.5cm}  \left.\left. - \frac12\int_0^T \left( A_{T,i} K_i(X_s) + A_{T,j} K_j(X_s) \right)^2 ds\right)\right].
\end{align*}
But this last expression is again a Girsanov-density and hence its expectation equals one. Consequently, 
\[ \textrm{Cov}(Z_i, Z_j) = \E_{b_0}[Z_i Z_j] - \E_{b_0}[Z_i]\E_{b_0}[Z_j] = 1-1^2 =0.\]
We thus may apply Lemma \ref{lemma_E_absvalue} and it remains to show that
\[ N^{-(1+\gamma)} \sum_{k=1}^N \E_{b_0}\left[ Z_k^{1+\gamma}\right] \rightarrow 0\]
for a suitable choice of $0<\gamma\leq 1$ and asymptotic $T\to\infty$. In a first step, we investigate one single summand $\E_{b_0}[ Z_k^{1+\gamma}]$. We have
\[ \E_{b_0}[ Z_k^{1+\gamma}] = \E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k} K_k(X_s) dW_s - \frac{1+\gamma}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right)\right].\]
We now split the second integral in the exponen and get with the occupation times formula in the second step
\begin{align*}
&-\frac{1+\gamma}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\\
&\hspace{0.5cm}= -\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac12 ((1+\gamma)^2 - 1-\gamma) \int_0^T A_{T,k}^2 K_k(X_s)^2 ds\\
&\hspace{0.5cm}=-\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\frac1T L_T^z(X) dz\\
&\hspace{0.5cm} = -\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\rho_{b_0}(y) dz \\
&\hspace{1.5cm} + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz \\
&\hspace{1.5cm}+ \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right)dz
\end{align*}
Inserting into the formula for $\E_{b_0}[Z_k^{1+\gamma}]$ and pulling the non-random factors out of the integral this leads to
\begin{align*}
\E_{b_0}[Z_k^{1+\gamma}] &= A_1\cdot A_2 \cdot \E\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k} K_k(X_s) dW_s - \frac{(1+\gamma)^2}{2} \int_0^T A_{T,k}^2 K_k(X_s)^2 ds \right.\right.\\
&\hspace{3cm}\left.\left.+ \frac12\gamma(1+\gamma)T\int_0^T A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz\right)\right]
\end{align*}
where 
\begin{align*}
A_1 &:= \exp\left( \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\rho_{b_0}(y) dz\right)\quad \textrm{ and }\\
A_2 &:=\exp\left(  \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right)dz\right).
\end{align*}
To further evaluate the term within the expectation we again add a suitable zero. Therefore, pick $p=p_T>1$ that will be specified later and the corresponding $q=q_T$ with $\frac1p+\frac1q =1$. Then we write the expectation in the following form
\begin{align*}
&\E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right.\\
&\hspace{1cm}  \cdot\exp\left( \frac12 (p-1)(1+\gamma)^2 \int_0^T A_{T,k}^2 K_k(X_s)^2 ds \right.\\
&\hspace{2.5cm} \left.\left. + \frac12\gamma(1+\gamma)T \int_\R A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz\right)\right]\\
&= \E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right.\\
&\hspace{1.5cm} \cdot \exp\left( \frac12 (p-1) (1+\gamma)^2 T \int_\R A_{T,k}^2 K_k(z)^2 \rho_{b_0}(y) dz \right.\\
&\hspace{2cm} \left. \left. +\left( \frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) T \int_\R A_{T,k}^2 K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]
\end{align*}
where we used the occupation times formula again in the second step and split $\frac1T L_T^z(X) = \rho_{b_0}(z) + \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right)$. Pulling out the non-random factor and applying Hölder's inequality yields
\[ \E_{b_0}[Z_k^{1+\gamma}]  = A_1\cdot A_2\cdot A_3\cdot A_4\cdot A_5,\]
where
\begin{align*}
A_3 &:= \E_{b_0}\left[ \exp\left( p(1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p^2(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right]^\frac1p, \\
A_4&:= \exp\left( \frac12 (p-1) (1+\gamma)^2 T \int_\R A_{T,k}^2 K_k(z)^2 \rho_{b_0}(y) dz \right),\quad \textrm{ and } \\
A_5&:= \E_{b_0}\left[ \exp\left( q\left(\frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) T \int_\R A_{T,k}^2 K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]^\frac1q
\end{align*}
The most interesting term will be $A_1$ and we consider it later within the sum (remember that we still just treat $Z_k^{1+\gamma}$ for some fixed $k$ here). The terms $A_2,\dots, A_5$ on the other side will turn out to be bound constants:
\begin{itemize}
\item[$A_2:$] According to Lemma \ref{bound_invariant_density} the invariant density is Lipschitz with constant $L^*$. Hence, on the support of $K_k$ we have $|\rho_{b_0}(y)-\rho_{b_0}(z)|\leq 2L^* h_T^{w_k}$. Hence,
\begin{align*}
A_2 &= \exp\left( \frac12\gamma(1+\gamma)T A_{T,k}^2 \int_\R K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right) dz\right)\\
&\leq  \exp\left( \frac12\gamma(1+\gamma)T A_{T,k}^2 \int_\R K_k(z)^2 \left|\rho_{b_0}(z) - \rho_{b_0}(y)\right| dz\right)\\
&\leq \exp\left( \frac12\gamma(1+\gamma) T A_{T,k}^2 2L^*(h_T^{w_k})^2 \|K\|_{L^2}^2\right)\\
&= \exp\left( \gamma(1+\gamma) \|K\|_{L^2}^2 L^* L^2 (1-\epsilon_T)^2 T (h_T^{w_k})^{2\beta+2}\right)\\
&= \exp\left(\gamma(1+\gamma) \|K\|_{L^2}^2L^* L^2 (1-\epsilon_T)^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} Th_T^{w_k} \frac{\log T}{T \rho_{b_k(y_k)}}\right).
\end{align*}
This term converges to one, as the exponent goes to zero due to the fact that $(1-\epsilon_T)\rightarrow 1$ and $h_T^{w_k} \log T\rightarrow 0$ as 
\[ h_T^{w_k} \log T \asymp \left( \frac{\log T}{T}\right)^{\frac{1}{2\beta+1}} \log T = T^{-\frac{1}{2\beta+1}} \left( \log T\right)^{\frac{2\beta +2}{2\beta +1}}.\]
\item[$A_3:$] For every $T$ the term $A_3$ is the expectation of a Girsanov-density and hence by martingale arguments it equals one, i.e. $A_3 =1$.
\item[$A_4:$] Here we use again Lemma $\ref{bound_invariant_density}$ to get $\|\rho_{b_0}\|_\infty\leq L^*$. Then we estimate
\begin{align*}
A_4 &= \exp\left( \frac12 (p-1) (1+\gamma)^2 T A_{T,k}^2 \int_\R K_k(z)^2 \rho_{b_0}(z) dz\right)\\
&\leq \exp\left( \frac12 (p-1)(1+\gamma)^2 L^* \|K\|_{L^2}^2 T A_{T,k}^2 h_T^{w_k}\right)\\
&= \exp\left( \frac12 (1+\gamma)^2 L^* \|K\|_{L^2}^2 L^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} \rho_{b_0}(y_k)^{-1} T(p-1)\frac{\log T}{T}\right).
\end{align*}
The last exponent converges to zero if $(p-1)\log T\rightarrow 0$ which is for example true, if we set 
\[ p= p_T = 1+ T^{-\frac14}.\]
Especially, $p>1$ which is import as we applied the Hölder inequality for it. Of course, many other choices of $p$ would do the same job here, but will see in the next step, that $p$ mustn't be too close to one and our choice perfectly applies for both $A_4$ and $A_5$.
\item[$A_5:$] In this case we have
\begin{align*}
A_5 &= \E_{b_0}\left[ \exp\left( q\left(\frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) TA_{T,k}^2 \right. \right. \\
&\hspace{1.5cm} \left. \left. \cdot \int_\R  K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]^\frac1q\\
&\leq \E_{b_0}\left[ \exp\left( \frac12(1+\gamma) q ((p-1)(1+\gamma) + \gamma) TA_{T,k}^2 h_T^{w_k} \|K\|_{L^2}^2 \left\|\frac1T L_T(X) - \rho_{b_0}\right\|_{\infty}\right) \right]^\frac1q \\
&= \E_{b_0}\left[ \exp\left( \tilde{c} c_p \log T \left\|\frac1T L_T(X) - \rho_{b_0}\right\|_{\infty}\right)\right]^\frac1q
\end{align*}
with
\begin{align*}
\tilde{c} &:= \frac12(1+\gamma)\|K\|_{L^2}^2 L^2\left(\frac{c_*}{L}\right)^\frac{1}{2\beta +1}\rho_{b_0}(y_k)^{-1}, \\
c_{p}&:= q((p-1)(1+\gamma) + \gamma).
\end{align*}
Note in the latter case that $q$ is determined by $p$ as its conjugate. By a series expanison of $\exp$ and dominated convergence \textbf{check applicability!!} as well as an application of Proposition \ref{moments_local-invariant} we get for the expectation
\begin{align*}
&\E_{b_0}\left[ \exp\left( \tilde{c} c_p \log T \left\|\frac1T L_T^z(X) - \rho_{b_0}(z)\right\|_{\infty}\right)\right]\\
&\hspace{1cm} =\E_{b_0}\left[ \sum_{k=0}^\infty\frac{(\tilde{c}c_p \log T\|\frac1T L_T - \rho_{b_0}\|_\infty )^k}{k!}\right]\\
&\hspace{1cm} = \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} \E_{b_0}\left[\left\|\frac1T L_T(X) - \rho_{b_0}\right\|_\infty^k\right]\\
&\hspace{1cm}\leq \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} c_1^k\left( \frac{k}{T} + \frac{1}{\sqrt{T}}\left( 1+\sqrt{k} + \sqrt{\log T}\right) + Te^{-c_2T}\right)^k \\
&\hspace{1cm}\leq \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} c_1^k k^k \left( \frac1T + \frac{1}{\sqrt{T}}\left( 2+\sqrt{\log T}\right) + Te^{-c_2T}\right)^k\\
&\hspace{1cm} = \sum_{k=0}^\infty\frac{k^k}{k!} (\tilde{c}c_1)^k (c_pB_T)^k 
\end{align*}
with
\[ B_T = \frac{\log T}{T} + \frac{\log T}{\sqrt{T}} \left( 2+\sqrt{\log T}\right) + T\log T e^{-c_2T}.\]
By Stirling's formula we get for $k\geq k_0$ that 
\[ \frac{k^k}{k!} = \frac{k^k}{\sqrt{2\pi k} k^k e^{-k}} = \frac{e^k}{\sqrt{2\pi k}} \leq e^k.\]
Moreover, we remember $p=p_T= 1+T^{-\frac14}$ from the term $A_4$. This choice gives $q = \frac{p}{p-1} = 1+ T^{\frac14}$ and 
\[c_p = (1+T^{-\frac14})(1+\gamma) + (1+T^{\frac14})\gamma \leq 2(1+\gamma)(1+T^\frac14).\]
Thus there exists a constant $C_{k_0}\geq 1$ such that after inserting all this we end up with
\begin{align*}
\sum_{k=0}^\infty\frac{k^k}{k!} (\tilde{c}c_1)^k (c_pB_T)^k& \leq C_{k_0} \sum_{k=0}^\infty (\tilde{c}c_1 e)^k\left( 2(1+\gamma)(1+T^\frac14) B_T\right)^k\\
&= C_{k_0} \sum_{k=0}^\infty (2(1+\gamma)\tilde{c}c_1 e)^k C_T^k,
\end{align*}
where
\[ C_T := (1+T^\frac14)B_T = \frac{\log T(1+T^\frac14)}{T} + \frac{\log T (1+T^\frac14)}{\sqrt{T}}\left( 2+\sqrt{\log T}\right) + T (1+T^\frac14) \log T e^{-c_2 T}.\]
The important feature now is that $C_T\rightarrow 0 $ for $T\to\infty$ and we have shown so far
\[ A_5 \leq \left( C_{k_0} \sum_{k=0}^\infty (2(1+\gamma)\tilde{c}c_1 e)^k C_T^k\right)^{\frac{1}{1+T^\frac14}}.\]
As the term within the bracket is greater than one, we can upper bound the whole expression by forgetting the exponent which is stricly smaller than one. Now it is time to choose $T$ large enougt such that $C_T\leq 2(1+\gamma)\tilde{c}c_1 e$. Then we have
\begin{align*}
A_5\leq C_{k_0}\sum_{k=0}^\infty \left( 2(1+\gamma)\tilde{c}c_1 eC_T\right)^k = \frac{C_{k_0}}{1-2(1+\gamma)\tilde{c}c_1 e C_T} \stackrel{T\to\infty}{\longrightarrow} C_{k_0}.
\end{align*}
\end{itemize}
Summing up, we have shown so far, that there exists a constant $C>1$ not depending on $k$ such that
\[ \E_{b_0}\left[ Z_k^{1+\gamma}\right]\leq C A_1 = C\exp\left( \frac{T}{2}\gamma(1+\gamma) A_{T,k}^2 \rho_{b_0}(y_k) \int_\R K_k(z)^2 dz\right).\] 
Next, we analyse the deterministic exponent and plug in the definition of $A_{T,k}$ and $K_k$. This yields
\begin{align*}
&\frac12\gamma(1+\gamma)\rho_{b_0}(y) T A_{T,k}^2 \int_\R K_k(z)^2 dz \\
&\hspace{1cm}  = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) T A_{T,k}^2 h_T^{w_k} \|K\|_{L^2}^2\\
&\hspace{1cm} = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) \|K\|_{L^2}^2 L^2 (1-\epsilon_T)^2 T (h_T^{w_k})^{2\beta+1}\\
&\hspace{1cm} = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) \|K\|_{L^2}^2 L^2 (1-\epsilon_T)^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} T\frac{\log T}{T\rho_{b_k}(y_k)}\\
&\hspace{1cm} =\frac12\gamma(1+\gamma)\|K\|_{L^2}^2 L^{2-\frac{2\beta+1}{\beta}} \frac{2L^{\frac{1}{\beta}}}{(2\beta+1)\|K\|_{L^2}^2} \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)} (1-\epsilon_T)^2 \log T\\
&\hspace{1cm}= \gamma(1+\gamma) \frac{1}{2\beta+1} \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}  (1-\epsilon_T)^2 \log T.
\end{align*}
It remains to show that the fraction of the two density is close enough to one. Thins also get easier, if we can express its order in $T$ without dependence on $k$. We have
\[ \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}  = \frac{C_{b_k,\sigma}}{C_{b_0,\sigma}} \exp\left(2\sigma^{-2}\int_0^{y_k} (b_0- b_k)(y) dy\right).\] 
By the same arguments as in step $(2)$ in the proof of Lemma  \ref{lemma_fixed_point} we see that the exponent is bounded by $c\left(\frac{\log T}{T}\right)^{\frac{\beta}{2\beta+1}}=ca_T$ for some constant $c>0$ and thus $\exp\left(2\sigma^{-2}\int_0^{y_k} (b_0- b_k)(y) dy\right) = 1+o_T(a_T)$. In the same proof we find
\[ C_{b_0,\sigma} \exp\left( -4\sigma^2 AL h_T^{w_k}\right) \leq C_{b_k,\sigma} \leq C_{b_0,\sigma} \exp\left( 4\sigma^2 AL h_T^{w_k}\right)\]
and with the same argument as above we see that $\frac{C_{b_k,\sigma}}{C_{b_0,\sigma}} = 1+o_T(a_T)$. We conclude
\[ \left|  \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}   -1\right| = o_T (a_T).\]
Now every ingredient is prepared and we finalize the proof. Remember that $N_T = c\left(\frac{T}{\log T}\right)^{\frac{1}{2\beta +1}}$ for some constant $c>0$. Then we have 
\begin{align*}
&N^{-(1+\gamma)} \sum_{k=1}^N \E_{b_0}\left[ Z_k^{1+\gamma}\right] \\
&\hspace{1cm}\leq CN^{-\gamma} \exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T))  (1-\epsilon_T)^2 \log T\right)\\
&\hspace{1cm}= C\exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T)) (1-\epsilon_T)^2 \log T - \gamma\log N\right)\\
&\hspace{1cm} = C\exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T))  (1-\epsilon_T)^2 \log T \right.\\
&\hspace{3.5cm} \left. - \gamma\frac{1}{2\beta+1}\left( \log T - \log\log T + \log c\right)\right)
\end{align*}
Set $\gamma=\epsilon_T$ we have $(\gamma(1+\gamma)(1-\epsilon_T)^2 = \epsilon_T - \epsilon_T^2 - \epsilon_T^3 + \epsilon_T^4$ and hence the last expression equals
\begin{align*}
C \exp\left(  \frac{1}{2\beta+1}\left( \left( o_T(a_T) - \epsilon_T^2 + o_T(\epsilon_T^3)\right)\log T - \epsilon_T\log\log T +\epsilon_T\log c\right)\right).
\end{align*}
Looking after the definition of $a_T$ we see that $o_T(a_T)\log T = o_T(1)$ and from the choice of $\epsilon_T$ we get $\epsilon_T^2\log T\rightarrow \infty$ and hence the whole expression tends to zero as the exponent converges to $-\infty$.
\end{proof}







\newpage

\subsubsection{Weak convergence}

We define $\mathcal{T}=  [-A,A]\times (0,1)$ and the processes $(Z_T(y,h))_{(y,h)\in\mathcal{T}}$ and $(Z(y,h))_{(y,h)\in\mathcal{T}}$ by
\[Z_T(y,h) := \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} \]
and
\[ Z(y,h) := \frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_{b_0}(z)} dW_z}{\| K_{y,h} \sqrt{\rho_{b_0}}\|_{L^2} }\]
where $(W_z)_{z\in [-A,A]}$ is a standard Brownian motion.\\
We remember
\[ \rho_T ((y,h), (y',h'))^2 = \frac1T \int_0^T \left( K_{y,h}(X_s) - K_{y',h'}(X_s)\right)^2 ds\]
and we define
\[ \rho((y,h), (y',h'))^2 = \int_\R \left( K_{y,h}(z) - K_{y',h'}(z)\right)^2 \rho_{b_0}(z) dz.\]



We will make use of the following result \textbf{(cite from anywhere, maybe Kutoyants)}.

\begin{proposition}\label{central_limit_diffusion}
Let $X$ be a diffusion with drift $b\in\Sigma(C,A,\gamma,\sigma)$. Then for any measurable function $f:\R\rightarrow\R$ with $\int_\R f(x) \rho_{b}(x) dx$ we have
\[ \frac{1}{\sqrt{T}}\int_0^T f(X_s) dW_s\ \stackrel{\mathcal{L}}{\Longrightarrow}\ \mathcal{N}\left( 0, \int_\R f(x)^2 \rho_b(x) dx\right).\]
\end{proposition}




Now the central result of this section is the following.

\begin{thm}\label{weak_conv}
We have weak convergence of our test statistic $T(X)$ under $\Pr_{b_0}$ against
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left( \| K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}^2\right) \right).\]
\end{thm}
\begin{proof}
\textbf{Convergence of finite-dimensional distributions.} \\
We choose $(y_k, h_k)\in\mathcal{T}$, $1\leq k\leq N$. To investigate the weak convergence of $(Z_T(y_1,h_1),\dots, Z_T(y_N, h_N))$ to $(Z(y_1,h_1),\dots, Z(y_N,h_N))$ we first use the Cramer-Wold device for the nominators. So let $t_1,\dots, t_n\in\R$ be arbitrary real numbers. Then we have by Proposition \ref{central_limit_diffusion}
\begin{align*}
&\sum_{k=1}^N t_k \frac{1}{\sqrt{T}} \int_0^T K_{y_k,h_k}(X_s) dW_s = \frac{1}{\sqrt{T}} \int_0^T \left( \sum_{k=1}^N t_k K_{y_k,h_k}(X_s)\right) dW_s\\
&\hspace{2cm} \stackrel{\mathcal{L}}{\Longrightarrow} \mathcal{N}\left( 0, \int_\R \left( \sum_{k=1}^N t_k K_{y_k,h_k}(x)\right)^2 \rho_{b_0}(x) dx\right).
\end{align*}
This distribution equals the distribution of
\[ \sum_{k=1}^N t_k \int_{-A}^A K_{y_k,h_k}(z) \sqrt{\rho_{b_0}(z)} dW_z = \int_{-A}^A \left( \sum_{k=1}^N t_k K_{y_k,h_k}(z) \right) \sqrt{\rho_{b_0}(z)} dW_z \]
which can be seen easily by Ito's isometry. Hence, 
\begin{align*}
&X_T := \left( \frac{1}{\sqrt{T}} \int_0^T  K_{y_1,h_1}(X_s) dW_s, \dots, \frac{1}{\sqrt{T}} \int_0^T  K_{y_N,h_N}(X_s) dW_s\right) \\
&\hspace{1cm} \stackrel{\mathcal{L}}{\Longrightarrow} \left( \int_{-A}^A K_{y_1,h_1}(z) \sqrt{\rho_{b_0}(z)} dW_z, \dots, \int_{-A}^A K_{y_N,h_N}(z) \sqrt{\rho_{b_0}(z)} dW_z \right)=:X.
\end{align*}
Furthermore, the vectors of the denominators converge almost surely, i.e.
\begin{align*}
&Y_T := \left( \sqrt{\frac1T \int_0^T K_{y_1,h_1}(X_s)^2 ds}, \dots, \sqrt{\frac1T \int_0^T K_{y_N,h_N}(X_s)^2 ds}\right)\\
&\hspace{2cm}\longrightarrow_{as} \left( \| K_{y_1,h_1}\sqrt{\rho_{b_0}}\|_{L^2},\dots, \| K_{y_N,h_N}\sqrt{\rho_{b_0}}\|_{L^2}\right) =:Y
\end{align*}
as for each $1\leq k\leq N$
\begin{align*}
&\left| \frac1T\int_0^T K_{y_k, h_k}(X_s)^2 ds - \| K_{y_k,h_k}\sqrt{\rho_{b_0}}\|_{L^2}^2\right| \\
&\hspace{1cm} = \left| \int_\R K_{y_k,h_k}(z)^2 \frac1T L_T^z(X) dz - \int_0^T K_{y_k,h_k}(z)^2 \rho_{b_0}(z) dz \right|\\
&\hspace{1cm}\leq \left\| \frac1T L_T(X) - \rho_{b_0}\right\| \int_\R K_{y_k,h_k}(z)^2 dz \rightarrow_{as} 0.
\end{align*}
By Slutzky's Lemma we then conclude $(X_T, Y_T)\stackrel{\mathcal{L}}{\Longrightarrow} (X,Y)$ and by the continuous mapping theorem we finally get
\[ (Z_T(y_1,h_1),\dots, Z_T(y_N, h_N))\stackrel{\mathcal{L}}{\Longrightarrow} (Z(y_1,h_1),\dots, Z(y_N, h_N)).\]


\textbf{Asymptotic stochastic equicontinuity}\\
By boundedness of the kernel function $K$ we see that
\[ \mathcal{F} := \left\{ \left( K_{y,h} - K_{y',h'}\right)2 \mid (y,h), (y',h')\in\mathcal{T}\right\} \]
is uniformely Glivenko-Cantelli. As $\E_{b_0}[\rho_T((y,h), (y',h'))^2] = \rho( (y,h), (y',h'))^2$ we thus get for any $\delta>0$
\[\lim_{T\to\infty} \Pr_{b_0}\left( \left\| \rho_T((y,h), (y',h'))^2 - \rho((y,h), (y',h'))^2 \right\|_{\mathcal{T}\times\mathcal{T}} >\delta\right) =0.\]
Let $\epsilon>0$. Then we have
\begin{align*}
&\Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon\right) \\
&\hspace{1cm} = \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon, \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} \leq \delta \right)\\
&\hspace{2cm} + \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon, \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} > \delta\right)\\
&\hspace{1cm} \leq\Pr_{b_0}\left( \sup_{\rho_T((y,h),(y',h'))\leq 2\delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon \right) + \Pr_{b_0}\left( \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} > \delta\right).
\end{align*} 
The latter summand is $o_{\Pr_{b_0}}$ as seen before, and by the multiscale lemma \textbf{cite!!!} we get stochastic equicontinuity of the first summand with respect to the metric $\rho_T$. Consequently, 
\[\lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon\right) =0.\]

Putting together the convergence of the finite-dimensional distributions and the asymptotic stochastic equicontinuity we get convergence in distribution of the processes indexed by $\mathcal{T}$, i.e.
\[ \left( Z_T(y,h)\right)_{(y,h)\in\mathcal{T}} \stackrel{\mathcal{L}}{\Longrightarrow} \left( Z(y,h)\right)_{(y,h)\in\mathcal{T}}.\]

Now define 
\[ \tilde{T}_T(\delta, \delta') := \sup_{(y,h)\in\mathcal{T}:\ \delta < \|K_{y,h}\|_{L^2}\leq \delta'} \left(\frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} - C\left( \frac1T \int_0^T K_{y,h}(X_s)^2 ds\right) \right) \]
as well as
\[ S(\delta, \delta') := \sup_{(y,h)\in\mathcal{T}:\ \delta < \|K_{y,h}\|_{L^2}\leq \delta'} \left(\frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_{b_0}(z)} dW_z}{\| K_{y,h} \sqrt{\rho_{b_0}}\|_{L^2} } - C\left( \| K_{y,h}\sqrt{\rho_{b_0}} \|_{L^2}^2\right) \right).\]
Applying the same Glivenko-Cantelli argument as above to $\mathcal{F}' := \left\{ K_{y,h}\mid (y,h)\in\mathcal{T}\right\}$ instead of $\mathcal{F}$ we see by the continuous mapping theorem that
\[  \sup_{(y,h)\in\mathcal{T}}\left| C\left( \frac1T \int_0^T K_{y,h}(X_s)^2 ds\right)- C\left( \| K_{y,h}\sqrt{\rho_{b_0}} \|_{L^2}^2\right) \right| \longrightarrow_{\Pr_{b_0}} 0.\]
Together with the above established weak convergence of the processes it follows for any fixed $\delta\in (0,1]$ that
\[ \tilde{T}_T(\delta,1)\ \stackrel{\mathcal{L}}{\Longrightarrow}\ S(\delta,1).\]
Again by an application of the multiscale lemma \textbf{cite!!!} we see that
\[ \lim_{\delta\searrow 0} \limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,\delta) \geq \epsilon\right) =0.\]


\textbf{Investigation of $Z(y,h)$}\\
Next, we note that we can also apply the multiscale lemma to the process $Z$ instead of $Z_T$. The requirements are easily checked for $\tilde{Z}(y,h) := \int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0}(z)} dW_z$ with semimetric $\rho$ and $\sigma(y,h) := \| K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}$ as $Z$ is Gaussian with
\[ \tilde{Z} \sim\mathcal{N}\left( 0, \|K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}^2\right).\]
First of all, this implies $S(0,1)<\infty$ almost surely and as above this gives for every $\epsilon>0$
\[ \lim_{\delta\searrow 0} \Pr_{b_0}\left( S(0,\delta)>\epsilon\right) =0.\]
For any $l\geq \lfloor \frac{1}{2A}\rfloor$ the random variables $Z_k := Z( \frac{k}{l}, \frac{1}{2l})$, $1\leq k\leq l$ are independent as the support of the functions $K_{\frac{k}{l}, \frac{1}{2l}}$ and $K_{\frac{k'}{l}, \frac{1}{2l}}$ is disjoint for $k\neq k'$. Moreover, they are standard Gaussians and hence their maximum is $(2\log l)^\frac12 + o_{\Pr}(1) = C(\frac{1}{l}) + o_{\Pr}(1)$ for $l\to\infty$. A simple substitution gives $\frac{c}{2l}=ch\leq \| K_{y,\frac{1}{2l}} \sqrt{\rho_{b_0}}\|_{L^2}^2 \leq Ch = \frac{C}{2l}$ for constants $c,C>0$ and $C$ may be chosen $\geq 1$. Then we have
\[ S(0,1) \geq \max_{1\leq k\leq l} Z_k - C\left(\frac{1}{l}\right) + o_l(1) \]
and conclude that $S(0,1)\geq 0$ almost surely, where we used that $C(\frac{C}{l}) = (2\log l + 2\log C)^\frac12 = (2\log l)^\frac12 + o_l(1)$.

\textbf{Conclusion}\\
Now the weak convergence of $\tilde{T}_T(\delta,1)$ to $S(\delta, 1)$ entail for $r>0$
\begin{align*}
&\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)>r\right) \\
&\hspace{1cm}\leq \lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(\delta,1)>r\right) +  \lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,\delta)>r\right)\\
&\hspace{1cm} \leq \lim_{\delta\searrow 0}\Pr_{b_0}\left( S(\delta,1)>r\right)\\
&\hspace{1cm} \leq \Pr_{b_0}\left( S(0,1)>r\right).
\end{align*}
Moreover, for arbitrary $\tilde{r}\in\R$ we have
\begin{align*}
\limsup_{T\to\infty}  \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq \tilde{r}\right) &\leq \inf_{\delta>0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(\delta,1)\leq \tilde{r}\right) \\
&\leq \inf_{\delta>0}\Pr_{b_0}\left( S(\delta,1)\leq \tilde{r}\right) \\
&= \Pr_{b_0}\left( S(0,1)\leq \tilde{r}\right)
\end{align*}
which in particular implies $\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq \tilde{r}\right) =0$ for $\tilde{r}<0$. Noting that this last computation also includes for $r\geq 0$
\begin{align*}
\limsup_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r) &= 1- \limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq  r\right)\\
&\geq 1- \Pr_{b_0}( S(0,1)\leq r) = \Pr_{b_0}( S(0,1)>r).
\end{align*} 
As both estimates for $\limsup_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r)$ may be repeated for $\liminf_{T\to\infty}$ we get $\lim_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r) = \Pr_{b_0}( S(0,1)>r)$ and the claim follows.
\end{proof}





\newpage

\subsubsection{Worst case for one-sided alternative}

We fix, $A,\gamma,\sigma>0$, $C\geq 1$ and set 
\[\mathcal{H}_{\leq} := \{ f\in \Sigma(C,A,\gamma,\sigma)\mid f\leq 0\textrm{ on } [-A,A]\}. \]

We want to show that an asymptotically worst case within this set of hypothesis is $f=0$ which is the reasonable expectation as it is the hypothesis closest to the alternative of functions being larger than zero anywhere within $[-A,A]$. So we remember 
\[ \mathcal{T} := (0,1]\times [-A+h, A-h] \]
and the test statistic
\[ T_b(X)  = \sup_{(y,h)\in\mathcal{T}} \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)\]
where
\[ \tilde{\Psi}_{y,h}^b(X) = \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} + \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
Clearly, the second summand is always negative for $b\in\mathcal{H}_{\leq}$ and vanishes for $b=0$, where the latter is understood as restricted to $[-A,A]$. Outside of this interval the drift clearly needs to deviate from zero in order to ensure ergodic properties of the solution or put differently, to ensure $b\in\Sigma(C,A,\gamma,\sigma)$. In this latter case we know that the invariant density $\rho_0=c$ is constant on $[-A, A]$ and hence the weak limit of the test statistic is given by
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C( \|cK_{y,h}\|_{L^2}^2)\right),\]
where
\[ Z(y,h) = \frac{\int_{-A}^A K_{y,h}(z) dW_z}{\|K_{y,h}\|_{L^2}}.\]


\begin{proposition}
For each $b\in\mathcal{H}_{\leq}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_b(X) > r\right) \leq \Pr\left( S>r\right),\]
where
\[ S := \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left(\|K_{y,h}\|_{L^2}^2\right) + C\left( (1\vee (L^*\wedge (2h)^{-1})^{-1}\right)\right).\]
\end{proposition}
\begin{proof}
Let $b\in\mathcal{H}_{\leq}$. The key idea is to split the set $\mathcal{T}$ in three parts: We choose $\delta,\epsilon>0$ and set
\begin{align*}
\mathcal{T}_1 &:= \left\{ (y,h)\in\mathcal{T} \mid h\geq\delta\textrm{ and } \min_{x\in [y-h,y+h]} \rho_b(x)b(x) < - \epsilon\right\}, \\
\mathcal{T}_2 &:_= \left\{ (y,h)\in\mathcal{T} \mid h <\delta\right\}, \textrm{ and }\\
\mathcal{T}_3 &:= \left\{ (y,h)\in\mathcal{T} \mid h\geq\delta\textrm{ and } \rho_b(x)b(x)\geq -\epsilon\textrm{ on } [y-h, y+h]\right\}.
\end{align*}
Note that all sets depend on $\delta$ and $\epsilon$. Then we have
\begin{align*}
\Pr(T_b(X)>r) &= \Pr\left( \sup_{(y,h)\in\mathcal{T}}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_1}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm}+\Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm}+\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right).
\end{align*}
Of course the inequality remains valid if we put $\lim_{\epsilon\searrow 0}\lim_{\delta\searrow 0}\lim_{T\to\infty}$ before both sides. The rationale behind the argument will be that the first probability converges to zero as the bias in $\tilde{\Psi}$ dominates the stochastic term, the second one vanishes by the multiscale lemma as in the proof of the weak convergence in Theorem \ref{weak_conv} and the last one smaller in stochastic order than $S$. Furthermore, we have seen in Theorem \ref{weak_conv} that both randoms variables $T_b(X)$ and $S$ are $\geq 0$ almost surely and it suffices to consider $r>0$(\textbf{for the first two sumands in $S$ this follows from Theorem \ref{weak_conv}, the third one is positive and bounded by a constant}).

\begin{itemize}
\item[(1)] We can bound $T_b(X)$ with the supremum taken over $\mathcal{T}_1$ by
\[ \sup_{(y,h)\in\mathcal{T}_1} \left( \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}  - C(\sigma_{y,h}^2)\right) + \sup_{(y,h)\in\mathcal{T}_1}\frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
The limit in distribution of the first term is given in Theorem \ref{weak_conv} and we are going to show that the second term converges to $-\infty$ almost surely. Then we can conclude
\[ \lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_1}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) =0.\]
First of all we write with the occupation times formula
\[ \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} = \sqrt{T}\frac{\int_\R K_{y,h}(z) b(z) \frac1T L_T^z dz}{\sqrt{\int_\R K_{y,h}(z)^2 \frac1T L_T^z dz}}.\]
We have almost sure convergence of the fraction against
\[ \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}} = \sqrt{h} \frac{\int_\R K(z) b(y+hz) \rho_b(y+hz)dz}{\sqrt{\int_\R K(z)^2 \rho_b(y+hz)dz}}\]
where equality follows from substitution. Keeping in mind that the expression is negative, upper-bounding it is the same as finding lower bounds of the absolute value. In particular, we may choose the denominator as large as possible by using the upper bound $L^*$ of the invariant density from Lemma \ref{bound_invariant_density} and choosing $h$ as small as possible. Thus we find
\[  \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}}\leq \sqrt{\delta} \left( \sqrt{L^*} \|K\|_{L^2}\right)^{-1} \int_\R K(z) b(y+hz) \rho_b(y+hz)dz.\]
From our condition on the set $\mathcal{T}_1$ we can find $z' \in [-1,1]$ such that $b(y+hz')\rho_b(y+hz')\leq -\epsilon$. As $b\rho_b$ is a continuous function on $[-A,A]$, it is uniformly continuous. Hence we find $\delta'>0$ (not depending on $y$ and $h$ which is the important part!) such that $b(y+hz)\rho_b(y+hz) <\frac{\epsilon}{2}$ for all $z$ that suffice $|y+hz' - y+hz| <\delta'$. This latter condition is equivalent to $|z-z'|\leq \frac{\delta'}{h}$. We get
\begin{align*}
\int_\R K(z) b(y+hz) \rho_b(y+hz)dz &\leq  - \frac{\epsilon}{2}\int_{B_{\frac{\delta'}{h}}(z')\cap [-1,1]} K(z) dz\\
&\leq  - \frac{\epsilon}{2}\int_{B_{\frac{\delta'}{\delta}}(z')\cap [-1,1]} K(z) dz.
\end{align*}
As $K$ is given by the triangular kernel that integral is minimized for $B_{\frac{\delta'}{\delta}}(z')\cap [-1,1] = [-1, -1+\frac{\delta'}{\delta}]$. As a triangle with both sides $\frac{\delta'}{\delta}$ its volume equals $\frac12 \left(\frac{\delta'}{\delta}\right)^2$ which finally gives
\[ \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}}\leq -\sqrt{\delta} \left( \sqrt{L^*} \|K\|_{L^2}\right)^{-1}\frac{\epsilon}{4} \left(\frac{\delta'}{\delta}\right)^2\]
and consequently
\[\sqrt{T}\frac{\int_\R K_{y,h}(z) b(z) \frac1T L_T^z dz}{\sqrt{\int_\R K_{y,h}(z)^2 \frac1T L_T^z dz}} \rightarrow_{as} -\infty.\]
As the bound derived for the second factor does not depend on the location parameters $(y,h)$ we can put the supremum before the expression and are done with the first case.

\item[(2)] As the second summand in $\tilde{\Psi}$ is negative, we may disregard it whereby we make the probability of overshooting greater and get from Theorem \ref{weak_conv} that
\begin{align*}
&\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\hspace{0.5cm}\leq \lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^0(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\hspace{0.5cm} = \Pr\left( \sup_{(y,h)\in\mathcal{T}_2} \left( \frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C(\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) >r\right)
\end{align*}
Now $\|K_{y,h}\|_{L^2}^2 = h\|K\|_{L^2}^2$ and we have in the notation of Theorem \ref{weak_conv}
\[ \lim_{\delta\searrow 0}\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \leq \lim_{\delta\searrow 0}\lim_{T\to\infty}\Pr\left( S(0,\delta)>r\right) =0.\]

\item[(3)] For the last part we first drop the condition $h\geq \delta$ and get
\[ \mathcal{T}_3\subset \left\{ (y,h)\in\mathcal{T}\mid \rho_b(x)b(x)\geq -\epsilon\textrm{ on } [y-h,y+h]\right\} =: \mathcal{T}_3'\]
which particularly implies
\begin{align*}
\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'}  \left(  \tilde{\Psi}_{y,h}^0(X) - C(\sigma_{y,h}^2) \right)>r \right),
\end{align*} 
where we again dropped the second summand of $\tilde{\Psi}$ in the second step as it is negative for $b\in\mathcal{H}_{\leq}$. By the weak limit in Theorem \ref{weak_conv}
\begin{align*}
&\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm} = \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) >r\right).
\end{align*}
Taking the limit $\lim_{\delta\searrow 0}$ doesn't change anything as neither side depends on $\delta$ and it remains to evaluate $\lim_{\epsilon\searrow 0}$.
If we write $\mathcal{T}_3'(\epsilon)=\mathcal{T}_3'$ we see that $\mathcal{T}_3'(\epsilon)\subset \mathcal{T}_3'(\epsilon')$ for $\epsilon\leq \epsilon'$ and 
\[ \lim_{\epsilon\searrow 0} \mathcal{T}_3'(\epsilon) = \left\{ (y,h)\in\mathcal{T}\mid \rho_b b=0 \textrm{ on } [y-h, y+h]\right\} =:\mathcal{T}_3''.\]
For each $(y,h)\in\mathcal{T}_3''$ we have that $\rho_b=c$ is constant on $[y-h,y+h]$ as $\rho_b'=\frac{2b\rho_b}{\sigma^2}$ and thus
\begin{align*}
&\lim_{\epsilon\searrow 0} \sup_{(y,h)\in\mathcal{T}_3'(\epsilon)} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right)\\
&\hspace{1cm} = \sup_{(y,h)\in\mathcal{T}_3''} \left(\frac{\int_{-A}^A K_{y,h}(z)dW_z}{\| K_{y,h}\|_{L^2}} - C\left( \|K_{y,h}c\|_{L^2}^2\right)\right)\\
&\hspace{1cm} \leq  \sup_{(y,h)\in\mathcal{T}_3''} \left(\frac{\int_{-A}^A K_{y,h}(z)dW_z}{\| K_{y,h}\|_{L^2}} - C\left( \|\tilde{c}K_{y,h}\|_{L^2}^2\right)\right)
\end{align*} 
with $\tilde{c} = 1\vee (L^*\wedge \frac{1}{2h})$. Here we used in the last step that $c\leq L^*$ is clear, as the invariant density is bounded by $L^*$. Furthermore, as it integrates to one, we have $2hc\leq 1\Leftrightarrow c\leq \frac{1}{2h}$. Finally, the reasoning is finished by noting that $C(\cdot)$ decreases with increasing argument. \\
For any $a>b>0$ we have $\sqrt{a-b}\geq \sqrt{a}-\sqrt{b}$ as
\[ (\sqrt{a}-\sqrt{b})^2 = a - 2\sqrt{ab}+b \leq a-2b+b = a-b.\]
By the definition of $C(\cdot)$ and the calculus rules of $\log$ we thus have
\begin{align*}
C\left( \|\tilde{c}K_{y,h}\|_{L^2}^2\right) &= \sqrt{2\log\left(\frac{1}{\tilde{c}K_{y,h}\|_{L^2}^2}\right)}\\
&= \sqrt{ 2\log\left( \frac{1}{\|K_{y,h}\|_{L^2}^2}\right) - 2\log(\tilde{c})} \\
&\geq  \sqrt{ 2\log\left( \frac{1}{\|K_{y,h}\|_{L^2}^2}\right)}  - \sqrt{2\log(\tilde{c})}\\
&= C(\|K_{y,h}\|_{L^2}^2) - C(\tilde{c}^{-1})
\end{align*}
Furthermore, we increase the random variable, by taking the supremum over a larger set, in this case $\mathcal{T}$ instead of $\mathcal{T}_3''$. This gives
\[\lim_{\epsilon\searrow 0} \sup_{(y,h)\in\mathcal{T}_3'(\epsilon)} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) \leq S.\]
Altogether, we have
\[ \lim_{\epsilon\searrow 0}\lim_{\delta\searrow 0}\lim_{T\to\infty}\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \leq \Pr\left( S>r\right).\]
\end{itemize}
\end{proof}











==> Sections/TrialsII.tex <==
\section{Trials......}



\begin{proof}[Proof of Continuity limit random variable]
We will show that the random variable
\[ S_b = \sup_{(y,h)\in\mathcal{T}}\left( \frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_b(z)} dW_z}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - C\left( \frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right)\right) \]
has not atom. Then in particular, both $U_1$ and $U_2$ have no atom and consequently, the same is true for their maximum, as for any $x\in\R$,
\[ \Pr\left( U_1\vee U_2 =x\right) \leq \Pr(U_1 =x) + \Pr(U_2=x) =0,\]
which finishes the claim.\\

First of all, $S_b$ has no positive atoms, which can be seen along the lines of the proof of Lemma~$2$ in \cite{Piterbarg} and we have to show that there is no atom in zero, i.e. $\Pr(S_b>0) =1$. 
By using $q_b\geq L_*$ from Lemma~\ref{uniform_lower_bound_invariant_density}, we find
\begin{align*}
C\left(\frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right) &= \sqrt{2\log\left(\frac{ \int_{-A}^A q_b(z) dz}{\int_{-A}^A K_{y,h}(z)^2 q_b(z) dz}\right)}\\
&\leq \sqrt{2\log\left(\frac{ \int_{-A}^A q_b(z)/L_* dz}{h \|K\|_{L^2}^2}\right)}
\end{align*}
and 
\[ S_b \geq \sup_{(y,h)\in\mathcal{T}}\left( \frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_b(z)} dW_z}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - C\left( \frac{L}{h \|K\|_{L^2}^2}\right)\right) =:\tilde{S}_b,\]
with $L=1\vee \int_{-A}^A q_b(z)/L_* dz$. 
Now, we can write
\begin{align*}
X(y,h) := \int_{-A}^A \frac{K_{y,h}(z)\sqrt{q_b(z)}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}^2} dW_z = Y_1(y,h) + h^\frac14 Y_2(y,h) 
\end{align*}
with
\begin{align*}
Y_1(y,h) &:= \frac{1}{\sqrt{h}\|K\|_{L^2}} \int_{-A}^A K_{y,h}(z) dW_z, \\
Y_2(y,h) &:= h^{-\frac14} \int_{-A}^A \left( \frac{K_{y,h}(z)\sqrt{q_b(z)}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - \frac{K_{y,h}(z)}{\sqrt{h}\|K\|_{L^2}} \right) dW_z.
\end{align*}
By Lemma~$1$ in \cite{Piterbarg}
\[ \Pr\left( \sup_{ 0\leq y\leq A-h} Y_1(y,h) > \sqrt{2\log(L/h\|K\|_{L^2}^2)} \textrm{ i.o.  as } h\searrow 0 \right) =1.\]
We now apply Lemma~\ref{lemma_H3} to this and the process $Y=Y_2$, which is possible due to Lemma~\ref{lemma_H2}, and conclude
\begin{align*}
\Pr\left( \sup_{ 0\leq y\leq A-h} X(y,h) > \sqrt{2\log(L/h\|K\|_{L^2}^2)} \textrm{ i.o.  as } h\searrow 0 \right) =1.
\end{align*}
Following the lines of the proof of Theorem~$1$ in \cite{Piterbarg} we then see
\[ \Pr(S_b >0) \geq \Pr(\tilde{S}_b >0) =1\]
and we conclude that $S_b$ has no atom in zero. 
\end{proof}






\begin{lemma}\label{lemma_H3}
Let $X(u)$ depend on a parameter $u>0$ and suppose that for all $K\geq 1$ we have
\[ \Pr\left( X(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right)=1. \]
Let $Y(u)$ be a family depending on $u>0$ and $Y^*(u) := \sup_{u'\leq u}Y(u)\in\mathcal{O}_\Pr(1)$ for $u\searrow 0$. Then for all $K\geq 1$ and $\alpha>0$,
\[ \Pr\left( X(u) + u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right)=1. \]
\end{lemma}
\begin{proof}
Let $\epsilon>0$. Choose $u_0>0$ small enough and $L>0$ large enough such that for 
\[ A_\epsilon := \left\{ \sup_{u\leq u_0} |Y(u)| \leq L\right\} >1-\epsilon.\]
\begin{align*}
&\Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right) \\
&\hspace{0.2cm} \geq \Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0, A_\epsilon\right)  \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K/u)}+u^\alpha L \textrm{ i.o.  as } u\searrow 0, A_\epsilon\right)  \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K/u)}+ u^\alpha L \textrm{ i.o.  as } u\searrow 0\right) - \Pr\left( A_\epsilon^c\right),
\end{align*}
where the last step uses
\[ \Pr(A\cap B) = \Pr(A) - \Pr(A\cap B^c) \geq \Pr(A) - \Pr(B^c).\]
Now choose $c>1$ large enough such that
\[ \sqrt{2\log(cK/u)} \geq \sqrt{2\log(K/u)} + u^\alpha L \]
for $u<u_0$, which is possible since the condition is equivalent to
\[ 2\log(c) \geq 2u^\alpha L \sqrt{2\log(K/u)} + u^{2\alpha} L^2 \]
and the right hand side converges to zero for $u\searrow 0$. For this $K'=cK$, 
\begin{align*}
&\Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right) \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K'/u)} \textrm{ i.o.  as } u\searrow 0\right) - \Pr\left( A_\epsilon^c\right).
\end{align*}
The first probability equals one by assumption and the claim follows by taking $\epsilon\searrow 0$.
\end{proof}





\begin{lemma}\label{lemma_H1}
Let $x\geq -1$. Then we have
\[ \left(1-\sqrt{1+x}\right)^2 \leq x^2.\]
\end{lemma}
\begin{proof}
We write
\begin{align}\label{eqp: H4}
\left( 1- \sqrt{1+x}\right)^2 -x^2 = \left( \sqrt{1+x}-1 + x\right)\left( \sqrt{1+x}-1 -x\right). 
\end{align} 
Now we distinguish cases: For $-1\leq x\leq 0$, we have 
\[ \sqrt{1+x}-1 + x \leq 0 \quad \textrm{ and }\quad \sqrt{1+x}-1-x\geq 0,\]
where the latter can be seen because it is equivalent to 
\[  \sqrt{1+x} \geq 1+x \Leftrightarrow 1+x \geq 1+2x+x^2 \Leftrightarrow 0\geq x+x^2,\]
which is true since $|x|\geq x^2$ for $|x|\leq 1$. Thus, the product on the right-hand side of \eqref{eqp: H4} is non-positive. For $x\geq 0$, we have
\[ \sqrt{1+x}-1 + x \geq 0 \quad \textrm{ and }\quad \sqrt{1+x}-1-x\leq 0,\]
where the last inequality follows from $\sqrt{1+x}\leq 1+x$ in this case. Again, the product in \eqref{eqp: H4} is non-positive.
\end{proof}






\begin{lemma}\label{lemma_H2}
Define 
\[ Y(y,h) := h^{-\frac14} \int_{-A}^A \frac{K_{y,h}(z)}{\sqrt{h}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h}\|K\|}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - 1\right) dW_z.\]
and based on this
\[ Y(h_0) := \sup_{h\leq h_0}\sup_{y\in [-A,A]} Y(y,h).\]
Then we have $Y(h_0) = \mathcal{O}_{\Pr}(1)$ for $h_0\searrow 0$.
\end{lemma}
\begin{proof}
First, $Y(y,h)$ is a continuous, zero-mean Gaussian process with corresponding covariance metric
\begin{align*}
d((y,h), (y',h'))^2&= \int_{-A}^A \left( \frac{K_{y,h}(z)}{h^{3/4}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h}\|K\|_{L^2}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - 1\right) \right.\\
&\hspace{1.5cm}  \left. - \frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h'}\|K\|_{L^2}}{\|K_{y',h'}\sqrt{q_b}\|_{L^2}} - 1\right)\right)^2 dz.
\end{align*}
Let $L>0$, then
\begin{align}\label{eqp: H1}
\begin{split}
&\Pr\left( |Y(h_0)| > L \right) \leq \frac{1}{L} \E\left[ \sup_{h\leq h_0}\sup_{y\in [-A,A]} |Y(y,h)| \right] \\
&\hspace{1cm}\leq \frac{1}{L} \E\left[ |Y(y_1,h_1)|\right] + \frac{48}{L} \int_0^\infty \sqrt{\log(N(r, (0,h_0]\times [-A,A], d))} dr
\end{split}
\end{align}
by Markov's inequality in the first and Dudley's theorem (Theorem $11.17$ in~\cite{Talagrand}) in the second step and arbitrary $(y_1, h_1)\in [-A,A]\times (0,h_0]$. We turn to bounding the covering numbers. 

First, we choose $h_0$ small enough such that $4L^* h_0 <L_*/2$. We have, writing $\|\cdot\| := \|\cdot\|_{L^2}$ from here on,
\begin{align*}
\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|} &= \sqrt{\frac{(q_b(y) + q_b(z) - q_b(y)) h\|K\|^2}{\int_{-A}^A K_{y,h}(z)^2 q_b(y) dz + \int_{-A}^A K_{y,h}(z)^2 (q_b(z)-q_b(y)) dz}} \\
&= \sqrt{\frac{(q_b(y) + q_b(z) - q_b(y))h\|K\|^2}{q_b(y) h\|K\|^2 + \int_{-A}^A K_{y,h}(z)^2 (q_b(z)-q_b(y)) dz}}
\end{align*}
Using $|q_b(z) - q_b(y)|\leq L^*h$ for $|z-y|\leq h$, we give an upper and lower bound for the last expression. We start with the upper bound
\begin{align*}
\sqrt{\frac{q_b(y) h\|K\|^2 + L^* \|K\|^2 h^2}{q_b(y) h\|K\|^2 - L^* \|K\|^2 h^2}} &= \sqrt{\frac{q_b(y) + L^*h}{q_b(y) - L^*h}} \\
& = \sqrt{ 1+ \frac{q_b(y) + L^*h - q_b(y) +L^*h}{q_b(y) - L^* h}}\\
&\leq \sqrt{1+4L^*/L_* h},
\end{align*}
where we used in the last line that $q_b(y)-L^*h \geq L_*-L^*h \geq L_*/2$ by choice of $h\leq h_0$. Similiarly, we find the lower bound
\begin{align*}
\sqrt{\frac{q_b(y) h\|K\|^2-  L^* \|K\|^2 h^2}{q_b(y) h\|K\| + L^* \|K\|^2 h^2}} &= \sqrt{\frac{q_b(y) - L^*h}{q_b(y) + L^*h}} \\
& = \sqrt{ 1+ \frac{q_b(y) - L^*h - q_b(y) -L^*h}{q_b(y) + L^* h}}\\
&\leq \sqrt{1-4L^*/L_* h}.
\end{align*}
In consequence, we conclude by Lemma \ref{lemma_H1}
\begin{align}\label{eqp: H2}
\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|}  - 1\right)^2 \leq c_1 h^2,
\end{align}
with $c_1 := 16(L^*/L_*)^2$. Then we have
\begin{align}\label{eqp: H3}
d((y,h), (y',h'))^2\leq 4A \left( h^{-3/2} c_1h^2 + (h')^{-3/2} c_1(h')^2 \right) \leq 8Ac_1\sqrt{h_0}.
\end{align}
Note that this bound is uniform in $(y,h), (y',h')$ which means that for $h_0\searrow 0$ the covering number $N(r, (0,h_0]\times [-A,A], d)$  converges to one for each $r>0$.
To apply the dominated convergence theorem to the integral on the right-hand side of \eqref{eqp: H1}, we need to find an integrable majorant. Therefore, we take $h_0$ small enough such that $8Ac_1\sqrt{h_0}<\frac12$ and it suffices to consider $r<\frac12$ because the integrator in \eqref{eqp: H1} vanishes for $r\geq \frac12$ by \eqref{eqp: H3}. \\



Let $r<\frac12$ and denote by $\beta$ the Hölder order of the kernel, where $\beta=1$ if it is Lipschitz or smoother. We split the interval $(0,h_0]$ into $I_1, \dots, I_n$ intervals of length at most $cr^{16/\beta}$ and $[-A,A]$ into $J_1,\dots, J_m$ intervals of length at most $cr^{16/\beta}$, where $c>0$ will be specified later. We will show that their number
\[ \left( 1 + 2A\right) c^{-1} r^{-16/\beta} \]
is a bound for the covering numbers. For this aim, let $(y,h), (y',h')\in I_k\times J_l$ and we will show that $d((y,h),(y',h'))^2 <r^2$.\\

Let $c_2<\frac12(8Ac_1)^{-2}$. Note that we can assume $h\geq c_2r^{4}$ for the rest of the proof that bounds the covering numbers, which can be seen as follows: For $h<c_2r^4$ and $c<c_2$,
\[ h' \leq c_2 r^4 + cr^{16/\beta} \leq  2c_2 r^4,\]
as $|h-h'|<cr^{16/\beta}$ because $h,h'\in J_l$. Applying the bound in \eqref{eqp: H3}, it follows directly that in this case
\[ d((y,h),(y',h')) |\leq 8Ac_1\sqrt{2c_2 r^4} < 8Ac_1\sqrt{(XAc_1)^{-2}} r^2 <r^2. \]


Consequently, assume $h\geq c_2r^4$ in the following. First, we bound $d((y,h),(y',h'))$ by the triangle inequality and $(a+b)^2 \leq 2a^2 + 2b^2$ as
\[ d((y,h),(y',h'))^2 \leq 2d((y,h),(y',h))^2 + 2d((y',h),(y',h'))^2. \]
Using the definition of $d$ and $(a+b)^2\leq 2a^2 + 2b^2$, we find $d((y,h),(y',h))^2 \leq A_1 + A_2$ with
\begin{align*}
A_1 &:= 2\int_{-A}^A \left( \frac{K_{y,h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h}(z)}{h^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2 dz, \\
A_2 &:= 2\int_{-A}^A \frac{K_{y',h}(z)^2}{h^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
For $A_1$ we have with \eqref{eqp: H2} and \eqref{eqp: B11} for a constant $c_3$,
\begin{align*}
A_1 & \leq \frac{2c_1h^2}{h^{3/2}\|K\|^2} \int_{-A}^A \left( K_{y,h}(z) - K_{y',h}(z)\right)^2 q_b(z) dz \\
&\leq \frac{2c_1c_3}{\|K\|^2} \lambda([y-h,y+h]\bigtriangleup [y'-h,y'+h]) \\
&\leq 4c_1c_3 \|K\|^{-2} |y-y'| \\
&< C_1 cr^{16}.
\end{align*}
For $A_2$, we have
\begin{align*}
A_2 &= \frac{2}{\sqrt{h}}\left( \frac{1}{\|K_{y,h}\sqrt{q_b}\|} - \frac{1}{\|K_{y',h}\sqrt{q_b}\|}\right)^2 \int_{-A}^A K_{y',h}(z)^2 q_b(z) dz \\
&= \frac{2}{\sqrt{h}}\left( \frac{\|K_{y',h}\sqrt{q_b}\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2.
\end{align*}
The square of the quotient of the $L^2$-norms is given by
\begin{align*}
\frac{\|K_{y',h}\sqrt{q_b}\|^2}{\|K_{y,h}\sqrt{q_b}\|^2} &= 1+ \frac{\int_{y'-h}^{y'+h} K_{y',h}(z)^2 q_b(z) dz - \int_{y-h}^{y+h} K_{y,h}(z)^2 q_b(z) dz}{\|K_{y,h}\sqrt{q_b}\|^2} \\
&= 1+ \frac{h\int_{-1}^1 K(z)^2 \left( q_b(y'+zh) - q_b(y+zh)\right) dz}{\|K_{y,h}\sqrt{q_b}\|^2} ,
\end{align*}
where the absolute value of the second summand is bounded by
\begin{align*}
\frac{h \|K\|^2 L^* |y-y'|}{h\|K\|^2 L_*} = \frac{L^*|y-y'|}{L_*},
\end{align*}
as $|q_b(y+zh)-q_b(y'+zh)|\leq L^* |y-y'|$. By Lemma \ref{lemma_H1}
\begin{align*}
A_2 &\leq \frac{2}{\sqrt{h}}\left( \frac{\|K_{y',h}\sqrt{q_b}\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2 \\
& \leq  \frac{2}{\sqrt{h}}\left(\frac{L^*}{L_*}\right)^2|y-y'|^2\\
& \leq 2(L^*/L_*)^2 |y-y'| \\
&< C_2c r^{16},
\end{align*} 
as $h^{-1}|y-y'| \leq c_2^{-1} r^{-2} c r^{16/\beta} <1$ for $c<c_2$. \\

We turn to $d((y',h),(y',h'))^2$ and bound $d((y',h),(y',h'))^2\leq B_1+B_2$ with
\begin{align*}
B_1 &:= 2\int_{-A}^A \left( \frac{K_{y',h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz \\
B_2 &:= 2\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h'} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
$B_1$ is bounded from above by $B_1\leq B_{1,1}+B_{1,2}$ with
\begin{align*}
B_{1,1} &:= 4\int_{-A}^A \left( \frac{K_{y',h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{h^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz, \\
B_{1,2} &:= 4\int_{-A}^A \left( \frac{K_{y',h'}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz.
\end{align*}
For $B_{1,1}$ we have as for $A_1$,
\begin{align*}
B_{1,1} &\leq \frac{4c_1 h^2}{h^{3/2}\|K\|^2}\int_{-A}^A \left( K_{y',h}(z) - K_{y',h'}(z)\right)^2 q_b(z) dz\\
& \leq \frac{4c_1c_3}{\|K\|^2} \lambda([y'-h,y'+h]\bigtriangleup [y'-h', y'+h']) \\
& \leq 6c_1c_3 \|K\|^{-2} |h-h'|\\
&\leq C_4 cr^{16}.
\end{align*} 
For $B_{1,2}$, a bound is given by
\begin{align*}
B_{1,2} &\leq \frac{4c_1 h^2}{\|K\|^2} \left( \frac{1}{h^{3/4}} - \frac{1}{(h')^{3/4}} \right)^2 \int_{-A}^A K_{y',h'}(z)^2 dz \\
&= 4c_1 h^2 h'\left( \frac{1}{h^{3/4}} - \frac{1}{(h')^{3/4}} \right)^2.
\end{align*}
By a Taylor expansion, we have
\[ h^{-\frac34} - (h')^{-\frac34} = -\frac34 \xi^{-\frac74} (h-h'),\]
where $\xi$ lies between $h$ and $h'$.
%in particular, it is bounded from below by 
%\[ \xi\geq h-cr^{16/\beta} \geq c_2r^4 -cr^{16/\beta}\geq c_2/2r^{4}$
%for $c<c_2$. 
Additionally, by the choice of $h\geq c_2r^4$ and $|h-h'|\leq cr^{16/\beta}$ we have $h/2\leq \xi, h'\leq 2h$. This yields
\begin{align*}
B_{1,2}&\leq 2c_1 h^2 h h^{-\frac{14}{4}} 2^{\frac{14}{4}} \left(\frac34\right)^2 |h-h'|^2 \\
&= 2^5 h^{-\frac12} |h-h'|^2\\
& \leq 2^5 |h-h'|\\
&\leq C_4 cr^{16},
\end{align*}
as $h^{-1}|h-h'| \leq c_2^{-1} r^{-2} c r^{16/\beta} <1$ for $c<c_2$.
For $B_2$, we bound $B_2\leq B_{2,1} + B_{2,2}$, where
\begin{align*}
B_{2,1} &:= 4\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz, \\
B_{2,2} &:= 4\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h'} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
For $B_{2,1}$, we find the upper bound
\begin{align*}
&\frac{4h}{(h')^{3/2}}\left( \frac{1}{\|K_{y',h}\sqrt{q_b}\|} - \frac{1}{\|K_{y',h'}\sqrt{q_b}\|}\right)^2 \int_{-A}^A K_{y',h'}(z)^2 q_b(z) dz \\
&\hspace{1cm} = \frac{4h}{(h')^{3/2}}\left( \frac{\|K_{y',h'}\sqrt{q_b}\|}{\|K_{y',h}\sqrt{q_b}\|} -1\right)^2
\end{align*}
We bound the quotient of the $L^2$-norms
\begin{align*}
\frac{\|K_{y',h'}\sqrt{q_b}\|^2}{\|K_{y',h}\sqrt{q_b}\|^2} &= 1+ \frac{\int_{y'-h'}^{y'+h'} K_{y',h'}(z)^2 q_b(z) dz - \int_{y'-h}^{y'+h} K_{y',h}(z)^2 q_b(z) dz}{\|K_{y',h}\sqrt{q_b}\|^2} \\
&= 1+ \frac{1}{\|K_{y',h}\sqrt{q_b}\|^2}\int_{-A}^A \left( K_{y',h'}(z) - K_{y',h}(z)\right)\left( K_{y',h'}(z) + K_{y',h}(z)\right) q_b(z) dz\\
&\leq 1+ \frac{2L^*}{\|K_{y',h}\sqrt{q_b}\|^2} \int_{-A}^A \left| \frac{z-y'}{h'} - \frac{z-y'}{h}\right|^\beta dz \\
&\leq 1+ \frac{4L^*A^2}{\|K_{y',h}\sqrt{q_b}\|^2} \frac{|h-h'|^\beta}{(hh')^\beta}\\
&\leq 1+ \frac{4L^*A^2}{h L_*\|K\|^2} \frac{|h-h'|^\beta}{(hh')^\beta}
\end{align*}
Again by Lemma \ref{lemma_H1} and using $h,h'\geq \frac12c_2/ r^4$ because
\[ h' \geq h- cr^{16/\beta} \geq c_2r^4 - c r^{16/\beta} \geq  \frac12 c_2 r^4\]
for $c<c_2$, 
\begin{align*}
B_{2,1} &\leq \frac{64 A^4 (L^*)^2}{(L_*)^2 \|K\|^4 h^{2\beta+1} (h')^{3/2 + 2\beta}} |h-h'|^{2\beta}\\
&\leq \frac{64 A^4 (L^*)^2}{(L_*)^2 \|K\|^4}\left( \frac{2}{c_2}\right)^{\frac52 + 4\beta} r^{-10 - 16\beta} |h-h'|^{2\beta} \\
&\leq C_5 c^{2\beta} r^6,
\end{align*}
where we used $r^{-10-16\beta} |h-h'|^{2\beta} \leq c^{2\beta} r^{-26+32}$. For $B_{2,2}$, we have the bound
\begin{align*}
B_{2,2} &\leq \frac{4}{(h')^{3/2} \|K_{y',h'}\sqrt{q_b}\|^2} \left(\sqrt{h}-\sqrt{h'}\right)^2 \int_{-A}^A K_{y',h'}(z)^2 q_b(z) dz \\
& = \frac{4}{(h')^{3/2}} \left(\sqrt{h}-\sqrt{h'}\right)^2
\end{align*}
By a Taylor expansion, 
\[ \sqrt{h} - \sqrt{h'} = \frac{1}{2\sqrt{\xi}} |h-h'|\]
for $\xi$ between $h$ and $h'$ and by the same reasoning as for $B_{1,2}$, we get from this
\begin{align*}
B_{2,2} &\leq  (h')^{-\frac32} \xi^{-1} |h-h'|^2 \\
&\leq \left(\frac{2}{c_2}\right)^{\frac52} r^{-10} |h-h'|^2\\
&\leq C_6 c^2 r^{32}.
\end{align*}
Collecting all the bounds, we have
\[ d((y,h),(y',h')) \leq \left( C_1+C_2+C_3+C_4+C_5+C_6\right) c^{2\beta} r^6, \]
which is $<r^2$ for $c$ sufficiently small. In conclusion, we have the majorant $(1+2A)c^{-1}r^{-16/\beta}$ of the covering numbers on the  right-hand side of \eqref{eqp: H1}. Integrability follows as
\begin{align*}
&\int_0^\frac12 \sqrt{\log((1+2A)c^{-1}r^{-16/\beta})} dr \\
&\hspace{1cm} = \int_0^\frac12 \sqrt{\log((1+2A)c^{-1}) + 16/\beta\log(1/r)} dr\\
&\hspace{1cm} \leq \int_0^\frac12 \sqrt{\log((1+2A)c^{-1})} dr + \int_0^\frac12 \sqrt{16/\beta\log(1/r)} dr,
\end{align*}
where the first integral is clearly finite, and for the second one, we have by substituting $r=e^{-u}$, 
\begin{align*}
\int_0^\frac12 \sqrt{16/\beta \log(1/r)} dr &\leq \sqrt{16/\beta} \int_0^1 \sqrt{\log(1/r)} dr \\
&=  \sqrt{16/\beta} \int_0^\infty \sqrt{\log(e^u)} e^{-u} dr\\
&= \sqrt{16/\beta} \Gamma\left(\frac32\right) <\infty.
\end{align*} 
Thus, the integral on the right-hand side of \eqref{eqp: H1} converges to zero for $h_0\searrow 0$. In particular, we can choose $h_0$ small enough and afterwards $L$ large enough such that the right-hand side of \eqref{eqp: H1} is bounded by $\epsilon$ and the claim follows.
\end{proof}





==> Version_ArXiv/Sections/Composite_Hypothesis.tex <==
\section{Testing of composite hypotheses}


\subsection{One-sided alternative}

We fix, $A,\gamma,\sigma>0$, $C\geq 1$ and set 
\[\mathcal{H}_{\leq 0} := \{ f\in \Sigma(C,A,\gamma,\sigma)\mid f\leq 0\textrm{ on } [-A,A]\}. \]
We will assume under the alternative, that $b$ belongs to some Hölder class $\mathcal{H}(1,L)$, $L>0$ and of couse admits ergodic properties, i.e. $b\in\Sigma(1,L,0)$.We measure the distance to $\mathcal{H}_{\leq 0}$ by
\[ \Delta(b) := \inf_{b_0\in\mathcal{H}_{\leq 0}} \| 1_{[-A,A]}(b_0 - b)\rho_b^\frac13\|_\infty \]
and it is easily seen that for $b\notin\mathcal{H}_{\leq 0}$ we have
\[ \Delta(b) = \sup_{x\in [-A,A]} \left( b(x) \rho_b(x)^\frac13\right).\]

We set
\[ \mathcal{T} := (0,1]\times [-A+h, A-h] \]
and considert the test statistic
\[ T_b(X)  = \sup_{(y,h)\in\mathcal{T}} \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)\]
where
\[ \tilde{\Psi}_{y,h}^b(X) = \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} + \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
This is the same statistic as $\Psi_{y,h}(X)$ in section $3$ when we choose $b_0=0$ on the interval $[-A,A]$. To built our test, we want to identify a worst case within the set $\mathcal{H}_{\leq 0}$ in order to have a non-degenerate random variable that delivers the quantiles for our test. \\
In a first step we want to show that an asymptotically worst case within this set of hypothesis is $f=0$ which is the reasonable expectation as it is the hypothesis closest to the alternative of functions being larger than zero anywhere within $[-A,A]$.

Clearly, the second summand is always negative for $b\in\mathcal{H}_{\leq 0}$ and vanishes for $b=0$, where the latter is understood as restricted to $[-A,A]$. Outside of this interval the drift clearly needs to deviate from zero in order to ensure ergodic properties of the solution or put differently, to ensure $b\in\Sigma(C,A,\gamma,\sigma)$. In this latter case we know that the invariant density $\rho_0=c$ is constant on $[-A, A]$ and hence the weak limit of the test statistic is given by
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C( \|cK_{y,h}\|_{L^2}^2)\right),\]
where
\[ Z(y,h) = \frac{\int_{-A}^A K_{y,h}(z) dW_z}{\|K_{y,h}\|_{L^2}}.\]
But it is not directly clear that $b_0=0$ is the worst case from these considerations, as the first summand contains the process $X$ which depends on the choice of drift and it is not clear that this term is also stochastically dominated by the choice $b_0=0$. But nevertheless, the assertion turns out to be true asymptotically: for negative choices of $b_0$ the first term may be larger, but this is compensated by the second term which in turn is negative. This is spelt out in detail in the next result and its proof in Appendix D.

\begin{proposition}\label{worst_case_one-sided}
For each $b\in\mathcal{H}_{\leq 0}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_b(X) > r\right) \leq \Pr\left( S>r\right),\]
where
\[ S := \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left(\|K_{y,h}\|_{L^2}^2\right) + C\left( (1\vee (L^*\wedge (2h)^{-1})^{-1}\right)\right).\]
\end{proposition}

As an application of Theorem \ref{Multiscale_Lemma} is immediate for $S$, we know that the critical value
\[ \kappa_{\leq 0, \alpha} := \min \{ r\in\R:\ \Pr(S\leq r)\geq 1-\alpha\}\]
is well defined and we reject the null hypothesis $\mathcal{H}_{\leq 0}$ at level $\alpha$ if $T_b(X)> \kappa_{\leq 0, \alpha}$. This turns again turns out to be optimal with the best possible constant. Note that the optimal recovery kernel $K_\beta$ in the case of $\beta=1$ is given by the triangular kernel $K(x) = 1_{\{|x|\leq 1\}}(1-|x|)$ with $\|K\|_{L^2}^2 = \frac23$. In this case the optimal constant of section $3$ is given by $c_* = L^\frac13$.

\begin{thm}\label{theorem_one-sided}
Let $(\epsilon_T)_{T\geq 0}$ be given such that $\lim_{T\to\infty} \epsilon_T =0$ and $\lim_{T\to\infty} \epsilon_T\sqrt{\log T} =\infty$, let $T_b$ be given with the choice of the rectangular kernel $K$ and 
\[ \rho_T := \left( \frac{\log T}{T}\right)^\frac13.\]
\begin{enumerate}
\item[(a)] For any test $\phi_T$ with $\E_0[\phi_T]\leq \alpha$ we have
\[ \limsup_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,0): \Delta(b)\geq (1-\epsilon_T) L^\frac13 \delta_T}} \E_b [ \phi_T(X)] \leq \alpha.\]
\item[(b)] Our test satisfies
\[ \lim_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,0): \Delta(b)\geq (1+\epsilon_T) L^\frac13 \delta_T}} \Pr_b\left( T_b(X)\geq \kappa_{\leq 0, \alpha}\right) =1.\]
\end{enumerate}
\end{thm}





\subsection{$\delta$-environment}
Now we turn to test for a $\delta$-environment. Pick a drift function $b_0\in\Sigma(C,A,\gamma,\sigma)$ and $\delta>0$ and define 
\[ \mathcal{H}_\delta(b_0) := \left\{ b\in \Sigma(C,A,\gamma,\sigma)\mid \| 1_{[-A,A]} (b-b_0)\|_\infty \leq \delta\right\}.\]
As an alternative we again choose some Hölder class $\mathcal{1,L}$, $L>0$ with ergodic properties of the solution. The distances is given in this case for $b\notin\mathcal{H}_\delta(b_0)$ as
\[ \Delta(b) = \sup_{x\in [-A,A]} \left( (|b(x)-b_0(x)| - \delta) \rho_b(x)^\frac13\right).\]
With the definition of $\Psi_{y,h}(X)$ from section $3$ we define a test statistic
\[ T_\delta(X) := \sup_{(y,h)\in\mathcal{T}} \left(\left| \Psi_{y,h}(X)\right| - C(\sigma_{y,h}^2) - \Psi_\delta\right),\]
where
\[ \Psi_\delta := \frac{\frac{\delta}{\sqrt{T}} \int_0^T K_{y,h}(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
As a worst case we expect the function $b_0\pm\delta$: on the one hand because this choice eliminates the term $\Psi_\delta$, on the other hand intuitively, as it is the boundery case to the alternative and therefore a predestinated candidate. But as in the case of a one-sided alternative it is not exactly clear, as the distribution of $X$ depends on the drift. But we may again show that we are on the right track.

\begin{proposition}\label{worst_case_delta}
For each $b\in\mathcal{H}_{\delta}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_\delta(X) > r\right) \leq \Pr\left( S_1\vee S_2>r\right),\]
where
\begin{align*}
S_1 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0+\delta}(z)} dW_z}{\|K_{y,h}\sqrt{\rho_{b_0+\delta}}\|_{L^2}}\right| - C\left(\|K_{y,h}\sqrt{\rho_{b_0+\delta}}\|_{L^2}^2\right)\right),\\
S_2 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0-\delta}(z)} dW_z}{\|K_{y,h}\sqrt{\rho_{b_0-\delta}}\|_{L^2}}\right| - C\left(\|K_{y,h}\sqrt{\rho_{b_0-\delta}}\|_{L^2}^2\right)\right).
\end{align*} 
\end{proposition}

We may apply Theorem \ref{Multiscale_Lemma} to both $S_1$ and $S_2$ to get a well defined critical value
\[ \kappa_{\delta,\alpha} := \min\{ r\in\R:\ \Pr(S_1\vee S_2 \leq r) \geq 1-\alpha\}.\]
Then our test rejects the null hypothesis $\mathcal{H}_\delta$ at level $\alpha$ if $T_\delta(X) >\kappa_{\delta,\alpha}$.


\begin{thm}\label{theorem_delta}
Let $(\epsilon_T)_{T\geq 0}$ be given such that $\lim_{T\to\infty} \epsilon_T =0$ and $\lim_{T\to\infty} \epsilon_T\sqrt{\log T} =\infty$, let $T_\delta$ be given with the choice of the rectangular kernel $K$ and 
\[ \rho_T := \left( \frac{\log T}{T}\right)^\frac13.\]
\begin{enumerate}
\item[(a)] For any test $\phi_T$ with $\E_0[\phi_T]\leq \alpha$ we have
\[ \limsup_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,b_0\pm\delta): \Delta(b)\geq (1-\epsilon_T) L^\frac13 \delta_T}} \E_b [ \phi_T(X)] \leq \alpha.\]
\item[(b)] Our test $T_\delta$ satisfies
\[ \lim_{T\to\infty} \inf_{\substack{ b\in\Sigma(1,L,b_0\pm\delta): \Delta(b)\geq (1+\epsilon_T) L^\frac13 \delta_T}} \Pr_b\left( T_\delta(X)\geq \kappa_{\delta, \alpha}\right) =1.\]
\end{enumerate}
\end{thm}




==> Version_ArXiv/Sections/Further_results.tex <==
\section{Sketch of the proof of Theorem \ref{lower_bound}}\label{Sec_supp}

The proof of the lower bound in Theorem \ref{lower_bound} relies on the construction of several drift functions that belong to the alternative $H_1(b_0,\eta)$, but are close to the null in the distance $\Delta_J$ the theorem is formulated for. The innovation is that constructing these alternatives close enough to the null leads to a fixed point problem.

The start of the proof is to deduce the classical inequality
\begin{align}\label{eq: lower_av_likelihood}
\inf_{\substack{b\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1-\epsilon_T)c_*\delta_T}} \E_b[\psi] - \alpha 
\leq  \E_{b_0+\eta}\left[ \left| \frac1N \sum_{k=1}^N \frac{d\Pr_{b_k}}{d\Pr_{b_{0}+\eta}}(X) - 1\right|\right]
\end{align}
that holds true for each test $\psi$ with $\sup_{b\in H_0(b_0,\eta)}\E_{b}[\psi]\leq\alpha$ and suitable alternatives $b_k$.
Those will be constructed in such a way that the last expression tends to zero for $T\to\infty$, in particular each $b_k$ and their number $N$ will depend on $T$. It will turn out from our construction that the likelihood ratios are not independent and proceeding with Cauchy-Schwarz' inequality does not yield tight enough bounds. For this purpose, we prove the following result.


\begin{proposition}\label{lemma_E_absvalue}
Let $Z_1,\dots, Z_m$ be strictly positive random variables with $\E[Z_i]=1$ and $\E[Z_i Z_j]\leq C_0$ for all $1\leq i,j\leq m$ and some constant $C_0\geq 1$. Then for all $\epsilon>0$ and $0<\nu\leq 1$ we have
\begin{align*}
\E\left[\left| \frac1m \sum_{i=1}^m Z_i - 1\right|\right] &\leq \sqrt{\epsilon} + \left( 2\epsilon^{-\nu} m^{-(1+\nu)} \sum_{i=1}^m \E[ Z_i^{1+\nu}] \right)^\frac12 + \sqrt{C_0-1}  \\
&\hspace{1cm} +2\epsilon^{-\nu}m^{-(1+\nu)}\sum_{i=1}^m \E[ Z_i^{1+\nu}].
\end{align*} 
\end{proposition}



The construction of the hypotheses $b_k$ that allow to achieve the optimal constant in Theorem \ref{lower_bound} is highly non-trivial as compared to the standard approach.
Typically, $b_k\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}$ with $\Delta_J(b_k)\geq (1-\epsilon_T)c_*\delta_T$ is constructed by adding a localized kernel to some boundary case of the null at location $y_k$, for different $k$, i.e. $b_k$ is of the form
\[ b_k = b_0 + \eta + \textrm{localized kernel at } y_k.\]
Furthermore, with $\Delta_J$ as defined in \eqref{eq: Delta_J}, $b_k$ should be smallest possible in the sense
\begin{align}\label{eq: lower_delta}
\begin{split}
\Delta_J(b_k) &=\sup_{x\in J} \Big(|b_k(x)-b_0(x)| - \eta\Big) \left(\frac{q_{b_k}(x)}{\sigma^2}\right)^\frac{\beta}{2\beta+1}\\
&=  (1-\epsilon_T)c_*\delta_T,
\end{split}
\end{align}  
where $q_{b_k}$ denotes the invariant density corresponding to the drift $b_k$. The problem is to find $y_k$ and the corresponding localized kernels such that \eqref{eq: lower_delta} ist satisfied. This is rather involved due to the dependence of $q_{b_k}$ on $b_k$ itself.
Our ansatz is as follows: we define
\[ b^w(x) := b_{0}(x) +\eta + L(1-\epsilon_T)(h_T^w)^\beta K_T^\beta\left(\frac{x-y^w}{h_T^w}\right)\]
with 
\[ h_T^w := \left(\frac{c_*}{L}\right)^\frac{1}{\beta} \left( \frac{\sigma^2 \log T}{T w}\right)^\frac{1}{2\beta+1},\]
and $y^w$ is a location that depends continuously on $w$. The particular dependence on $w$ in $h_T^w$ is inspired by the optimal bandwidth for detection where the bandwidth depends in the same way on the invariant density.
For such a drift function $b^w$, \eqref{eq: lower_delta} is equivalent to the following fixed point problem. 

\medskip
\noindent
\textit{Fixed point problem:}
\[ w = q_{b^w}(y^w) K_T(0)^\frac{2\beta+1}{\beta}.\]
The following result states that there exists a solution. Its proof can be found in Appendix \ref{App_lower}.


\begin{lemma}\label{lemma_fixed_point}
Let $R>0$. Choose $y\in [-A', A'] $ and set $y^w = y+Rh_T^w$. Then for $T\geq T_0$ large enough and $\frac12<c_T<1$, there exists $\tilde{w}\in [c_TL_*, c_T L^*]$, such that 
\[ \tilde{w}= c_Tq_{b^{\tilde{w}}}(y^{\tilde{w}}). \]
\end{lemma}


With this lemma, we can define the drifts $b_k$ satifying \eqref{eq: lower_delta} interatively. As the height and support of the additive localized kernel depends on $h_T^w$, it will be different with varying location. % as illustrated in Figure \ref{figure2}.


%\begin{figure}[h]
%\begin{tikzpicture}
%\draw [thick] (0,0) -- (12,0);
%%\draw [red] (2,0) -- (2.5,1) -- (3,0);
%%\draw [green] (3,0) -- (5,2) -- (7,0);
%%\draw [blue] (7,0) -- (8,1.5) -- (9,0);
%\filldraw[black] (1,0) circle (1pt) node[anchor=north] {-A};
%\filldraw[black] (11,0) circle (1pt) node[anchor=north] {A};
%\filldraw[black] (2,0) circle (1pt) node[anchor=north] {-A'};
%\filldraw[black] (10,0) circle (1pt) node[anchor=north] {A'};
%\filldraw[black] (2.5,0) circle (1pt) node[anchor=north] {$y_1$};
%\filldraw[black] (5,0) circle (1pt) node[anchor=north] {$y_2$};
%\filldraw[black] (8,0) circle (1pt) node[anchor=north] {$y_3$};
%
%\draw[|-|, red] (2.5,-0.75)--(3,-0.75) node[below,midway]{$h_1$};
%\draw[|-|, green] (5,-0.75)--(7,-0.75) node[below,midway]{$h_2$};
%\draw[|-|, blue] (8,-0.75)--(9,-0.75) node[below,midway]{$h_3$};
%
%
%\draw[red, domain=2:2.35] plot (\x,{1.5*(1-(2*(2.5-\x))^(0.75))});
%\draw[red, domain=2.35:2.65] plot (\x,{1.5*(1-0.3^(0.75))});
%\draw[red, domain=2.65:3] plot (\x,{1.5*(1-(2*(\x-2.5))^(0.75))});
%
%\draw[green, domain=3:4.85] plot (\x,{2.5*(1-((5-\x)/2)^(0.75))});
%\draw[green, domain=4.85:5.15] plot (\x,{2.5*(1-0.075^(0.75))});
%\draw[green, domain=5.15:7] plot (\x,{2.5*(1-((\x-5)/2)^(0.75))});
%
%
%\draw[blue, domain=7:7.85] plot (\x,{2*(1-(8-\x)^(0.75))});
%\draw[blue, domain=7.85:8.15] plot (\x,{2*(1-0.15^(0.75))});
%\draw[blue, domain=8.15:9] plot (\x,{2*(1-(\x-8)^(0.75))});
%\end{tikzpicture}
%\caption{\small{The construction principle of our localized kernels, illustrated with the optimal recovery kernel $K_{0.75}$. First, the red hat is constructed from $-A$, then the green one starting at $y_1+h_1$ and finally the blue hat. One can see that depending on the solution $w$ of each fixed point problem the height and width of each hat varies.}}\label{figure2}
%\end{figure}





By the aforementioned Proposition \ref{lemma_E_absvalue}, the proof is now reduced to bounding the $(1+\gamma)$-moments of likelihood ratios of diffusions driven by different drifts. Those are available using Girsanov's theorem and the further calculation heavily depends on the occupation times formula \ref{occupation_times_formula} and the concentration result \ref{moments_local-invariant} for the empirical density. 






==> Version_ArXiv/Sections/Implementation.tex <==
\section{Computability and numerical example}\label{Sec_Implementation}
In this section we first discuss how the test statistic $T_T^\eta(X)$ given in \eqref{eq: T_eta} can be computed for a given observation $X=(X_t)_{t\in [0,T]}$. In a second part, an extended simulation study is given.


\subsection{Computability of the test statistic $T_T^\eta$}
When implementing the test statistic $T_T^\eta(X)$ for an observed path $X$ one has to evaluate several Lebesgue integrals and the stochastic It\^{o} integral $\int_0^T K_{y,h}(X_s) dX_s$. Given a continuously differentiable kernel $K$ we have seen in Section \ref{Sec_Stability} that by It\^{o}'s formula
\[ \int_0^T K_{y,h}(X_s) dX_s = \int_{X_0}^{X_T} K_{y,h}(z) dz - \frac{\sigma^2}{2} \int_0^T (K_{y,h})'(X_s) ds \]
and based on this we established a version $\tilde\Psi_{T,y,h}^{b_0}(X)$ of $\Psi_{T,y,h}^{b_0}(X)$, given in \eqref{eq: tilde_psi}, that is defined pathwise. Working with this version directly yields a way to compute the local statistics for any given path $X$ and we have seen in Theorem \ref{Upper_bound} that for a rate optimal procedure, we can indeed choose a kernel that is continuously differentiable. 
%Moreover, the proof of Theorem \ref{thm_continuity} established continuity of the mapping
%\begin{align*}
%\mathcal{T}\ &\rightarrow\ \ \ \R,\\
%(y,h) &\mapsto\  \tilde\Psi_{T,y,h}^{b_0}(X).
%\end{align*}
%In consequence, the test statistic $T_T^\eta$ is measurable as it reduces to a supremum over a countable set.


%\begin{remark}[The case $\beta\leq 1$]
%For $\beta\leq 1$ we defined $T_T^\eta$ with the optimal recovery kernel $K_\beta$ that is not differentiable. However, as it has compact support, we can approximate $K=K_\beta$ uniformly by $K^n$ that are continuously differentiable by the Stone-Weierstraß theorem. By dominated convergence for stochastic integrals we than have
%\[ \int_0^T K_{y,h}^n(X_s) dX_s \rightarrow \int_0^T K_{y,h}(X_s) dX_s\]
%in probability and the left-hand side may be rewritten as
%\[ \int_{X_0}^{X_T} K_{y,h}^n(z) dz - \frac{\sigma^2}{2h}\int_0^T (K_{y,h}^n)'(X_s) ds.\]
%This representation is again a continuous in $(y,h)$ version of $\int_0^T K_{y,h}^n(X_s) dX_s$. In Lemma \ref{lemma_approx_K_beta} we show that for a certain choice of $K^n$ its convergence is uniform in $(y,h)\in\mathcal{T}$ for any path $X$ fullfilling $c_1 q_b \leq \frac{1}{\sigma^2 T} L_T^\cdot(X)\leq c_2  q_b$ for some constants $0<c_1\leq c_2$ and hence the limit is also continuous in $(y,h)$, in particular, it is measurable.
%\end{remark}




\begin{remark}[Grid of bandwidths]\label{remark_bandwidth}
In practice, one has to restrict to a finite subset $\mathcal{T}'\subset\mathcal{T}$ when computing the statistic $T_T^\eta$. The proof of Theorem \ref{Upper_bound} reveals that the minimal bandwidth used for detection is of order $(\log T/T)^{1/(2\beta+1)}$. Hence, it suffices to choose $h$ from the finite set
\[ \mathcal{H}_T := \left\{ k T^{-1} \mid k=1,2,\dots, \lfloor AT\rfloor \right\}. \]
The same distance of points should be applied to define a grid for $y$, i.e. we choose this parameter from
\[ \mathcal{Y}_T := \left\{ -A + kT^{-1} \mid k=1,2,\dots \lfloor 2AT\rfloor \right\} \]
and the finite set $\mathcal{T}'$ of location and bandwidth parameters for implementation may be chosen as $\mathcal{T}' = (\mathcal{Y}_T\times \mathcal{H}_T)\cap\mathcal{T}$, assuming $T\in\Q$.
\end{remark}



\begin{remark}[Quantiles for the simple null]
%Remember the test $\phi_T^{b_0}$ given in \eqref{eq: phi_0} for the simple null. % Here we definded the test statistic $T_T^{b_0}(X)$ in \eqref{eq: T_simple} and the corresponding quantiles in \eqref{eq: quantile_simple}. 
From a practical point of view it is much more convenient to replace the quantile $\kappa_{T,\alpha}^{\neq b_0}$ in the test $\phi_T^{b_0}$ given in \eqref{eq: phi_0} by the quantile
\[ \kappa_\alpha^{b_0} := \min\left\{ r\in\R \mid \Pr\left( S_{b_0}\leq r\right)\geq 1-\alpha\right\} \]
of the limiting statistic $S_{b_0}$ from Theorem \ref{weak_conv} which can be easily simulated by Monte Carlo methods as the explicit form of the invariant density $q_{b_0}$ is known.
\end{remark}











\subsection{Numerical example}

In this section we will give a numerical illustration of the testing procedure of Section~\ref{Sec_similarity} for the parameter specification $b_0(x) =-x$ together with $A=\sigma^2=1$.\\
%To compute the test $\phi_T^\eta(X)$ given in \eqref{eq: phi_eta} for simulated data, we first need to specify the quantiles $\kappa_{\eta,\alpha}$ given in \eqref{eq: kappa_eta_alpha}. 
The quantiles $\kappa_{\eta,\alpha}$ given in \eqref{eq: kappa_eta_alpha} are estimated by the empirical quantiles of $N=10000$ independent samples of $U_1\vee U_2+4\sqrt{A\eta/\sigma^2}$. Results for different $\eta$ and $\alpha$ are given in Table~\ref{Table_quant}. It can be seen that the influence of $\eta$ on the quantiles is mostly due to the additive correction term $4\sqrt{A\eta/\sigma^2}$. An algorithm for their derivation is provided in Section~\ref{App_implementation}. Note that $q_{b_0\pm\eta}$ is given explicitly for the specification $b_0(x)=-x$ by the stationary density of an Ornstein-Uhlenbeck process which is known to be Gaussian. 


\begin{center}
\begin{table}[h]
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.3781$ & $1.6775$ & $2.2468$ \\
$0.05$ & $1.4222$ & $1.7311$ &  $2.3178$ \\
$0.1$ & $1.4473$ & $1.7391$ & $2.3726$ \\
$0.2$ & $1.4503$ & $1.7497$ & $2.3047$ \\
$0.3$ & $1.4646$ & $1.7458$ & $2.3403$ \\
$0.4$ & $1.4642$ & $1.7692$ & $2.3748$ \\
$0.5$ & $1.5021$ & $1.7670$ & $2.3114$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.3781$ & $1.6775$ & $2.2468$ \\
$0.05$ & $2.3166$ & $2.6256$ &  $3.2122$ \\
$0.1$ & $2.7122$ & $3.0040$ & $3.6375$ \\
$0.2$ & $3.2391$ & $3.5386$ & $4.0935$ \\
$0.3$ & $3.6555$ & $3.9367$ & $4.5312$ \\
$0.4$ & $3.9900$ & $4.2990$ & $4.9046$ \\
$0.5$ & $4.3305$ & $4.5954$ & $5.1398$ \\
\end{tabular}
\medskip
\caption{\small{Quantiles of $U_1\vee U_2$ (left) and $U_1\vee U_2+4\sqrt{A\eta/\sigma^2}$ (right) for different $\eta$ and $\alpha$. The simulated quantiles are taken from a sample of $N=10000$, the parameters of the algorithm in Section~\ref{App_implementation} are chosen as $n_1 =100$ and $n_2=100$.}}\label{Table_quant}
\end{table}
\end{center}





To demonstrate the detection power of our test, we simulate data that follows the SDE in \eqref{eq: SDE} with
\[ b_{alt}(x) := -x  - 0.8 K\left(\frac{x+0.6}{0.15}\right) + 0.15 K\left(\frac{x}{0.2}\right) + 0.5 K\left(\frac{x-0.5}{0.1}\right),\]
where
\begin{align}\label{eq: K_alt}
K(x) := \frac{15}{16} \left( 1-x^2\right)^2 \1_{\{|x|\leq 1\}}.
\end{align} 
By Remark~\ref{remark_fixed_point}, our results hold true in the case of a fixed starting point of the diffusion and we assume $X_0=0$ for simplicity in implementation. A display of $b_{alt}$ is included in Figure~\ref{Figure_2}. The simulation is done with a time horizon $T=10000$ on an equidistant grid with width $0.001$, i.e. we simulate $10^7$ values of the diffusion according to the Euler-Maruyama scheme (cf. Section~$9.1$ and $10.2$ in \cite{Kloeden}). In Figure~\ref{Figure_2} the minimal intervals of $D_{\alpha}^\eta$ given in Remark~\ref{remark_D_alpha} are depicted for $\alpha=0.05$ and the two values $\eta_1=0.05$ and $\eta_2=0.2$. Here, an interval $I\in D_\alpha^\eta$ is called minimal, if for any interval $I\neq J\in D_\alpha^\eta$ we have $J\nsubseteq I$. The test statistic is computed with the kernel given in \eqref{eq: K_alt}.  




%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot01}
%\end{minipage}
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot03}
%\end{minipage}%
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot02}
%\end{minipage}
%\begin{minipage}{0.5\textwidth}
%\includegraphics[scale=0.3]{Plot04}
%\end{minipage}


\begin{center}
\begin{figure}
%\begin{table}[h]
\begin{tabular}{cc}
\includegraphics[scale=0.3]{Plot01} & \includegraphics[scale=0.3]{Plot03}\\
\includegraphics[scale=0.3]{Rplot_new3} & \includegraphics[scale=0.3]{Rplot_new2}
\end{tabular}
\caption{\small{Both upper pictures show the drift $b_{alt}$ together with its $\eta$-environment for $\eta_1=0.05$ (left) and $\eta_2=0.2$ (right). In the bottom the minimal intervals are depicted for both cases according to the parameter specification given in the text and $\alpha=0.05$.}}\label{Figure_2}
%\end{table}
\end{figure}
\end{center}







In the following table the proportion of detections is given for various values of $\eta$ and $\alpha$ for $N=400$ simulated paths. It also contains this proportion 'locally' to show which of the three possible violations from $H_0(b_0,\eta)$ is detected (it depends on $\eta$ if $b_{alt}$ lies outside an $\eta$-environment of $b_0$ or not).


\begin{center}
\begin{table}[h]
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $1.00$ & $1.00$ \\
$0.1$ & $1.00$ & $1.00$ & $1.00$ \\
$0.2$ & $1.00$ & $1.00$ & $1.00$ \\
$0.3$ & $0.98$ & $0.97$ & $0.91$ \\
$0.4$ & $0.47$ & $0.36$ & $0.19$ \\
$0.5$ & $0.14$ & $0.11$ & $0.07$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $1.00$ & $1.00$ \\
$0.1$ & $1.00$ & $1.00$ & $1.00$ \\
$0.2$ & $1.00$ & $1.00$ & $1.00$ \\
$0.3$ & $0.98$ & $0.96$ & $0.88$ \\
$0.4$ & $0.42$ & $0.32$ & $0.17$ \\
$0.5$ & $0.12$ & $0.09$ & $0.06$ \\ 
\end{tabular}
\hfill
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{} \\
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $0.99$ & $0.98$ & $0.94$ \\
$0.05$ & $0.75$ & $0.64$ & $0.46$ \\
$0.1$ & $0.49$ & $0.40$ & $0.23$ \\
$0.2$ & $0.14$ & $0.11$ & $0.06$ \\
$0.3$ & $0.04$ & $0.03$ & $0.02$ \\
$0.4$ & $0.01$ & $0.01$ & $0.00$ \\
$0.5$ & $0.00$ & $0.00$ & $0.00$ \\
\end{tabular}
\quad
\begin{tabular}{c|ccc}
\multicolumn{4}{c}{} \\
\textbf{$\eta$} & \textbf{$\alpha=0.1$} & \textbf{$\alpha=0.05$} & \textbf{$\alpha = 0.01$} \\
\hline
$0$  & $1.00$ & $1.00$ & $1.00$ \\
$0.05$ & $1.00$ & $0.99$ & $0.96$ \\
$0.1$ & $0.92$ & $0.85$ & $0.60$ \\
$0.2$ & $0.33$ & $0.28$ & $0.19$ \\
$0.3$ & $0.16$ & $0.12$ & $0.08$ \\
$0.4$ & $0.06$ & $0.05$ & $0.03$ \\
$0.5$ & $0.02$ & $0.02$ & $0.01$ \\
\end{tabular}
\medskip
\caption{\small{Proportions of rejection of the null for different $\eta$ and $\alpha$ and $N=400$ simulated paths. We count, if there is any detected interval (upper left), a minimal interval intersecting with $[-0.75,-0.45]$ (upper right), $[-0.2,0.2]$ (bottom left) or $[0.4,0.6]$ (bottom right).}}\label{Table_prop_rejection}
\end{table}
\end{center}






==> Version_ArXiv/Sections/Intro_App.tex <==
\begin{frontmatter}

% "Title of the paper"
\title{\vspace{-0.3cm} Supplement to "Sharp adaptive similarity testing with pathwise stability for ergodic diffusions"}
\runtitle{Supplement to "Similarity testing for ergodic diffusions"}


\author{\fnms{Johannes} \snm{Brutsche}\ead[label=e1]{johannes.brutsche@stochastik.uni-freiburg.de}}
%\address{\printead{e1}}
\and
\author{\fnms{Angelika} \snm{Rohde}\ead[label=e2]{???}}
%\address{\printead{e2}}
%\affiliation{???}


%\begin{aug}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Only one address is permitted per author. %%
%% Only division, organization and e-mail is %%
%% included in the address.                  %%
%% Additional information can be included in %%
%% the Acknowledgments section if necessary. %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\author{\fnms{Johannes} \snm{Brutsche}\ead[label=e1]{johannes.brutsche@stochastik.uni-freiburg.de}}
%\and
%\author{\fnms{Angelika} \snm{Rohde}\ead[label=e2]{angelika.rohde@stochastik.uni-freiburg.de}}
%\affiliation{University of Freiburg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Addresses                                %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\address{Institute of Mathematics\\ Ernst-Zermelo-Straße 1\\ 79104 Freiburg\\ Germany \\ \printead{e1,e2} }
%\address{Institute of Mathematics\\ Ernst-Zermelo-Straße 1\\ 79104 Freiburg\\ Germany \\ \printead{e2}}
%\end{aug}

\runauthor{J. Brutsche and A. Rohde}

\affiliation{Albert-Ludwigs-Universit\"at Freiburg}

\end{frontmatter}



%This supplement is organised as follows. In Section~\ref{App_prelim} we give a brief overview on scalar ergodic diffusions. This includes well-known results that are frequently used in the proofs in the other sections and some own results taylored to our context, where a proof is provided. Section~\ref{App_Multiscale} introduces to multiscale theory based on empirical processes and contains the proof of Theorem~\ref{Multiscale_Lemma}. The subsequent Section~\ref{App_weak} presents many general results on uniform weak convergence and based on those the proof of the uniform weak convergence result in Theorem~\ref{weak_conv}. Section~\ref{App_least} contains the proof of our main result, Theorem~\ref{worst_case_delta}, that was sketched in Section~\ref{Sec_weak} and identifies a stochastic dominating random variable for the test statistic $T_T^\eta$ on which the quantiles for our test $\phi_T^\eta$ are based. It also includes the proof of Remark~\ref{remark_Piterbarg} which establishes that this dominating random variable has not atoms. In Section~\ref{App_lower} we give the proof of the minimax lower bound, Theorem~\ref{lower_bound}, that was already sketched in Section~\ref{Sec_supp}. Subsequently, Section~\ref{App_Upper} contains the proofs of the corresponding upper bounds given in Theorem~\ref{Upper_bound}, \ref{thm_adaptivity} and \ref{thm_simple_hypothesis}. Finally, proofs of the stability results of Theorem~\ref{thm_continuity} and \ref{prop_stability} together with Remark~\ref{remark_stability} are given in Section~\ref{App_stability}. This presentation also includes preliminaries on fractional calculus and fractional Brownian motion, as well as the proof of Proposition~\ref{lemma_X^H-X}. 


\vspace{-0.1cm}
This supplementary material is organized as follows:\\
\vspace{-0.2cm}

\tableofcontents
\addtocontents{toc}{\protect\setcounter{tocdepth}{3}}



\section{Notation}

For any set $E$ and function $f:E\rightarrow \R$ we denote
\[ \|f\|_E := \sup_{x\in E} |f(x)|. \]
When $E=\R$ we denote $\|f\|_\infty := \sup_{x\in\R} |f(x)|$. For a compact set $K\subset \R^n$ we denote by $\mathcal{C}(K)$ the set of continuous functions $f:K\rightarrow\R$ and consider it as a normed space with the norm $\|\cdot\|_K$. Moreover, we set 
\[ l_\infty(E) :=\{ f:E\rightarrow \R: \|f\|_E <\infty\}. \]
We denote by $\|\cdot\|_{L^p(\Pr)}$ the $L^p$-norm with respect to the probability measure $\Pr$. On the other hand, for a subset $I\subset\R$ we write $\|\cdot\|_{L^p(I)}$ for the $L^p$-norm with respect to the Lebesgue measure $\lambda(\cdot)$ on $\R$ and denote the corresponding $L^p$-space by $L^p(I)$. If $I=\R$, we simply write $\|\cdot\|_{L^p}$. By $\|\cdot\|_2$ we denote the Euclidean norm on $\R^d$.\\
For real numbers $a,b\in\R$ we use the notation $a\wedge b:=\min\{a,b\}$ and $a\vee b :=\max\{a,b\}$, as well as $a_+ := \max\{a,0\}$ and $\textrm{sign}(a) = a/|a|$. For functions, in particular random variables, maximum and minimum are understood pointwise and also abbreviated with $\wedge$ and $\vee$. The cardinality of a finite set $B$ is denoted by $\#B$.\\
We use the Landau symbols $\mathcal{O}(a_T)$ and $o(a_T)$, where 
\[ b_T=\mathcal{O}(a_T)\Leftrightarrow \limsup_{T\to\infty} \left|\frac{b_T}{a_T}\right|<\infty\quad \textrm{ and }\quad b_T=o(a_T)\Leftrightarrow \lim_{T\to\infty} \left|\frac{b_T}{a_T}\right| =0.\] 
In case $a_T=1$, we write $\mathcal{O}_T(1)$ and $o_T(1)$ to indicate the running index.\\
By $\rightarrow_{as}$, $\rightarrow_{\Pr}$ and $\rightarrow_{\mathcal{D}}$ we denote almost sure convergence, convergence in probability and convergence in distribution, respectively. By $\Rightarrow$ we denote weak convergence of measures. $X_n=o_\Pr(1)$ means that $(X_n)_{n\in\N}$ converges to zero in probability and $X_n=\mathcal{O}_\Pr(1)$ that $(X_n)_{n\in\N}$ is stochastically bounded. We frequently use the notation
\[ \Pr( A,B ) := \Pr(A\cap B).\]
Furthermore, throughout the whole paper, we fix constans $A,\gamma,\sigma>0$ and $C\geq 1$ that are used in the definition of the drift function class $\Sigma(C,A,\gamma,\sigma)$ given in Section~\ref{Sec_Notation}. Additionally, $L_*$ and $L^*$ are fixed as the constants for the uniform lower and upper bounds on the invariant density $q_b$ over the class $\Sigma(C,A,\gamma,\sigma)$ that are provided by Lemma~\ref{bound_invariant_density} and \ref{uniform_lower_bound_invariant_density}.







==> Version_ArXiv/Sections/Introduction.tex <==
\section{Introduction}

\paragraph{Motivation}
In many areas such as physics or financial mathematics, numerous time-continuous dynamics are naturally described by a diffusion process. Moreover,
diffusions arise frequently as scaling limits of jump process modelings. For instance, the stochastic SIS model in epidemiology reveals an Ornstein-Uhlenbeck process as a scaling limit. Therefore, stochastic differential equations have become an important subject of investigation in nonparametric statistics. 

Within the standard nonparametric scalar diffusion model where Brownian motion is the driving noise, the aim of our paper is to develop an efficient multiple test to infer about \textit{similarity} of an unknown drift $b$ to some reference drift $b_0$: At prescribed significance, we want to identify simultaneously those regions where violation from similiarity occurs, without a priori knowledge of their number, size and location.
Here, a drift $b$ is said to be similar to $b_0$ at tolerance $\eta\geq 0$ within some interval $I$ if
\[ b_0(x)-\eta \leq b(x)\leq b_0(x) +\eta\quad \textrm{ for all } x\in I.\]
Once regions of deviation from similarity are identified at level of significance $\alpha$, the null hypothesis of the \textit{similarity testing problem}
%we can even claim at the same significance that they \textit{do exist}, i.e. we also come up with a solution to the testing problem 
\begin{align}\label{eq: Testing_problem}
H_0:\ \sup_{x\in I}|b(x)-b_0(x)| \leq \eta \quad \textrm{ versus }\quad H_1:\ \sup_{x\in I} |b(x)-b_0(x)|>\eta
\end{align} 
is rejected. 
Sometimes, it is unrealistic to assume that the reference $b_0$ is exactly specified, and testing for exact equality $b=b_0$ is impossible. But even if the reference $b_0$ is available, testing $b=b_0$ may miss the point in many applications because 'sufficiently close' is equally convenient. 
The relevance of testing hypotheses of the form \eqref{eq: Testing_problem} for $\eta>0$ has meanwhile been widely acknowledged in many different fields of statistical inference such as financial, medical, pharmaceutical or environmental statistics, see \cite{Altman}, \cite{Buecher}, \cite{Dette}, \cite{Fogarty}, \cite{McBride}, \cite{Romano} and \cite{Wellek} including references cited therein. Note that testing for similarity avoids the consistency problem mentioned in~\cite{Berkson}, i.e. that any consistent test will detect arbitrary small deviations in the drift if the sample size is sufficiently large. 


\vspace{-0.2cm}

\tiny
\begin{center}
\begin{figure}[h]
\begin{tikzpicture}
\draw [thick] (0,0) -- (10,0);

%\filldraw[black] (1,0) circle (1pt) node[anchor=north] {$-A$};
%\filldraw[black] (9,0) circle (1pt) node[anchor=north] {$A$};

\draw[blue, domain=0.5:9.5] plot (\x,{2+0.01*(\x-5)^3}) node(1){};
\draw[blue, domain=0.5:9.5, dotted] plot (\x,{1.5+0.01*(\x-5)^3}) node(2){};
\draw[blue, domain=0.5:9.5, dotted] plot (\x,{2.5+0.01*(\x-5)^3}) node(3){};

\draw[green, domain=0.5:4] plot (\x,{2+0.01*(\x-5)^3 +0.3*sin(70*\x)}) {};
\draw[green, domain=4:4.7] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (\x-4)^2}) {};
\draw[green, domain=4.7:5.3] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +1.5*(\x-4.7)^2)}) {};
%\draw[green, domain=5.3:6.5] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +2*(5.3-4.7)^2) + sin(150*(\x-5.3) -1}) {};
%\draw[green, domain=6.5:9.5] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +2*(5.3-4.7)^2) + sin(150*(6.5-5.3) -1 -sin(300*(\x-6.5+pi/2) }) {};

\draw[green, domain=5.3:7.5] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +1.5*(5.3-4.7)^2) + 0.7*(\x-5.3)^(1/1.5) }) {};
\draw[green, domain=7.5:8.5] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +1.5*(5.3-4.7)^2) + 0.7*(7.5-5.3)^(1/1.5) -0.3*(\x-7.5)^(1.8) }) {};
\draw[green, domain=8.5:9.5] plot (\x,{2+0.01*(4-5)^3 +0.3*sin(70*4) - (4.7-4)^2 +1.5*(5.3-4.7)^2) + 0.7*(7.5-5.3)^(1/1.5) -0.3*(8.5-7.5)^(1.8) - 0.25*sin(220*(\x-8.5) }) {};

\draw[-, green, dotted] (4.45,0)--(4.45,1.5);
\draw[-, green, dotted] (5.15,0)--(5.15,1.5);
\draw[-, green, dotted] (6.5,0)--(6.5,2.54);
\draw[-, green, dotted] (8.1,0)--(8.1,2.82);
\draw [green, thick] (4.45,0) -- (5.15,0);
\draw [green, thick] (6.5,0) -- (8.1,0);


\draw[|-|, red] (4,2)--(4,2.5) node[right, midway]{$\eta$};

\node [right, color=blue] at (1) {$b_0$};
%\node [right, color=cyan] at (2) {$b_0-\eta$};
%\node [right, color=cyan] at (3) {$b_0+\eta$};

\end{tikzpicture}
\caption{\small{An illustration of a function $b_0$ and its $\eta$-environment, together with some other drift function and the intervals of deviation from the null.}}\label{Fig_1}
\end{figure}
\end{center}
\normalsize


\vspace{-0.5cm}

Since, as mentioned above, diffusion models arise frequently as scaling limits of jump processes, another aspect is of particular importance: Small perturbations in the jump process modeling lead to a different drift in the limiting diffusion, but they \textit{might} change the process class of the driving noise as well. In consequence, when testing for similarity of the drift to the drift of a reference model, the true noise may only be close to that of this reference model, and testing is only meaningful under some stability properties with respect to the driving noise specification.

Besides, in applications where a nontrivial dependence structure in time is present, the driving noise is not given by Brownian motion. In such situations, fractional diffusion models have become increasingly popular (cf. \cite{Ait}, \cite{Gatheral}, \cite{Mishura} and references therein). However, in contrast to standard diffusion, fractional diffusions neither belong to the process class of Markov processes nor semimartingales. Thus, the number of tools for statistical analysis is rather limited. In view of the non-availablity of efficient nonparametric testing procedures in such cases, stability justifies to use tests developed for the standard diffusion model at least in situations where the driving noise is close to Brownian motion in a suitable sense.





%For example in stochastic epidemic modelling, jump processes describing the number of infected people are approximated by diffusion models for large size of population (cf. Pardoux and Kurtz...). In such situations, small perturbations of the state-discrete model lead to a different drift in the limiting diffusion and they \textit{might} change the process class of the driving noise. \\

 

%At the same time, the procedure should be robust under small deviation from Brownian motion as the driving noise process. A detailed investigation for fractional driving noise, which is neither a semimartingale nor a Markov process, is provided for Hurst indices close to the Brownian motion case.\\
%Although being conceptually two completely different aspects, both the similarity hypothesis and the stability property robustify the statistical analysis of the diffusion model:

%The assumption of independent increments for the driving noise is a limitation in application where nontrivial dependence structures in time appear in several settings, see .... for examples of fractional diffusion models. In these cases a stability property for $H\approx 1/2$ of the similarity testing is desirable from two perspectives. First, one may not realize from discrete oberservations that the driving noise is in fact no Brownian motion and the model is missspecified. Secondly, non-availablity of advanced testing procedures for fractional models up to now suggests to use tests developed for the wrong model at least in a neighborhood of the Brownian case.








 

\paragraph{Main contributions}
For $\eta>0$, the null in \eqref{eq: Testing_problem} is a composite hypothesis, and our goal is to construct for any significance level $\alpha\in (0,1)$ a multiple testing procedure $\phi_\eta$ to infer about local deviations from similarity under the constraint
\begin{align*}
\sup_{b\in H_0} \E_b\left[ \phi_\eta\right] \leq \alpha.
\end{align*} 
To this aim, we employ the multiscale approach that has been proven to be successful in a large variety of scenarios (cf. \cite{Datta}, \cite{Walther}, \cite{Duembgen/Spokoiny}, \cite{Koenig}, \cite{Proksch}, \cite{Rohde_2} and  \cite{Rohde}), though not including stochastic differential equations. 
%The identification of regions of violation from similarity relies on local likelihood ratio statistics. A test statistic $T_\eta(X)$ for~\eqref{eq: Testing_problem} based on observations $X=(X_t)_{t\in [0,T]}$ is then given as a supremum combination of those. There exists a vast amount of testing problems in the literature where this multiscale approach has been applied (cf. \cite{Datta}, \cite{Walther}, \cite{Duembgen/Spokoiny}, \cite{Koenig}, \cite{Proksch}, \cite{Rohde_2} and  \cite{Rohde}). The closest in spirit to our procedure is the test developed in \cite{Duembgen/Spokoiny} and related works such as \cite{Datta}, \cite{Walther} and \cite{Rohde}.
While composite hypotheses in the context of multiscale testing have been 
studied in situations where the boundary of the hypothesis is least favourable in the sense of stochastic ordering (cf. \cite{Walther}, \cite{Duembgen/Spokoiny}), the situation for the composite similarity hypothesis for the drift of ergodic diffusions is substantially more intricate. 
Although our multiscale test statistic is motivated by the idea of simultaneously testing $b\leq b_0+\eta$ and $b\geq b_0-\eta$ pointwisely, %\textit{assuming} that these one-sided composite hypotheses can be tested for their boundary cases. However,
there is no evidence that the boundary cases are least favourable for the null hypothesis of similarity. Indeed, the stochastic order relation required for this purpose may be missing even for the corresponding local likelihood ratio statistics. The reason is that their distribution does not only depend on local values of the drift $b$, but on the entire drift function via the invariant density.\\


Our main contributions are the following: 

\begin{itemize}
\item[(i)] Based on a multiscale statistic in the spirit as described above and for any significance level $\alpha\in (0,1)$, we construct a threshold level such that the resulting test $\phi_T^\eta$ for the testing problem \eqref{eq: Testing_problem} satisfies
\begin{align}\label{eq: level_asymp}
\limsup_{T\to\infty} \sup_{b\in H_0} \E_b\left[ \phi_T^\eta\right] \leq \alpha,
\end{align} 
where $T$ denotes the time horizon of the diffusion's observation. Note that \eqref{eq: level_asymp} is a substantially stronger statement than the pointwise relation $\limsup_{T\to\infty} \E_b[\phi_T^\eta]\leq\alpha$ for all $b\in H_0$. For the derivation of \eqref{eq: level_asymp}, we construct a random variable $Y_\eta$
%However, it is not clear that these are least favourable cases in the sense of stochastic ordering, leaving open the specification of a threshold level to define a test $\phi_T^\eta$ based on $T_T^\eta$ that fullfills \eqref{eq: level_H0_intro} for fixed $T$. This issue remains in the limit $T\to\infty$ due to the influence of the invariant density of the observed diffusion process, although $b_0\pm\eta$ seem to be \textit{close} to being least favourable cases. We find this last observation to be true in the following sense:
\begin{itemize}
\item that provably dominates the test statistic \textit{uniformly} on the similiarity hypothesis in stochastic order asymptotically and %, i.e. for $r\in\R$,
%\[ \limsup_{T\to\infty} \sup_{b\in H_0} \Pr_b\left( T_T^\eta(X)\geq r\right) \leq \Pr(Y_\eta\geq r), \textrm{ and}\] 
\item whose distribution depends continuously on the level $\eta$ of similarity, and $Y_0$ equals the limiting distribution of the test statistic under the simple null.
\end{itemize}

The cornerstone of the construction of $Y_\eta$ is the identification of the weak limit of the multiscale test statistic \textit{uniformly} in $b\in H_0$. Whereas weak limit results for supremum statistics like ours have been derived in various settings (cf. \cite{Walther}, \cite{Proksch}, \cite{Rohde_2} and \cite{Rohde}), the additional uniformity in the drift parameter accounting for the composite null in \eqref{eq: Testing_problem} is new and considerably more involved on a mathematical level.




\item[(ii)] We prove optimality and adaptivity for the similarity test in the minimax sense, as introduced in \cite{Ingster1} and \cite{Ingster2}.
We exemplarily consider the case of alternatives belonging to some Hölder class $\mathcal{H}(\beta, L)$ where deviations are measured in weighted supremum norm which is the equivalent to weighted risk definitions in sharp adaptive drift estimation like \cite{Dalalyan} or \cite{Strauch_2}. Our similarity test is shown to be rate-optimal in the minimax sense, adaptive in both the unknown parameters $\beta$ and $L$, optimal in the constant for the regime $\beta\leq 1$ and here, even sharp adaptive in $L$. %, whereas this condition turns out to be unneccessary for the simple null where we establish sharp adaptive results over any class $\mathcal{H}(\beta, L)$. 
The hypotheses construction in the proof of the lower bound involves a delicate fixed point problem as the drift itself appears in the invariant density which pops up in the deviation measure between null and alternative.


\item[(iii)] We address the problem of stability for fractional diffusion models
where the driving Brownian motion is replaced by a fractional Brownian motion with Hurst index $H\in (0,1)$. Note that $H=1/2$ corresponds to standard Brownian motion.
We prove that the test statistic built from observations in the fractional diffusion model has strong performance properties as the fractional driving noise approaches Brownian motion in the following sense:
\begin{itemize}
\item The test is \textit{uniformly} over the hypothesis of similarity of approximate level $\alpha$, i.e. (slightly simplified)
\begin{align}\label{eq: level_alpha_H}
\limsup_{T\to\infty} \limsup_{H\to\frac12}\sup_{b\in H_0} \E_b^H\left[\phi_T^\eta \right] \leq \alpha,  
\end{align} 
where $\E_b^H$ denotes the expectation when applied to fractional diffusion with Hurst index $H$ and drift $b$.

\item We prove that the minimax optimality is preserved in a certain sense as the fractional driving process approaches Brownian motion.
\end{itemize}


As our test statistic for $\phi_T^\eta$ involves a stochastic integral which is not even defined for fractional diffusion observations a priori,
we first introduce a pathwise continuation of the statistic as a function of the data that is continuous with respect to the topology of uniform convergence. Then, \textit{uniformly} over the similarity hypothesis, we prove that the test statistic built from observations for fractional driving noise converges for $H\to 1/2$ in probability to that built for standard Brownian motion. This uniformity, which is substantially harder to derive than the corresponding pointwise result for any fixed drift, is crucial in order to deduce \eqref{eq: level_alpha_H}.
The preservation of minimax properties relies on $L^1(\Pr)$-convergence of likelihood ratios of the fractional diffusion model to those of the standard model. This derivation is based on (deterministic) fractional calculus (cf. \cite{Samko}).


%Although the ansatz for constructing the multiple test is equally reasonable for fractional diffusions, the corresponding likelihood ratios are rather bulky and by far less accessible for sophisticated multiscale analysis which is already involved in the case of Brownian motion. 
%For fractional diffusions close to standard Brownian diffusion, the standard Brownian diffusion model, being mathematically much easier, may still provide an excellent description of the fractional dynamics.



\item[(iv)] We outline how to extend our results to the multidimensional case. While the construction of a multiscale test statistic is possible in higher dimension, an identification of a dominating random variable as in (i) for $\eta>0$ is not available a priori. % However, the identification of a quantile is immediate in 
However, in case of the simple null hypothesis $\eta=0$, minimax rate-optimality can be attained. This extension is mainly of technical nature as local time does not exist in higher dimension. % it is possible to achieve rate-optimality for the minimax results described in (ii). \\ %Whether the efficiency constant is attained in higher dimension remain open, because the argument used to prove solvability of the fixed point problem mentioned in (ii) is not available in higher dimension. \\
Our stability results for the fractional diffusion model do neither transfer straightforwardly. Instead, we present a pathwise stability approach based on the theory of rough paths which was first introduced by Lyons in \cite{Lyons}. The presentation includes a rough path version of our test that is close in spirit to a similar rough path version of maximum likelihood estimators in \cite{Diehl/Friz}.


%We outline how to extend our results to the multidimensional case.
%An extension for the construction of the test statistic and minimax results are mainly of technical nature as local time does not exist in higher dimension. \textcolor{blue}{In particular, an extension for the simple null is straightforward, whereas the identification of threshold as in (i) does not transfer as there are infinitely many boundary cases in higher dimension.
%Even for the simple null}, our stability results for the fractional diffusion model do not transfer straightforwardly. Instead, we present a pathwise stability approach based on the theory of rough paths which was first introduced by Lyons in \cite{Lyons}. The presentation includes a rough path version of our test that is close in spirit to a similar rough path version of maximum likelihood estimators in \cite{Diehl/Friz}.
\end{itemize}







The article is organized as follows. Model description and notation are given in Section~\ref{Sec_Notation}. In Section~\ref{Sec_simple}, we tackle the technical difficulties of constructing a powerful multiscale statistic for the simple null $b=b_0$ which are due to the context of ergodic diffusions. 
Section~\ref{Sec_similarity} contains the results described in (i), including the development of a multiscale test for the composite similarity hypothesis. 
Power properties as summarized in (ii) are given in Section~\ref{Sec_Power}.
The stability results (iii) are content of Section~\ref{Sec_Stability}. % Section~\ref{Sec_Implementation} includes computational aspects and an extended simulation study.
In Section~\ref{Sec_weak}, a route of proof of the main result in (i) is presented. Here, the crucial limit theorem for the supremum statistic with weak convergence \textit{uniformly} over the null hypothesis is stated.
An outline of the proof of the lower bound with the fixed point argument of (ii) is presented in Section~\ref{Sec_supp}. Section~\ref{Sec_outlook} outlines the extension of our results to the multidimensional case as described in (iv).
All proofs as well as an extended simulation study are deferred to the supplementary material.



%which is built by correcting a least favourable case of the weak limit by some additive constant depending on the similiarity level $\eta$.
%In Section~\ref{Sec_Power} the power properties are given for both the similiarity test and the simple null. Proving the lower bound with optimal constant relies on the construction of boundary alternatives involving a fixed point problem. As a new contribution, this is outlined in Section~\ref{Sec_supp}. The investigation concerning pathwise stability results and the fractional model missspecification are presented in Section~\ref{Sec_Stability}. Subsequent, a numerical example is given in Section~\ref{Sec_Implementation} and the outlook to the multidimensional case is presented in Section~\ref{Sec_outlook}.













%Last but not least, we want our test to depend continuously on the data, i.e. that it produces similar results of oberservations $(X_t)_{t\geq 0}$ and $(\tilde{X}_t)_{t\geq 0}$ that are close in some metric. With this property an investigation of the test's behavior under model missspecification becomes feasible. For example, the noise may be described by a fractional Brownian motion $W^H$ with Hurst parameter $H$ close to $\frac12$, the case of standard Brownian motion. Although the true Hurst index can be recovered as a path property, robustness properties of the test are of practical relevance in such a situation. First, because estimating $H$ may be accompanied by minor errors and second, because the test still produces reasonable results under this robustness property for $H\approx\frac12$.\\ 

%The testing problem of similarity clearly comes up with a composite null.
%In such a setting one usually considers a least favourable case within this hypothesis to built the test upon. This means that for a test $T$ we have a stochastic order of the form
%\[ \sup_{b\in H_0} \Pr_b( T\geq r) \leq \Pr_{\tilde{b}} (T\geq r) \]
%for all $r\in\R$ and a least favourable drift $\tilde{b}$. In a regression setting it is not hard to see that intuition holds true and the least favourable case is given by the boundary of the null, see \cite{Duembgen/Spokoiny}. In our case this would correspond to those $b$ fullfilling $\|b-b_0\|=\eta$. However, the model of an ergodic diffusion imposes new technical difficulties which makes identification of a least favourable case substantially more difficult. This is described in more detail in Section $3.2$.\\

%The power investigation follows the minimax approch introduced by Ingster in \cite{Ingster1} and \cite{Ingster2} that allows the alternative to be an entire function class that separates the null hypothesis from the alternative by some distance. 
%In our case the alternative will belong to some Hölder class $\mathcal{H}(\beta, L)$ and deviations are measured in weighted supremum norm. This setup raises another specification for our test, namely we want it to detect in a minimax optimal way without a priori knowledge of $\beta$ and $L$.\\
%The first who considered such kind of testing problem in supremum norm with a sharp adaptive result were Dümbgen and Spokoiny in \cite{Duembgen/Spokoiny} for a deterministic drift and the convex hypotheses that the drift is negative, nonincreasing or convex.\\
%Inspired by this work, we start building a multiscale test for the simple null by combining certain local test statistics that account for our lack of knowledge where the deviation occurs and of what form it is. \\
%Nevertheless, the diffusion setting imposes many new technical difficulties. On a conceptual level there are two important aspects of it. First, some arguments from empirical process theory have to be adopted to combine them with stochastic analysis. This particularly implies bounding random covering numbers for a semi-metric given in terms of the quadratic variation of $X$ and finding sub-gaussian tail bounds for certain local test statistics. This is important to design a non-degenerate multiscale test statistic.\\
%Secondly, for each drift $b$ we have to take the invariant distribution with Lebesgue density $q_b$ into account. Intuitively, deviations are harder to detect at a certain location $y$ when the process spends less time in a neighborhood of $y$ which corresponds to a lower value of $q_b(y)$. For this reason we have to use a weighted supremum norm for our power consideration to establish optimality not only in the rate, but also in the constant. The weight is given in terms of the invariant density, similar to the weighted $L^2$-risk in Dalalyans sharp adaptive drift estimation result in \cite{Dalalyan}. But to our knowledge, our usage of the weighted sup-norm is new in the literature about nonparametric statistics of ergodic diffusions.\\
%%Another obstacle involving the invariant density is the identification of a least favourable case within the null $\mathcal{H}_\eta(b_0)$. Compared to \cite{Duembgen/Spokoiny} it is not at all clear that they are given by the boundary cases $b_0\pm\eta$. To overcome this, we establish uniform weak convergence results of our test statistic to identify an asymptotically least favourable case. \\
%Once this is done, we are able to establish rate optimal adaptive lower and upper bounds in the minimax sense. For similarity testing we even get the optimal constant in the regime $\beta\leq 1$, whereas this condition turns out to be unneccessary for the simple null where we get sharp adaptive results over any class $\mathcal{H}(\beta, L)$. \\



%Althought adaptive procedures solve the problem of dealing with unknown smoothness parameters, a model misspecification is not covered at all. In Diehl et al. \cite{Diehl/Friz} pathwise stability of maximum likelihood estimators was considered using rough path theory. This theory was originally developed by Lyons in the mid 1990's and culminated in the landmark paper \cite{Lyons}. Both \cite{Friz/Hairer} and \cite{ Friz/Victoir} are excellent sources on the subject. In Section $4$ we deal with the problem of misspecification of the noise and suppose the SDE is not driven by a Brownian motion, but a fractional Brownian motion with Hurst index $H\approx\frac12$ close to the case of a standard Brownian motion. The question arising from a practical point of view is wether the test completely misbehaves in such a situation or if it is robust in a certain sense and produces still reasonable results. To the best of our knowledge this kind of problem has not been addressed in the realm of nonparametric statistics althought first attempts have been made to estimate parameters of fractional diffusion models \textbf{keep this part?}.\\
%We take first steps in this direction and show that our test still detects with probability $1-\epsilon$ for $H$ close enough to $\frac12$. The key insight here is that we are able to formulate a rough version of our test statistic using rough integration that allows to insert solutions of fractional diffusions and that we can show its continuity in the Hurst parameter. Moreover, we show by continuity of the likelihood ratios of the fractional and the classical model that no substantial improvement of this test is possible in the limit $H\to\frac12$.\\




%The main contributions of this article are the following.
%
%\begin{enumerate}
%\item[(1)] We develop a test  that checks if the drift $b$ is sufficiently similar to some reference drift on some compact interval, i.e. if $b\in\mathcal{H}_\eta(b_0)$. If not, we want to detect the regions of violation with prescribed significance.\\
%We show that it is rate-optimal in the minimax sense and even exact for alternatives belonging to Hölder classes $\mathcal{H}(\beta, L)$ for $\beta\leq 1$. For the boundary case of the simple null $\eta=0$ the test is exact for all $\beta>0$.
%\item[(2)] It is intuitive that the invariant density $q_b(y)$ amounts to how small detectable deviations at location $y$ may be. This dependence is explained in a mathematically rigorous way. It is crucial to get the best possible constants in the power considerations. On the other hand, its appearance impedes the construction of alternatives within the lower bound and gives rise to a fixed-point problem (see Section $5$ for details).
%\item[(3)] Developing the similarity test includes identification of an asymptotically least favourable case within the null $\mathcal{H}_\eta(b_0)$ - which is a highly non-trivial task: In principal, if $b_1(y)-b_0(y)$ is smaller than $b_2(y)-b_0(y)$ we would expect this deviation to be harder to detect, but a larger invariant density $q_{b_1}(y)> q_{b_2}$ could make up for the smaller difference.
%\item[(4)] To identify an asymptotically least favourable case, we derive weak limits of our test statistic that are uniform over the composite hypothesis and in fact uniform over the whole class $\Sigma(C,A,\gamma,\sigma)$ as this requires no extra tools. This includes some results about uniform weak convergence that may be interesting on their own.
%\item[(5)] Computability of the test is discussed and a simulation study is given.
%\end{enumerate}




==> Version_ArXiv/Sections/Multiscale_Test.tex <==
\section{The multiscale test for similarity}\label{Sec_similarity}

In this section we construct a test statistic for the similarity testing problem presented in the introduction. In particular, it comprises the derivation of a quantile that ensures validity on the composite null which is a highly non-trivial contribution as indicated in Section \ref{SubSec_one-sided}.\\
Before we start, we fix some additional notation to formulate the testing problem in a mathematical rigorous way. Therefore, letting $\eta\geq 0$ and choosing a reference drift $b_0$ we formulate the composite null hypothesis as
\[ H_0(b_0,\eta) := \left\{ b\mid \| b-b_0\|_{[-A,A]} \leq \eta\right\} \cap \Sigma(C,A,\gamma,\sigma).\]
This composite hypothesis will be testet against its complement in $\Sigma(C,A,\gamma,\sigma)$, i.e.
\begin{align}\label{eq: H1_eta}
H_1(b_0,\eta) := \left\{ b\mid \| b-b_0\|_{[-A,A]} > \eta\right\} \cap \Sigma(C,A,\gamma,\sigma).
\end{align}
In this notation $\eta$ describes the extent of similarity. The smaller $\eta$, the more similar are $b_0$ and $H_0(b_0,\eta)$. In particular, we also cover the case $\eta=0$ where the null is the simple hypothesis $\{b_0\}$ from the preceeding section. 
%Being a minor restriction, we assume $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$. This choice of $b_0$ ensures that both $b_0\pm\eta\in \mathcal{H}_\eta(b_0)$ as shown in Appendix A. 





\subsection*{Construction of the similarity test}

The first insight for constructing the similarity test is that $\{ \|b-b_0\|_{[-A,A]} \leq \eta\} $ may be written as
\begin{align*}
\bigcap_{y\in [-A,A]} \{ b(y)\leq b_0(y)+\eta\} \cap \{ b(y)\geq b_0(y)-\eta \},
\end{align*}
proposing that testing for similarity is the same as testing for two one-sided hypotheses. The construction from Section~\ref{SubSec_one-sided} then suggests the statistic
\begin{align}\label{eq: Motivation_test_similarity}
\begin{split}
&\max\left\{ \Psi_{T,y,h}^{b_0+\eta}(X), -\Psi_{T,y,h}^{b_0-\eta}(X)\right\} \\
&\hspace{2cm} \leq \max\left\{ \Psi_{T,y,h}^{b_0} - \Lambda_{T,y,h}^\eta(X), -\Psi_{T,y,h}^{b_0}(X) - \Lambda_{T,y,h}^\eta(X)\right\}\\
&\hspace{2cm} \leq \left|\Psi_{T,y,h}^{b_0}(X)\right| - \Lambda_{T,y,h}^\eta(X)
\end{split}
\end{align}
for testing for deviation at a certain location $y$ with 
\[ \Lambda_{T,y,h}^\eta(X) := \frac{\eta \int_0^T K_{y,h}(X_s) ds}{\sigma\sqrt{ \int_0^T K_{y,h}(X_s)^2 ds}}.\]
Combining those localized statistics in the same way as in Section~\ref{Sec_simple} for $(y,h)\in\mathcal{T}$ given in \eqref{eq: cT} then yields the ansatz
\begin{align}\label{eq: T_eta}
T_T^\eta(X) := \sup_{(y,h)\in\mathcal{T}} \left(\left| \Psi_{T,y,h}^{b_0}(X)\right| - \Lambda_{T,y,h}^\eta(X)- C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2) \right)
\end{align} 
as a test statistic for $H_0(b_0,\eta)$ against $H_1(b_0,\eta)$ given in \eqref{eq: H1_eta}.
As our test has to be valid on $H_0(b_0,\eta)$ we have to identify a value $\kappa$ such that
\begin{align}\label{eq: kappa_T}
\sup_{b\in H_0(b_0,\eta)} \Pr_b\left( T_T^\eta(X) >\kappa \right) \leq \alpha.
\end{align} 
In order to guarantee high power on the alternative, $\kappa$ should be chosen as small as possible to fullfill \eqref{eq: kappa_T}. However, the standard approach which is identifying a least favourable case $\tilde{b}\in H_0(b_0,\eta)$, namely
\[ \sup_{b\in H_0(b_0,\eta)} \Pr_b\left( T_T^{\eta}(X) > \kappa\right) \leq \Pr_{\tilde b}\left(T_T^{\eta}(X) > \kappa\right),  \] 
and choosing $\kappa$ as the quantile of $T_T^\eta$ under $\Pr_{\tilde{b}}$ fails: One might expect that least favourable cases are given by the boundary cases $b_0\pm\eta$ in terms of stochastic order, 
%\begin{align*}\label{eq: stoch_order}
%\sup_{b\in\mathcal{H}_\eta(b_0)} \Pr_b\left( T_T^\eta(X) \geq r\right) \leq \Pr_{b_0\pm\eta}\left( T_T^\eta(X)\geq r\right) 
%\end{align*}
but this is totally unclear which can be seen as follows. 
%Bounding the variables $|\Psi_{T,y,h}^{b_0}(X)| - \Lambda_{T,y,h}^\eta(X)$ within the supremum in \eqref{eq: T_eta} by the triangle inequality gives
When decomposing $|\Psi_{T,y,h}^{b_0}(X)|$ into
\begin{align}\label{eq: 8.1}
\left| \frac{\int_0^T K_{y,h}(X_s) dW_s}{\sqrt{  \int_0^T K_{y,h}(X_s)^2 ds}} +\frac{\int_0^T K_{y,h}(X_s)(b(X_s) - b_0(X_s)) ds}{\sqrt{  \int_0^T K_{y,h}(X_s)^2 ds}}  \right|, %- \frac{\eta  \int_0^T K_{y,h}(X_s) ds}{\sigma \sqrt{ \int_0^T K_{y,h}(X_s)^2 ds}} 
\end{align} 
%\begin{align}\label{eq: 8.1}
%\left| \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h}(X_s) dW_s}{\sqrt{ \frac1T \int_0^T K_{y,h}(X_s)^2 ds}}\right| + \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h}(X_s)  ( |b(X_s) - b_0(X_s)|-\eta ) ds}{\sigma \sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} 
%\end{align} 
the construction reveals that for any  $b\in H_0(b_0,\eta)$, the first summand within the absolute value is tight, whereas the absolute value of the second one is bounded by $\Lambda_{T,y,h}^\eta(X)$ and equal to $\Lambda_{T,y,h}^\eta(X)$ for the boundary cases $b=b_0\pm\eta$. Although this suggests these boundary cases to be least favourable candidates in the sense of stochastic ordering, the distribution of the first summand in \eqref{eq: 8.1} still depends on $b$ -- as a process in $(y,h)$ even asymptotically in terms of finite dimensional distributions -- and no stochastic order relationship as in \cite{Duembgen/Spokoiny} is available. Moreover, the distribution of the argument of $C(\cdot)$ in \eqref{eq: T_eta} depends on $b$ as well. Nevertheless, $b_0\pm \eta$ seems to be \textit{close} to the least favourable case. Indeed, we find this closeness to be true \textit{uniformly} in the limit $T\to\infty$.




\begin{thm}\label{worst_case_delta}
Let $T_T^\eta$ be given as in \eqref{eq: T_eta} with a non-negative kernel function $K$ of bounded variation supported in $[-1,1]$ with $\|K\|_{[-1,1]}\leq 1$. % which is bounded by one. 
Furthermore, assume that $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$. Pick a relatively compact subset of $H_0(b_0,\eta)$, again denoted by $H_0(b_0,\eta)$. Then we have for any $r\in\R$,  
\[ \limsup_{T\to\infty} \sup_{b\in H_0(b_0,\eta)}\Pr_b\left( T_T^\eta(X) \geq r\right) \leq \Pr\left( U_1\vee U_2 + 4\sqrt{A\eta/\sigma^2} \geq r\right),\]
where $U_1\vee U_2$ denotes the (pointwise) maximum of $U_1$ and $U_2$ given by
\begin{align*}
U_1 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_{b_0+\eta}(z)} dW_z}{\|K_{y,h}\sqrt{q_{b_0+\eta}}\|_{L^2}}\right| - C\left(\frac{\|K_{y,h}\sqrt{q_{b_0+\eta}}\|_{L^2}^2}{\| \1_{[-A,A]}\sqrt{q_{b_0+\eta}}\|_{L^2}^2}\right)\right),\\
U_2 &:= \sup_{(y,h)\in\mathcal{T}} \left( \left|\frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_{b_0-\eta}(z)} dW_z}{\|K_{y,h}\sqrt{q_{b_0-\eta}}\|_{L^2}}\right| - C\left(\frac{\|K_{y,h}\sqrt{q_{b_0-\eta}}\|_{L^2}^2}{\| \1_{[-A,A]}\sqrt{q_{b_0-\eta}}\|_{L^2}^2}\right)\right).
\end{align*} 
\end{thm}


The proof of this result is the most elaborate one in this article and Section \ref{Sec_weak} contains a route of it together with a uniform weak convergence result of the supremum statistic developed in Section \ref{Sec_simple}. This uniform weak convergence is both the most important ingredient for Theorem \ref{worst_case_delta} and interesting on its own. In addition, some general results about uniform weak convergence are derived that may be of independent interest and can be found in Section \ref{Sec_weak} as well. The complete proof of Theorem \ref{worst_case_delta}, which can be found in Appendix \ref{App_least}, is then a sophisticated combination of this weak convergence result and stochastic analysis tools together with the explicit representation of the invariant density that occurs in the limiting statistic. 




\begin{remark}\label{remark_Piterbarg}
It is shown in \cite{Piterbarg} that a supremum statistic like $U_1$, without the normalizing factor $\sqrt{q_b}$ in nominator and denominator, has a distribution without point mass. We prove that this is also true for $U_1\vee U_2$ in Appendix~\ref{SubSecD2}, which is important to conclude that our test based on the test statistic $T_T^\eta$ is uniformly asymptotically of level $\alpha$, see \eqref{eq: asym_level_alpha} below.
\end{remark}



%\begin{remark}
%Theorem \ref{worst_case_delta} is the reason for working with the normalization of $\hat\sigma_T(y,h)$ by $\hat\sigma_{\max}$. In principle, this is not crucial for deriving our asymptotic power results, but it allows to specify the additive correction constant $2\sqrt{A\eta}$ without any further assumptions.
%\end{remark}






The limiting statistics $U_1$ and $U_2$ in Theorem \ref{worst_case_delta} are almost surely finite which can be seen analogeously to Theorem \ref{Multiscale_Lemma} and hence the quantiles
\begin{align}\label{eq: kappa_eta_alpha}
\kappa_{\eta, \alpha} := \min \left\{ r\in\R:\ \Pr( U_1\vee U_2 + 4\sqrt{A\eta/\sigma^2} \leq r)\geq 1-\alpha \right\}
\end{align} 
are well-defined. %We reject the null $\mathcal{H}_{\eta}(b_0)$ at level $\alpha$ if 
%\[ T_T^\eta(X)> \kappa_{\eta, \alpha}. \]
For the testing problem $H_0(b_0,\eta)$ versus the alternative~\eqref{eq: H1_eta}, the test 
\begin{align}\label{eq: phi_eta}
\phi_T^\eta(X) = \1_{\left\{ T_T^\eta(X)> \kappa_{\eta,\alpha}\right\}} 
\end{align} 
is by Theorem \ref{worst_case_delta} uniformly (over $H_0(b_0,\eta)$) asymptotically of level $\alpha$, i.e.
\begin{align}\label{eq: asym_level_alpha}
\limsup_{T\to\infty}\sup_{b\in H_0(b_0,\eta)} \Pr_b\left(\phi_T^\eta(X) =1 \right) \leq \alpha. 
\end{align} 



\begin{remark}[Simultaneous detection of regions of deviation]\label{remark_D_alpha}
The test statistic $T_T^\eta(X)$ exceeds the $(1-\alpha)$-significance level if, and only if, the random family
\[ \mathcal{D}_\alpha^\eta := \left\{ (y,h)\in\mathcal{T}: |\Psi_{T,y,h}^{b_0}(X)| - \Lambda_{T,y,h}^\eta(X) > C\left( \hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2\right) + \kappa_{\eta,\alpha} \right\} \]
is non-empty. Therefore, one may conclude that with confidence $1-\alpha$ there is a deviation from $H_0(b_0,\eta)$ on \textbf{every} interval $[y-h, y+h]$ with $(y,h)\in\mathcal{D}_\alpha$. An illustration is given in the simulation study in Section \ref{SubSec_Imp2} of the supplementary material.
\end{remark}










==> Version_ArXiv/Sections/Outlook.tex <==
\section{The multidimensional case}\label{Sec_outlook}

The theory of ergodic diffusions solving a stochastic differential equation of the form \eqref{eq: SDE} is not limited to the scalar case and neither is the statistical analysis. The aim of this section is to depict how our results from Section \ref{Sec_simple}--\ref{Sec_Stability} can be transferred to this multidimensional setting, where conceptually two different kinds of problem arise: 

\begin{itemize}
\item While the construction of a multiscale test statistic is rather straightforward in higher dimension, a generalization of Theorem~\ref{worst_case_delta}, which was already highly non-trivial in dimension $d=1$, is not available a priori. However, the identification of a quantile is immediate in case of the simple null hypothesis $b=b_0$, corresponding to $\eta=0$. Here, also rate-optimality in the minimax sense transfers to higher dimension, where the main obstacle is that no local time and occupation times formula is available in dimension $d>1$. This is merely of technical nature and alternative tools are outlined in Subsection~\ref{SubSec_construction}. 

\item The stability results of Section \ref{Sec_Stability} do need a completely different approach. For the stochastic integrals in our test statistic, we can no longer have a continuous dependence on the data in supremum metric for $d>1$, see Section~$7$ in \cite{Diehl/Friz}. To overcome this problem, we may employ rough path theory to construct a rough path extension of our test. Such an extension, similar in spirit to \cite{Diehl/Friz}, gives a pathwise definition of the test statistic. A continuity result in analogy to Theorem~\ref{thm_continuity} can then be derived with respect to the $\alpha$-Hölder rough path metric instead of the supremum metric. 
%An investigation of multidimensional fractional diffusions is then possible with this pathwise defined test statistic for a fixed drift function $b$. However, transferring the uniformity in the drift $b$ which was crucial for \eqref{eq: level_H} remains an open problem.
Whether higher dimensional analogues of the strong results of Section~\ref{SubSec_fractional_model} with uniformity over the drift can be deduced in this way remains, however, totally unclear.
As to the best of our knowledge, rough path arguments have not yet been used in the literature on nonparametric statistics, the rough path extension of the test is presented in Subsection~\ref{SubSec_stability} in greater detail.
\end{itemize}
 






\subsection{Construction of the test statistic}\label{SubSec_construction}

The similarity hypothesis in dimension $d$ is of the form
\[ H_0: \sup_{x\in I} \|b(x)-b_0(x)\|\leq \eta, \]
where $\|\cdot\|$ denotes some norm on $\R^d$ and $I\subset\R^d$ some rectangle. For the reason of coordinatewise visualization, the maximum norm plays a favourite role. In this case, a natural approach is built upon the idea of constructing multiscale statistics $T_1^\eta, \dots, T_d^\eta$ for the testing problem in each of the $d$ components of the drift and then taking their maximum. For $\eta=0$, these componentwise statistics $T_i^\eta$ can be based on local test statistics in the spirit of those given in \eqref{eq: Psi} for the scalar case, because Girsanov's theorem is equally available in higher dimension. For the similarity hypothesis $\eta>0$, the statistic $T_i^\eta$ for any of the $d$ components can be built according to \eqref{eq: Motivation_test_similarity}.\\ %Depending on the alternative under consideration, one may study disturbances belonging to some isotropic or anisotropic Hölder class. In the latter case, the bandwidth varies in each dimension. \\
For the simple null hypothesis $b=b_0$, the corresponding test $\phi_{b_0}$ is defined as
\[ \phi_{b_0}(X) = \1_{\left\{ \max_{i=1,\dots, d} T_i^\eta(X) >\kappa\right\}}, \]
where $\kappa$ is the $(1-\alpha)$-quantile of the statistic $\max_{i=1,\dots, d} T_i^\eta(X)$ under $\Pr_{b_0}$. Finiteness of the statistic follows as in Theorem~\ref{Multiscale_Lemma}. The uniform concentration results for stochastic time integrals used in its proof cannot be based on the local time any longer which does not exists in dimension $d>1$. Instead, they may be derived using alternative techniques, as for example in \cite{Strauch_2} (cf. Lemma~$2$), see also~\cite{Strauch_3}. Additionally, Proposition~\ref{Exp_ineq} has to be generalized.

For the composite similarity hypothesis, however, the construction of a suitable threshold $\kappa$ remains open. Although the uniform weak limit result Theorem~\ref{weak_conv} generalizes to higher dimension, the identification of a stochastically dominating random variable in the spirit of Theorem~\ref{worst_case_delta} does not. Indeed, while there are only two boundary cases $b_0\pm\eta$ on $[-A,A]$ in dimension $d=1$, there are infinitely many in dimension $d>1$.


%It remains to specify a threshold to construct a test based on the multiscale test statistic described above. For the simple null, this is immediate as we can take the quantile of the statistic. Because a multidimensional version of the uniform limit theorem of the multiscale statistic can be derived with the same techniques as for Theorem~\ref{weak_conv} in dimension one, we can also work with the quantiles of the weak limit that can easily be computed numerically, see Remark~\ref{remark_quantile_simple}. \\
%However, for the composite similarity hypothesis with $\eta>0$, the identification of a stochastically dominating random variable as in Theorem~\ref{worst_case_delta} is not straightforward because there exists infinitely many boundary cases in dimension $d>1$ and not only two as for $d=1$. Basically, one can follow steps (i) and (ii) of the proof of Theorem~\ref{worst_case_delta} to restrict the problem to the boundary of $H_0$, but step (iii) does not transfer as this boundary is not finite.\\

Minimax results in higher dimension are known for multiscale testing, see for example \cite{Datta} and \cite{Rohde}. At least in the case of the simple null, where the extension of the test is straightfoward, rate-optimality in Theorems~\ref{lower_bound} and~\ref{thm_simple_hypothesis} transfers to higher dimension by replacing technical arguments based on the local time and occupation times formula by other concentration results. However, the identification of the optimal constant in the lower bound relies on the solvability of a multidimensional fixed point problem in the spirit of Lemma~\ref{lemma_fixed_point}, but the argument used in its proof is not available in higher dimension.

%This includes the fixed point problem presented in Section \ref{Sec_supp}, whose proof basically relied on the explicit representation of the invariant density $q_b$ and its continuous dependence on $b$ that is also not restricted to dimension $d=1$.












\subsection{Stability of the test statistic}\label{SubSec_stability}

The fractional diffusion model \eqref{eq: SDE_H} can also be considered in higher dimension. However, establishing continuity properties of the test statistic becomes more difficult. In the proof of Theorem \ref{thm_continuity}, the crucial step was so show that the stochastic integrals $\int_0^T K_{y,h}(X_s) dX_s$ in the test statistic depend continuously on the data in supremum metric. Whereas this continuous dependence could be established in dimension one, this no longer is true in dimension $d>1$. An explicit counterexample involving a two-dimensional Ornstein-Uhlenbeck process was constructed by Friz et al. in \cite{Diehl/Friz}, Section~$7$, in the context of maximum likelihood estimation for multidimensional diffusions. To overcome this lack of continuity, they consider the observation as a rough path that allows for continuity statements about rough integrals in rough path metric. This strategy can be adopted to our testing problem as outlined in the following.




\subsection*{Brief description of rough path theory}
Here, we summarize the basic definitions of rough path theory. The presentation is not exhaustive at all, but it will enable the reader to comprehend the rough path extension of our test statistic. The notation follows \cite{Friz/Hairer}, which is also an excellent reference on the subject together with \cite{Friz/Victoir}. In the following, we use the notation $X_{s,t} := X_t - X_s$ and $\|\cdot\|$ for the Euclidean norm.\\

For $\alpha\in (\frac13, \frac12]$, we define the space of $\alpha$-Hölder rough paths, denoted by $\mathscr{C}^\alpha([0,T],\R^d)$, as pairs $(X,\mathbb{X})=:\mathbf{X}$ of functions $X:[0,T]\rightarrow \R^d$ and $\mathbb{X}:[0,T]^2\rightarrow \R^d\otimes\R^d$, with $\otimes$ denoting the tensor product, with the following properties:
\[ \|X\|_\alpha := \sup_{s\neq t\in [0,T]}\frac{\|X_{s,t}\|}{|t-s|^\alpha} <\infty,\quad\quad \|\mathbb{X}\|_{2\alpha} := \sup_{s\neq t\in [0,T]}\frac{\|\mathbb{X}_{s,t}\|}{|t-s|^{2\alpha}}<\infty\]
and we have the so-called \textit{Chen relation}
\[ \mathbb{X}_{s,t} - \mathbb{X}_{s,u} - \mathbb{X}_{u,t} = X_{s,u}\otimes X_{u,t}, \quad s,u,t\in [0,T].\]
If additionally, 
\[ 2\textrm{Sym}(\mathbb{X}_{s,t}) = X_{s,t}\otimes X_{s,t}, \]
where $\textrm{Sym}: \R^d\otimes\R^d\rightarrow \R^d\otimes\R^d$ is given by $v\mapsto \frac12(v+v^*)$ and $v^*$ being characterized by $(v_1\otimes v_2)^* =v_2\otimes v_1$, we call the rough path $(X,\mathbb{X})$ a \textit{geometric rough path}. \\ %and denote the set of all geometric rough paths by $\mathscr{C}_g^\alpha([0,T],\R^d)$.\\
Although the second order process $\mathbb{X}$ is by definition a two-parameter object, it is already fully determined by knowledge of $t\mapsto (X_{0,t}, \mathbb{X}_{0,t})$ by the Chen relation. This makes it reasonable to talk about a path.\\
An illustrative example for our purpose is a Brownian motion $W$ combined with one of the following second order processes:
\[ \mathbb{W}_{s,t}^{\textrm{It\^{o}}} = \int_s^t W_u dW_u \quad \textrm{ or }\quad \mathbb{W}_{s,t}^{\textrm{Strat}} = \int_s^t W_u \circ dW_u,\]
where $\circ$ indicates Stratonovich integration. Note the important fact that usually, there is some choice for the second order process which can be thought of as the definition of the integral of the first order process against itself (and not the other way around!).\\
For $\mathbf{X},\mathbf{Y}\in\mathscr{C}^\alpha([0,T],\R^d)$, the $\alpha$-Hölder rough path metric is given by
\[ d_\alpha(\mathbf{X},\mathbf{Y}) := \|X_0-Y_0\| +\sup_{s\neq t\in[0,T]}\frac{\|X_{s,t}-Y_{s,t}\|}{|t-s|^\alpha} + \sup_{s\neq t\in [0,T]}\frac{\|\mathbb{X}_{s,t}-\mathbb{Y}_{s,t}\|}{|t-s|^{2\alpha}}.\]
Finally, we need an integration theory for rough paths. Let $\mathcal{L}(\R^d, \R^m)$ denote the linear maps from $\R^d$ to $\R^m$ which can be identified with their matrix representation in $\R^{dm}$. For any $F:\R^d\rightarrow \mathcal{L}(\R^d, \R^m)$ which is bounded and twice differentiable (considered as a function from $\R^d\rightarrow\R^{dm}$) with derivative $DF$, this derivative is in turn understood as a map from $\R^d$ to $\mathcal{L}(\R^d\otimes\R^d,\R^m)\cong \mathcal{L}(\R^d,\mathcal{L}(\R^d,\R^m))$, see  Section~$1.4$ in \cite{Friz/Hairer}. For those $F$, the rough integral against $\mathbf{X}$ is defined as 
\[ \int_0^T F(X_s)d\mathbf{X}_s := \lim_{|\mathcal{P}|\to 0} \sum_{[s,t]\in\mathcal{P}} F(X_s) X_{s,t} + DF(X_s)\mathbb{X}_{s,t},\]
where for an arbitary partition $\mathcal{P}$ of $[0,T]$, $|\mathcal{P}|$ denotes the length of its largest segment. The limit on the right-hand side exists by the fundamental Theorem~$4.4$ in \cite{Friz/Hairer}.
For our setup, the most useful properties of the rough integral are continuity as a function in $\mathbf{X}$ with respect to the $\alpha$-Hölder rough path metric (cf. \cite{Friz/Hairer}, Theorem~$4.16$) and that by inserting $\mathbf{X}=(W,\mathbb{W}^\textrm{Strat})$, it coincides with the Stratonovich integral almost surely (cf. \cite{Friz/Hairer}, Corollary~$5.2$). %Thus, we will be able to reformulate our test as depending on a rough path without changing it compared to our version with the It\^{o}-integral. 




\subsection*{Building a rough path version of our test}

It is well-known that there exists a geometric rough path lift of standard It\^{o} diffusions which gives rise to a rough integration theory that coincides with Stratonovich integration (see Proposition $17.1$ in \cite{Friz/Victoir}). Our starting point is the reformulation of the It\^{o} stochastic integral within our test statistic in terms of the Stratonovich integral
%\begin{align}\label{eq: Out1}
%\int_0^T K_{y,h}(X_s) dX_s = \int_0^T K_{y,h}(X_s) \circ dX_s - \frac12 \int_0^T \textrm{Trace}( DK_{y,h}(X_s)) ds
%\end{align}
(cf. \cite{Kallenberg}, p. 410). %To build a rough path version auf our test statistic, we first replace the It\^{o} integral in the definition of multidimensional analogs of the local statistics \eqref{eq: Psi} by the right-hand side of~\eqref{eq: Out1}. 
Because for the standard It\^{o} diffusion the rough integral coincides with the Stratonovich integral with probability one, the idea is to substitute the appearing Stratonovich integral by the rough path integral $\int_0^T K_{y,h}(X_s)d\mathbf{X}_s$. This gives a rough path version $\mathbf{\tilde\Psi}_{T,y,h}^{b_0}(\mathbf{X})$ of the $d$-dimensional vector of local statistic \eqref{eq: Psi} %$\Psi_{T,y,h}^{b_0}(X)$ 
that is well-defined not only for It\^{o} diffusions, but for arbitrary rough paths. Based on this, we obtain a rough path version of the similarity test statistic
\[ \mathbf{T}_T^\eta(\mathbf{X}) := \max_{i=1,\dots, d} \sup_{(y,h)\in\mathcal{T}_T}\left( \left|\left(\mathbf{\tilde{\Psi}}_{T,y,h}^{b_0}(\mathbf{X})\right)_i\right| -\Lambda_{T,y,h}^\eta(X) - C\bigg(\frac{\hat\sigma_T(y,h)^2}{\hat\sigma_{T,\max}^2}\bigg) \right).\]
Details on how the lifted rough path can be approximated numerically from an observed process can be found in Section~$8.1$ in \cite{Diehl/Friz}. Therefore, the statistic $\mathbf{T}_T^\eta$ is actually solely dependent on the observed process $X$.
The definition of $\hat\sigma_T(y,h)$, $\hat\sigma_{T,\max}$ and $\Lambda_{T,y,h}^\eta(X)$ remains unchanged when switching to the rough path extension as they only depend on the first component of $\mathbf{X}=(X,\mathbb{X})$, whereas, of course, they have to be adjusted to the multidimensional setting.
Following the lines for a pathwise construction of the test in Section \ref{Sec_Stability}, one again has to restrict the preimage of the map $\mathbf{T}_T^\eta$ to some subset $\mathbb{D}_{A,T}^\alpha$ of $\alpha$-Hölder rough paths, for which the denominators of the local test statistics do not vanish.
Applying the It\^{o} formula for rough paths given in Proposition~$5.6$ in \cite{Friz/Hairer} shows that the rough path approach to define $\mathbf{\tilde \Psi}_{T,y,h}^{b_0}$ in dimension $d=1$ yields again the statistic $\tilde\Psi_{T,y,h}^{b_0}$ of Section~\ref{Sec_Stability}. Thus, the rough test statistic described above is indeed an extension to dimension $d>1$ of what has been done in Section~\ref{Sec_Stability}.



%\begin{align*}
%&\mathbf{\tilde\Psi}_{T,y,h}^{b_0}(\mathbf{X}) = \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h}(X_s) d\mathbf{X}_s}{\sigma\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}\\
%&\hspace{3cm} - \frac{\frac{1}{\sqrt{T}}\int_0^T \left( K_{y,h}(X_s)b_0(X_s) + \frac{1}{2} \textrm{Tr}(DK_{y,h}(X_s))\right) ds}{\sigma\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2  ds}}.
%\end{align*} 
%For the same reason as in the one-dimensional case, we restrict to $\mathcal{T}_T$ instead of $\mathcal{T}$, when defining the global test statistic and set
%\[ \mathbf{T}_T^\eta(\mathbf{X}) := \sup_{(y,h)\in\mathcal{T}_T}\left( \left|\mathbf{\tilde{\Psi}}_{T,y,h}^{b_0}(\mathbf{X})\right| -\Lambda_{T,y,h}^\eta(X) - C\left(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2\right) \right).\]
%Here the definition of $\hat\sigma_T(y,h), \hat\sigma_{T,\max}$ and $\Lambda_{T,y,h}^\eta(X)$ remains unchanged as they only depend on the first component of $\mathbf{X}=(X,\mathbb{X})$. \\
%Applying the It\^{o} formula for rough paths given in Proposition $5.6$ in \cite{Friz/Hairer} shows that the rough path approach to define $\mathbf{\tilde \Psi}_{T,y,h}^{b_0}$ in dimension $d=1$ yields again the statistic $\tilde\Psi_{T,y,h}^{b_0}$ of Section \ref{Sec_Stability}. Thus, the rough test statistic described above is indeed an extension to dimension $d>1$ of what has been done in Section \ref{Sec_Stability}.





\subsection*{Stability properties}

%As the $d_\alpha$-metric ensures continuity of rough integrals, it is straightforward to establish for any fixed $T>0$ continuity of the map
%\begin{align*}
%\mathbf{\tilde{\Psi}}_{T,y,h}^{b_0}:\ \mathbb{D}_{A,T}\times \mathcal{T}_T\ \ &\longrightarrow\ \ \ \R,\\
%(\mathbf{X}, (y,h))\ &\ \mapsto\ \ \mathbf{\tilde{\Psi}}_{T,y,h}^{b_0}(\mathbf{X}),
%\end{align*}
%where the left side is equipped with the product topology induced by $d_\alpha$ and twice the absolute value on real numbers. By the same preliminary lemmas on continuity of suprema as used in the one-dimensinal case to prove Theorem \ref{thm_continuity}, this can be extended to continuity of
As rough integration is continuous with respect to $d_\alpha$-Hölder rough path metric we can establish continuity of
\begin{align*}
\mathbf{T}_T^\eta:\ \mathbb{D}_{A,T}^\alpha &\longrightarrow \ \ \ \R,\\
\mathbf{X}\ &\ \mapsto \ \ \mathbf{T}_T^\eta(\mathbf{X}),
\end{align*}
with respect to %the $\alpha$-Hölder rough path metric. 
this metric along the lines of the proof of Theorem~\ref{thm_continuity}. Finally, Friz et al. established in Theorem $16$ in \cite{Diehl/Friz} that the solution of the multidimensional fractional diffusion
\[ dX_t^H = b(X_t^H) dt + \sigma dW_t^H\]
can be lifted to a random geometric $\alpha$-Hölder rough path $\mathbf{X}^H = (X^H, \mathbb{X}^H)$ for every $\alpha\in (\frac13,H\wedge \frac12)$ that has a continuous modification in $H=\frac12$ with respect to $d_\alpha$-metric for any $\alpha\in (\frac13,\frac12)$. Thus, the subsequent almost sure continuity statement
\[ \mathbf{T}_T^\eta(\mathbf{X}^H) \longrightarrow \mathbf{T}_T^\eta(\mathbf{X}) \]
for $H\to 1/2$ follows immediately. 
Whether higher dimensional analogues of our strong results of Section~\ref{SubSec_fractional_model} with uniformity over the drift can be deduced in this way remains, however, totally unclear.









==> Version_ArXiv/Sections/Power_considerations.tex <==
\section{Minimax optimality and sharp adaptivity}\label{Sec_Power}

In this section we will show that the similarity test $\phi_T^\eta$ possesses minimax optimality and adaptivity properties. To this aim we restrict the alternative $H_1(b_0,\eta)$ given in \eqref{eq: H1_eta} to Hölder-regular deviations $b-b_0$. In most situations, precise knowledge of the regularity of this deviation is unrealistic and we will establish that a suitable chocie of the kernel $K$ in the definition of the test statistic $T_T^\eta$ in \eqref{eq: T_eta} allows for (sharp) adaptive results.





\subsection{Measuring distances from $H_0(b_0,\eta)$}

When establishing minimax rates and optimal constants it is crucial to specify a distance between a given function $b$ and the null $H_0(b_0,\eta)$. We define this distance as
\begin{align}\label{eq: Delta_J}
\Delta_J(b) := \inf_{\tilde{b}\in H_0(b_0,\eta)} \left\| |b - \tilde{b}| \left(\frac{q_b}{\sigma^2}\right)^\frac{\beta}{2\beta+1}\right\|_J
\end{align} 
with compact $J\subset (-A,A)$ to avoid boundary effects. For $b\notin H_0(b_0,\eta)$ it is given by
\[ \Delta_J(b) = \sup_{x\in J} \Big(|b(x)-b_0(x)| - \eta\Big) \left(\frac{q_b(x)}{\sigma^2}\right)^\frac{\beta}{2\beta+1}\]
which corresponds to the boundary cases $\tilde{b} = b_0\pm\eta$. Note that the occurence of $q_b$ and $\sigma^2$ meet our intuition: deviations at a point $y$ can be exptected to be easier to detect if the process spends more time around $y$, i.e. when $q_b(y)$ is large. On the other hand, detecting is more challenging the more noise we have, i.e. the larger $\sigma^2$ is. The reason we do not shift the factor $(q_b/\sigma^2)^{\beta/(2\beta+1)}$ into rate or constant is that $q_b$ depends on the location. For testing in supremum norm this is the equivalent to weighted risk definitions used in sharp adaptive drift estimation, see for example \cite{Dalalyan} and \cite{Strauch_2}.





\subsection{Optimal power properties}
For $\beta, L>0$ the Hölder class $\mathcal{H}(\beta,L)$ is given by the set of functions functions $f:\R\rightarrow\R$ such that for each $k=0,\dots,\lfloor \beta\rfloor$ the Hölder-condition
\[ \left| f^{(\lfloor\beta\rfloor)}(x) - f^{(\lfloor\beta\rfloor)}(y)\right| \leq L|x-y|^{\beta-\lfloor\beta\rfloor}\]
is valid, where $f^{(n)}$ denotes the $n$-th derivative of $f$. Our power results specify those functions in
\[ \bigcup_{\beta, L>0} H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\} ,\]
close enough to the null $H_0(b_0,\eta)$ in the distance $\Delta_J$ that can be detected by $\phi_T^\eta$ given in \eqref{eq: phi_eta} with probability tending to one. For this aim, we define the rate
\[ \delta_T =\delta_T(\beta) := \left(\frac{\log T}{T}\right)^{\frac{\beta}{2\beta +1}} \]
and constant
\begin{align}\label{eq: c_optimal}
c_* = c_*(\beta,L) := \left( \frac{2L^{\frac{1}{\beta}}}{(2\beta +1)\|K_\beta\|_{L^2}^2}\right)^{\frac{\beta}{2\beta+1}}.
\end{align} 
Here $K_\beta$ is the unique solution of the following optimization problem:
\begin{align}\label{eq: optimal_recovery}
\textrm{Minimize } \|K\|_{L^2} \textrm{ over all } K\in\mathcal{H}(\beta,1) \textrm{ with } K(0)\geq 1.
\end{align} 
We call $K_\beta$ the optimal recovery kernel. In the case $0<\beta\leq 1$ it is not difficult to see that
\[ K_\beta (x) = \1_{\{|x|\leq 1\}} \left(1-|x|^\beta\right),\]
as we even have $K_\beta (x) \leq f(x)$ for all $x\in [-1,1]$ and $f\in\mathcal{H}(\beta,1)$ in this case. For $\beta =2$ an explicit solution is known (see~\cite{Leonov}). For details on how this function can be constructed numerically, see \cite{Donoho} and \cite{Leonov}. Furthermore, for all $\beta>0$, $K_\beta$ is compactly supported, an even function and satisfies $K_\beta (0)=1>|K_\beta(x)|$ for $x\neq 0$. \\ 

%To show that our test $\phi_T^\eta$ is indeed the best possible, we establish the corresponding lower bound. As our result on identifying the least favourable case is not required for this, we do not impose the condition $K\geq 0$ within the proof and get the optimal constant $c_*$ for all $\beta>0$.


For the power consideration we start with the lower bound. In the next theorem we will show that for every test of level $\alpha$ of the hypothesis $H_0(b_0,\eta)$ there exist drift functions in the alternative that deviate $(1-\epsilon_T)c_*\delta_T$ from $H_0(b_0,\eta)$ in the semimetric $\Delta_J$ which will not be detected with probability $1-\alpha-o(1)$ or larger. In particular, this is even true in the knowledge of both smoothness parameters $\beta$ and $L$.

\begin{thm}\label{lower_bound}
Let $\eta\geq 0$ and $\psi_T$ be a test that is uniformly over $H_0(b_0,\eta)$ of level $\alpha$, i.e. $\sup_{b\in H_0(b_0,\eta)}\E_{b}[\psi_T]\leq\alpha$, for some drift function $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$. Then for arbitrary numbers $\epsilon_T>0$ with $\lim_{T\to\infty}\epsilon_T =0$ and $\lim_{T\to\infty}\epsilon_T \sqrt{\log T} =\infty$,
\[ \limsup_{T\to\infty}\ \inf_{\substack{b\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1-\epsilon_T)c_*\delta_T}}\ \E_{b}\left[\psi_T\right]\ \leq\ \alpha\]
for any fixed compact interval $J\subset (-A,A)$.
\end{thm}

Although the proof of this result follows common ideas that have to be applied in the context of stochastic analysis, there appear two unusual obstacles. The first relates to the definition of local alternatives. Those are commonly defined via some disturbance function $g$.
%; here, the alternative is of the form $b_0 \pm\eta + g$ due to the composite null. 
However, in our case we cannot just add some hat $g$ with absolute height $(1-\epsilon_T)c_*\delta_T$ on boundary cases of the null hypothesis, because the distance $\Delta_J$ involves a scaling by the invariant density of the local alternative itself, which in turn depends on the choice of $g$. This leads to a fixed point problem which in Appendix~\ref{App_lower} is proven to be solvable, enabling us to construct alternatives $b$ with $\Delta_J(b)=(1-\epsilon_T)c_*\delta_T$. The second obstruction is that the likelihoods of the above constructed hypotheses are not independent as for example in \cite{Walther} or \cite{Duembgen/Spokoiny}, but only  uncorrelated asymptotically, see Proposition~\ref{lemma_E_absvalue} and Remark~\ref{remark_E_absvalue}. More details are provided in the route of the proof in Section~\ref{Sec_supp}.\\



Next, we establish the corresponding upper bounds of $\phi_T^\eta$ in \eqref{eq: phi_eta}. Note that the validity of Theorem~\ref{worst_case_delta} cannot be guaranteed for kernels of higher order than one because such kernels necessarily take negative values.

%In case $\beta\leq 1$, Theorem \ref{worst_case_delta} is applicable with the choice $K_\beta$ as $K_\beta\geq 0$ with support $[-1,1]$. Here, $\phi_T^\eta$ attains both the rate and constant of the lower bound in Theorem \ref{lower_bound}. As $K_\beta$ does not depend on $L$ the test is therefore sharp adaptive in $L$. In case $\beta>1$, $K_\beta$ may be negative and we have to replace it with a kernel that is non-negative in order to guarantee that the test keeps the significance level on the hypothesis. This does not yield the optimal constant, but still a rate optimal testing procedure. 


\begin{thm}\label{Upper_bound}
Let $\beta, L>0$, $\eta>0$, $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$ and let $K$ be a non-negative kernel of bounded variation supported in $[-1,1]$ with $\|K\|_{[-1,1]}=1$.
Then for arbitrary numbers $\epsilon_T>0$ with $\lim_{T\to\infty}\epsilon_T =0$ and $\lim_{T\to\infty} \epsilon_T \sqrt{\log T}=\infty$ there exists a constant $c=c(\beta, L, K)$ such that for the test $\phi_T^\eta$ given in~\eqref{eq: phi_eta},
\[ \lim_{T\to\infty}\ \inf_{\substack{b\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1+\epsilon_T)c\delta_T}}\ \Pr_b\left( \phi_T^\eta(X) =1\right)\ =\ 1\]
for any fixed compact interval $J\subset (-A,A)$. In the case $\beta\in (0,1]$ we can choose $K=K_\beta$ and the result is true for $c=c_*$.
\end{thm}


This result may be read as follows: If the underlying drift function of our diffusion deviates from the composite null $H_0(b_0,\eta)$ in distance $\Delta_J$ by at least $(1+\epsilon_T)c\delta_T$, then the test detects the deviation and rejects the null hypothesis of similiarity with probability close to one. Hence, for any non-negative kernel of bounded variation supported in $[-1,1]$, the test $\phi_T^\eta$ is minimax rate-optimal as it attains over the whole range of $\beta, L>0$ the corresponding rate of the lower bound in Theorem \ref{lower_bound}. In case $\beta\leq 1$, it is even optimal in the constant. The next theorem even states that rate-adaptivity is attained uniformly over parameter ranges of the form $[\beta_1,\beta_2]\times [L_1,L_2]$ and sharp adaptivity for fixed $\beta$ over $L\in [L_1,L_2]$.


\begin{thm}[Adaptivity]\label{thm_adaptivity}
%Let $\beta, L>0$, $\eta>0$, $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$ and let $K$ be a non-negative kernel of bounded variation supported in $[-1,1]$.
Let $\beta, L>0$ and $b_0,K$ and $\epsilon_T$ be specified as in Theorem~\ref{Upper_bound}.
Then for a compact subset $[\beta_1,\beta_2]\times[L_1, L_2]\subset (0,\infty)^2$ the test $\phi_T^\eta$ is rate-adaptive in both parameters $\beta$ and $L$ in the sense
\[  \lim_{T\to\infty}\ \inf_{(b,L)\in [\beta_1,\beta_2]\times [L_1,L_2]}\ \inf_{\substack{b\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1+\epsilon_T)c(\beta, L,K)\delta_T}}\ \Pr_b\left( \phi_T^\eta(X) =1\right)\ =\ 1.\]
For $\beta\leq 1$ we have sharp adaptivity in the parameter $L\in [L_1,L_2]\subset (0,\infty)$ in the sense
\[  \lim_{T\to\infty}\ \inf_{L\in [L_1,L_2]}\ \inf_{\substack{b\in H_1(b_0,\eta) \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1+\epsilon_T)c_*\delta_T}}\ \Pr_b\left( \phi_T^\eta(X) =1\right)\ =\ 1.\]
\end{thm}




%\begin{remark}[Lower bound on the bandwidth]\label{remark_h_min}
%In the proof of Theorem \ref{Upper_bound} a certain bandwidth $h_T=h_T(L, K)$ is used for detection. For $L\in [L_1,L_2]\subset (0,\infty)$ belonging to some compact interval one then finds a lower bound $h_{\min}(T,L_2)$ on the bandwidth $h_T$ that is sufficient for rate optimal detection. This is important from a practical point of view as the supremum over $\mathcal{T}$ within the test statistic $T_T^\eta$ can only be computed for some finite grid that necessarily has a lower bound of the parameter $h$.
%\end{remark}



%\begin{remark}\label{remark_boundary}
%The proof of Theorem \ref{Upper_bound} actually shows that the interval $J$ where we detect the alternativ can be chosen time-dependent as
%\[ J_T := \left[ -A + \left(\frac{(1+\epsilon_T)c\rho_T}{LL_*}\right)^\frac{1}{\beta}, A - \left(\frac{(1+\epsilon_T) c \rho_T}{LL_*}\right)^\frac{1}{\beta} \right]. \]
%\[ J_T := \left[ -A + \left((1+\epsilon_T)c\rho_T/(LL_*)\right)^\frac{1}{\beta}, A - \left((1+\epsilon_T) c \rho_T/(LL_*)\right)^\frac{1}{\beta} \right]. \]
%As $\rho_T\rightarrow 0$, we cover a growing part of the interval $[-A,A]$. This modification works, as the bandwidth $h_T$ specified in the proof fullfills 
%\[ h_T \leq  \left(\frac{(1+\epsilon_T) c \rho_T}{LL_*}\right)^\frac{1}{\beta}\]
%\[ h_T \leq  \left((1+\epsilon_T) c \rho_T/(LL_*)\right)^\frac{1}{\beta}\]
%and thus, for each $y\in J_T$ we have $[y-h_T, y+h_T]\subset [-A,A]$. The appearance of $L_*$ is due to the fact that the optimal bandwidth at location $y_T$ depends on $q_b(y_T)$.\\
%The full interval $J=[-A,A]$ can be treated by using suitable boundary kernels as was done in \cite{Lepski/Tsybakov}.
%\end{remark}







For $\eta=0$ the hypothesis $H_0(b_0,\eta)$ reduces to the simple hypothesis $b=~b_0$ (on $[-A,A]$). % As we do not need an identification of a least-favourable case 
Here, we find minimax optimality including the efficiency constant even on the full range $\beta,L>0$.
%Following the considerations in Remark \ref{remark_adaptivity}, it is then sharp adaptive in $L$ for all $\beta>0$.



\begin{thm}\label{thm_simple_hypothesis}
Let $\beta,L>0$ and $b_0$ and $\epsilon_T$ be specified as in Theorem~\ref{Upper_bound}.
%Then we have the following for the simple hypothesis:
%For any fixed non-degenerate inverval $J\subset (-A,A)$, let $\psi_T$ be a level-$\alpha$-test, i.e. $\E_{b_0}[\psi_T]\leq\alpha$. Then
%\[ \limsup_{T\to\infty} \inf_{\substack{b\in\mathcal{H}(\beta,L,b_0,0):\ \Delta_J(b)\geq (1+\epsilon_T)c_*\delta_T}} \E_{b}\left[\psi_T\right]\leq \alpha.\]
Then the test $\phi_T^{b_0}$ given in \eqref{eq: phi_0} with the kernel $K=K_\beta$ satisfies for any compact interval $J\subset (-A,A)$
\[ \lim_{T\to\infty}\ \inf_{\substack{b\in H_{\neq} \cap\{ b-b_0\in \mathcal{H}(\beta, L)\}:\\ \Delta_J(b)\geq (1-\epsilon_T)c_*\delta_T}}\ \Pr_b\left( \phi_T^{b_0}=1\right)\ =\ 1.\]

\end{thm}







\begin{remark}[Diffusions started at a fixed point]\label{remark_fixed_point}
For technical convenience, all of our results were derived under the assumption that the diffusion $X$ is stationary, i.e. $X_0\sim\mu_b$. However, it is not necessary. In Remark~\ref{remark_fixed_start} and \ref{remark_fixed_start_upper} we give the details how Theorem~\ref{worst_case_delta}, \ref{lower_bound}, \ref{Upper_bound}, \ref{thm_adaptivity} and \ref{thm_simple_hypothesis} can be established for $X$ started at a fixed point $x_0\in [-A,A]$.
\end{remark}


















==> Version_ArXiv/Sections/Preliminaries.tex <==
\section{Model assumptions and notation}\label{Sec_Notation}


For the problem of similarity testing, we assume throughout that a continuous record of observations $(X_t)_{t\in [0,T]}$ is available, where $X$ denotes an It\^{o} diffusion satisfying the one-dimensional homogeneous stochastic differential equation (SDE) of the form
\begin{align}\label{eq: SDE}
dX_t = b(X_t) dt + \sigma dW_t,\quad X_0 = \xi,
\end{align} 
with drift $b:\R\rightarrow\R$, $\sigma>0$, $W=(W_t)_{t\geq 0}$ a standard one-dimensional Brownian motion and initial condition $\xi$ independent of $W$. In this setup, the diffusion coefficient is identifiable using the semimartingale quadratic variation of the diffusion and the problem of its estimation does not arise. This remains also true if $\sigma$ was replaced by $\sigma(X_t)$ in \eqref{eq: SDE}. For conciseness and clarity in the representation, we however restrict attention to constant diffusion coefficient. The extension of our results to a non-constant diffusion coefficient is straightforward, except for Section~\ref{Sec_Stability} because a suitable notion of stochastic integrals is then needed to even define the fractional SDE.\\
For arbitrary but fixed constants $A,\gamma, \sigma >0$ and $C\geq 1$, the  drift $b$ belongs to 
\begin{align*}
\Sigma(C,A,\gamma, \sigma) &:=\left\{ b\in \textrm{Lip}_\textrm{loc}(\R):\ |b(x)|\leq C(1+|x|)\ \forall x\in\R \textcolor{white}{\frac12} \right.\\
&\hspace{3cm}\left.\textrm{ and } \frac{b(x)}{\sigma^2}\textrm{sign}(x)\leq -\gamma\ \forall |x|\geq A\right\}.
\end{align*}
Here, $\textrm{Lip}_\textrm{loc}(\R)$ denotes the local Lipschitz functions on $\R$, see Appendix~\ref{A1_SubSec}. The first two constraints ensure that the SDE \eqref{eq: SDE} has a unique strong solution and the last one is a typical assumption to guarantee ergodicity and the existance of an invariant measure. For each $b\in\Sigma(C,A,\gamma,\sigma)$ we denote this invariant measure by $\mu_b$ and it is a classical result (cf. \cite{Kutoyants}, Theorem~$1.16$) that it admits the invariant probability density
\[ q_b(x) := \frac{1}{C_{b,\sigma}} \exp\left( \int_0^x \frac{2b(y)}{\sigma^2} dy\right) \quad\textrm{ for all } x\in\R,\]
with normalizing constant $C_{b,\sigma}$.
For $x<0$ the integral should be read as $\int_0^x f(y)dy = -\int_{x}^0 f(y) dy$.
For ease of representation, we assume that $\xi\sim\mu_b$ such that $X$ is stationary and ergodic. Extensions are possible, see Remark~\ref{remark_fixed_point}.\\
Subsequently, we add $b$ as subscript to expectation and probability, $\E_b$ and $\Pr_b$, to emphasize that $X$ inside satisfies \eqref{eq: SDE} with drift $b$.

For any set $I\subset \R$ and bounded function $f:I\rightarrow \R$ we denote
\[ \|f\|_I := \sup_{z\in I} |f(z)|.\]
For any compact set $K\subset\R$ we denote by $\mathcal{C}(K)$ the set of continuous functions $f: K\rightarrow\R$. Unless stated otherwise, we denote by $\|\cdot\|_{L^2}$ the $L^2$-norm with respect to the Lebesgue measure on $\R$.


==> Version_ArXiv/Sections/Simple_null.tex <==
\section{The case of the simple null $b=b_0$}\label{Sec_simple}

Although our main contribution is the development of a test for similiarity, we start with the hypothesis $b=b_0$ as a preliminary step before the similiarity test is presented in the next section. 
Besides being of independent interest, this presentation comprises solutions to technical difficulties that arise merely from the setting of ergodic diffusions in the context of multiscale testing - and not those attributed to the composite null.\\ 
The precise testing problem we address in this section is given for some $b_0\in\Sigma(C/2, A, \gamma,\sigma)$ by
\begin{align}\label{eq: H_0-simple}
H_0:\ \|b-b_0\|_{[-A,A]} =0 
\end{align} 
versus one of the following alternatives:
\begin{align*}
&H_{\neq}:\ \left\{\|b-b_0\|_{[-A,A]}>0 \right\} \cap\Sigma(C,A,\gamma,\sigma), \\
&H_{>}:\ \left\{\exists x\in [-A,A]:\ b(x)-b_0(x)>0 \right\} \cap\Sigma(C,A,\gamma,\sigma), \\
&H_{<}:\ \left\{\exists x\in [-A,A]:\ b(x)-b_0(x)<0 \right\} \cap\Sigma(C,A,\gamma,\sigma).
\end{align*}  
The intersection with $\Sigma(C,A,\gamma,\sigma)$ accounts for the fact that we only test against ergodic diffusions. In a first step, we consider $H_0$ against the two-sided alternative $H_{\neq}$. Afterwards in Subsection \ref{SubSec_one-sided} we consider the alternatives $H_<$ and $H_>$. 




\subsection{Testing the two-sided alternative}
Suppose that we want to test a simple drift hypothesis $b_0$ against a simple alternative $b_1$. Then by the Neyman-Pearson-Lemma, an optimal test is given by the likelihood ratio statistic $d\Pr_{b_1}/d\Pr_{b_0}(X)$, in our particular case given by means of Girsanov's theorem as 
\[ \frac{d\Pr_{\xi_1}}{d\Pr_{\xi_0}}(X_0)\exp\left( \int_0^T \frac{b_1(X_s) - b_0(X_s)}{\sigma^2} dX_s - \frac12\int_0^T \frac{b_1(X_s)^2 - b_0(X_s)^2}{\sigma^2} ds\right).\]
When moving on to the composite alternative $\{\|b-b_0\|_{[-A,A]}>0\}$ which can be represented as
\[ \bigcup_{\delta>0}\bigcup_{y \in [-A,A]} \{ |b(y) -b_0(y)|\geq \delta\}, \]
alternatives of the form $b=b_0+K_{y}$ for some localized deviation $K_y$ with $K_y(y)=\delta$ seem to be hardest to detect for each set of the union. If some regularity of the alternative $b$ is imposed, deviation $|b(y)-b_0(y)|=\delta$ implies that $|b(x)-b_0(x)|\neq 0$ for all $x$ within some neighborhood of $y$ as well. The size of this neighborhood depends on the regularity of the alternative which is typically unknown.
The idea is now to develop a multiple test in the spirit of \cite{Duembgen/Spokoiny} that simultaneously tests all locations with likelihood ratio statistics of localized deviations 
\[ K_{y,h}(x) := K\left(\frac{x-y}{h}\right), \quad x\in\R, \]
with different scaling parameters $h>0$. As our approach combines standardized local $\log$-likelihood ratio statistics, the particular value $\delta$ will cancel out.

%Following the motivation for a multiple test of Dümbgen and Spokoiny in \cite{Duembgen/Spokoiny}, the next step is to test against $\{\|b-b_0\|_{[-A,A]}>\delta\}$ for some $\delta>0$ which is given by 
%\[ \bigcup_{y \in [-A,A]} \{ |b(y) -b_0(y)|>\delta\}.\]
%Looking for least favourable cases within each set of the union suggests to test against alternatives $b$ with $b-b_0= K_{y,h}$, where
%\[ K_{y,h}(x) := K\left(\frac{x-y}{h}\right) \]
%is a rescaled version of some compactly supported kernel $K:\R\rightarrow\R$ that will be specified later. Then the likelihood ratio statistic $d\Pr_{b_0+K_{y,h}}/d\Pr_{b_0}$ is optimal to test $H_0$ against $\{ |b(y)-b_0(y)|>\delta\}$. Later on, those local test statistics will be combined in a certain way to arrive at a test against $H_1$.





\subsubsection*{Suitable standardization of the local likelihood statistics}
Omitting the initial values, the $\log$-likelihood ratio of local deviation $b=b_0+K_{y,h}$ and $b_0$ is given by
\[  \frac{1}{\sigma^2}\int_0^T K_{y,h}(X_s) dX_s - \frac{1}{2\sigma^2} \int_0^T \left( 2b_0(X_s) K_{y,h}(X_s) + K_{y,h}(X_s)^2 \right) ds. \]
For our construction of the multiple test, standardization under $\Pr_{b_0}$ is required. Whereas an additive correction for centering under $\Pr_{b_0}$ is obvious, we do not divide by the standard deviation of the stochastic integral $\sigma^{-1}\int_0^T K_{y,h}(X_s) dW_s$ for normalizing the variance, but choose its random analogue, the square root of its quadratic variation, which is purely data dependent. Thus, the standardized local $\log$-likelihood statistic is given by
\begin{align}\label{eq: Psi}
\Psi_{T,y,h}^{b_0}(X) := \frac{\int_0^TK_{y,h}(X_s) dX_s}{\sigma\sqrt{ \int_0^T K_{y,h}(X_s)^2 ds}} -\frac{\int_0^T K_{y,h}(X_s) b_0(X_s) ds}{\sigma\sqrt{ \int_0^T K_{y,h}(X_s)^2 ds}}.
\end{align} 
The deeper reason behind normalizing with the quadratic variation is that it
provides a suitable standardization of the martingale part $\int_0^T K_{y,h}(X_s)dW_s$ for \textit{any} drift $b$. This enables us to attain efficiency when moving on to the construction of a multiple test for the \textit{composite} null hypothesis of similarity in Section~\ref{Sec_similarity}.
%to allow for precise control of the tails of our local deviation statistic under $\Pr_{b_0}$,  see Proposition \ref{Exp_ineq}. 
Note that under $\Pr_{b_0}$,
\begin{align*}
\Psi_{T,y,h}^{b_0}(X) = \frac{\int_0^TK_{y,h}(X_s) dW_s}{\sqrt{\int_0^T K_{y,h}(X_s)^2 ds}}. 
\end{align*} 



\subsection*{Developing the multiple test}
The following result shows that the local statistics $\Psi_{T,y,h}^{b_0}(X)$ in \eqref{eq: Psi} can be combined for all $(y,h)$ within
\begin{align}\label{eq: cT}
\mathcal{T} := \left\{ (y,h)\in\Q^2 \mid h\in (0,A] \textrm{ and } y\in [-A+h, A-h]\right\}
\end{align} 
in a specific way that enables to construct the desired multiple test.
%This together suggests to use the statistic $\sup_{(y,h)\in\mathcal{T}}\Psi_{T,y,h}^{b_0}(X)$ which needs to be additively corrected for the supremum to make the statistic tight under the null. This is quite challenging in our setting, as the localized statistics are neither independent nor identically distributed. However, we are able to specify this additive correction as fully spelt out in the next theorem.


\begin{thm}\label{Multiscale_Lemma}
Let $\Psi_{T,y,h}^{b_0}(X)$ be given as above for a kernel $K$ of bounded variation with support $[-1,1]$ and $\|K\|_{[-1,1]} \leq 1$. Furthermore, set
\[ \hat\sigma_T(y,h)^2 := \frac1T \int_0^T K_{y,h}(X_s)^2 ds \quad \textrm{ and }\quad \hat\sigma_{T,\max}^2 := \frac1T \int_0^T \1_{[-A,A]}(X_s)^2 ds.\]
%and
%\[ \hat\sigma_{T,\max}^2 := \frac1T \int_0^T \1_{[-A,A]}(X_s)^2 ds.\]
Then under $\Pr_{b_0}$ the sequence (indexed in $T$)
\[\sup_{(y,h)\in\mathcal{T}}\left( \left|\Psi_{T,y,h}^{b_0}(X)\right| - C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2)\right)\]
is tight, where $C(\cdot)$ is given by
\[ C(r) :=(2\log(1/r))^\frac12. \]
\end{thm}


The proof of this result is deferred to Appendix~\ref{App_Multiscale} and relies on a delicate interplay of stochastic analysis and sophisticated empirical processes. Various variants of identifying the above correction $C(\cdot)$ have been established in the theory of multiscale testing, see for example \cite{Walther}, \cite{Duembgen/Spokoiny}  or \cite{Rohde}. We derive another version of such results, where the sub-gaussian tail bounds of the local test statistics allow for an additional $\log$-factor, see Proposition \ref{Multiscale_preparation}. %Applying this Proposition strongly relies on tools from stochastic analysis, in particular the local time of a diffusion and the occupation times formula together with an exponential tail bound for martingales. Additionally, using the quadratic variation for standardization requires us to bound \textit{random} covering numbers.\\
%Of particular interest is the additive correction term $C(\cdot)$ that loosely speaking compensates the two suprema.
%$D(\cdot)$ on the other hand is bounded and strictly positive on $(0,1]$ with $\lim_{r\to 0} D(r) =0$.\\
%Being defined as a supremum, it is not directly clear that $T_T^{b_0}(X)$ is measurable, but follows from the fact that the local test statistics $\Psi_{T,y,h}^{b_0}(X)$ are continuous in $(y,h)\in\mathcal{T}$. This is explained in detail together with the computability of the estimator in Section \ref{Sec_Implementation}.\\
With these preliminaries we now define the global test statistic
\begin{align}\label{eq: T_simple}
T_T^{b_0}(X) := \sup_{(y,h)\in\mathcal{T}} \left( |\Psi_{T,y,h}^{b_0}(X)| - C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2)\right).
\end{align} 
%Note that from the properties of $D(\cdot)$ and 
Theorem \ref{Multiscale_Lemma} ensures that the corresponding quantiles
\begin{align}\label{eq: quantile_simple}
\kappa_{T,\alpha}^{\neq b_0} := \min\left\{ r\in\R\mid \Pr_{b_0}\left( T_T^{b_0}(X)\leq r\right) \geq 1-\alpha\right\} 
\end{align} 
are well-defined and form a bounded sequence. An asymptotic power investigation of the resulting test
\begin{align}\label{eq: phi_0}
\phi_T^{b_0}(X) = \1_{\left\{ T_T^{b_0}(X)> \kappa_{T,\alpha}^{\neq b_0}\right\}} 
\end{align}
is given in Section \ref{Sec_Power}.




%\begin{remark}[Normalizing the deviation metric]
%The appearance of $\hat\sigma_{T,\max}^2$ is another normalization, in this case the normalization of the deviation metric $\hat\sigma_T$. It does not affect $\Psi_{T,y,h}^{b_0}(X)$ as added in both nominator and denominator it cancels out, but is later used for technical reasons in the identification of the least favourable case in the setting of the composite null. Furthermore, it ensures that the deviation metric $\hat\sigma_T/\hat\sigma_{T,\max}$ is bounded by one.
%\end{remark}



%\begin{remark}[Simultaneous detection of regions of deviation]\label{remark_detection}
%As outlined in the introduction we are not only interested in the testing problem \eqref{eq: Testing_problem} but also want to identify the regions of deviation. Therefore note that the above test statistic $T_T^{b_0}$ exceeds the $(1-\alpha)$-significance level if, and only if, the random family
%\[ \mathcal{D}_\alpha := \left\{ (y,h)\in\mathcal{T}:\ |\Psi_{T,y,h}^{b_0}(X)| > C\left( \hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2\right) + \kappa_{T,\alpha} \right\} \]
%is non-empty. In particular one may conclude that with confidence $1-\alpha$ there is a deviation from $b_0$ on \textit{every} interval $[y-h, y+h]$ with $(y,h)\in\mathcal{D}_\alpha$.
%\end{remark}




\subsection{Testing for one-sided alternatives}\label{SubSec_one-sided}

Following the same approach that was taken to construct the test against $H_{\neq}$ we construct a test of $H_0$ versus $H_>$. The same reasoning yields the test statistic
\begin{align*}
T_T^{>b_0}(X) := \sup_{(y,h)\in\mathcal{T}} \left( \Psi_{T,y,h}^{b_0}(X) - C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2)\right)
\end{align*} 
which equals that in \eqref{eq: T_simple} except for the missing absolute value signs around $\Psi_{T,y,h}^{b_0}$. They drop out as we only test against $b$ being larger than $b_0$. By Theorem \ref{Multiscale_Lemma} the corresponding quantile 
\[ \kappa_{T,\alpha}^{>b_0} := \min\left\{ r\in\R\mid \Pr_{b_0}\left( T_T^{<b_0}(X)\leq r\right) \geq 1-\alpha\right\} \]
is well-defined.
For testing against $H_<$ the same approach with local alternatives of the form $b = b_0- K_{y,h}$ leads to the test statistic
\begin{align*}
T_T^{<b_0}(X) := \sup_{(y,h)\in\mathcal{T}} \left( -\Psi_{T,y,h}^{b_0}(X) - C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2)\right)
\end{align*}
with the quantile $\kappa_{T,\alpha}^{<b_0}$ under $\Pr_{b_0}$ defined correspodingly.\\

It is important to note that we restrict attention to the \textit{simple} null hypothesis \eqref{eq: H_0-simple}, where the quantiles $\kappa_{T,\alpha}^{\neq b_0}, \kappa_{T,\alpha}^{<b_0}$ and $\kappa_{T,\alpha}^{>b_0}$ of our test statistics have to be determined under $\Pr_{b_0}$. As exemplarily the one-sided alternative $H_>$ is also a reasonable alternative for the composite null $\{ b\leq b_0\}$, the question arises whether
\[ \sup_{b\in\{b\leq b_0\}} \Pr_b\left( T_T^{>b_0}(X) > \kappa_{T,\alpha}^{>b_0}\right) \leq \Pr_{b_0}\left(T_T^{>b_0}(X) > \kappa_{T,\alpha}^{>b_0}\right),  \]
in order to guarantee validity on the composite null $\{b\leq b_0\}$. However, it is totally unclear if this inequality is true, see Section \ref{Sec_similarity}. This missing stochastic order relationship crucially complicates the construction of the similarity test.










==> Version_ArXiv/Sections/Stability.tex <==
\section{Stability of the similarity test under model misspecification}\label{Sec_Stability}

In this section we investigate the behaviour of the test $\phi_T^\eta$ under misspecification of the driving noise in \eqref{eq: SDE}. An application of the test statistic for data $X$ given by the wrong model is reasonable from two different angles:
\begin{itemize}
\item On the one hand, one might \textit{not realize} that the data does not arise from the model \eqref{eq: SDE} and hence use the test statistic $T_T^\eta$. 
\item On the other hand, suppose one \textit{knows} that the model \eqref{eq: SDE} is wrong but up to now, no test for the assumed true model is available. Then one might use our similiarity test based on the wrong model if the latter is close to the assumed true model in some sense, as this is so far the only way to address the similarity testing problem.
\end{itemize}

Both questions ask for some continuity property of $X\mapsto T_T^\eta(X)$. However, as the definition of $T_T^\eta(X)$ involves a stochastic (It\^{o}-) integral, it is not even clear how it could be defined for data $X$ that is not given by a semimartingale. Moreover, as all results in Sections \ref{Sec_simple}, \ref{Sec_similarity} and \ref{Sec_Power} use very specific properties of the It\^{o} diffusion \eqref{eq: SDE}, any deviation from this model assumption might cause a failure of those results. Thus, the availability of continuity results on $X\mapsto T_T^\eta(X)$ is a priori not clear at all.\\
In Subsection \ref{SubSec_cont} we will propose a natural extension of our test statistic $T_T^\eta$ that is defined pathwise and is in fact well defined for any continuous path $X$. Furthermore, we establish continuity 
of this extended test statistic with respect to the topology of uniform convergence. In Subsection \ref{SubSec_fractional_model} we particularly focus on fractional misspecification of the driving noise. 
We establish that even uniformly in the drift, the extended test statistic is stable as the fractional noise approaches Brownian motion. This uniformity, which is substantially harder to derive than the corresponding pointwise result for any fixed drift, is crucial in order to deduce that the test is actually uniformly (over the drift) asymptotically of level $\alpha$ in this limiting scenario, see \eqref{eq: level_H}.
Moreover, we prove that the minimax optimality is preserved in a certain sense as the fractional driving process approaches Brownian motion.






\subsection{Continuity properties of the test statistic}\label{SubSec_cont}

As mentioned in the introduction of this section, the first obstacle appearing is that the test statistic $T_T^\eta(X)$ given in \eqref{eq: T_eta} can only be evaluated for semimartingles as it involves the It\^{o} integral \[  \int_0^T K_{y,h}(X_s) dX_s, \]
where ther kernel $K$ satisfies the requirements of Theorem \ref{worst_case_delta}. To give a pathwise definition, we have to generalize the test statistic. To this aim, we assume in addition the kernel $K$ to be continuously differentiable and apply It\^{o}'s formula to $f(x) = \int_0^x K_{y,h}(y) dy$ which gives for the diffusion $X$ solving~\eqref{eq: SDE}
\[ \int_0^T K_{y,h}(X_s) dX_s= \int_{X_0}^{X_T} K_{y,h}(z) dz - \frac{\sigma^2}{2}\int_0^T (K_{y,h})'(X_s) ds.\]
On the right-hand side, it is perfectly possible to insert any continuous function $f\in\mathcal{C}([0,T])$. Therefore, we define
\begin{align*}
\tilde{I}_T:\ \mathcal{C}([0,T]) &\longrightarrow\ \R, \\
 f\ \ \  & \longmapsto\ \int_{f(0)}^{f(T)} K_{y,h}(z) dz - \frac{\sigma^2}{2}\int_0^T (K_{y,h})'(f(s)) ds.
\end{align*} 
$\tilde I_T$ is measurable as it is continuous with respect to $\|\cdot\|_{[0,T]}$. 
Let 
\[ D_{A,T}:= \{ f\in\mathcal{C}([0,T]) \mid -A,A\in f([0,T]) \} \]
be the set of real-valued continuous functions $f$ on $[0,T]$ whose image set $f([0,T])$ contains the interval $[-A,A]$.
For any $f\in D_{A,T}$ we denote
\begin{align}\label{eq: tilde_psi}
\tilde\Psi_{T,y,h}^{b_0}(f) &:=  \frac{\tilde I_T(f)}{\sigma\sqrt{ \int_0^T K_{y,h}(f(s))^2 ds}} -\frac{\int_0^T K_{y,h}(f(s)) b_0(f(s)) ds}{\sigma\sqrt{ \int_0^T K_{y,h}(f(s))^2 ds}}.
\end{align} 
Based on those $\tilde\Psi_{T,y,h}^{b_0}(f)$% with $(y,h)\in\mathcal{T}_T$
, the final extended test statistic is given pathwise by
\[ \tilde T_T^{\eta}(f) := \sup_{(y,h)\in\mathcal{T}_T} \left(\left| \tilde\Psi_{T,y,h}^{b_0}(f)\right|- \Lambda_{T,y,h}^\eta(X) - C(\hat\sigma_T(y,h)^2/\hat\sigma_{T,\max}^2) \right) .\]
Here, $\hat\sigma_T(y,h), \hat\sigma_{T,\max}, \Lambda_{T,y,h}^\eta(X)$ and $C(\cdot)$ are defined as in Section~\ref{Sec_simple} and~\ref{Sec_similarity} where no problem occurs as all involved integrals are  classical integrals. Note that in the respective definitions of $\tilde\Psi_{T,y,h}^{b_0}(f)$ and $\tilde T_T^\eta(f)$, no division by zero occurs due to the restriction of $f$ to $D_{A,T}$.
Additionally, as a consequence of Remark \ref{remark_bandwidth} in Appendix~\ref{Sec_Implementation} on implementation, it is sufficient to restrict attention to $\mathcal{T}_T := \left\{ (y,h)\in\mathcal{T}\mid h\geq h_{\min}(T)\right\}$.% Finally, we can introduce the test
%\[ \tilde\phi_T^\eta(f) := \1_{\left\{ \tilde T_T^\eta(f) >\kappa_{\eta,\alpha}\right\}} .\]




\begin{thm}\label{thm_continuity}
The mapping $\tilde{T}_T^\eta: D_{A,T}\longrightarrow\R$ is continuous with respect to the topology of uniform convergence.
\end{thm}










\subsection{Fractional misspecification of the noise}\label{SubSec_fractional_model}


As an example beyond a common semimartingale or Markovian setup with non-trivial dependence structure in time, we consider dynamics of the form
\begin{align}\label{eq: SDE_H}
dX_t^H = b(X_t^H) dt + \sigma dW_t^H, \quad X_0^H =x_0,
\end{align} 
where $W^H$, $H\in (0,1)$, is a fractional Brownian motion, i.e. a Gaussian process with covariance structure
\begin{align}\label{eq: R_H}
R_H(t,s) = \E\left[ W_t^H W_s^H\right] = \frac12\left( t^{2H} + s^{2H} - |t-s|^{2H}\right). 
\end{align} 
Although developing a similarity test for this fractional model and arbitrary $H$ is obstructed by missing developments in stochastic analysis that enable to perform sophisticated empirical process theory, for $H\approx 1/2$ the model in \eqref{eq: SDE} may be a good description of the true dynamics in \eqref{eq: SDE_H}. We propose to still use $\phi_T^\eta$ based on the wrong model in this context. For justification, we subsequently prove that for $H\approx 1/2$, the test statistic $\tilde T_T^\eta(X^{H,b})$ is close to $\tilde T_T^\eta(X^{b})$, uniformly in $b$. %and $\tilde\phi_T^\eta$ is close to the best possible test.




%\subsection*{The fractional diffusion model}

%Throughout this section we fix a time horizon $T$ and a probability space $(\Omega, \mathcal{A}, \Pr)$ that supports a Brownian motion $W=(W_t)_{t\in [0,T]}$. As we are interested in convergence for varying Hurst parameter $H$ it is important that all $W^H$ are defined on the same probability space. Therefore, we define $W^H=(W_t^H)_{t\in [0,T]}$ by
Throughout this section we fix a probability space $(\Omega, \mathcal{A}, \Pr)$ that supports a Brownian motion $W=(W_t)_{t\geq 0}$. As we are interested in convergence for varying Hurst parameter $H$ it is important that all $W^H$ are defined on the same probability space. Therefore, we define $W^H=(W_t^H)_{t\in [0,T]}$ by
\[ W_t^H := \int_0^t K_H(t,s) dW_s, \]
where $K_H$ is some kernel function specified in \eqref{eq: K_H}. One also has that $W^H|_{H=1/2} = W$ is a standard Brownian motion. \\
Existance of a strong solution to \eqref{eq: SDE_H} was established in \cite{Nualart} under the condition 
\begin{enumerate}
\item[(i)] $|b(x)|\leq C(1+|x|)$ if $H\leq \frac12$ and 
\item[(ii)] $|b(x) - b(y)|\leq C|x-y|^\alpha$ for some $1>\alpha>1-\frac{1}{2H}$ in the case $H>\frac12$.
\end{enumerate}
In fact, in the second case one can also use Lipschitz continuous $b$ as in \cite{Tudor}. As we are interested to compare our results on the case $H=1/2$ with the fractional model, we restrict ourselves to Lipschitz continuous $b\in\Sigma(C,A,\gamma,\sigma)$. For such $b$ we denote the solution process of \eqref{eq: SDE_H} by $X^{H,b}$ and by $X^b$ the solution of \eqref{eq: SDE} for drift $b$ and initial condition $x_0$, respectively. \\


As a first result, we have $X^{H,b}\rightarrow X^b$ in probability uniformly on $[0,T]$ as $H\to 1/2$. For any fixed Lipschitz continuous drift function $b$, this convergence seems to be well-known in the literature. Here, the convergence is required \textit{uniformly} over Lipschitz balls for the crucial conclusion \eqref{eq: level_H}, and hence an own proof is presented in Appendix \ref{App_stability} which relies on Dudley's Theorem about suprema of Gaussian processes and identities for fractional integrals. 

\begin{proposition}\label{lemma_X^H-X}
%Let $b:\R\rightarrow\R$ be Lipschitz continuous with $|b(x)|\leq C(1+|x|)$. %Denote by $X^{H,b}$ the solution of \eqref{eq: SDE_H} and by $X^b$ a solution of \eqref{eq: SDE} with starting point $X_0=x_0$. 
For every $\epsilon,L>0$, we have
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)}\Pr\left( \|  X^{H,b} - X^b \|_{[0,T]} >\epsilon\right)\ \stackrel{H\to\frac12}{\longrightarrow}\ 0.\]
%Moreover, the above convergence is uniform over drifts $b\in \Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)$ for any $L>0$. 
%\[ \sup_{\mathcal{H}(1,L)\cap \Sigma(C,A,\gamma,\sigma)} \Pr\left(\|  X_b^H - X_b\|_{[0,T]} >\epsilon\right)\ \stackrel{H\to\frac12}{\longrightarrow}\ 0.\]
\end{proposition}

The preceeding Proposition \ref{lemma_X^H-X} shows that for small deviations of $H$ from $1/2$ the diffusion model \eqref{eq: SDE} is still a good description of the dynamics of $X^{H,b}$.\\
As a consequence of this Proposition and Theorem \ref{thm_continuity}, the next theorem states that uniformly in $b$, $\tilde T_T^\eta$ is stable as $H$ approaches $1/2$ conditional on the event that the statistics are defined.



\begin{thm}\label{prop_stability}
Conditional on the event $\{X^{H,b},X^{b}\in D_{A,T}\}$, the test statistic $\tilde T_T^\eta(X^{H,b})$ converges to $\tilde T_T^\eta(X^{b})$ in probability uniformly over drift functions $b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)$ for any $L>0$, i.e. for every $\epsilon>0$,
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)}\Pr\left( \left. \left| \tilde T_T^\eta(X^{H,b}) - \tilde T_T^\eta(X^{b}) \right| >\epsilon \ \right| X^{H,b},X^{b}\in D_{A,T} \right) \stackrel{H\to\frac12}{\longrightarrow} 0\]
for $T$ sufficiently large. Moreover, we have for the conditioning event
\begin{align*}
&\liminf_{T\to\infty} \liminf_{H\to\frac12} \inf_{b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)}  \Pr\left( X^{H,b}, X^{b}\in D_{A,T}\right)\\
&\hspace{1cm}=\liminf_{H\to\frac12} \liminf_{T\to\infty} \inf_{b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L)}\Pr\left( X^{H,b}, X^{b}\in D_{A,T}\right)  =1.
\end{align*} 
\end{thm}


The idea of the proof is to use the continuity of $\tilde T_T^\eta$ from Theorem \ref{thm_continuity}. However, continuity solely is not sufficient to derive the uniformity in $b$ as stated in Theorem \ref{prop_stability}. By showing tightness of the family of measures $\{\Pr^{X^{H,b}} : b\in\Sigma(C,A,\gamma,\sigma)\cap\mathcal{H}(1,L), H\in \{H_n:n\in\N\}\}$ for any sequence $(H_n)_{n\in\N}$ with $H_n\to\frac12$, we are able to restrict attention to a compact subset of $D_{A,T}$ in $\mathcal{C}([0,T])$. On this, $\tilde T_T^\eta$ is uniformly continuous and we can apply the uniform continuous mapping theorem for convergence in probability, see Lemma \ref{lemma_CMT_uniform}. The proof of tightness does not follow the route of verifying asymptotic stochastic equicontinuity, but is instead based on the Gronwall lemma, Proposition \ref{lemma_X^H-X}, the Arzelà-Ascoli theorem and Prohorov's theorem, see Lemma \ref{lemma_X^H_tight}.



\begin{remark}\label{remark_stability}
With the uniform convergence in conditional probability in Proposition \ref{prop_stability}, it is reasonable to define a test $\tilde\phi_T^\eta$ based on $\tilde T_T^\eta$ as it was done in \eqref{eq: phi_eta} for the Brownian diffusion.  For some $\kappa> \kappa_{\eta,\alpha}$, where $\kappa_{\eta,\alpha}$ is given in \eqref{eq: kappa_eta_alpha}, we set
\[ \tilde\phi_T^\eta\left(X^H\right) := \1_{\left\{ \tilde T_T^\eta(X^H)>\kappa\right\}}.\]
Then one obtains as a corollary of Propsition \ref{prop_stability} that this test $\tilde\phi_T^\eta$ is in the limit $H\to\frac12$ uniformly (over $H_0(b_0,\eta)\cap\mathcal{H}(1,L)$) asymptotically of level $\alpha$ in the sense that
\begin{align}\label{eq: level_H}
\limsup_{T\to\infty} \limsup_{H\to\frac12}\sup_{b\in H_0(b_0,\eta)\cap\mathcal{H}(1,L)} \Pr_b\left(\tilde\phi_T^\eta(X^H) =1 \right) \leq \alpha. 
\end{align} 
\end{remark}



%For $H\to\frac12$ we have the following convergence in probability:
%\[ \tilde T_T^{\eta}\left(X^H\right) \longrightarrow_\Pr \tilde T_T^{\eta}\left(X^{1/2}\right). \]
%Alternative......: For all $\epsilon>0$ there exists a sequence $\delta(T) := \delta(T,\epsilon)>0$ such that
%\[ \limsup_{T\to\infty} \sup_{|H-\frac12|< \delta(T)} \Pr\left( \left| \tilde T_T^\eta(X^H) - \tilde T_T^\eta(X^{1/2})\right|>\epsilon\right) = 0.\]
%
%Other alternative....: Denote by $X_T^H$ and $X_T^{1/2}$ the solution to equation \eqref{eq: SDE_H} up to time $T>0$. For all $\epsilon>0$ we have
%\[ \lim_{H\to\frac12} \Pr\left( \left| \tilde T_T^\eta(X_T^H) - \tilde T_T^\eta(X_T^{1/2})\right|>\epsilon\right) \leq 2\Pr\left( X_T^{1/2}\notin D_{A+\epsilon}\right).\]



%Is Remark then: For every $\epsilon>0$ there exists $\delta(T)>0$ such that
%\[ \limsup_{T\to\infty} \sup_{|H-\frac12|< \delta(T)} \Pr\left( \tilde T_T^\eta(X^H) >\kappa_{\eta,\alpha}\right) \leq \limsup_{T\to\infty} \Pr\left( \tilde T_T^\eta(X^{1/2}) >\kappa_{\eta,\alpha}-\epsilon\right).\]









%\subsection*{The likelihood of the fractional diffusion model and lower bounds}\label{SubSec_likelihood}

Finally, we show that the test $\tilde\phi_T^\eta$ is indeed powerful for $H\approx 1/2$ by establishing a lower bound in the spirit of Theorem \ref{lower_bound} for $H$ being close to the Brownian case $H=1/2$.
%This relies on a change of measure formula for solutions of \eqref{eq: SDE_H} with constant volatility. It is known in the literature and stated in Proposition \ref{Girsanov_fBM} that $X_b^H$ solving \eqref{eq: SDE_H} is a fractional Brownian motion with start in $x_0$ under the measure $\tilde\Pr$ defined by 
%\[ \frac{d\tilde\Pr}{d\Pr} = Z_T^H(b_\cdot^H), \]
%where the definition of the likelihood $Z_T^H$ is given in the precise formulation of the Proposition in Appendix \ref{App_stability}. \\


%The next result may be read as follows: for every test $\psi_T^H$ of level $\alpha$ of the hypothesis $H_0(b_0,\eta)$ in the model \eqref{eq: SDE_H} with $H\in (0,1)$ and every $H'$ too close enough to $1/2$ there exists an alternative function that deviates at least $(1-\epsilon_T)c_*\delta_T$ from $H_0(b_0,\eta)$ in the semimetric $\Delta_J$ that will not be detected by $\psi_T^{H'}$ with probability $1-\alpha-o(1)$ or larger.


\begin{thm}\label{Continuity_lower_H}
Let $x_0\in [-A,A]$ and $b_0\in\Sigma(C/2-\eta,A,\gamma+\eta/\sigma^2,\sigma)$. Then for every $\epsilon>0$ there exists a sequence $\delta(T):=\delta(T,\epsilon)>0$ such that
\[ \limsup_{T\to\infty} \sup_{\substack{H:\ |H-\frac12|<\delta(T)}} \sup_{\psi_T^H}\ \inf_{\substack{b\in H_1(b_0,\eta)\cap \{b-b_0\in\mathcal{H}(\beta,L)\}:\\ \Delta_J(b)\geq (1-\epsilon_T)c_*\delta_T}} \E\left[\psi_T^H(X^{H,b})\right]\leq \alpha +\epsilon,\]
where $\sup_{\psi_T^H}$ is taken over tests $\psi_T^H$ with $\sup_{b\in H_0(b_0,\eta)}\E\left[ \psi_T^H(X^{H,b})\right] \leq \alpha$.
\end{thm}


The idea of the proof is to bound $\sup_{b\in H_0(b_0,\eta)}\E\left[ \psi_T^H(X^{H,b})\right]-\alpha$ from above by an expression involving an average of likelihoods of certain unfavourable alternatives as it was done in the proof of Theorem \ref{lower_bound}. Then we prove 
\begin{align}\label{eq: L1_Z_H}
\E\left[\left| Z_T^H(b_k(X_\cdot^{H,b})) - Z_T^{1/2}(b_k( X_\cdot^b))\right|\right] \stackrel{H\to\frac12}{\longrightarrow} 0
\end{align} 
where $Z_T^{H}$ denotes the likelihood from Girsanov's theorem, to apply Theorem \ref{lower_bound} for the case of $X^b$.
The $L^1(\Pr)$-convergence in \eqref{eq: L1_Z_H} is established by rewriting the explicit form of $Z_T^H$ in terms of fractional integrals and derivatives and then derive continuity results of those. Note that the likelihood ratios $Z_T^H$ for $H\neq 1/2$ are far more complicated than in case of $H=1/2$, see Appendix \ref{SubSub_fBM}.







==> Version_ArXiv/Sections/Trials.tex <==
\section{Trials}



\begin{lemma}
Suppose that $c_1\leq \frac1T L_T^x(X)\leq c_2$. Then we have for all $u,\delta>0$
\[N\left( (u\delta)^\frac12, \{ (y,h)\in\mathcal{T}: \sigma((y,h))^2\leq\delta\}, \rho\right) \leq ....u^{-2}\delta^{-1},\]
where
\[ \sigma((y,h))^2 := \frac1T\int_0^T K_{y,h}(X_s)^2 ds\]
and
\[ \rho( (y,h), (y',h')) :=\frac1T \int_0^T \left( K_{y,h}(X_s) - K_{y',h'}(X_s)\right)^2 ds.\]
\end{lemma}
\begin{proof}
We split the interval $[a,b]$ into a partition $(M_k)_{1\leq k\leq N}$ such that $\lambda(M_k)=\frac{u\delta}{2c_2\|K\|_{TV}}$ for $1\leq k\leq N-1$ and $\lambda(M_N)\leq \frac{u\delta}{2c_2\|K\|_{TV}}$. Then we have
\[ \lambda([a,b]) = \sum_{k=1}^N \lambda(M_k)\geq (N-1)\frac{u\delta}{2c_2\|K\|_{TV}}, \]
or equivalently
\[ N\leq 1+ \frac{2(b-a)c_2\|K\|_{TV}}{u\delta}.\]
Take $(y,h)\in\mathcal{T}$ such that $\sigma(y,h)^2\leq\delta$, i.e.
\[ \frac1T\int_0^T K_{y,h}(X_s)^2 ds = \int_\R K_{y,h}(z)^2 \frac1T L_T^z(X) dz \leq \delta.\]
Now using the lower bound for the averaged local time we get
\[ \delta\geq c_1\int_\R K_{y,h}(z)^2 dz = c_1\int_{y-h}^{y+h} K\left(\frac{z-y}{h}\right)^2 dz = c_1h\int_{-1}^1 K(z)^2 dz = hc_1\| K\|_{L^2}^2,\]
which implies $h\leq \delta c_1^{-1}\|K\|_{L^2}^{-2}$. Now suppose $y-h\in M_i$ and $y+h\in M_j$. As we know the length of the intervals $M_k$ we conclude
\[ (i-j-1)\frac{u\delta}{2c_2\|K\|_{TV}} \leq \frac{2\delta}{c_1\|K\|_{L^2}^2}\quad\Leftrightarrow\quad i-j\leq 1+\frac{4c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2} u^{-1}.\]
Furthermore, we know that there are at most 
\begin{align*}
&\left( 1+\frac{4c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2} u^{-1}\right)\left( 1+2(b-a)c_2\|K\|_{TV}(u\delta)^{-1}\right)\\
&\hspace{1.5cm}\leq  8c_2\|K\|_{TV} \max\left\{ b-a, \frac{2}{c_1\|K\|_{L^2}^2}, \frac{4(b-a)c_2\|K\|_{TV}}{c_1\|K\|_{L^2}^2}\right\} u^{-2}\delta^{-1}
\end{align*} 
such pairs. Thus the proof is finished if we could show that there is at most one such point $(y,h)$ in a maximal subset $\mathcal{T}'$ of $\{ (y,h)\in\mathcal{T}: \sigma(y,h)^2\leq \delta\}$ with $\rho((y,h),(y',h'))^2>u\delta$ for arbitrary $(y,h),(y',h')\in\mathcal{T}'$. We pick $(y,h), (y',h')\in\mathcal{T}$ such that $y-h, y'-h'\in M_i$ and $y+h, y'+h'\in M_j$ and are done if we can show that for those $\rho((y,h),(y',h'))^2\leq u\delta$.\\
As $K$ is of bounded variation, there exists a probability measure $\mu$ on $[-1,1]$ and a measurable function $g$ with $|g|\leq \|K\|_{TV}$ such that for almost all $x\in [-1,1]$ we have
\[ K(x) = \int_{-1}^x g d\mu.\]
Since $K$ is bounded by one, we have
\begin{align*}
&\frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds\\
&\hspace{1.5cm} \leq \frac1T\int_0^T \left| K_{y,h}(X_s)-K_{y',h'}(X_s)\right| ds\\
&\hspace{1.5cm} = \int_\R\left| K\left(\frac{z-y}{h}\right) - K\left(\frac{z-y'}{h'}\right)\right| \frac1T L_T^z(X) dz\\
&\hspace{1.5cm} \leq c_2 \int_\R \left| \int_{-1}^{\frac{z-y}{h}} g(u) d\mu(u)- \int_{-1}^{\frac{z-y'}{h'}} g(u) d\mu(u)\right| dz\\
&\hspace{1.5cm} \leq c_2\int_\R \left|\int_{\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}}^{\max\left\{1, \frac{z-y}{h}, \frac{z-y'}{h'}\right\}} g(u) d\mu(u)\right| dz\\
&\hspace{1.5cm} \leq c_2\int_\R \int_{\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}}^{\max\left\{ 1,\frac{z-y}{h}, \frac{z-y'}{h'}\right\}} |g(u)| d\mu(u) dz\\
&\hspace{1.5cm} \leq c_2\|K\|_{TV} \int_\R\int_{-1}^1 1_{B_z((y,h),(y',h'))} (u) d\mu(u) dz\\
&\hspace{1.5cm} = c_2 \|K\|_{TV} \int_{-1}^1 \int_\R 1_{B_z((y,h),(y',h'))} (u) dz d\mu(u),
\end{align*}
with
\[B_z((y,h),(y',h')) = \left[\min\left\{-1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}, \max\left\{1,\frac{z-y}{h},\frac{z-y'}{h'}\right\}\right]\]
and an application of Fubini's theorem in the last step. Now $u\in B_z((y,h),(y',h'))$ if and only if
\[ -1\leq \frac{z-y}{h}\leq u\leq \frac{z-y'}{h'}\leq 1\quad \textrm{ or }\quad -1\leq\frac{z-y'}{h'}\leq u\leq \frac{z-y}{h}\leq 1.\]
The first condition is equivalent to $uh'+y'\leq z\leq uh+y$, the second one to $uh+y\leq z\leq uh'+y'$. Thus, the inner integral equals $|y' + uh' - y - uh|$ and we get
\begin{align*}
\frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds&\leq c_2 \|K\|_{TV}\int_{-1}^1 |y'+uh'-y-uh| d\mu(u)\\
&\leq c_2 \|K\|_{TV}\max_{u=\pm 1} |y-y' +u( h-h')|\\
&\leq c_2\|K\|_{TV} \lambda([y-h,y+h]\bigtriangleup [y'-h',y'+h']),
\end{align*}
where the second inequality follows from the fact, that $|y-y' + u(h-h')|$ is maximized for $u=\textrm{sign}(y-y')\textrm{sign}(h-h')$.\\
As we chose $(y,h),(y',h')\in\mathcal{T}$ to fullfill $y-h,y'-h'\in M_i$ and $y+h,y'+h'\in M_j$ we know that
$\lambda([y-h,y+h]\bigtriangleup [y'-h',y'+h']) \leq 2\frac{u\delta}{2c_2\|K\|_{TV}}$. Hence,
\[ \frac1T\int_0^T \left( K_{y,h}(X_s)-K_{y',h'}(X_s)\right)^2 ds\leq 2c_2\|K\|_{TV}\frac{u\delta}{2c_2\|K\|_{TV}} = u\delta\]
and the proof is complete.
\end{proof}








\subsection{Alternative Proof of the upper bound}

First of all, we introduce the most important function spaces needed for the proof \textbf{(later put them in front part of the paper)}.
\begin{enumerate}
\item[(1)] For positive numbers $\beta, L$ we define the Hölder class $\mathcal{H}(\beta, L)$ as the set of $l=\lfloor \beta\rfloor$ times differentiable functions $f:S \rightarrow\R$, $S\subset\R$ whose derivative $f^{(l)}$ satisfies
\[ \left| f^{(l)}(x) - f^{(l)}(y)\right| \leq L|x-y|^{\beta -l}\quad \textrm{ for all } x,y\in S.\]
\item[(2)] For constants $M,\gamma, \sigma >0$ and $C\geq 1$ we set
\[ \Sigma(C,A,\gamma, \sigma) :=\left\{ b\in \textrm{Lip}_{loc}(\R):\ |b(x)|\leq C(1+|x|)\ \forall x\in\R\textrm{ and } \frac{b(x)}{\sigma^2}\textrm{sgn}(x)\leq -\gamma\ \forall |x|\geq A\right\}.\]
For all this functions $b\in\Sigma(C,A,\gamma, \sigma)$ there exists a unique strong solution of the SDE $dX_t = b(X_t) dt +\sigma dW_t$ with ergodic properties and invariant density
\[ \rho_b(x) := \frac{1}{C_{b,\sigma} \sigma^2} \exp\left( \int_0^x \frac{2b(y)}{\sigma^2} dy\right) \quad\textrm{ for all } x\in\R,\]
with the normalising constant $C_{b,\sigma}:= \int_\R \frac{1}{\sigma^2}\exp\left(\int_0^u \frac{2b(y)}{\sigma^2} dy\right)du$. We will denote the corresponding invariant measure by $\mu_b$.
%Moreover, we can deduce from this assumption some regularity properties of the invariant density $\phi_b$. In particular, there exists a constant $\mathcal{L}=\mathcal{L}(C,A,\gamma,\sigma)$ such that
%\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \max\left\{ \|\phi_b\|_\infty, \|\phi_b'\|_\infty\right\} <\mathcal{L}, \]
%and for any $\theta>0$ we have
%\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)}\sup_{x\in\R} |x|^\theta\phi_b(x) <\infty.\]

%\item[(3)] Last but not least we set for $\beta, L>0$
%\[ \Sigma(\beta, L) := \Sigma(\beta, L, C,A,\gamma) := \left\{ b\in\Sigma(C,A,\gamma,1): \phi_b\in\mathcal{H}(\beta+1, L)\right\}.\]

\item[(3)] Last but not least set for $\beta, L>9$
\begin{align*}
\Sigma(\beta, L) := \Sigma(\beta, L, C,A,\gamma,b_0)  := \left\{ b_1\in \Sigma(C,A,\gamma,1) : (b_1-b_0) \in\mathcal{H}(\beta,L)\right\}.
\end{align*}
\end{enumerate}








\subsubsection{Regularity of drift and invariant density}

\begin{lemma}
For $f\in\mathcal{H}(\beta +1, L)$, we have $f'\in\mathcal{H}(\beta,L)$.
\end{lemma}
\begin{proof}
As $1+\beta>1$ we know from the definition of the Hölder class that $f$ is at least one time differentiable and $f'$ exists. Furthermore, as $\lfloor\beta+1\rfloor = 1+\lfloor \beta\rfloor$, $f'$ is $l=\lfloor\beta\rfloor$ times differentiable and
\begin{align*}
\left| (f')^{(\lfloor\beta\rfloor)}(x) - (f')^{(\lfloor\beta\rfloor)}(y)\right| &= \left| f^{(1+\lfloor\beta\rfloor)}(x) - f^{(\lfloor\beta\rfloor)}(y)\right|\\
& \leq L|x-y|^{\beta+1 - (1+\lfloor\beta\rfloor)} = L|x-y|^{\beta-\lfloor\beta\rfloor}.
\end{align*}
\end{proof}




\begin{lemma}\label{bound_invariant_density}
There exists a constant $L = L(C,A,\gamma,\sigma)$ such that
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \max\left\{ \|\rho_b\|_\infty, \| \rho_b'\|_\infty\right\} \leq L.\]
\end{lemma}
\begin{proof}[Proof]
Let $b\in\Sigma(C,A,\gamma,\sigma)$. First we look for an upper bound of the normalizing factor $C_{b,\sigma}^{-1}\sigma^{-2}$ which equivalent to looking for a lower bound of $C_{b,\sigma}$. By the at most linear growth condition we get
\[ \left| \int_0^x 2\sigma^{-2} b(y) dy\right| \leq 2\sigma^{-2} \int_0^{|x|} |b(y)|dy \leq 2\sigma^{-2} \int_0^{|x|} C(1+|y|)dy \leq 2C\sigma^{-2}(1+|x|)|x|.\]
Hence on the interval $[-a,a]$ with $a\leq 1$ we have
\[ \exp\left( \int_0^x \frac{b(y)}{\sigma^2} dy \right) \geq \exp\left( - 2C\sigma^{-2} (1+a)a\right) \geq \exp\left( - 2C\sigma^{-2}\right).\]
Setting $a=\frac{1}{C}$ we get by non-negativity of $\exp$ that
\[ C_{b,\sigma} \geq \int_{-C^{-1}}^{C^{-1}} \sigma^{-2} \exp\left(\int_0^u 2\sigma^{-2} b(y) dy\right) du \geq \frac{2}{C\sigma^2} \exp\left( -2C\sigma^{-2}\right).\]
Thus,
\[ \frac{1}{C_{b,\sigma}\sigma^2} \leq \frac{C\sigma^2}{2} e^{2C\sigma^{-2}},\]
so the normalizing constant of the invariant density $\rho_b$ is bounded by some constant depending only on $C$ and $\sigma$.\\
We now turn to $\exp\left(\int_0^x 2\sigma^{-2} b(y) dy\right)$ and see that it suffices to bound the exponent by some constant. For $x>0$ we may upper-bound via
\begin{align*}
\int_0^x 2\sigma^{-2} b(y) dy &\leq \int_0^{A\wedge x} 2\sigma^{-2}b(y) dy + \int_{A\wedge x}^x 2\sigma^{-2}b(y) dy \\
&\leq 2\sigma^{-2} C(1+A) A + 2\int_{A\wedge x}^x -\gamma dy\\
&= 2\sigma^{-2} C(1+A) A -2\gamma(x-A\wedge x)\\
&\leq 2\sigma^{-2} C(1+A) A + 2A\gamma.
\end{align*} 
Similarly, we ge for $x<0$
\begin{align*}
\int_0^x 2\sigma^{-2} b(y) dy &= -\int_0^{-x} 2\sigma^{-2} b(y) dy\\
&= - \int_0^{A\wedge(-x)} 2\sigma^{-2}b(y) dy - \int_{A\wedge (-x)}^{-x}2\sigma^{-2}b(y) dy\\
&\leq 2\sigma^{-2} C(1+A)A - 2\int_{A\wedge (-x)}^{-x} \gamma dy\\
&= 2\sigma^{-2} C(1+A)A - 2\gamma (-x - A\wedge (-x))\\
&\leq 2\sigma^{-2} C(1+A)A +2A\gamma.
\end{align*}
So finally, we have the bound
\[ \rho_b(x) \leq \frac{C\sigma^2}{2} e^{2C\sigma^{-2}} e^{2\sigma^{-2}C(1+A)A + 2A\gamma}.\]
Now we consider $\|\rho_b'\|_\infty$ and use $\rho_b' = 2b\rho_b$. Unfortunately, $b$ is not bounded by some constant so we are not done immediately. 
But we have shown above that
\[ \exp\left( \int_0^x 2\sigma^{-2} b(y) dy\right) \leq \exp\left( 2\sigma^{-2}C(1+A)A + 2A\gamma - 2\gamma |x|\right).\]
This gives
\begin{align*}
|\rho_b'(x)| \leq |2b(x) \rho_b(x)| &\leq C\sigma^{-2} e^{2C\sigma^{-2}} (1+|x|)e^{\tilde{c} - 2\gamma |x|}\\
&\leq C\sigma^{-2} e^{2C\sigma^{-2}}  \left( e^{\tilde{c}} + |x|e^{\tilde{c} - 2\gamma |x|}\right)
\end{align*} 
with  $\tilde{c} = 2\sigma^{-2}C(1+A)A + 2A\gamma$. Now the function $|x| e^{\tilde{c} - 2\gamma|x|}$ is bounded and maximized for $|x| = \frac{1}{2\gamma}$. Thus,
\[ |\rho_b'(x)| \leq C\sigma^{-2} e^{2C\sigma^{-2}}  \left( e^{\tilde{c}} + \frac{1}{2\gamma}e^{\tilde{c}-1}\right)\]
and the proof is finished by taking $L$ as the maximum of both the upper bounds.
\end{proof}


\begin{lemma}\label{local_time-Invariant}
Let $h_T = c\left(\frac{\log T}{T}\right)^\alpha$, $\alpha>0$. Furthermore, let $b\in\Sigma(C,A,\gamma,\sigma)$. Then for every $z\in [y-h_T, y+h_T]$
\[ \frac1T L_T^z(X) - \rho_b(y) = o_{\Pr}\left( (\log T)^{-1}\right).\]
\end{lemma}
\begin{proof}[Proof]
We first split in the obious way
\[ \frac1T L_T^z(X) - \rho_b(y) = \left( \frac1T L_T^z(X) -\rho(z)\right) + \left( \rho_b(z)-\rho_b(y)\right).\]
As $\rho_b$ is differentiable with bounded derivative it is Lipschitz continuous, more precisely we get with Lemma \ref{bound_invariant_density}
\[ \left|\rho_b(z)-\rho_b(y)\right| \leq L(C,A,\gamma,\sigma) |y-z| \leq 2L(C,A,\gamma,\sigma) h_T.\]
Using the definition of $h_T$ it follows $ (\rho_b(y)-\rho_b(z))1_{[y-h_T, y+h_T]}(z)\in o_T\left((\log T)^{-1}\right)$.\\
For the other term we use the fact that
\[ \sqrt{T} \left(\frac1T L_T^z(X) - \rho_b(z)\right) \] 
converges in distribution to a centered Gaussian random map according to Lemma $56$ in \textbf{Diss Willems/Strauch...look for the paper}. Hence, $\sqrt{T}\left(\frac1T L_T^z(X) - \rho_b(z)\right)\in \mathcal{O}_{\Pr}(1)$ and consequently
$\log T\left(\frac1T L_T^z(X) - \rho_b(z)\right)\in o_{\Pr}(1)$ and the claim follows.
\end{proof}








\subsubsection{The choice of the kernel}

Let $K= K(\cdot,\beta)$ be the unique solution of the following optimization problem:
\[ \textrm{Minimize } \|K\|_{L^2} \textrm{ over all } K\in\mathcal{H}(\beta,1) \textrm{ with } K(0)\geq 1.\]

In the case $0<\beta\leq 1$ it is not difficult to see that
\[ K(x) = 1_{|x|\leq 1} \left(1-|x|^\beta\right),\]
as we even have $K(x) \leq f(x)$ for all $x\in [-1,1]$ and $f\in\mathcal{H}(\beta,1)$ in this case. For $\beta =2$ an explicit solution is known (see Leonov...). Furthermore, for all $\beta>0$ $K$ is compactly supported, an even function and satisfies $K(0)=1>|K(x)|$ for $x\neq 0$. We will denote this compact support by $[-R,R]$.\\

For any scale parameter $h>0$ and location parameter $y\in\R$ we denote
\[ K_{y,h}(x) = K\left(\frac{x-y}{h}\right) \]
and this function is clearly supported in $[y-Rh, y+Rh]$.

\begin{lemma}\label{Lemma_rescaling}
For any $\delta>0$ the function $\tilde{K}:= \pm\delta K_{y,h}$ belongs to $\mathcal{H}(\beta, \delta h^{-\beta})$ and minimizes $\|\tilde{K}\|_{L^2}$ over this class under the additional constraint $\pm \tilde{K}(y)\geq \delta$.
\end{lemma}
\begin{proof}[Proof]
Clearly, as it holds for $K$, $\tilde{K}$ is $\lfloor \beta\rfloor$-times differentiable and we have
\begin{align*}
\left| \tilde{K}^{\lfloor\beta\rfloor}(x) - \tilde{K}^{\lfloor\beta\rfloor}(x')\right| &= \delta h^{-\lfloor\beta\rfloor} \left| K^{\lfloor\beta\rfloor}\left(\frac{x-y}{h}\right) - K^{\lfloor\beta\rfloor}\left(\frac{x'-y}{h}\right) \right| \\
&\leq \delta h^{-\lfloor\beta\rfloor}\left|\frac{x-y}{h} - \frac{x'-y}{h}\right|^{\beta-\lfloor\beta\rfloor} \\
&= \delta h^{-\beta} |x-x'|^{\beta-\lfloor\beta\rfloor},
\end{align*}
which establishes $\tilde{K}\in\mathcal{H}(\beta, \delta h^{-\beta})$.\\
For every $K$ with $K(0)\geq 1$, we have $\pm\tilde{K}(y) = \delta K(0)\geq\delta$ and for $L^2$-norm we have
\[ \|\tilde{K}\|_{L^2} = \left(\int_\R \delta^2 K\left(\frac{x-y}{h}\right)^2 dx\right)^\frac12 = \delta h^{-\frac12} \left(\int_\R K(x)^2 dx\right)^\frac12 = \delta h^{-\frac12} \|K\|_{L^2},\]
so this norm is minimized, if $\|K\|_{L^2}$ is minimized and we are done.
\end{proof}










\begin{proof}[Alternative Proof of Theorem \ref{Upper_bound}]
Denote $K_{y,h}(X_s) = K\left(\frac{X_s-y}{h}\right)$. For every $y$, the probability $\Pr(T(X)>\kappa_\alpha)$ of rejecting the null hypothesis is bounded from below by
\begin{align*}
&\Pr_{b_1}\left( \left| \Psi_T(y,h_T)\right| > C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right) + \kappa_\alpha\right) \\
&\hspace{0.5cm} =\Pr_{b_1}\left(\frac{\left| \frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s  + \frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left( b_1(X_s) - b_0(X_s)\right) ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right.\\
&\hspace{4cm}\left. > C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right)+\kappa_\alpha\right)\\
&\hspace{0.5cm} \geq \Pr_{b_1}\left( -\textrm{sign}\left(\int_0^T K_{y,h_T}(X_s)\left( b_1(X_s) - b_0(X_s)\right) ds\right) \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right. \\
&\hspace{2cm} \left. < \frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac2T\int_0^T K_{y,h_T}(X_s)^2 ds\right)+\kappa_\alpha\right).
\end{align*}
The idea of the proof is to proceed as follows: First, we show that the left side of the inequality forms a tight sequence and hence the claim is established once we show that the right side diverges to infinity in a second step.\\
As $z$ is taken from a compact set $A$, we find constants $c_1, c_2>0$ such that $c_1\leq \phi_b\leq c_2$. Now define the set
\[\mathcal{C}_T :=\left\{ \sup_{z\in A} \left| \frac1T \L_T^z(X) - \phi_b(z)\right| <\frac{c_1}{2}\right\}.\] 
By the result of van Zanten \textbf{tex this somewhere)} we have $\Pr_{b_1}(\mathcal{C}_T) \rightarrow 1$ for $T\to\infty$ and on $\mathcal{C}_T$ it holds that
\[ \frac12 \phi_b(z)\leq \frac1T \L_T^z(X)\leq \frac32 \phi_b(z).\]
Now let $\epsilon>0$ and take $T\geq T_0$ large enough such that $\Pr_{b_1}(\mathcal{C}_T)>1-\frac{\epsilon}{2}$. For $K>0$ we can write
\begin{align*}
&\Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K\right)\\
&\hspace{0.5cm} = \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T\right) + \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T^c\right)
\end{align*}
The second term is bounded by $\Pr(\mathcal{C}_T^c)<\frac{\epsilon}{2}$. For the first own we use the occupation times formula to get
\[ \frac1T \int_0^T K_{y,h_T}(X_s)^2 ds = \int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz\]
and on $\mathcal{C}_T$ we can upper- and lower-bound the averaged local time to get
\[ \frac12 \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz \leq \frac1T\int_0^T K_{y,h_T}(X_s)^2 ds \leq \frac32 \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz.\]
Now we apply Proposition \ref{Exp_ineq} with $\theta = \int_\R K_{y,h_T}(z)^2 \phi_b(z) dz$ and $S=\sqrt{3}$ to get
\[ \Pr_{b_1}\left(\left|\frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)dW_s}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}}\right| >K,\ \mathcal{C}_T\right) \leq 4K\sqrt{e} (1+\log(\sqrt{3}))\exp\left(-\frac{K^2}{2}\right).\]
Clearly, we can choose $K$ large enough to bound this term again by $\frac{\epsilon}{2}$ and the proof of the thightness is finished.\\

Now we want to show that
\[ \left( 1+\epsilon_T\right)\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds\right)\rightarrow \infty\]
for all $b_1-b_0\in\Sigma(\beta, L)$ such that $\|(b_1-b_0)\rho_{b_1}^\frac{\beta}{2\beta+1}\|_\infty \geq \delta_T$. Let $b_1$ be such a function with $\left|(b_1(y)-b_0(y)\rho_{b_1}(y)^\frac{\beta}{2\beta+1}\right|>\delta_T$, or equivalently
\[ |b_1(y) - b_0(y) | > c_*\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^{\frac{\beta}{2\beta+1}} =:\tilde{\delta}_T.\]
We define 
\[ h_T := \left(\frac{c_*}{L}\right)^{\frac{1}{\beta}}\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^{\frac{1}{2\beta+1}}.\]
Then from Lemma \ref{Lemma_rescaling} we know that $\tilde{\delta}_T K_{y,h_T}\in\mathcal{H}(\beta, \tilde{\delta}_T h_T^{-\beta}) = \mathcal{H}(\beta, L)$ and minimizes the $L^2$-norm over his class for all functions $f$ satisfying $f(y)\geq\delta$. In particular, this implies
\[ \left| \int_\R \tilde{\delta}_T K_{y,h_T}(z) (b_1(z)-b_0(z)) dz \right| \geq \tilde{\delta}_T^2 \int_\R K_{y,h_T}(z)^2 dz.\]
By the occupation times formula and Lemma \ref{local_time-Invariant} we may write
\begin{align*}
&\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} = \frac{\sqrt{T}\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) \frac1T L_T^z(X)dz\right|}{\sqrt{\int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz}}\\
&\hspace{1cm}=\frac{\sqrt{T}\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) \left( \rho_{b_1}(y) + \frac1T L_T^z(X) - \rho_{b_1}(y)\right)dz\right|}{\sqrt{\int_\R K_{y,h_T}(z)^2\left(\rho_{b_1}(y) + \frac1T L_T^z(X) - \rho_{b_1}(y)\right) dz}}\\
&\hspace{1cm} = \frac{\sqrt{T} \left(\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})\right)\left|\int_\R K_{y,h_T}(z)\left(b_1(z) - b_0(z)\right) dz\right|}{\sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})}\sqrt{\int_\R K_{y,h_T}(z)^2dz}}\\
&\hspace{1cm} = \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T}\frac{\tilde{\delta}_T^{-1} \left|\int_\R \tilde{\delta}_T K_{y,h_T}(z) ( b_1(z)-b_0(z)) dz \right|}{\sqrt{\int_\R K_{y,h_T}(z)^2dz}}\\
&\hspace{1cm}\geq \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T} \frac{\tilde{\delta}_T \int_\R K_{y,h_T}(z)^2 dz}{\sqrt{\int_\R K_{y,h_T}(z)^2 ds}}\\
&\hspace{1cm} = \sqrt{\rho_{b_1}(y) + o_{\Pr}((\log T)^{-1})} \sqrt{T h_T} \tilde{\delta}_T \| K\|_{L^2}
\end{align*}
where the last step follows by substitution of $\tilde{x}=\frac{x-y}{h_T}$ in the integral. Now be definition of $h_T$ and $\tilde{\delta}_T$ we have
\begin{align*}
\sqrt{Th_T}\tilde{\delta}_T &= T^\frac12 \left(\frac{c_*}{L}\right)^{\frac{1}{2\beta}} \left( \frac{\log T}{T\rho_{b_1}(y)}\right)^\frac{1}{2(2\beta+1)} c_*\left(\frac{\log T}{T \rho_{b_1}(y)}\right)^\frac{\beta}{2\beta+1}\\
&= c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \rho_{b_1}(y)^{-\frac{1}{2(2\beta+1)} - \frac{\beta}{2\beta+1}} T^{\frac12 - \frac{1}{2(2\beta+1)} - \frac{\beta}{2\beta+1}} (\log T)^{\frac{1}{2(2\beta+1)} + \frac{\beta}{2\beta+1}}\\
&= c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \rho_{b_1}(y)^{-\frac12} (\log T)^{\frac12},
\end{align*}
as $\frac{1}{2(2\beta+1)} + \frac{\beta}{2\beta+1} = \frac{1+2\beta}{2(2\beta+1)} = \frac12$. So we arrive at
\begin{align*}
\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} &\geq \sqrt{1+o_{\Pr}((\log T)^{-1})} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2}\sqrt{\log T}\\
&= \sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2}.
\end{align*}


Next, we treat the compensating term $C(\cdot)$ in a similar way. We have
\begin{align*}
C\left(\frac1T \int_0^T K_{y,h_T}(X_s)^2 ds\right) &= C\left( \int_\R K_{y,h_T}(z)^2 \frac1T L_T^z(X) dz\right) \\
&= C\left( (\rho_{b_1}(y)+o_{\Pr}(1)) \int_\R K_{y,h_T}(z)^2 dz\right) \\
&= C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right).
\end{align*}
With the definition of $C$ we proceed the following way:
\begin{align*}
&C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right) = \left( 2\log\left(\frac{1}{(\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T}\right)\right)^\frac12\\
&\hspace{1cm} = \left( -2 \log\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right)\right)^\frac12\\
&\hspace{1cm} = \left( - 2\log(h_T) - 2\log((\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 )\right)^\frac12\\
&\hspace{1cm}= \left( -2\log(h_T) +\mathcal{O}_{\Pr}(1)\right)^\frac12.
\end{align*}
Now with our definition of $h_T$ we have
\[ \log(h_T) = \frac{1}{\beta} \log\left( \frac{c_*}{L}\right) + \frac{1}{2\beta+1}\left( \log\log T - \log T - \log(\rho_{b_1}(y)) \right)\]
and consequently,
\[ C\left( (\rho_{b_1}(y) + o_{\Pr}(1)) \|K\|_{L^2}^2 h_T\right) = \left( \frac{2}{2\beta+1} \log T - \frac{2}{2\beta+1}\log\log T  + \mathcal{O}_{\Pr}(1)\right)^\frac12.\]
Now we can put everything together and evaluate the whole expression. With an application of Lemma \ref{log-terms} in the second step this yields
\begin{align*}
&\left( 1+\epsilon_T\right)\frac{\left|\frac{1}{\sqrt{T}}\int_0^T K_{y,h_T}(X_s)\left(b_1(X_s) - b_0(X_s)\right)ds\right|}{\sqrt{\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds}} -C\left(\frac1T\int_0^T K_{y,h_T}(X_s)^2 ds\right)\\
&\hspace{0.5cm} \geq (1+\epsilon_T)\sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2} - \left( \frac{2}{2\beta+1} \log T - \frac{2}{2\beta+1}\log\log T  + \mathcal{O}_{\Pr}(1)\right)^\frac12\\
&\hspace{0.5cm} = (1+\epsilon_T)\sqrt{\log(T) + o_{\Pr}(1)} c_*^\frac{2\beta+1}{2\beta} L^{-2\beta} \|K\|_{L^2} - \sqrt{\frac{2}{2\beta+1} \log T} + o_{\Pr}(1)\\
& \textbf{here we need the def of $c_*$ which will be in the theorem...} c_* = \left( \frac{2L^{\frac1\beta}}{(2\beta+1)\|K\|_{L^2}^2}\right)^{\frac{\beta}{2\beta+1}}\\
&\hspace{0.5cm} = \sqrt{\frac{2}{2\beta+1}} \left( \sqrt{\log T + o_{\Pr}(1)}- \sqrt{\log T} + \epsilon_T\sqrt{\log T + o_{\Pr}(1)}\right) + o_{\Pr}(1)\\
&= \sqrt{\frac{2}{2\beta +1}} \left( o_{\Pr}(1) + \epsilon_T\sqrt{\log T + o_{\Pr}(1)}\right) + o_{\Pr}(1) \rightarrow \infty.
\end{align*}
In the last step we have used that $\epsilon_T\sqrt{T}\rightarrow \infty$ and hence $\epsilon_T\sqrt{\log T + o_T(1)}\rightarrow\infty$ next to
\begin{align*}
\sqrt{\log T + o_{\Pr}(1)}- \sqrt{\log T} &= \frac{\log T + o_{\Pr}(1) - \log T}{\sqrt{\log T + o_{\Pr}(1)} + \sqrt{\log T}}\\
&= \frac{o_{\Pr}(1)}{\sqrt{\log T+o_{\Pr}(1)} + \sqrt{\log T}} =o_{\Pr}(1).
\end{align*} 
\end{proof}













\subsubsection{Sharp lower bound}

Like in any other proof of lower bounds we will reduce the problem to some challenging hypothesis - in our case some small deviations of the drift that will not be detected. In order to construct those, we choose a kernel function $K:\R\rightarrow\R$ with $K\in\mathcal{C}_c^\infty(\R)$, $\textrm{supp}(K) = [-1,1]$, $|K(x)|\leq 1$, $K(0)=1$ and $K\in\mathcal{H}(\beta, 1)$. We set
\[ h_T^w := \left(\frac{c_*}{L}\right)^\frac{1}{\beta} \left( \frac{\log T}{T w}\right)^\frac{1}{2\beta+1}.\]
Then we pick some drift $b_0\in\Sigma\left( \frac{C}{2},A, \gamma, 1\right)$ for the zero hypothesis and define the alternatives
\[ b_j^w(x) := b_0(x) + L(h_T^w)^\beta K\left(\frac{x-y_j^w}{h_T^w}\right),\]
where $y_j^w$ is some location depending continuously on $w$. To be valid hypotheses we need three conditions on $b_j^w$: 
\begin{itemize}
\item The SDE with drift $b_j^w$ should be ergodic, more precisely, we need $b_j^w\in \Sigma(C,A,\gamma, \sigma)$,
\item we need $b_0 - b_j^w\in\mathcal{H}(\beta, L)$,
\item the support of the $b_j-b_0$ should be disjoint which corresponds to a good choise of $y_hj^w$, and
\item we want 
\[\left|(b_j^w(y_j^w) - b_0(y_j^w))\rho_{b_j^w}(y_j^w)^\frac{\beta}{2\beta+1}\right| = L(h_T^w)^\beta K(0)\left|\rho_{b_j^w}(y_j^w)\right|^\frac{\beta}{2\beta+1} = c_*\left(\frac{\log T}{T}\right)^\frac{\beta}{2\beta+1}.\]
Using our definition of $h_T^w$ this is equivalent to
\[ w = \rho_{b_j^w}(y_j^w).\]
\end{itemize} 
As we are dealing with asymptotics, it is in fact enough to verify those conditions for $T\geq T_0$. The first two are standard and will be established in Lemmata \ref{lemma_cond_2} and \ref{lemma_cond_1}. The third condition will be dealt with in the proof of the main theorem by constructing the alternatives inductively. The last one could in fact be relaxed to $\geq$ instead of equality, but is self-evident to expect the hardest detectable alternative in the case of equality which is what we assume above. It also has the nice feature that is gives rise to a fixed-point problem: We associate to any $w$ in some suitable chosen interval a drift function $b_j^w$ which again is associated to a drift function $\rho_{b_j^w}$ which is known in the ergodic case. This drift can be evaluated at $y_j^w$ and we ask if it possible to chose $w$ in such a way that the outcome of the concatenation of these mapings is again $w$.




\begin{lemma}\label{lemma_cond_2}
For the drift functions $b_0$ and $b_j^w$ defined above we have $b_0-b_j^w\in\mathcal{H}(\beta, L)$
\end{lemma}
\begin{proof}
As $b_0 - b_j^w = L (h_T^w)^\beta K\left( \frac{\cdot - y_j^w}{h_T^w}\right)$ we know that this difference is $\lfloor\beta\rfloor$-times differentiable as this holds for $K$. Furthermore, 
\begin{align*}
&\left| (b_0-b_j^w)^{(\lfloor\beta\rfloor)}(x) - (b_0-b_j^w)^{(\lfloor\beta\rfloor)}(x')\right| \\
&\hspace{1cm}= L(h_T^w)^{\beta-\lfloor\beta\rfloor}\left| K^{(\lfloor\beta\rfloor)}\left( \frac{x-y_j^w}{h_T^w}\right) - K^{(\lfloor\beta\rfloor)}\left(\frac{x'-y_j^w}{h_T^w}\right)\right|\\
&\hspace{1cm}\leq L(h_T^w)^{\beta-\lfloor\beta\rfloor}\left| \frac{x-y_j^w}{h_T^w} - \frac{x'-y_j^w}{h_T^w}\right|^{\beta- \lfloor\beta\rfloor}\\
&\hspace{1cm}= L|x-x'|^{\beta-\lfloor\beta\rfloor},
\end{align*}
where we used in the second step that $K\in\mathcal{H}(\beta, 1)$.
\end{proof}




\begin{lemma}\label{lemma_cond_1}
For the drift $b_j^w$ defined above we have $b_j^w\in \Sigma(C,A,\gamma, \sigma)$ for all $T$ large enough to ensure $L(h_T^w)^\beta\leq \frac{C}{2}$.
\end{lemma}
\begin{proof}
We have $b_j^w(x) = b_0(x)$ for $|x|\geq A$ and hence $\frac{b_j^w(x)}{\sigma^2}\textrm{sgn}(x) \leq -\gamma$ for those $x$ as the condition is fullfilled for $b_0$. Furthermore, as $b_0$ and $K$ are locally Lipschitz, the same holds true for $b_j^w$. Last but not least, 
\[ |b_j^w(x)| \leq |b_0(x)| + L(h_T^w)^\beta \left| K\left(\frac{x-y_j^w}{h_T^w}\right)\right| \leq \frac{C}{2}(1+|x|) + L(h_T^w)^\beta \leq C(1+|x|).\]
\end{proof}



\begin{lemma}\label{lemma_fixed_point}
Choose $y\in\R$ and set $y_j^w = y+h_T^w$. Then for $T\geq T_0$ large enougt, there exists $\tilde{w}>0$ such that $\rho_{b_j^{\tilde{w}}}(y_j^{\tilde{w}}) = \tilde{w}$.
\end{lemma}
\begin{proof}
Denote by $f$ the concatenation of the following maps
\begin{equation*}
\begin{matrix}
& \R_{>0} & \longrightarrow & (\mathcal{C}^0, \|\cdot\|_\infty)\times \R &\longrightarrow & (\mathcal{C}^0, \|\cdot\|_\infty)\times \R &\longrightarrow &\R_{\geq 0}, \\
& w & \mapsto & \begin{pmatrix}b_j^{w}\\ y_j^w\end{pmatrix} &\mapsto & \begin{pmatrix}\rho_{b_j^w}\\ y_j^w\end{pmatrix} &\mapsto  & \rho_{b_j^w}(y_j^w).
\end{matrix}
\end{equation*}
Our proof will establish
\begin{itemize}
\item[(1)] continuity of $f:\R_{> 0}\rightarrow\R_{\geq 0}$, 
\item[(2)] existance of a compact interval $I\subset\R_{>0}$ such that $f(I)\subset I$. 
\end{itemize}
Then it follows that there exists a fixed point $\tilde{w}$ within the interval $I$ and the proof is complete.\\
We begin with statement $(1)$. The map $f$ consists of three parts and we will show continuity for each arrow seperately, each time $j$ and $T$. In each case the preimage of the map is the image of the previous mapping understood as a subspace of the given space in the diagram above. 
\begin{itemize}
\item[(a)] The first map $w\mapsto b_j^w$ can be split into $w\mapsto h_T^w \mapsto b_j^w$ as $y_j^w$ is also a function of $h_T^w$. In this composition continuity of the first part is obvious. For the second one we consider $w, w'>0$ and estimate with the fact that $K\in\mathcal{C}_c^\infty$
\begin{align*}
&\left| b_j^w(x) - b_j^{w'}(x)\right|\leq L\left| (h_T^w)^\beta K\left(\frac{x-y_j^w}{h_T^w}\right) - (h_T^{w'})^\beta K\left(\frac{x-y_j^{w'}}{h_T^{w'}}\right)\right|\\
&\hspace{0.5cm}\leq L\left| (h_T^w - h_T^{w'}) K\left(\frac{x-y_j^w}{h_T^w}\right) + h_T^{w'}\left( K\left(\frac{x-y_j^{w'}}{h_T^{w'}}\right) - K\left(\frac{x-y_j^w}{h_T^w}\right)\right)\right|\\
&\hspace{0.5cm} \leq \|K\|_\infty |h_T^w - h_T^{w'}| + h_T^{w'} \|K'\|_\infty\left| \frac{x-y_j^{w'}}{h_T	^{w'}} - \frac{x-y_j^w}{h_T^w}\right|\\
&\hspace{0.5cm} = \|K\|_\infty |h_T^w - h_T^{w'}| + h_T^{w'} \|K'\|_\infty\left| \frac{h_T^w ( x-y_j^{w'}) - h_T	^{w'} (x-y_j^w)}{h_T^{w'}h_T^w}\right|
\end{align*}
For the  numerator of the last term we have
\begin{align*}
h_T^w ( x-y_j^{w'}) - h_T	^{w'} (x-y_j^w) &= (h_T^w - h_T^{w'})x - h_T^w y_j^{w'} + h_T^{w'}y_j^w\\
&=  (h_T^w - h_T^{w'})x  - h_T^w ( y_j^{w'} - y_j^w) + y_j^w (h_T^{w'} - h_T^w) \\
&= (h_T^w - h_T^{w'})\left( x  + h_T^w - y_j^w\right)
\end{align*}
which yields 
\[ \left| b_j^w(x) - b_j^{w'}(x)\right|\leq \left( \|K\|_\infty + \frac{|y-x|}{h_T^w}\right) \left|h_T^w - h_T^{w'}\right|.\]
As the difference $b_j^w- b_j^{w'}$ vanishes outside $[-A,A]$ the factor is bounded in $x$ and we get continuity in supremum norm.\\
Continuity in the second parameter is again obvious as $y_j^w = 2j h_T^w$ is again a continuous function in $w$.

\item[(b)] Nothing happens in the second component, so we only have to work for the first one. Our hypotheses are of the form $b_j^w = b_0 + g_j^w$, so $\|b_j^w - b_j^{w'}\|_\infty = \|g_j^w - g_j^{w'}\|_\infty$ and the $g_j^w$ are supported within $[-A,A]$, i.e. the supremum norm of the difference vanishes outside this interval. The invariant density is of the form
\[ \rho_{b_{j^w}}(x) = \frac{1}{C_{b_j^w,\sigma}\sigma^2}\exp\left( \int_0^x \frac{2b_j^w}{\sigma^2} dy\right),\]
and we show continuity of $b_j^w\mapsto C_{b_j^w,\sigma}$ and $b_j^w\mapsto \exp\left(\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy \right)$ where the latter is understood as a continuous function in $(\mathcal{C}^0, \|\cdot\|_\infty)$.\\
Let $\epsilon>0$, then there exists $\delta>0$ such that 
\[ \left\| \exp\left(\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy \right)-\exp\left(\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy \right)\right\| <\epsilon\]
if 
\[ \left\|\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy-\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy\right\|_\infty<\delta.\]
But the last expression can be bound in terms of $\|b_j^w - b_j^{w'}\|_\infty$ as
\begin{align*}
&\left|\int_0^x \frac{2b_j^w(y)}{\sigma^2} dy-\int_0^x \frac{2b_j^{w'}(y)}{\sigma^2} dy\right| \leq 2\sigma^{-2} \left| \int_0^x b_j^w(y) - b_j^{w'}(y) dy\right|\\
&\hspace{1cm} \leq 2\sigma^{-2} \int_0^{|x|} \left| g_j^w(y) - g_j^{w'}(y)\right| dy \leq 2\sigma^{-2} \int_{-A}^A\left| g_j^w(y) - g_j^{w'}(y)\right| dy \\
&\hspace{1cm} \leq 4A\sigma^{-2} \|g_j^w - g_j^{w'}\|_\infty = 4A\sigma^{-2} \|b_j^w - b_j^{w'}\|_\infty.
\end{align*}
We move on to $b_j^w\mapsto C_{b_j^w,\sigma}$. By the triangle inequality we directly get
\begin{align*}
&\left| C_{b_j^w, \sigma} - C_{b_j^{w'}, \sigma}\right| \leq \sigma^{-2} \int_\R\left|\exp\left( \int_0^y 2\sigma^{-2} b_j^w(u) du \right) - \exp\left(\int_0^y 2\sigma^{-2} b_j^{w'}(u) du \right)\right| dy \\
& \hspace{0.5cm}= \sigma^{-2} \int_\R \exp\left(\int_0^y 2\sigma^{-2} b_0(u) du \right) \left|\exp\left( \int_0^y 2\sigma^{-2} g_j^w(u) du \right) - \exp\left(\int_0^y 2\sigma^{-2} g_j^{w'}(u) du \right)\right| dy\\
&\hspace{0.5cm} \leq C_{b_0,\sigma} \left\|\exp\left( \int_0^\cdot 2\sigma^{-2} g_j^w(u) du \right) - \exp\left(\int_0^\cdot 2\sigma^{-2} g_j^{w'}(u) du \right)\right\|_\infty
\end{align*}
So $|C_{b_j^w, \sigma} - C_{b_j^{w'}, \sigma}|<\epsilon$ if the last supremum norm ist $<\frac{\epsilon}{C_{b_0,\sigma}}$ which can be archived for $\|g_j^w - g_j^{w'}\|_\infty = \|b_j^w - b_j^{w'}\|_\infty$ small enough according to the first part of (b).

\item[(c)] We add zero and get
\[ \left| \rho_{b_j^w}(y_j^w) - \rho_{b_j^{w'}}(y_j^{w'}\right| \leq \left| \rho_{b_j^w}(y_j^w) - \rho_{b_j^w}(y_j^{w'})\right| + \left| \rho_{b_j^w}(y_j^{w'}) - \rho_{b_j^{w'}}(y_j^{w'})\right|.\]
For arbitrary $\epsilon>0$ and $|y_j^w - y_j^{w'}|<\delta$, $\delta>0$ appropriate, the first summand can be chosen $\leq\epsilon$ as evaluation of a continuous function is a continuous mapping. The same holds trivially true for the second summand for $\| \rho_{b_j^w}-\rho_{b_j^{w'}}\|_\infty< \epsilon$.
\end{itemize}

We now turn to the statement $(2)$. From Lemma \ref{bound_invariant_density} we know that there exists a constant $L^*=L^*(C,A,\gamma,\sigma)$ such that for every drift function $b\in\Sigma(C,A,\gamma,\sigma)$ we have $\|\rho_b\|_\infty\leq L^*$. Set
\[ I := \left[\frac14 \min_{-A\leq x\leq A}\rho_{b_0}(x) , L^*\right] =: [L_*, L^*]. \]
Now we want to show that for large enough $T$ this interval fulfills $f(I)\subset I$. Choose $w\in [L_*,L^*]$. If $T$ is large enough to ensure
\[ L (h_T^w)^\beta = c_* \left(\frac{\log T}{Tw}\right)^\frac{\beta}{2\beta+1} \leq  c_* \left(\frac{\log T}{TL_*}\right)^\frac{\beta}{2\beta+1}  \leq \frac{C}{2}\]
we know by Lemma \ref{lemma_cond_1} that $b_j^w\in\Sigma(C,A,\gamma,\sigma)$ and hence 
\[ \rho_{b_j^w}(y_j^w) \leq \| \rho_{b_j^w}\|_\infty \leq L^*.\]
For the lower bound first note that due to $\|K\|_\infty\leq 1$
\[ \left| \int_0^x g_j^w(y) dy\right| \leq \int_0^{|x|} g_j^w(y) dy \leq \int_{-A}^A g_j^w(y) dy \leq 2A L(h_T^w)^\beta \leq 2AL (h_T^{L_*})^\beta.\]
So we may choose $T\geq T_0$ large enough such that $2AL(h_T^{L_*})^\beta\leq \min\left\{ \frac{\sigma^2\log 2}{2}, \log 2\right\}$. Then we have for the constant 
\begin{align*}
C_{b_j^w,\sigma} &= \sigma^{-2}\int_\R \exp\left( \int_0^y 2\sigma^{-2}b_0(u) du \right)\exp\left( \int_0^y 2\sigma^{-2} g_j^w(u) du \right) dy\\
&\leq  \exp\left(4\sigma^{-2} AL(h_T^{L_*})^\beta\right) \int_\R \sigma^{-2}\exp\left( \int_0^y 2\sigma^{-2} b_0(u) du \right) dy\\
&\leq 2 C_{b_0,\sigma}
\end{align*}
or equivalently, $(\sigma^2 C_{b_j^w, \sigma})^{-1} \geq \frac12 (\sigma^2 C_{b_0,\sigma})^{-1}$. By the same argument and the same choice of $T\geq T_0$ we get
\begin{align*}
\exp\left( \int_0^{y_j^w} b_j^w(y) dy\right) &= \exp\left( \int_0^{y_j^w} b_0(x) dx\right)\exp\left( \int_0^{y_j^w} g_j^w(y) dy\right)\\
& \geq \exp\left( \int_0^{y_j^w} b_0(x) dx\right) \exp\left(-\log 2\right).
\end{align*} 
Combining this, we get
\begin{align*}
\rho_{b_j^w}(y_j^w) &= \frac{1}{C_{b_j^w, \sigma}\sigma^2} \exp\left( \int_0^{y_j^w} 2\sigma^{-2} b_j^w(u) du \right)\\
&\hspace{1cm}\geq \frac12 \frac{1}{C_{b_0,\sigma}} \exp\left( \int_0^{y_j^w} b_0(x) dx\right)\frac12= \frac14 \rho_{b_0}(y_j^w) \geq L_*.
\end{align*}  
\end{proof}





\begin{lemma}\label{lemma_E_absvalue}
Let $Z_1,\dots, Z_m$ be stricly positive, uncorrelated random variables with $\E[Z_i]=1$ for all $1\leq i\leq m$. Then for all $\epsilon>0$ and $0<\gamma\leq 1$ we have
\begin{align*}
\E\left[\left| \frac1m \sum_{i=1}^m Z_i - 1\right|\right] &\leq \sqrt{\epsilon} + \left( 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{i=1}^m \E[ Z_i^{1+\gamma}] \right)^\frac12 + 2\epsilon^{-\gamma}m^{-(1+\gamma)}\sum_{i=1}^m \E[ Z_i^{1+\gamma}].
\end{align*} 
\end{lemma}
\begin{proof}
First of all, we note that from $\E[Z_i]=0$ and the uncorrelatedness we get $\E[Z_i Z_j] =1$ for $i\neq j$.\\
With $1=\E[Z_i] = \E[ Z_i 1_{\{Z_i\leq \epsilon m\}} + Z_i 1_{\{Z_i > \epsilon m\}}] = \E[Z_i 1_{\{Z_i \leq \epsilon m\}}] + \E[Z_i 1_{\{Z_i > \epsilon m\}}]$ and the fact that $Z_i\geq 0$ we get
\begin{align*}
&\E\left[\left| \frac1m \sum_{i=1}^m Z_i -1\right|\right] \\
&\hspace{0.5cm}= \E\left[ \left| \frac1m\sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right) + \frac1m\sum_{i=1}^m \left( Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right) \right|\right] \\
&\hspace{0.5cm}\leq \frac1m\E\left[ \left| \sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right)\right|\right] + \frac1m\E\left[\left|\sum_{i=1}^m \left( Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right) \right|\right]\\
&\hspace{0.5cm}\leq \frac1m\E\left[ \left| \sum_{i=1}^m \left( Z_i1_{\{Z_i \leq \epsilon m\}} - \E[ Z_i 1_{\{Z_i \leq  \epsilon m\}}]\right)\right|^2\right]^\frac12 +\frac1m \E\left[\sum_{i=1}^m \left| Z_i1_{\{Z_i > \epsilon m\}} - \E[Z_i 1_{\{Z_i > \epsilon m\}}]\right| \right]\\
&\hspace{0.5cm}\leq \frac1m \textrm{Var}\left( \sum_{i=1}^m  Z_i1_{\{Z_i \leq \epsilon m\}}\right)^\frac12 + \frac1m \E\left[ \sum_{i=1}^m \left| Z_i 1_{\{ Z_i>\epsilon m\}} \right| +  \left|\E[Z_i 1_{\{Z_i > \epsilon m\}}] \right| \right]\\
&\hspace{0.5cm}\leq \frac1m \textrm{Var}\left( \sum_{i=1}^m  Z_i1_{\{Z_i \leq \epsilon m\}}\right)^\frac12 + \frac2m \sum_{i=1}^m \E\left[ Z_i 1_{\{ Z_i>\epsilon m\}}\right]\\
&\hspace{0.5cm}= \frac1m \left( \sum_{i=1}^m \textrm{Var}\left( Z_i 1_{\{ Z_i\leq \epsilon m\}}\right) + \sum_{i,j=1}^m \textrm{Cov}\left(  Z_i 1_{\{ Z_i\leq \epsilon m\}},  Z_j 1_{\{ Z_j\leq \epsilon m\}}\right)\right)^\frac12 + \frac2m \sum_{i=1}^m \E\left[ Z_i 1_{\{ Z_i>\epsilon m\}}\right]\\
&\hspace{0.5cm} =: \frac1m\left( A_1 + A_2\right)^\frac12 + A_3.
\end{align*}
Now we treat eacht term $A_i$ seperately. As a variance the term $A_1+A_2$ is positive and it suffices to find an upper bound for it without taking the absolute value. In particular we may drop negative summands without double-checking that they are in absolute value smaller than the remaining positive ones. For the first one a bound is straightforward as
\[ A_1 \leq \sum_{i=1}^m \E\left[ Z_i^2 1_{\{ Z_i\leq \epsilon m\}}\right] \leq \epsilon m \sum_{i=1}^m \E\left[ Z_i1_{\{ Z_i\leq \epsilon m\}}\right] \leq \epsilon m\sum_{i=1}^m \E[Z_i] = \epsilon m^2.\]
For the second term we first note that 
\[1_{\{ Z_i\leq \epsilon m\}} = 1-1_{\{ Z_i> \epsilon m\}}\]
and similarly
\begin{align*}
1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}} &= 1- 1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j > \epsilon m\}} - 1_{\{ Z_i> \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}}-1_{\{ Z_i> \epsilon m\}}1_{\{ Z_j> \epsilon m\}}\\
&=: 1- A_{ij}.
\end{align*} 
Now we can start with
\begin{align*}
A_2 &= \sum_{i,j=1}^m \E\left[ Z_iZ_j 1_{\{ Z_i\leq \epsilon m\}}1_{\{ Z_j\leq \epsilon m\}}\right]  - \E\left[Z_i1_{\{ Z_i\leq \epsilon m\}}\right]\E\left[Z_j1_{\{ Z_j\leq \epsilon m\}}\right] \\
&= \sum_{i,j=1}^m \E\left[ Z_iZ_j ( 1- A_{ij})\right] - \E\left[ Z_i (1-1_{\{ Z_i>\epsilon m\}})\right]\E\left[ Z_j (1-1_{\{ Z_j> \epsilon m\}})\right]\\
&= -\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] + \sum_{i,j=1}^m \E[Z_iZ_j] - \left( \E[Z_i] - \E[Z_i1_{\{ Z_i>\epsilon m\}}]\right)\left(\E[Z_j] - \E[Z_j1_{\{ Z_j> \epsilon m\}}]\right)\\
&=-\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] + \sum_{i,j=1}^m 1- \left( 1 - \E[Z_i1_{\{ Z_i>\epsilon m\}}]\right)\left(1- \E[Z_j1_{\{ Z_j> \epsilon m\}}]\right)\\
&= -\sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right]\\
&\hspace{1cm} + \sum_{i,j=1}^m  1- \left( 1- \E[Z_i1_{\{ Z_i>\epsilon m\}}]-\E[Z_j1_{\{ Z_j>\epsilon m\}}] + \E[Z_i1_{\{ Z_i>\epsilon m\}}]\E[Z_j1_{\{ Z_j>\epsilon m\}}]\right)\\
&= - \sum_{i,j=1}^m \E\left[Z_iZ_j A_{ij}\right] +\E[Z_i1_{\{ Z_i>\epsilon m\}}]\E[Z_j1_{\{ Z_j>\epsilon m\}}] + \sum_{i,j=1}^m  \E[Z_i1_{\{ Z_i>\epsilon m\}}]+\E[Z_j1_{\{ Z_j>\epsilon m\}}] 
\end{align*}
As $Z_i\geq 0$ and $A_{i,j}\geq 0$ the first of the summands is negative and we get
\[ A_2 \leq \sum_{i,j=1}^m  \E[Z_i1_{\{ Z_i>\epsilon m\}}]+\E[Z_j1_{\{ Z_j>\epsilon m\}}] = 2m\sum_{i=1}^m \E[Z_i1_{\{ Z_i>\epsilon m\}}]. \]
Now we use the indicator in the last remaining expectation to estimate for $0<\gamma\leq 1$
\[ \E[Z_i1_{\{ Z_i>\epsilon m\}}]j \leq (\epsilon m)^{-\gamma} \E\left[Z_i^{1+\gamma}1_{\{ Z_i>\epsilon m\}}\right]\leq  (\epsilon m)^{-\gamma} \E\left[Z_i^{1+\gamma}\right]. \]
Altogether we arrive at 
\[ A_2 \leq 2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right].\]
Using $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for $a,b\geq 0$ we finally get
\begin{align*}
\frac1m(A_1 + A_2)^\frac12 &\leq \frac1m\left( \epsilon m^2 + 2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12\\
&\leq \frac1m\left( \sqrt{\epsilon} m + \left(2\epsilon^{-\gamma} m^{1-\gamma} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12 \right)\\
&= \sqrt{\epsilon} + \left( 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{i=1}^m\E\left[Z_i^{1+\gamma}\right]\right)^\frac12
\end{align*}
which are exactly the first to summands in the assertion of the lemma. We close the proof by the estimation of $A_3$. But here we simply use the same trick with $0<\gamma\leq 1$ and directly get
\[ A_3 \leq 2\epsilon^{-\gamma} m^{-(1+\gamma)} \sum_{k=1}^m \E\left[Z_i^{1+\gamma}\right].\]
\end{proof}





Within the proof of the sharp lower bound, we will make use of the following:

\begin{proposition}\label{moments_local-invariant}
Let $X$ be a diffusion with $b\in\Sigma(C,A,\gamma,\sigma)$. Then there exist constants $c_1, c_2>0$m such that, for any $p, T\geq 1$, 
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} \left(\E_{b}\left[ \left\| \frac1T L_T(X) - \rho_b\right\|_\infty^p\right]\right)^\frac1p \leq c_1\left( \frac{p}{T} + \frac{1}{\sqrt{T}}\left( 1+ \sqrt{p} + \sqrt{\log T}\right) + Te^{-c_2T}\right).\]
\end{proposition}
\begin{proof}
See Willems/Strauch, Lemma 43 in Dissertation....check for the paper!!!
\end{proof}




\begin{proof}[Proof of the sharp lower bound]
We first begin building our hypothesis. $b_0$ and $h_T^w$ are chosen as above and we proceed inductively:
\begin{itemize}
\item In the first step we set $y_1^w := -A + h_T^w$. Then by Lemma \ref{lemma_fixed_point} there exists $w_1>0$ such that $\rho_{b_j^{w_1}}(y_j^{w_1}) = w_1$ and we set $b_1 := b_1^{w_1}$, $y_1:=y_1^{w_1}$. Clearly, the support of $b_1-b_0$ is given by $[-A, -A + 2h_T^{w_1}] = [y_j-h_T^{w_1}, y_j+h_T^{w_1}]$.
\item If $b_j$ is constructed with $y_j$ we put $y_{j+1}^w := y_j + h_T^{w_j}+ h_T^w$. Again Lemma \ref{lemma_fixed_point} ensures existance of $w_{j+1}>0$ with $\rho_{b_{j+1}^{w_{j+1}}}(y_{j+1}^{w_{j+1}}) = w_{j+1}$ and we set $b_{j+1} := b_{j+1}^{w_{j+1}}, y_{j+1}:= y_{j+1}^{w_{j+1}}$. The support of $b_{j+1}-b_0$ is given by $[y_j + h_T^{w_j}, y_j + h_T^{w_j}+2h_T^{w_{j+1}}] = [y_{j+1}- h_T^{w_{j+1}}, y_{j+1}+h_T^{w_{j+1}}]$ and hence is disjoint of all $b_j-b_0$ constructed before.
\item The construction ends when for the first time the right endpoint of the newly constructed interval $[y_N - h_T^{w_N}, y_N+h_T^{w_N}]$ is greater than $A$.
\end{itemize}
From Lemma \ref{bound_invariant_density} we get a constant $L^* =L^*(C,A.\gamma,\sigma)$ such that every drift $b\in\Sigma(C,A,\gamma,\sigma)$ admits an invariant density $\rho_b$ with $\|\rho_b\|_\infty\leq L^*$. In particular, we have $w_j\leq L^*$ for all $j=1,\dots, N$. Next, we specify $N$. From the construction of the hypothesis we have $2A \geq \sum_{j=1}^N 2h_T^{w_j}$. Hence, 
\begin{align*}
A \geq \sum_{j=1}^N h_T^{w_j} &= \sum_{j=1}^N \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{Tw_j}\right)^{\frac{1}{2\beta +1}} \\
&= \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{T}\right)^{\frac{1}{2\beta +1}} \sum_{j=1}^N \left(\frac{1}{w_j}\right)^{\frac{1}{2\beta +1}}\\
&\geq \left(\frac{c^*}{L}\right)^\frac{1}{\beta}\left(\frac{\log T}{T}\right)^{\frac{1}{2\beta +1}} N \left(\frac{1}{L^*}\right)^{\frac{1}{2\beta+1}}.
\end{align*}
This can be transformed into an inequality of the form $N\leq\dots$ and from our construction algorithm we know that $N$ is the largest integer fullfilling this inequality, thus
\[ N =N_T = \left\lfloor \frac{A}{(L^*)^{\frac{1}{2\beta+1}}} \left(\frac{L}{c^*}\right)^\frac{1}{\beta}\left(\frac{T}{\log T}\right)^{\frac{1}{2\beta +1}} \right\rfloor.\]
Before we proceed, we fix the notation 
\[ A_{T,j} := (1-\epsilon_T) L\left( h_T^{w_j}\right)^\beta\quad \textrm{ and }\quad K_j(\cdot) := K_{y_j, h_T^{w_j}}(\cdot)\]
so we can write $b_j = b_0 + A_{T,j} K_j$.\\


Now, let $\phi$ be test with $\E_{b_0}[\phi]\leq\alpha$. Then we have
\begin{align*}
\inf_{b\in\Sigma(\beta, L): \|(b-b_0)\phi_b^{\beta/(2\beta+1)}\|_\infty\geq (1-\epsilon_T)c_* \delta_T} \E_b[\phi] - \alpha &\leq \min_{1\leq k\leq N} \E_{b_k}[\phi] - \E_{b_0}[\phi]\\
&\leq \E_{b_0}\left[ \left(\frac1N \sum_{k=1}^N \frac{d\Pr_{b_k}}{d\Pr_{b_0}}(X) - 1\right) \phi\right]\\
&\leq  \E_{b_0}\left[ \left| \frac1N \sum_{k=1}^N \frac{d\Pr_{b_k}}{d\Pr_{b_0}}(X) - 1\right|\right].
\end{align*}
For ease of notation we introduce
\[ Z_k := \frac{d\Pr_{b_k}}{d\Pr_{b_0}} (X) \]
and note that $\E_{b_0}[Z_k] = 1$ for each $1\leq k\leq N$. Furthermore, the $Z_k$ are pairwise uncorrelated. To see this, we calculate $\E_{b_0}[Z_iZ_j]$ for $i\neq j$. In this case we have $K_i(X_s) K_j(X_s) =0$ as the supports of $K_i$ and $K_j$ are disjoint which will be used in the third step:
\begin{align*}
\E_{b_0}[Z_i Z_j] &= \E_{b_0}\left[ \exp\left( \int_0^T A_{T,i} K^i(X_s) dW_s - \frac12\int_0^T A_{T,i}^2 K_i^2(X_s)^2 ds\right) \right.\\
&\hspace{1.5cm} \cdot\left. \exp\left( \int_0^T A_{T,j}K_j(X_s) dW_s - \frac12\int_0^T A_{T,j}^2 K_j(X_s)^2 ds\right)\right]\\
&= \E_{b_0}\left[ \exp\left( \int_0^T \left(A_{T_i}K_i(X_s) + A_{T_j}K_j(X_s)\right) dW_s \right.\right.\\
&\hspace{2.5cm}  \left.\left. - \frac12\int_0^T \left( A_{T,i}^2 K_i(X_s)^2 + A_{T,j}^2 K_j(X_s)^2 \right) ds\right)\right]\\
&= \E_{b_0}\left[ \exp\left( \int_0^T \left(A_{T_i}K_i(X_s) + A_{T_j}K_j(X_s)\right) dW_s \right.\right.\\
&\hspace{2.5cm}  \left.\left. - \frac12\int_0^T \left( A_{T,i} K_i(X_s) + A_{T,j} K_j(X_s) \right)^2 ds\right)\right].
\end{align*}
But this last expression is again a Girsanov-density and hence its expectation equals one. Consequently, 
\[ \textrm{Cov}(Z_i, Z_j) = \E_{b_0}[Z_i Z_j] - \E_{b_0}[Z_i]\E_{b_0}[Z_j] = 1-1^2 =0.\]
We thus may apply Lemma \ref{lemma_E_absvalue} and it remains to show that
\[ N^{-(1+\gamma)} \sum_{k=1}^N \E_{b_0}\left[ Z_k^{1+\gamma}\right] \rightarrow 0\]
for a suitable choice of $0<\gamma\leq 1$ and asymptotic $T\to\infty$. In a first step, we investigate one single summand $\E_{b_0}[ Z_k^{1+\gamma}]$. We have
\[ \E_{b_0}[ Z_k^{1+\gamma}] = \E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k} K_k(X_s) dW_s - \frac{1+\gamma}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right)\right].\]
We now split the second integral in the exponen and get with the occupation times formula in the second step
\begin{align*}
&-\frac{1+\gamma}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\\
&\hspace{0.5cm}= -\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac12 ((1+\gamma)^2 - 1-\gamma) \int_0^T A_{T,k}^2 K_k(X_s)^2 ds\\
&\hspace{0.5cm}=-\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\frac1T L_T^z(X) dz\\
&\hspace{0.5cm} = -\frac{(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\rho_{b_0}(y) dz \\
&\hspace{1.5cm} + \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz \\
&\hspace{1.5cm}+ \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right)dz
\end{align*}
Inserting into the formula for $\E_{b_0}[Z_k^{1+\gamma}]$ and pulling the non-random factors out of the integral this leads to
\begin{align*}
\E_{b_0}[Z_k^{1+\gamma}] &= A_1\cdot A_2 \cdot \E\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k} K_k(X_s) dW_s - \frac{(1+\gamma)^2}{2} \int_0^T A_{T,k}^2 K_k(X_s)^2 ds \right.\right.\\
&\hspace{3cm}\left.\left.+ \frac12\gamma(1+\gamma)T\int_0^T A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz\right)\right]
\end{align*}
where 
\begin{align*}
A_1 &:= \exp\left( \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2\rho_{b_0}(y) dz\right)\quad \textrm{ and }\\
A_2 &:=\exp\left(  \frac{T}{2} \gamma(1+\gamma)\int_\R A_{T,k}^2 K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right)dz\right).
\end{align*}
To further evaluate the term within the expectation we again add a suitable zero. Therefore, pick $p=p_T>1$ that will be specified later and the corresponding $q=q_T$ with $\frac1p+\frac1q =1$. Then we write the expectation in the following form
\begin{align*}
&\E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right.\\
&\hspace{1cm}  \cdot\exp\left( \frac12 (p-1)(1+\gamma)^2 \int_0^T A_{T,k}^2 K_k(X_s)^2 ds \right.\\
&\hspace{2.5cm} \left.\left. + \frac12\gamma(1+\gamma)T \int_\R A_{T,k}^2 K_k(z)^2 \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right) dz\right)\right]\\
&= \E_{b_0}\left[ \exp\left( (1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right.\\
&\hspace{1.5cm} \cdot \exp\left( \frac12 (p-1) (1+\gamma)^2 T \int_\R A_{T,k}^2 K_k(z)^2 \rho_{b_0}(y) dz \right.\\
&\hspace{2cm} \left. \left. +\left( \frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) T \int_\R A_{T,k}^2 K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]
\end{align*}
where we used the occupation times formula again in the second step and split $\frac1T L_T^z(X) = \rho_{b_0}(z) + \left(\frac1T L_T^z(X) - \rho_{b_0}(z)\right)$. Pulling out the non-random factor and applying Hölder's inequality yields
\[ \E_{b_0}[Z_k^{1+\gamma}]  = A_1\cdot A_2\cdot A_3\cdot A_4\cdot A_5,\]
where
\begin{align*}
A_3 &:= \E_{b_0}\left[ \exp\left( p(1+\gamma)\int_0^T A_{T,k}K_k(X_s) dW_s - \frac{p^2(1+\gamma)^2}{2}\int_0^T A_{T,k}^2 K_k(X_s)^2 ds\right) \right]^\frac1p, \\
A_4&:= \exp\left( \frac12 (p-1) (1+\gamma)^2 T \int_\R A_{T,k}^2 K_k(z)^2 \rho_{b_0}(y) dz \right),\quad \textrm{ and } \\
A_5&:= \E_{b_0}\left[ \exp\left( q\left(\frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) T \int_\R A_{T,k}^2 K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]^\frac1q
\end{align*}
The most interesting term will be $A_1$ and we consider it later within the sum (remember that we still just treat $Z_k^{1+\gamma}$ for some fixed $k$ here). The terms $A_2,\dots, A_5$ on the other side will turn out to be bound constants:
\begin{itemize}
\item[$A_2:$] According to Lemma \ref{bound_invariant_density} the invariant density is Lipschitz with constant $L^*$. Hence, on the support of $K_k$ we have $|\rho_{b_0}(y)-\rho_{b_0}(z)|\leq 2L^* h_T^{w_k}$. Hence,
\begin{align*}
A_2 &= \exp\left( \frac12\gamma(1+\gamma)T A_{T,k}^2 \int_\R K_k(z)^2 \left(\rho_{b_0}(z) - \rho_{b_0}(y)\right) dz\right)\\
&\leq  \exp\left( \frac12\gamma(1+\gamma)T A_{T,k}^2 \int_\R K_k(z)^2 \left|\rho_{b_0}(z) - \rho_{b_0}(y)\right| dz\right)\\
&\leq \exp\left( \frac12\gamma(1+\gamma) T A_{T,k}^2 2L^*(h_T^{w_k})^2 \|K\|_{L^2}^2\right)\\
&= \exp\left( \gamma(1+\gamma) \|K\|_{L^2}^2 L^* L^2 (1-\epsilon_T)^2 T (h_T^{w_k})^{2\beta+2}\right)\\
&= \exp\left(\gamma(1+\gamma) \|K\|_{L^2}^2L^* L^2 (1-\epsilon_T)^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} Th_T^{w_k} \frac{\log T}{T \rho_{b_k(y_k)}}\right).
\end{align*}
This term converges to one, as the exponent goes to zero due to the fact that $(1-\epsilon_T)\rightarrow 1$ and $h_T^{w_k} \log T\rightarrow 0$ as 
\[ h_T^{w_k} \log T \asymp \left( \frac{\log T}{T}\right)^{\frac{1}{2\beta+1}} \log T = T^{-\frac{1}{2\beta+1}} \left( \log T\right)^{\frac{2\beta +2}{2\beta +1}}.\]
\item[$A_3:$] For every $T$ the term $A_3$ is the expectation of a Girsanov-density and hence by martingale arguments it equals one, i.e. $A_3 =1$.
\item[$A_4:$] Here we use again Lemma $\ref{bound_invariant_density}$ to get $\|\rho_{b_0}\|_\infty\leq L^*$. Then we estimate
\begin{align*}
A_4 &= \exp\left( \frac12 (p-1) (1+\gamma)^2 T A_{T,k}^2 \int_\R K_k(z)^2 \rho_{b_0}(z) dz\right)\\
&\leq \exp\left( \frac12 (p-1)(1+\gamma)^2 L^* \|K\|_{L^2}^2 T A_{T,k}^2 h_T^{w_k}\right)\\
&= \exp\left( \frac12 (1+\gamma)^2 L^* \|K\|_{L^2}^2 L^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} \rho_{b_0}(y_k)^{-1} T(p-1)\frac{\log T}{T}\right).
\end{align*}
The last exponent converges to zero if $(p-1)\log T\rightarrow 0$ which is for example true, if we set 
\[ p= p_T = 1+ T^{-\frac14}.\]
Especially, $p>1$ which is import as we applied the Hölder inequality for it. Of course, many other choices of $p$ would do the same job here, but will see in the next step, that $p$ mustn't be too close to one and our choice perfectly applies for both $A_4$ and $A_5$.
\item[$A_5:$] In this case we have
\begin{align*}
A_5 &= \E_{b_0}\left[ \exp\left( q\left(\frac12 (p-1)(1+\gamma)^2 + \frac12\gamma(1+\gamma)\right) TA_{T,k}^2 \right. \right. \\
&\hspace{1.5cm} \left. \left. \cdot \int_\R  K_k(z)^2\left(\frac1T L_T^z(X)-\rho_{b_0}(z)\right) dz\right)\right]^\frac1q\\
&\leq \E_{b_0}\left[ \exp\left( \frac12(1+\gamma) q ((p-1)(1+\gamma) + \gamma) TA_{T,k}^2 h_T^{w_k} \|K\|_{L^2}^2 \left\|\frac1T L_T(X) - \rho_{b_0}\right\|_{\infty}\right) \right]^\frac1q \\
&= \E_{b_0}\left[ \exp\left( \tilde{c} c_p \log T \left\|\frac1T L_T(X) - \rho_{b_0}\right\|_{\infty}\right)\right]^\frac1q
\end{align*}
with
\begin{align*}
\tilde{c} &:= \frac12(1+\gamma)\|K\|_{L^2}^2 L^2\left(\frac{c_*}{L}\right)^\frac{1}{2\beta +1}\rho_{b_0}(y_k)^{-1}, \\
c_{p}&:= q((p-1)(1+\gamma) + \gamma).
\end{align*}
Note in the latter case that $q$ is determined by $p$ as its conjugate. By a series expanison of $\exp$ and dominated convergence \textbf{check applicability!!} as well as an application of Proposition \ref{moments_local-invariant} we get for the expectation
\begin{align*}
&\E_{b_0}\left[ \exp\left( \tilde{c} c_p \log T \left\|\frac1T L_T^z(X) - \rho_{b_0}(z)\right\|_{\infty}\right)\right]\\
&\hspace{1cm} =\E_{b_0}\left[ \sum_{k=0}^\infty\frac{(\tilde{c}c_p \log T\|\frac1T L_T - \rho_{b_0}\|_\infty )^k}{k!}\right]\\
&\hspace{1cm} = \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} \E_{b_0}\left[\left\|\frac1T L_T(X) - \rho_{b_0}\right\|_\infty^k\right]\\
&\hspace{1cm}\leq \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} c_1^k\left( \frac{k}{T} + \frac{1}{\sqrt{T}}\left( 1+\sqrt{k} + \sqrt{\log T}\right) + Te^{-c_2T}\right)^k \\
&\hspace{1cm}\leq \sum_{k=0}^\infty \frac{(\tilde{c}c_p\log T)^k}{k!} c_1^k k^k \left( \frac1T + \frac{1}{\sqrt{T}}\left( 2+\sqrt{\log T}\right) + Te^{-c_2T}\right)^k\\
&\hspace{1cm} = \sum_{k=0}^\infty\frac{k^k}{k!} (\tilde{c}c_1)^k (c_pB_T)^k 
\end{align*}
with
\[ B_T = \frac{\log T}{T} + \frac{\log T}{\sqrt{T}} \left( 2+\sqrt{\log T}\right) + T\log T e^{-c_2T}.\]
By Stirling's formula we get for $k\geq k_0$ that 
\[ \frac{k^k}{k!} = \frac{k^k}{\sqrt{2\pi k} k^k e^{-k}} = \frac{e^k}{\sqrt{2\pi k}} \leq e^k.\]
Moreover, we remember $p=p_T= 1+T^{-\frac14}$ from the term $A_4$. This choice gives $q = \frac{p}{p-1} = 1+ T^{\frac14}$ and 
\[c_p = (1+T^{-\frac14})(1+\gamma) + (1+T^{\frac14})\gamma \leq 2(1+\gamma)(1+T^\frac14).\]
Thus there exists a constant $C_{k_0}\geq 1$ such that after inserting all this we end up with
\begin{align*}
\sum_{k=0}^\infty\frac{k^k}{k!} (\tilde{c}c_1)^k (c_pB_T)^k& \leq C_{k_0} \sum_{k=0}^\infty (\tilde{c}c_1 e)^k\left( 2(1+\gamma)(1+T^\frac14) B_T\right)^k\\
&= C_{k_0} \sum_{k=0}^\infty (2(1+\gamma)\tilde{c}c_1 e)^k C_T^k,
\end{align*}
where
\[ C_T := (1+T^\frac14)B_T = \frac{\log T(1+T^\frac14)}{T} + \frac{\log T (1+T^\frac14)}{\sqrt{T}}\left( 2+\sqrt{\log T}\right) + T (1+T^\frac14) \log T e^{-c_2 T}.\]
The important feature now is that $C_T\rightarrow 0 $ for $T\to\infty$ and we have shown so far
\[ A_5 \leq \left( C_{k_0} \sum_{k=0}^\infty (2(1+\gamma)\tilde{c}c_1 e)^k C_T^k\right)^{\frac{1}{1+T^\frac14}}.\]
As the term within the bracket is greater than one, we can upper bound the whole expression by forgetting the exponent which is stricly smaller than one. Now it is time to choose $T$ large enougt such that $C_T\leq 2(1+\gamma)\tilde{c}c_1 e$. Then we have
\begin{align*}
A_5\leq C_{k_0}\sum_{k=0}^\infty \left( 2(1+\gamma)\tilde{c}c_1 eC_T\right)^k = \frac{C_{k_0}}{1-2(1+\gamma)\tilde{c}c_1 e C_T} \stackrel{T\to\infty}{\longrightarrow} C_{k_0}.
\end{align*}
\end{itemize}
Summing up, we have shown so far, that there exists a constant $C>1$ not depending on $k$ such that
\[ \E_{b_0}\left[ Z_k^{1+\gamma}\right]\leq C A_1 = C\exp\left( \frac{T}{2}\gamma(1+\gamma) A_{T,k}^2 \rho_{b_0}(y_k) \int_\R K_k(z)^2 dz\right).\] 
Next, we analyse the deterministic exponent and plug in the definition of $A_{T,k}$ and $K_k$. This yields
\begin{align*}
&\frac12\gamma(1+\gamma)\rho_{b_0}(y) T A_{T,k}^2 \int_\R K_k(z)^2 dz \\
&\hspace{1cm}  = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) T A_{T,k}^2 h_T^{w_k} \|K\|_{L^2}^2\\
&\hspace{1cm} = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) \|K\|_{L^2}^2 L^2 (1-\epsilon_T)^2 T (h_T^{w_k})^{2\beta+1}\\
&\hspace{1cm} = \frac12\gamma(1+\gamma)\rho_{b_0}(y_k) \|K\|_{L^2}^2 L^2 (1-\epsilon_T)^2 \left(\frac{c_*}{L}\right)^{\frac{2\beta+1}{\beta}} T\frac{\log T}{T\rho_{b_k}(y_k)}\\
&\hspace{1cm} =\frac12\gamma(1+\gamma)\|K\|_{L^2}^2 L^{2-\frac{2\beta+1}{\beta}} \frac{2L^{\frac{1}{\beta}}}{(2\beta+1)\|K\|_{L^2}^2} \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)} (1-\epsilon_T)^2 \log T\\
&\hspace{1cm}= \gamma(1+\gamma) \frac{1}{2\beta+1} \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}  (1-\epsilon_T)^2 \log T.
\end{align*}
It remains to show that the fraction of the two density is close enough to one. Thins also get easier, if we can express its order in $T$ without dependence on $k$. We have
\[ \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}  = \frac{C_{b_k,\sigma}}{C_{b_0,\sigma}} \exp\left(2\sigma^{-2}\int_0^{y_k} (b_0- b_k)(y) dy\right).\] 
By the same arguments as in step $(2)$ in the proof of Lemma  \ref{lemma_fixed_point} we see that the exponent is bounded by $c\left(\frac{\log T}{T}\right)^{\frac{\beta}{2\beta+1}}=ca_T$ for some constant $c>0$ and thus $\exp\left(2\sigma^{-2}\int_0^{y_k} (b_0- b_k)(y) dy\right) = 1+o_T(a_T)$. In the same proof we find
\[ C_{b_0,\sigma} \exp\left( -4\sigma^2 AL h_T^{w_k}\right) \leq C_{b_k,\sigma} \leq C_{b_0,\sigma} \exp\left( 4\sigma^2 AL h_T^{w_k}\right)\]
and with the same argument as above we see that $\frac{C_{b_k,\sigma}}{C_{b_0,\sigma}} = 1+o_T(a_T)$. We conclude
\[ \left|  \frac{\rho_{b_0}(y_k)}{\rho_{b_k}(y_k)}   -1\right| = o_T (a_T).\]
Now every ingredient is prepared and we finalize the proof. Remember that $N_T = c\left(\frac{T}{\log T}\right)^{\frac{1}{2\beta +1}}$ for some constant $c>0$. Then we have 
\begin{align*}
&N^{-(1+\gamma)} \sum_{k=1}^N \E_{b_0}\left[ Z_k^{1+\gamma}\right] \\
&\hspace{1cm}\leq CN^{-\gamma} \exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T))  (1-\epsilon_T)^2 \log T\right)\\
&\hspace{1cm}= C\exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T)) (1-\epsilon_T)^2 \log T - \gamma\log N\right)\\
&\hspace{1cm} = C\exp\left( \gamma(1+\gamma) \frac{1}{2\beta+1} (1+o_T(a_T))  (1-\epsilon_T)^2 \log T \right.\\
&\hspace{3.5cm} \left. - \gamma\frac{1}{2\beta+1}\left( \log T - \log\log T + \log c\right)\right)
\end{align*}
Set $\gamma=\epsilon_T$ we have $(\gamma(1+\gamma)(1-\epsilon_T)^2 = \epsilon_T - \epsilon_T^2 - \epsilon_T^3 + \epsilon_T^4$ and hence the last expression equals
\begin{align*}
C \exp\left(  \frac{1}{2\beta+1}\left( \left( o_T(a_T) - \epsilon_T^2 + o_T(\epsilon_T^3)\right)\log T - \epsilon_T\log\log T +\epsilon_T\log c\right)\right).
\end{align*}
Looking after the definition of $a_T$ we see that $o_T(a_T)\log T = o_T(1)$ and from the choice of $\epsilon_T$ we get $\epsilon_T^2\log T\rightarrow \infty$ and hence the whole expression tends to zero as the exponent converges to $-\infty$.
\end{proof}







\newpage

\subsubsection{Weak convergence}

We define $\mathcal{T}=  [-A,A]\times (0,1)$ and the processes $(Z_T(y,h))_{(y,h)\in\mathcal{T}}$ and $(Z(y,h))_{(y,h)\in\mathcal{T}}$ by
\[Z_T(y,h) := \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} \]
and
\[ Z(y,h) := \frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_{b_0}(z)} dW_z}{\| K_{y,h} \sqrt{\rho_{b_0}}\|_{L^2} }\]
where $(W_z)_{z\in [-A,A]}$ is a standard Brownian motion.\\
We remember
\[ \rho_T ((y,h), (y',h'))^2 = \frac1T \int_0^T \left( K_{y,h}(X_s) - K_{y',h'}(X_s)\right)^2 ds\]
and we define
\[ \rho((y,h), (y',h'))^2 = \int_\R \left( K_{y,h}(z) - K_{y',h'}(z)\right)^2 \rho_{b_0}(z) dz.\]



We will make use of the following result \textbf{(cite from anywhere, maybe Kutoyants)}.

\begin{proposition}\label{central_limit_diffusion}
Let $X$ be a diffusion with drift $b\in\Sigma(C,A,\gamma,\sigma)$. Then for any measurable function $f:\R\rightarrow\R$ with $\int_\R f(x) \rho_{b}(x) dx$ we have
\[ \frac{1}{\sqrt{T}}\int_0^T f(X_s) dW_s\ \stackrel{\mathcal{L}}{\Longrightarrow}\ \mathcal{N}\left( 0, \int_\R f(x)^2 \rho_b(x) dx\right).\]
\end{proposition}




Now the central result of this section is the following.

\begin{thm}\label{weak_conv}
We have weak convergence of our test statistic $T(X)$ under $\Pr_{b_0}$ against
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left( \| K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}^2\right) \right).\]
\end{thm}
\begin{proof}
\textbf{Convergence of finite-dimensional distributions.} \\
We choose $(y_k, h_k)\in\mathcal{T}$, $1\leq k\leq N$. To investigate the weak convergence of $(Z_T(y_1,h_1),\dots, Z_T(y_N, h_N))$ to $(Z(y_1,h_1),\dots, Z(y_N,h_N))$ we first use the Cramer-Wold device for the nominators. So let $t_1,\dots, t_n\in\R$ be arbitrary real numbers. Then we have by Proposition \ref{central_limit_diffusion}
\begin{align*}
&\sum_{k=1}^N t_k \frac{1}{\sqrt{T}} \int_0^T K_{y_k,h_k}(X_s) dW_s = \frac{1}{\sqrt{T}} \int_0^T \left( \sum_{k=1}^N t_k K_{y_k,h_k}(X_s)\right) dW_s\\
&\hspace{2cm} \stackrel{\mathcal{L}}{\Longrightarrow} \mathcal{N}\left( 0, \int_\R \left( \sum_{k=1}^N t_k K_{y_k,h_k}(x)\right)^2 \rho_{b_0}(x) dx\right).
\end{align*}
This distribution equals the distribution of
\[ \sum_{k=1}^N t_k \int_{-A}^A K_{y_k,h_k}(z) \sqrt{\rho_{b_0}(z)} dW_z = \int_{-A}^A \left( \sum_{k=1}^N t_k K_{y_k,h_k}(z) \right) \sqrt{\rho_{b_0}(z)} dW_z \]
which can be seen easily by Ito's isometry. Hence, 
\begin{align*}
&X_T := \left( \frac{1}{\sqrt{T}} \int_0^T  K_{y_1,h_1}(X_s) dW_s, \dots, \frac{1}{\sqrt{T}} \int_0^T  K_{y_N,h_N}(X_s) dW_s\right) \\
&\hspace{1cm} \stackrel{\mathcal{L}}{\Longrightarrow} \left( \int_{-A}^A K_{y_1,h_1}(z) \sqrt{\rho_{b_0}(z)} dW_z, \dots, \int_{-A}^A K_{y_N,h_N}(z) \sqrt{\rho_{b_0}(z)} dW_z \right)=:X.
\end{align*}
Furthermore, the vectors of the denominators converge almost surely, i.e.
\begin{align*}
&Y_T := \left( \sqrt{\frac1T \int_0^T K_{y_1,h_1}(X_s)^2 ds}, \dots, \sqrt{\frac1T \int_0^T K_{y_N,h_N}(X_s)^2 ds}\right)\\
&\hspace{2cm}\longrightarrow_{as} \left( \| K_{y_1,h_1}\sqrt{\rho_{b_0}}\|_{L^2},\dots, \| K_{y_N,h_N}\sqrt{\rho_{b_0}}\|_{L^2}\right) =:Y
\end{align*}
as for each $1\leq k\leq N$
\begin{align*}
&\left| \frac1T\int_0^T K_{y_k, h_k}(X_s)^2 ds - \| K_{y_k,h_k}\sqrt{\rho_{b_0}}\|_{L^2}^2\right| \\
&\hspace{1cm} = \left| \int_\R K_{y_k,h_k}(z)^2 \frac1T L_T^z(X) dz - \int_0^T K_{y_k,h_k}(z)^2 \rho_{b_0}(z) dz \right|\\
&\hspace{1cm}\leq \left\| \frac1T L_T(X) - \rho_{b_0}\right\| \int_\R K_{y_k,h_k}(z)^2 dz \rightarrow_{as} 0.
\end{align*}
By Slutzky's Lemma we then conclude $(X_T, Y_T)\stackrel{\mathcal{L}}{\Longrightarrow} (X,Y)$ and by the continuous mapping theorem we finally get
\[ (Z_T(y_1,h_1),\dots, Z_T(y_N, h_N))\stackrel{\mathcal{L}}{\Longrightarrow} (Z(y_1,h_1),\dots, Z(y_N, h_N)).\]


\textbf{Asymptotic stochastic equicontinuity}\\
By boundedness of the kernel function $K$ we see that
\[ \mathcal{F} := \left\{ \left( K_{y,h} - K_{y',h'}\right)2 \mid (y,h), (y',h')\in\mathcal{T}\right\} \]
is uniformely Glivenko-Cantelli. As $\E_{b_0}[\rho_T((y,h), (y',h'))^2] = \rho( (y,h), (y',h'))^2$ we thus get for any $\delta>0$
\[\lim_{T\to\infty} \Pr_{b_0}\left( \left\| \rho_T((y,h), (y',h'))^2 - \rho((y,h), (y',h'))^2 \right\|_{\mathcal{T}\times\mathcal{T}} >\delta\right) =0.\]
Let $\epsilon>0$. Then we have
\begin{align*}
&\Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon\right) \\
&\hspace{1cm} = \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon, \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} \leq \delta \right)\\
&\hspace{2cm} + \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon, \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} > \delta\right)\\
&\hspace{1cm} \leq\Pr_{b_0}\left( \sup_{\rho_T((y,h),(y',h'))\leq 2\delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon \right) + \Pr_{b_0}\left( \|\rho_T-\rho\|_{\mathcal{T}\times\mathcal{T}} > \delta\right).
\end{align*} 
The latter summand is $o_{\Pr_{b_0}}$ as seen before, and by the multiscale lemma \textbf{cite!!!} we get stochastic equicontinuity of the first summand with respect to the metric $\rho_T$. Consequently, 
\[\lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \sup_{\rho((y,h),(y',h'))\leq \delta}\left| Z_T(y,h) - Z_T(y',h')\right|>\epsilon\right) =0.\]

Putting together the convergence of the finite-dimensional distributions and the asymptotic stochastic equicontinuity we get convergence in distribution of the processes indexed by $\mathcal{T}$, i.e.
\[ \left( Z_T(y,h)\right)_{(y,h)\in\mathcal{T}} \stackrel{\mathcal{L}}{\Longrightarrow} \left( Z(y,h)\right)_{(y,h)\in\mathcal{T}}.\]

Now define 
\[ \tilde{T}_T(\delta, \delta') := \sup_{(y,h)\in\mathcal{T}:\ \delta < \|K_{y,h}\|_{L^2}\leq \delta'} \left(\frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} - C\left( \frac1T \int_0^T K_{y,h}(X_s)^2 ds\right) \right) \]
as well as
\[ S(\delta, \delta') := \sup_{(y,h)\in\mathcal{T}:\ \delta < \|K_{y,h}\|_{L^2}\leq \delta'} \left(\frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_{b_0}(z)} dW_z}{\| K_{y,h} \sqrt{\rho_{b_0}}\|_{L^2} } - C\left( \| K_{y,h}\sqrt{\rho_{b_0}} \|_{L^2}^2\right) \right).\]
Applying the same Glivenko-Cantelli argument as above to $\mathcal{F}' := \left\{ K_{y,h}\mid (y,h)\in\mathcal{T}\right\}$ instead of $\mathcal{F}$ we see by the continuous mapping theorem that
\[  \sup_{(y,h)\in\mathcal{T}}\left| C\left( \frac1T \int_0^T K_{y,h}(X_s)^2 ds\right)- C\left( \| K_{y,h}\sqrt{\rho_{b_0}} \|_{L^2}^2\right) \right| \longrightarrow_{\Pr_{b_0}} 0.\]
Together with the above established weak convergence of the processes it follows for any fixed $\delta\in (0,1]$ that
\[ \tilde{T}_T(\delta,1)\ \stackrel{\mathcal{L}}{\Longrightarrow}\ S(\delta,1).\]
Again by an application of the multiscale lemma \textbf{cite!!!} we see that
\[ \lim_{\delta\searrow 0} \limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,\delta) \geq \epsilon\right) =0.\]


\textbf{Investigation of $Z(y,h)$}\\
Next, we note that we can also apply the multiscale lemma to the process $Z$ instead of $Z_T$. The requirements are easily checked for $\tilde{Z}(y,h) := \int_{-A}^A K_{y,h}(z)\sqrt{\rho_{b_0}(z)} dW_z$ with semimetric $\rho$ and $\sigma(y,h) := \| K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}$ as $Z$ is Gaussian with
\[ \tilde{Z} \sim\mathcal{N}\left( 0, \|K_{y,h}\sqrt{\rho_{b_0}}\|_{L^2}^2\right).\]
First of all, this implies $S(0,1)<\infty$ almost surely and as above this gives for every $\epsilon>0$
\[ \lim_{\delta\searrow 0} \Pr_{b_0}\left( S(0,\delta)>\epsilon\right) =0.\]
For any $l\geq \lfloor \frac{1}{2A}\rfloor$ the random variables $Z_k := Z( \frac{k}{l}, \frac{1}{2l})$, $1\leq k\leq l$ are independent as the support of the functions $K_{\frac{k}{l}, \frac{1}{2l}}$ and $K_{\frac{k'}{l}, \frac{1}{2l}}$ is disjoint for $k\neq k'$. Moreover, they are standard Gaussians and hence their maximum is $(2\log l)^\frac12 + o_{\Pr}(1) = C(\frac{1}{l}) + o_{\Pr}(1)$ for $l\to\infty$. A simple substitution gives $\frac{c}{2l}=ch\leq \| K_{y,\frac{1}{2l}} \sqrt{\rho_{b_0}}\|_{L^2}^2 \leq Ch = \frac{C}{2l}$ for constants $c,C>0$ and $C$ may be chosen $\geq 1$. Then we have
\[ S(0,1) \geq \max_{1\leq k\leq l} Z_k - C\left(\frac{1}{l}\right) + o_l(1) \]
and conclude that $S(0,1)\geq 0$ almost surely, where we used that $C(\frac{C}{l}) = (2\log l + 2\log C)^\frac12 = (2\log l)^\frac12 + o_l(1)$.

\textbf{Conclusion}\\
Now the weak convergence of $\tilde{T}_T(\delta,1)$ to $S(\delta, 1)$ entail for $r>0$
\begin{align*}
&\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)>r\right) \\
&\hspace{1cm}\leq \lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(\delta,1)>r\right) +  \lim_{\delta\searrow 0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,\delta)>r\right)\\
&\hspace{1cm} \leq \lim_{\delta\searrow 0}\Pr_{b_0}\left( S(\delta,1)>r\right)\\
&\hspace{1cm} \leq \Pr_{b_0}\left( S(0,1)>r\right).
\end{align*}
Moreover, for arbitrary $\tilde{r}\in\R$ we have
\begin{align*}
\limsup_{T\to\infty}  \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq \tilde{r}\right) &\leq \inf_{\delta>0}\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(\delta,1)\leq \tilde{r}\right) \\
&\leq \inf_{\delta>0}\Pr_{b_0}\left( S(\delta,1)\leq \tilde{r}\right) \\
&= \Pr_{b_0}\left( S(0,1)\leq \tilde{r}\right)
\end{align*}
which in particular implies $\limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq \tilde{r}\right) =0$ for $\tilde{r}<0$. Noting that this last computation also includes for $r\geq 0$
\begin{align*}
\limsup_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r) &= 1- \limsup_{T\to\infty} \Pr_{b_0}\left( \tilde{T}_T(0,1)\leq  r\right)\\
&\geq 1- \Pr_{b_0}( S(0,1)\leq r) = \Pr_{b_0}( S(0,1)>r).
\end{align*} 
As both estimates for $\limsup_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r)$ may be repeated for $\liminf_{T\to\infty}$ we get $\lim_{T\to\infty} \Pr_{b_0}\left(\tilde{T}_T(0,1)\right)> r) = \Pr_{b_0}( S(0,1)>r)$ and the claim follows.
\end{proof}





\newpage

\subsubsection{Worst case for one-sided alternative}

We fix, $A,\gamma,\sigma>0$, $C\geq 1$ and set 
\[\mathcal{H}_{\leq} := \{ f\in \Sigma(C,A,\gamma,\sigma)\mid f\leq 0\textrm{ on } [-A,A]\}. \]

We want to show that an asymptotically worst case within this set of hypothesis is $f=0$ which is the reasonable expectation as it is the hypothesis closest to the alternative of functions being larger than zero anywhere within $[-A,A]$. So we remember 
\[ \mathcal{T} := (0,1]\times [-A+h, A-h] \]
and the test statistic
\[ T_b(X)  = \sup_{(y,h)\in\mathcal{T}} \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)\]
where
\[ \tilde{\Psi}_{y,h}^b(X) = \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} + \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
Clearly, the second summand is always negative for $b\in\mathcal{H}_{\leq}$ and vanishes for $b=0$, where the latter is understood as restricted to $[-A,A]$. Outside of this interval the drift clearly needs to deviate from zero in order to ensure ergodic properties of the solution or put differently, to ensure $b\in\Sigma(C,A,\gamma,\sigma)$. In this latter case we know that the invariant density $\rho_0=c$ is constant on $[-A, A]$ and hence the weak limit of the test statistic is given by
\[ \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C( \|cK_{y,h}\|_{L^2}^2)\right),\]
where
\[ Z(y,h) = \frac{\int_{-A}^A K_{y,h}(z) dW_z}{\|K_{y,h}\|_{L^2}}.\]


\begin{proposition}
For each $b\in\mathcal{H}_{\leq}$ and $r\in\R$  we have
\[ \lim_{T\to\infty} \Pr\left( T_b(X) > r\right) \leq \Pr\left( S>r\right),\]
where
\[ S := \sup_{(y,h)\in\mathcal{T}} \left( Z(y,h) - C\left(\|K_{y,h}\|_{L^2}^2\right) + C\left( (1\vee (L^*\wedge (2h)^{-1})^{-1}\right)\right).\]
\end{proposition}
\begin{proof}
Let $b\in\mathcal{H}_{\leq}$. The key idea is to split the set $\mathcal{T}$ in three parts: We choose $\delta,\epsilon>0$ and set
\begin{align*}
\mathcal{T}_1 &:= \left\{ (y,h)\in\mathcal{T} \mid h\geq\delta\textrm{ and } \min_{x\in [y-h,y+h]} \rho_b(x)b(x) < - \epsilon\right\}, \\
\mathcal{T}_2 &:_= \left\{ (y,h)\in\mathcal{T} \mid h <\delta\right\}, \textrm{ and }\\
\mathcal{T}_3 &:= \left\{ (y,h)\in\mathcal{T} \mid h\geq\delta\textrm{ and } \rho_b(x)b(x)\geq -\epsilon\textrm{ on } [y-h, y+h]\right\}.
\end{align*}
Note that all sets depend on $\delta$ and $\epsilon$. Then we have
\begin{align*}
\Pr(T_b(X)>r) &= \Pr\left( \sup_{(y,h)\in\mathcal{T}}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_1}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm}+\Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm}+\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right).
\end{align*}
Of course the inequality remains valid if we put $\lim_{\epsilon\searrow 0}\lim_{\delta\searrow 0}\lim_{T\to\infty}$ before both sides. The rationale behind the argument will be that the first probability converges to zero as the bias in $\tilde{\Psi}$ dominates the stochastic term, the second one vanishes by the multiscale lemma as in the proof of the weak convergence in Theorem \ref{weak_conv} and the last one smaller in stochastic order than $S$. Furthermore, we have seen in Theorem \ref{weak_conv} that both randoms variables $T_b(X)$ and $S$ are $\geq 0$ almost surely and it suffices to consider $r>0$(\textbf{for the first two sumands in $S$ this follows from Theorem \ref{weak_conv}, the third one is positive and bounded by a constant}).

\begin{itemize}
\item[(1)] We can bound $T_b(X)$ with the supremum taken over $\mathcal{T}_1$ by
\[ \sup_{(y,h)\in\mathcal{T}_1} \left( \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}  - C(\sigma_{y,h}^2)\right) + \sup_{(y,h)\in\mathcal{T}_1}\frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}}.\]
The limit in distribution of the first term is given in Theorem \ref{weak_conv} and we are going to show that the second term converges to $-\infty$ almost surely. Then we can conclude
\[ \lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_1}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) =0.\]
First of all we write with the occupation times formula
\[ \frac{\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s)b(X_s) ds}{\sqrt{\frac1T \int_0^T K_{y,h}(X_s)^2 ds}} = \sqrt{T}\frac{\int_\R K_{y,h}(z) b(z) \frac1T L_T^z dz}{\sqrt{\int_\R K_{y,h}(z)^2 \frac1T L_T^z dz}}.\]
We have almost sure convergence of the fraction against
\[ \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}} = \sqrt{h} \frac{\int_\R K(z) b(y+hz) \rho_b(y+hz)dz}{\sqrt{\int_\R K(z)^2 \rho_b(y+hz)dz}}\]
where equality follows from substitution. Keeping in mind that the expression is negative, upper-bounding it is the same as finding lower bounds of the absolute value. In particular, we may choose the denominator as large as possible by using the upper bound $L^*$ of the invariant density from Lemma \ref{bound_invariant_density} and choosing $h$ as small as possible. Thus we find
\[  \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}}\leq \sqrt{\delta} \left( \sqrt{L^*} \|K\|_{L^2}\right)^{-1} \int_\R K(z) b(y+hz) \rho_b(y+hz)dz.\]
From our condition on the set $\mathcal{T}_1$ we can find $z' \in [-1,1]$ such that $b(y+hz')\rho_b(y+hz')\leq -\epsilon$. As $b\rho_b$ is a continuous function on $[-A,A]$, it is uniformly continuous. Hence we find $\delta'>0$ (not depending on $y$ and $h$ which is the important part!) such that $b(y+hz)\rho_b(y+hz) <\frac{\epsilon}{2}$ for all $z$ that suffice $|y+hz' - y+hz| <\delta'$. This latter condition is equivalent to $|z-z'|\leq \frac{\delta'}{h}$. We get
\begin{align*}
\int_\R K(z) b(y+hz) \rho_b(y+hz)dz &\leq  - \frac{\epsilon}{2}\int_{B_{\frac{\delta'}{h}}(z')\cap [-1,1]} K(z) dz\\
&\leq  - \frac{\epsilon}{2}\int_{B_{\frac{\delta'}{\delta}}(z')\cap [-1,1]} K(z) dz.
\end{align*}
As $K$ is given by the triangular kernel that integral is minimized for $B_{\frac{\delta'}{\delta}}(z')\cap [-1,1] = [-1, -1+\frac{\delta'}{\delta}]$. As a triangle with both sides $\frac{\delta'}{\delta}$ its volume equals $\frac12 \left(\frac{\delta'}{\delta}\right)^2$ which finally gives
\[ \frac{\int_\R K_{y,h}(z) b(z)\rho_b(z) dz}{\sqrt{\int_\R K_{y,h}(z)^2 \rho_b(z) dz}}\leq -\sqrt{\delta} \left( \sqrt{L^*} \|K\|_{L^2}\right)^{-1}\frac{\epsilon}{4} \left(\frac{\delta'}{\delta}\right)^2\]
and consequently
\[\sqrt{T}\frac{\int_\R K_{y,h}(z) b(z) \frac1T L_T^z dz}{\sqrt{\int_\R K_{y,h}(z)^2 \frac1T L_T^z dz}} \rightarrow_{as} -\infty.\]
As the bound derived for the second factor does not depend on the location parameters $(y,h)$ we can put the supremum before the expression and are done with the first case.

\item[(2)] As the second summand in $\tilde{\Psi}$ is negative, we may disregard it whereby we make the probability of overshooting greater and get from Theorem \ref{weak_conv} that
\begin{align*}
&\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\hspace{0.5cm}\leq \lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^0(X) - C(\sigma_{y,h}^2) \right)>r \right) \\
&\hspace{0.5cm} = \Pr\left( \sup_{(y,h)\in\mathcal{T}_2} \left( \frac{\int_{-A}^A K_{y,h}(z) \sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C(\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) >r\right)
\end{align*}
Now $\|K_{y,h}\|_{L^2}^2 = h\|K\|_{L^2}^2$ and we have in the notation of Theorem \ref{weak_conv}
\[ \lim_{\delta\searrow 0}\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_2}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \leq \lim_{\delta\searrow 0}\lim_{T\to\infty}\Pr\left( S(0,\delta)>r\right) =0.\]

\item[(3)] For the last part we first drop the condition $h\geq \delta$ and get
\[ \mathcal{T}_3\subset \left\{ (y,h)\in\mathcal{T}\mid \rho_b(x)b(x)\geq -\epsilon\textrm{ on } [y-h,y+h]\right\} =: \mathcal{T}_3'\]
which particularly implies
\begin{align*}
\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\leq \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'}  \left(  \tilde{\Psi}_{y,h}^0(X) - C(\sigma_{y,h}^2) \right)>r \right),
\end{align*} 
where we again dropped the second summand of $\tilde{\Psi}$ in the second step as it is negative for $b\in\mathcal{H}_{\leq}$. By the weak limit in Theorem \ref{weak_conv}
\begin{align*}
&\lim_{T\to\infty} \Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right)\\
&\hspace{1cm} = \Pr\left( \sup_{(y,h)\in\mathcal{T}_3'} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) >r\right).
\end{align*}
Taking the limit $\lim_{\delta\searrow 0}$ doesn't change anything as neither side depends on $\delta$ and it remains to evaluate $\lim_{\epsilon\searrow 0}$.
If we write $\mathcal{T}_3'(\epsilon)=\mathcal{T}_3'$ we see that $\mathcal{T}_3'(\epsilon)\subset \mathcal{T}_3'(\epsilon')$ for $\epsilon\leq \epsilon'$ and 
\[ \lim_{\epsilon\searrow 0} \mathcal{T}_3'(\epsilon) = \left\{ (y,h)\in\mathcal{T}\mid \rho_b b=0 \textrm{ on } [y-h, y+h]\right\} =:\mathcal{T}_3''.\]
For each $(y,h)\in\mathcal{T}_3''$ we have that $\rho_b=c$ is constant on $[y-h,y+h]$ as $\rho_b'=\frac{2b\rho_b}{\sigma^2}$ and thus
\begin{align*}
&\lim_{\epsilon\searrow 0} \sup_{(y,h)\in\mathcal{T}_3'(\epsilon)} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right)\\
&\hspace{1cm} = \sup_{(y,h)\in\mathcal{T}_3''} \left(\frac{\int_{-A}^A K_{y,h}(z)dW_z}{\| K_{y,h}\|_{L^2}} - C\left( \|K_{y,h}c\|_{L^2}^2\right)\right)\\
&\hspace{1cm} \leq  \sup_{(y,h)\in\mathcal{T}_3''} \left(\frac{\int_{-A}^A K_{y,h}(z)dW_z}{\| K_{y,h}\|_{L^2}} - C\left( \|\tilde{c}K_{y,h}\|_{L^2}^2\right)\right)
\end{align*} 
with $\tilde{c} = 1\vee (L^*\wedge \frac{1}{2h})$. Here we used in the last step that $c\leq L^*$ is clear, as the invariant density is bounded by $L^*$. Furthermore, as it integrates to one, we have $2hc\leq 1\Leftrightarrow c\leq \frac{1}{2h}$. Finally, the reasoning is finished by noting that $C(\cdot)$ decreases with increasing argument. \\
For any $a>b>0$ we have $\sqrt{a-b}\geq \sqrt{a}-\sqrt{b}$ as
\[ (\sqrt{a}-\sqrt{b})^2 = a - 2\sqrt{ab}+b \leq a-2b+b = a-b.\]
By the definition of $C(\cdot)$ and the calculus rules of $\log$ we thus have
\begin{align*}
C\left( \|\tilde{c}K_{y,h}\|_{L^2}^2\right) &= \sqrt{2\log\left(\frac{1}{\tilde{c}K_{y,h}\|_{L^2}^2}\right)}\\
&= \sqrt{ 2\log\left( \frac{1}{\|K_{y,h}\|_{L^2}^2}\right) - 2\log(\tilde{c})} \\
&\geq  \sqrt{ 2\log\left( \frac{1}{\|K_{y,h}\|_{L^2}^2}\right)}  - \sqrt{2\log(\tilde{c})}\\
&= C(\|K_{y,h}\|_{L^2}^2) - C(\tilde{c}^{-1})
\end{align*}
Furthermore, we increase the random variable, by taking the supremum over a larger set, in this case $\mathcal{T}$ instead of $\mathcal{T}_3''$. This gives
\[\lim_{\epsilon\searrow 0} \sup_{(y,h)\in\mathcal{T}_3'(\epsilon)} \left(\frac{\int_{-A}^A K_{y,h}(z)\sqrt{\rho_b(z)} dW_z}{\| K_{y,h}\sqrt{\rho_b}\|_{L^2}} - C\left( \|K_{y,h}\sqrt{\rho_b}\|_{L^2}^2\right)\right) \leq S.\]
Altogether, we have
\[ \lim_{\epsilon\searrow 0}\lim_{\delta\searrow 0}\lim_{T\to\infty}\Pr\left( \sup_{(y,h)\in\mathcal{T}_3}  \left(  \tilde{\Psi}_{y,h}^b(X) - C(\sigma_{y,h}^2) \right)>r \right) \leq \Pr\left( S>r\right).\]
\end{itemize}
\end{proof}











==> Version_ArXiv/Sections/TrialsII.tex <==
\section{Trials......}



\begin{proof}[Proof of Continuity limit random variable]
We will show that the random variable
\[ S_b = \sup_{(y,h)\in\mathcal{T}}\left( \frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_b(z)} dW_z}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - C\left( \frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right)\right) \]
has not atom. Then in particular, both $U_1$ and $U_2$ have no atom and consequently, the same is true for their maximum, as for any $x\in\R$,
\[ \Pr\left( U_1\vee U_2 =x\right) \leq \Pr(U_1 =x) + \Pr(U_2=x) =0,\]
which finishes the claim.\\

First of all, $S_b$ has no positive atoms, which can be seen along the lines of the proof of Lemma~$2$ in \cite{Piterbarg} and we have to show that there is no atom in zero, i.e. $\Pr(S_b>0) =1$. 
By using $q_b\geq L_*$ from Lemma~\ref{uniform_lower_bound_invariant_density}, we find
\begin{align*}
C\left(\frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right) &= \sqrt{2\log\left(\frac{ \int_{-A}^A q_b(z) dz}{\int_{-A}^A K_{y,h}(z)^2 q_b(z) dz}\right)}\\
&\leq \sqrt{2\log\left(\frac{ \int_{-A}^A q_b(z)/L_* dz}{h \|K\|_{L^2}^2}\right)}
\end{align*}
and 
\[ S_b \geq \sup_{(y,h)\in\mathcal{T}}\left( \frac{\int_{-A}^A K_{y,h}(z)\sqrt{q_b(z)} dW_z}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - C\left( \frac{L}{h \|K\|_{L^2}^2}\right)\right) =:\tilde{S}_b,\]
with $L=1\vee \int_{-A}^A q_b(z)/L_* dz$. 
Now, we can write
\begin{align*}
X(y,h) := \int_{-A}^A \frac{K_{y,h}(z)\sqrt{q_b(z)}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}^2} dW_z = Y_1(y,h) + h^\frac14 Y_2(y,h) 
\end{align*}
with
\begin{align*}
Y_1(y,h) &:= \frac{1}{\sqrt{h}\|K\|_{L^2}} \int_{-A}^A K_{y,h}(z) dW_z, \\
Y_2(y,h) &:= h^{-\frac14} \int_{-A}^A \left( \frac{K_{y,h}(z)\sqrt{q_b(z)}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - \frac{K_{y,h}(z)}{\sqrt{h}\|K\|_{L^2}} \right) dW_z.
\end{align*}
By Lemma~$1$ in \cite{Piterbarg}
\[ \Pr\left( \sup_{ 0\leq y\leq A-h} Y_1(y,h) > \sqrt{2\log(L/h\|K\|_{L^2}^2)} \textrm{ i.o.  as } h\searrow 0 \right) =1.\]
We now apply Lemma~\ref{lemma_H3} to this and the process $Y=Y_2$, which is possible due to Lemma~\ref{lemma_H2}, and conclude
\begin{align*}
\Pr\left( \sup_{ 0\leq y\leq A-h} X(y,h) > \sqrt{2\log(L/h\|K\|_{L^2}^2)} \textrm{ i.o.  as } h\searrow 0 \right) =1.
\end{align*}
Following the lines of the proof of Theorem~$1$ in \cite{Piterbarg} we then see
\[ \Pr(S_b >0) \geq \Pr(\tilde{S}_b >0) =1\]
and we conclude that $S_b$ has no atom in zero. 
\end{proof}






\begin{lemma}\label{lemma_H3}
Let $X(u)$ depend on a parameter $u>0$ and suppose that for all $K\geq 1$ we have
\[ \Pr\left( X(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right)=1. \]
Let $Y(u)$ be a family depending on $u>0$ and $Y^*(u) := \sup_{u'\leq u}Y(u)\in\mathcal{O}_\Pr(1)$ for $u\searrow 0$. Then for all $K\geq 1$ and $\alpha>0$,
\[ \Pr\left( X(u) + u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right)=1. \]
\end{lemma}
\begin{proof}
Let $\epsilon>0$. Choose $u_0>0$ small enough and $L>0$ large enough such that for 
\[ A_\epsilon := \left\{ \sup_{u\leq u_0} |Y(u)| \leq L\right\} >1-\epsilon.\]
\begin{align*}
&\Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right) \\
&\hspace{0.2cm} \geq \Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0, A_\epsilon\right)  \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K/u)}+u^\alpha L \textrm{ i.o.  as } u\searrow 0, A_\epsilon\right)  \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K/u)}+ u^\alpha L \textrm{ i.o.  as } u\searrow 0\right) - \Pr\left( A_\epsilon^c\right),
\end{align*}
where the last step uses
\[ \Pr(A\cap B) = \Pr(A) - \Pr(A\cap B^c) \geq \Pr(A) - \Pr(B^c).\]
Now choose $c>1$ large enough such that
\[ \sqrt{2\log(cK/u)} \geq \sqrt{2\log(K/u)} + u^\alpha L \]
for $u<u_0$, which is possible since the condition is equivalent to
\[ 2\log(c) \geq 2u^\alpha L \sqrt{2\log(K/u)} + u^{2\alpha} L^2 \]
and the right hand side converges to zero for $u\searrow 0$. For this $K'=cK$, 
\begin{align*}
&\Pr\left( X(u) +u^\alpha Y(u) > \sqrt{2\log(K/u)} \textrm{ i.o.  as } u\searrow 0\right) \\
&\hspace{0.2cm} \geq \Pr\left( X(u) > \sqrt{2\log(K'/u)} \textrm{ i.o.  as } u\searrow 0\right) - \Pr\left( A_\epsilon^c\right).
\end{align*}
The first probability equals one by assumption and the claim follows by taking $\epsilon\searrow 0$.
\end{proof}





\begin{lemma}\label{lemma_H1}
Let $x\geq -1$. Then we have
\[ \left(1-\sqrt{1+x}\right)^2 \leq x^2.\]
\end{lemma}
\begin{proof}
We write
\begin{align}\label{eqp: H4}
\left( 1- \sqrt{1+x}\right)^2 -x^2 = \left( \sqrt{1+x}-1 + x\right)\left( \sqrt{1+x}-1 -x\right). 
\end{align} 
Now we distinguish cases: For $-1\leq x\leq 0$, we have 
\[ \sqrt{1+x}-1 + x \leq 0 \quad \textrm{ and }\quad \sqrt{1+x}-1-x\geq 0,\]
where the latter can be seen because it is equivalent to 
\[  \sqrt{1+x} \geq 1+x \Leftrightarrow 1+x \geq 1+2x+x^2 \Leftrightarrow 0\geq x+x^2,\]
which is true since $|x|\geq x^2$ for $|x|\leq 1$. Thus, the product on the right-hand side of \eqref{eqp: H4} is non-positive. For $x\geq 0$, we have
\[ \sqrt{1+x}-1 + x \geq 0 \quad \textrm{ and }\quad \sqrt{1+x}-1-x\leq 0,\]
where the last inequality follows from $\sqrt{1+x}\leq 1+x$ in this case. Again, the product in \eqref{eqp: H4} is non-positive.
\end{proof}






\begin{lemma}\label{lemma_H2}
Define 
\[ Y(y,h) := h^{-\frac14} \int_{-A}^A \frac{K_{y,h}(z)}{\sqrt{h}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h}\|K\|}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - 1\right) dW_z.\]
and based on this
\[ Y(h_0) := \sup_{h\leq h_0}\sup_{y\in [-A,A]} Y(y,h).\]
Then we have $Y(h_0) = \mathcal{O}_{\Pr}(1)$ for $h_0\searrow 0$.
\end{lemma}
\begin{proof}
First, $Y(y,h)$ is a continuous, zero-mean Gaussian process with corresponding covariance metric
\begin{align*}
d((y,h), (y',h'))^2&= \int_{-A}^A \left( \frac{K_{y,h}(z)}{h^{3/4}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h}\|K\|_{L^2}}{\|K_{y,h}\sqrt{q_b}\|_{L^2}} - 1\right) \right.\\
&\hspace{1.5cm}  \left. - \frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|_{L^2}} \left( \frac{\sqrt{q_b(z)} \sqrt{h'}\|K\|_{L^2}}{\|K_{y',h'}\sqrt{q_b}\|_{L^2}} - 1\right)\right)^2 dz.
\end{align*}
Let $L>0$, then
\begin{align}\label{eqp: H1}
\begin{split}
&\Pr\left( |Y(h_0)| > L \right) \leq \frac{1}{L} \E\left[ \sup_{h\leq h_0}\sup_{y\in [-A,A]} |Y(y,h)| \right] \\
&\hspace{1cm}\leq \frac{1}{L} \E\left[ |Y(y_1,h_1)|\right] + \frac{48}{L} \int_0^\infty \sqrt{\log(N(r, (0,h_0]\times [-A,A], d))} dr
\end{split}
\end{align}
by Markov's inequality in the first and Dudley's theorem (Theorem $11.17$ in~\cite{Talagrand}) in the second step and arbitrary $(y_1, h_1)\in [-A,A]\times (0,h_0]$. We turn to bounding the covering numbers. 

First, we choose $h_0$ small enough such that $4L^* h_0 <L_*/2$. We have, writing $\|\cdot\| := \|\cdot\|_{L^2}$ from here on,
\begin{align*}
\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|} &= \sqrt{\frac{(q_b(y) + q_b(z) - q_b(y)) h\|K\|^2}{\int_{-A}^A K_{y,h}(z)^2 q_b(y) dz + \int_{-A}^A K_{y,h}(z)^2 (q_b(z)-q_b(y)) dz}} \\
&= \sqrt{\frac{(q_b(y) + q_b(z) - q_b(y))h\|K\|^2}{q_b(y) h\|K\|^2 + \int_{-A}^A K_{y,h}(z)^2 (q_b(z)-q_b(y)) dz}}
\end{align*}
Using $|q_b(z) - q_b(y)|\leq L^*h$ for $|z-y|\leq h$, we give an upper and lower bound for the last expression. We start with the upper bound
\begin{align*}
\sqrt{\frac{q_b(y) h\|K\|^2 + L^* \|K\|^2 h^2}{q_b(y) h\|K\|^2 - L^* \|K\|^2 h^2}} &= \sqrt{\frac{q_b(y) + L^*h}{q_b(y) - L^*h}} \\
& = \sqrt{ 1+ \frac{q_b(y) + L^*h - q_b(y) +L^*h}{q_b(y) - L^* h}}\\
&\leq \sqrt{1+4L^*/L_* h},
\end{align*}
where we used in the last line that $q_b(y)-L^*h \geq L_*-L^*h \geq L_*/2$ by choice of $h\leq h_0$. Similiarly, we find the lower bound
\begin{align*}
\sqrt{\frac{q_b(y) h\|K\|^2-  L^* \|K\|^2 h^2}{q_b(y) h\|K\| + L^* \|K\|^2 h^2}} &= \sqrt{\frac{q_b(y) - L^*h}{q_b(y) + L^*h}} \\
& = \sqrt{ 1+ \frac{q_b(y) - L^*h - q_b(y) -L^*h}{q_b(y) + L^* h}}\\
&\leq \sqrt{1-4L^*/L_* h}.
\end{align*}
In consequence, we conclude by Lemma \ref{lemma_H1}
\begin{align}\label{eqp: H2}
\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|}  - 1\right)^2 \leq c_1 h^2,
\end{align}
with $c_1 := 16(L^*/L_*)^2$. Then we have
\begin{align}\label{eqp: H3}
d((y,h), (y',h'))^2\leq 4A \left( h^{-3/2} c_1h^2 + (h')^{-3/2} c_1(h')^2 \right) \leq 8Ac_1\sqrt{h_0}.
\end{align}
Note that this bound is uniform in $(y,h), (y',h')$ which means that for $h_0\searrow 0$ the covering number $N(r, (0,h_0]\times [-A,A], d)$  converges to one for each $r>0$.
To apply the dominated convergence theorem to the integral on the right-hand side of \eqref{eqp: H1}, we need to find an integrable majorant. Therefore, we take $h_0$ small enough such that $8Ac_1\sqrt{h_0}<\frac12$ and it suffices to consider $r<\frac12$ because the integrator in \eqref{eqp: H1} vanishes for $r\geq \frac12$ by \eqref{eqp: H3}. \\



Let $r<\frac12$ and denote by $\beta$ the Hölder order of the kernel, where $\beta=1$ if it is Lipschitz or smoother. We split the interval $(0,h_0]$ into $I_1, \dots, I_n$ intervals of length at most $cr^{16/\beta}$ and $[-A,A]$ into $J_1,\dots, J_m$ intervals of length at most $cr^{16/\beta}$, where $c>0$ will be specified later. We will show that their number
\[ \left( 1 + 2A\right) c^{-1} r^{-16/\beta} \]
is a bound for the covering numbers. For this aim, let $(y,h), (y',h')\in I_k\times J_l$ and we will show that $d((y,h),(y',h'))^2 <r^2$.\\

Let $c_2<\frac12(8Ac_1)^{-2}$. Note that we can assume $h\geq c_2r^{4}$ for the rest of the proof that bounds the covering numbers, which can be seen as follows: For $h<c_2r^4$ and $c<c_2$,
\[ h' \leq c_2 r^4 + cr^{16/\beta} \leq  2c_2 r^4,\]
as $|h-h'|<cr^{16/\beta}$ because $h,h'\in J_l$. Applying the bound in \eqref{eqp: H3}, it follows directly that in this case
\[ d((y,h),(y',h')) |\leq 8Ac_1\sqrt{2c_2 r^4} < 8Ac_1\sqrt{(XAc_1)^{-2}} r^2 <r^2. \]


Consequently, assume $h\geq c_2r^4$ in the following. First, we bound $d((y,h),(y',h'))$ by the triangle inequality and $(a+b)^2 \leq 2a^2 + 2b^2$ as
\[ d((y,h),(y',h'))^2 \leq 2d((y,h),(y',h))^2 + 2d((y',h),(y',h'))^2. \]
Using the definition of $d$ and $(a+b)^2\leq 2a^2 + 2b^2$, we find $d((y,h),(y',h))^2 \leq A_1 + A_2$ with
\begin{align*}
A_1 &:= 2\int_{-A}^A \left( \frac{K_{y,h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h}(z)}{h^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2 dz, \\
A_2 &:= 2\int_{-A}^A \frac{K_{y',h}(z)^2}{h^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y,h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
For $A_1$ we have with \eqref{eqp: H2} and \eqref{eqp: B11} for a constant $c_3$,
\begin{align*}
A_1 & \leq \frac{2c_1h^2}{h^{3/2}\|K\|^2} \int_{-A}^A \left( K_{y,h}(z) - K_{y',h}(z)\right)^2 q_b(z) dz \\
&\leq \frac{2c_1c_3}{\|K\|^2} \lambda([y-h,y+h]\bigtriangleup [y'-h,y'+h]) \\
&\leq 4c_1c_3 \|K\|^{-2} |y-y'| \\
&< C_1 cr^{16}.
\end{align*}
For $A_2$, we have
\begin{align*}
A_2 &= \frac{2}{\sqrt{h}}\left( \frac{1}{\|K_{y,h}\sqrt{q_b}\|} - \frac{1}{\|K_{y',h}\sqrt{q_b}\|}\right)^2 \int_{-A}^A K_{y',h}(z)^2 q_b(z) dz \\
&= \frac{2}{\sqrt{h}}\left( \frac{\|K_{y',h}\sqrt{q_b}\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2.
\end{align*}
The square of the quotient of the $L^2$-norms is given by
\begin{align*}
\frac{\|K_{y',h}\sqrt{q_b}\|^2}{\|K_{y,h}\sqrt{q_b}\|^2} &= 1+ \frac{\int_{y'-h}^{y'+h} K_{y',h}(z)^2 q_b(z) dz - \int_{y-h}^{y+h} K_{y,h}(z)^2 q_b(z) dz}{\|K_{y,h}\sqrt{q_b}\|^2} \\
&= 1+ \frac{h\int_{-1}^1 K(z)^2 \left( q_b(y'+zh) - q_b(y+zh)\right) dz}{\|K_{y,h}\sqrt{q_b}\|^2} ,
\end{align*}
where the absolute value of the second summand is bounded by
\begin{align*}
\frac{h \|K\|^2 L^* |y-y'|}{h\|K\|^2 L_*} = \frac{L^*|y-y'|}{L_*},
\end{align*}
as $|q_b(y+zh)-q_b(y'+zh)|\leq L^* |y-y'|$. By Lemma \ref{lemma_H1}
\begin{align*}
A_2 &\leq \frac{2}{\sqrt{h}}\left( \frac{\|K_{y',h}\sqrt{q_b}\|}{\|K_{y,h}\sqrt{q_b}\|} - 1\right)^2 \\
& \leq  \frac{2}{\sqrt{h}}\left(\frac{L^*}{L_*}\right)^2|y-y'|^2\\
& \leq 2(L^*/L_*)^2 |y-y'| \\
&< C_2c r^{16},
\end{align*} 
as $h^{-1}|y-y'| \leq c_2^{-1} r^{-2} c r^{16/\beta} <1$ for $c<c_2$. \\

We turn to $d((y',h),(y',h'))^2$ and bound $d((y',h),(y',h'))^2\leq B_1+B_2$ with
\begin{align*}
B_1 &:= 2\int_{-A}^A \left( \frac{K_{y',h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz \\
B_2 &:= 2\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h'} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
$B_1$ is bounded from above by $B_1\leq B_{1,1}+B_{1,2}$ with
\begin{align*}
B_{1,1} &:= 4\int_{-A}^A \left( \frac{K_{y',h}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{h^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz, \\
B_{1,2} &:= 4\int_{-A}^A \left( \frac{K_{y',h'}(z)}{h^{3/4}\|K\|}-\frac{K_{y',h'}(z)}{(h')^{3/4}\|K\|}\right)^2 \left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|} - 1\right)^2 dz.
\end{align*}
For $B_{1,1}$ we have as for $A_1$,
\begin{align*}
B_{1,1} &\leq \frac{4c_1 h^2}{h^{3/2}\|K\|^2}\int_{-A}^A \left( K_{y',h}(z) - K_{y',h'}(z)\right)^2 q_b(z) dz\\
& \leq \frac{4c_1c_3}{\|K\|^2} \lambda([y'-h,y'+h]\bigtriangleup [y'-h', y'+h']) \\
& \leq 6c_1c_3 \|K\|^{-2} |h-h'|\\
&\leq C_4 cr^{16}.
\end{align*} 
For $B_{1,2}$, a bound is given by
\begin{align*}
B_{1,2} &\leq \frac{4c_1 h^2}{\|K\|^2} \left( \frac{1}{h^{3/4}} - \frac{1}{(h')^{3/4}} \right)^2 \int_{-A}^A K_{y',h'}(z)^2 dz \\
&= 4c_1 h^2 h'\left( \frac{1}{h^{3/4}} - \frac{1}{(h')^{3/4}} \right)^2.
\end{align*}
By a Taylor expansion, we have
\[ h^{-\frac34} - (h')^{-\frac34} = -\frac34 \xi^{-\frac74} (h-h'),\]
where $\xi$ lies between $h$ and $h'$.
%in particular, it is bounded from below by 
%\[ \xi\geq h-cr^{16/\beta} \geq c_2r^4 -cr^{16/\beta}\geq c_2/2r^{4}$
%for $c<c_2$. 
Additionally, by the choice of $h\geq c_2r^4$ and $|h-h'|\leq cr^{16/\beta}$ we have $h/2\leq \xi, h'\leq 2h$. This yields
\begin{align*}
B_{1,2}&\leq 2c_1 h^2 h h^{-\frac{14}{4}} 2^{\frac{14}{4}} \left(\frac34\right)^2 |h-h'|^2 \\
&= 2^5 h^{-\frac12} |h-h'|^2\\
& \leq 2^5 |h-h'|\\
&\leq C_4 cr^{16},
\end{align*}
as $h^{-1}|h-h'| \leq c_2^{-1} r^{-2} c r^{16/\beta} <1$ for $c<c_2$.
For $B_2$, we bound $B_2\leq B_{2,1} + B_{2,2}$, where
\begin{align*}
B_{2,1} &:= 4\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz, \\
B_{2,2} &:= 4\int_{-A}^A \frac{K_{y',h'}(z)^2}{(h')^{3/2}\|K\|^2}\left( \frac{\sqrt{q_b(z)}\sqrt{h} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|}-\frac{\sqrt{q_b(z)}\sqrt{h'} \|K\|}{\|K_{y',h'}\sqrt{q_b}\|} \right)^2 dz.
\end{align*}
For $B_{2,1}$, we find the upper bound
\begin{align*}
&\frac{4h}{(h')^{3/2}}\left( \frac{1}{\|K_{y',h}\sqrt{q_b}\|} - \frac{1}{\|K_{y',h'}\sqrt{q_b}\|}\right)^2 \int_{-A}^A K_{y',h'}(z)^2 q_b(z) dz \\
&\hspace{1cm} = \frac{4h}{(h')^{3/2}}\left( \frac{\|K_{y',h'}\sqrt{q_b}\|}{\|K_{y',h}\sqrt{q_b}\|} -1\right)^2
\end{align*}
We bound the quotient of the $L^2$-norms
\begin{align*}
\frac{\|K_{y',h'}\sqrt{q_b}\|^2}{\|K_{y',h}\sqrt{q_b}\|^2} &= 1+ \frac{\int_{y'-h'}^{y'+h'} K_{y',h'}(z)^2 q_b(z) dz - \int_{y'-h}^{y'+h} K_{y',h}(z)^2 q_b(z) dz}{\|K_{y',h}\sqrt{q_b}\|^2} \\
&= 1+ \frac{1}{\|K_{y',h}\sqrt{q_b}\|^2}\int_{-A}^A \left( K_{y',h'}(z) - K_{y',h}(z)\right)\left( K_{y',h'}(z) + K_{y',h}(z)\right) q_b(z) dz\\
&\leq 1+ \frac{2L^*}{\|K_{y',h}\sqrt{q_b}\|^2} \int_{-A}^A \left| \frac{z-y'}{h'} - \frac{z-y'}{h}\right|^\beta dz \\
&\leq 1+ \frac{4L^*A^2}{\|K_{y',h}\sqrt{q_b}\|^2} \frac{|h-h'|^\beta}{(hh')^\beta}\\
&\leq 1+ \frac{4L^*A^2}{h L_*\|K\|^2} \frac{|h-h'|^\beta}{(hh')^\beta}
\end{align*}
Again by Lemma \ref{lemma_H1} and using $h,h'\geq \frac12c_2/ r^4$ because
\[ h' \geq h- cr^{16/\beta} \geq c_2r^4 - c r^{16/\beta} \geq  \frac12 c_2 r^4\]
for $c<c_2$, 
\begin{align*}
B_{2,1} &\leq \frac{64 A^4 (L^*)^2}{(L_*)^2 \|K\|^4 h^{2\beta+1} (h')^{3/2 + 2\beta}} |h-h'|^{2\beta}\\
&\leq \frac{64 A^4 (L^*)^2}{(L_*)^2 \|K\|^4}\left( \frac{2}{c_2}\right)^{\frac52 + 4\beta} r^{-10 - 16\beta} |h-h'|^{2\beta} \\
&\leq C_5 c^{2\beta} r^6,
\end{align*}
where we used $r^{-10-16\beta} |h-h'|^{2\beta} \leq c^{2\beta} r^{-26+32}$. For $B_{2,2}$, we have the bound
\begin{align*}
B_{2,2} &\leq \frac{4}{(h')^{3/2} \|K_{y',h'}\sqrt{q_b}\|^2} \left(\sqrt{h}-\sqrt{h'}\right)^2 \int_{-A}^A K_{y',h'}(z)^2 q_b(z) dz \\
& = \frac{4}{(h')^{3/2}} \left(\sqrt{h}-\sqrt{h'}\right)^2
\end{align*}
By a Taylor expansion, 
\[ \sqrt{h} - \sqrt{h'} = \frac{1}{2\sqrt{\xi}} |h-h'|\]
for $\xi$ between $h$ and $h'$ and by the same reasoning as for $B_{1,2}$, we get from this
\begin{align*}
B_{2,2} &\leq  (h')^{-\frac32} \xi^{-1} |h-h'|^2 \\
&\leq \left(\frac{2}{c_2}\right)^{\frac52} r^{-10} |h-h'|^2\\
&\leq C_6 c^2 r^{32}.
\end{align*}
Collecting all the bounds, we have
\[ d((y,h),(y',h')) \leq \left( C_1+C_2+C_3+C_4+C_5+C_6\right) c^{2\beta} r^6, \]
which is $<r^2$ for $c$ sufficiently small. In conclusion, we have the majorant $(1+2A)c^{-1}r^{-16/\beta}$ of the covering numbers on the  right-hand side of \eqref{eqp: H1}. Integrability follows as
\begin{align*}
&\int_0^\frac12 \sqrt{\log((1+2A)c^{-1}r^{-16/\beta})} dr \\
&\hspace{1cm} = \int_0^\frac12 \sqrt{\log((1+2A)c^{-1}) + 16/\beta\log(1/r)} dr\\
&\hspace{1cm} \leq \int_0^\frac12 \sqrt{\log((1+2A)c^{-1})} dr + \int_0^\frac12 \sqrt{16/\beta\log(1/r)} dr,
\end{align*}
where the first integral is clearly finite, and for the second one, we have by substituting $r=e^{-u}$, 
\begin{align*}
\int_0^\frac12 \sqrt{16/\beta \log(1/r)} dr &\leq \sqrt{16/\beta} \int_0^1 \sqrt{\log(1/r)} dr \\
&=  \sqrt{16/\beta} \int_0^\infty \sqrt{\log(e^u)} e^{-u} dr\\
&= \sqrt{16/\beta} \Gamma\left(\frac32\right) <\infty.
\end{align*} 
Thus, the integral on the right-hand side of \eqref{eqp: H1} converges to zero for $h_0\searrow 0$. In particular, we can choose $h_0$ small enough and afterwards $L$ large enough such that the right-hand side of \eqref{eqp: H1} is bounded by $\epsilon$ and the claim follows.
\end{proof}





==> Version_ArXiv/Sections/weak.tex <==
\section{Sketch of the proof of Theorem \ref{worst_case_delta}}\label{Sec_weak}


In Subsection \ref{SubSec_sketch} a route of proof for Theorem \ref{worst_case_delta} is given. It is built on a uniform weak convergence result for the supremum statistic $T_T^{b_0}(X)$ given in \eqref{eq: T_simple}. This crucial uniform weak convergence result is formulated in Theorem \ref{weak_conv}. A route of its proof is explained in Subsection \ref{SubSec_weak}, which strongly relies on the abstract Proposition~\ref{prop_unif_weak}.


\subsection{Sketch of proof of Theorem \ref{worst_case_delta}}\label{SubSec_sketch}

The idea of the proof is to upper bound 
\[ \limsup_{T\to\infty}\sup_{b\in H_0(b_0,\eta)}\Pr_b(T_T^\eta(X) \geq r)\] 
by decomposing the set $\mathcal{T}$ (over which the supremum $\sup_{(y,h)\in\mathcal{T}}$ in the definition \eqref{eq: T_eta} of $T_T^\eta(X)$ is taken) into three subsets $\mathcal{T}_1,\mathcal{T}_2(b)$ and $\mathcal{T}_3(b)$: 
\begin{itemize}
\item $\mathcal{T}_1$ consists of all $(y,h)\in\mathcal{T}$ with \textit{very small} $h$. Using the same techniques from empirical process theory as for the proof of Theorem \ref{Multiscale_Lemma}, we show that uniformly in $b$ the supremum over $\mathcal{T}_1$ is negligible as $T\rightarrow\infty$.
\item $\mathcal{T}_2(b)$ consists of those $(y,h)\in\mathcal{T}$ such that $b\in H_0(b_0,\eta)$ is \textit{bounded away from the boundary cases $b_0\pm\eta$} on $[y-h,y+h]$ while $h$ is \textit{not too small}. It is shown that the supremum in $T_T^\eta$ given in \eqref{eq: T_eta}, restricted to those $(y,h)$, converges to $-\infty$ uniformly in $b$ as $T\rightarrow\infty$. Hence, the supremum in \eqref{eq: T_eta} is not attained asymptotically at $(y,h)\in\mathcal{T}_2(b)$.
\item $\mathcal{T}_3(b)$ contains those $(y,h)\in\mathcal{T}$ for which $b\in H_0(b_0,\eta)$ is \textit{close to some boundary case $b_0\pm\eta$} on $[y-h,y+h]$ while $h$ is \textit{not too small}. Uniformly over $b$, the probability that the supremum over $\mathcal{T}_3(b)$ exceeds a given $r$ is proven to be upper bounded by $\Pr( U_1\vee U_2+ 4\sqrt{A\eta/\sigma^2}\geq r)$ in the limit $T\rightarrow\infty$. 
\end{itemize}
The last item is the most involved part of the proof and is explained in what follows. First, it is crucial to determine $\limsup_{T\to\infty} $ of
\begin{align}\label{eqp: 8.2}
\sup_{b\in H_0(b_0,\eta)} \Pr_b\left( \sup_{(y,h)\in\mathcal{T}_3(b)} \left(  \left| \frac{\frac{1}{\sqrt{T}}\int_0^T K_{y,h}(X_s) dW_s}{\hat\sigma_T(y,h)}\right| -C\left(\frac{\hat\sigma_T(y,h)^2}{\hat\sigma_{T,\max}^2}\right)\right) \geq r\right). 
\end{align}  
This is severely challenging for two reasons: 
\begin{itemize}
\item First, the random variable is defined as a supremum over normalized stochastic integrals, whose distribution depends via the process $X$ on the parameter $b$, while $X$ itself is stochastically dependent on $W$.
\item Secondly, we need to establish the result uniformly over $b$ belonging to $H_0(b_0,\eta)$, which is mathematically substantially more involved as compared to other weak limit results of supremum statistics.
\end{itemize}
The probability in \eqref{eqp: 8.2} corresponds to the overshooting probability of an upper bound on the test statistic $T_T^\eta$ obtained by applying the triangle inequality to \eqref{eq: 8.1}. Note that the expression within the probability now has the same distribution as $T_T^b(X)$ given in \eqref{eq: T_simple} under $\Pr_b$.
Thus, we have to investigate the weak limit of $T_T^b(X)$ \textit{uniformly} over $H_0(b_0,\eta)$ which substantially increases the technical effort. This uniformity strongly relies on $b\in\Sigma(C,A,\gamma,\sigma)$, but does not use $\|b-b_0\|_{[-A,A]}\leq\eta$ and hence it is derived on the whole class $\Sigma(C,A,\gamma,\sigma)\supset H_0(b_0,\eta)$. This yields the following Theorem \ref{weak_conv}. Its proof is deferred to Appendix \ref{App_weak}, while a route is presented in Subsection \ref{SubSec_weak} below.


\begin{thm}\label{weak_conv}
Define the random variable
\[ Z_b(y,h) := \int_{-A}^A K_{y,h}(z) \sqrt{q_b(z)} dW_z \]
with a Brownian motion $W$ on $[-A,A]$, 
\[ \sigma_b(y,h):=\| K_{y,h} \sqrt{q_b}\|_{L^2} \quad \textrm{ and }\quad \sigma_{b,\max} :=\|\1_{[-A,A]}\sqrt{q_b}\|_{L^2}, \] 
and based on those
\[ S_b :=  \sup_{(y,h)\in\mathcal{T}} \left( \frac{\left|Z_b(y,h)\right|}{\sigma_b(y,h)}  - C\left(\frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right)\right). \]
Then the following uniform weak convergence holds true:
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} d_{BL}^b\left( T_T^b(X),S_b \right)\stackrel{T\to \infty}{\longrightarrow} 0.\]
\end{thm}
Here, $d_{BL}$ denotes the dual bounded Lipschitz metric which metrizes weak convergence and is given in Appendix \ref{SubSec_C1}. The superscript $b$ in $d_{BL}^b$ indicates the dependence of the distribution of $X$ on $b$.\\

To continue with \eqref{eqp: 8.2}, note that it is almost immediate from our proof that Theorem \ref{weak_conv} remains true for $\mathcal{T}$ replaced by $\mathcal{T}_3(b)$. This allows to conclude that for any $\delta>0$, $\limsup_{T\to\infty}$ of \eqref{eqp: 8.2} is bounded from above by
\begin{align}\label{eqp: 8.3}
\sup_{b\in H_0(b_0,\eta)} \Pr\left( \sup_{(y,h)\in\mathcal{T}_3(b)} \left(  \frac{|Z_b(y,h)|}{\sigma_b(y,h)}-C\bigg(\frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\bigg)\right) \geq r-\delta\right),
\end{align} 
see Step (3) in Appendix \ref{App_least}. The remaining problem is the dependence of the random variable within the probability in \eqref{eqp: 8.3} on $b$. It is finally shown that $U_1\vee U_2 + 4\sqrt{A\eta/\sigma^2}$ stochastically dominates the random variables appearing in \eqref{eqp: 8.3} as a suppressed (in this sketch of proof) hyperparameter that specifies \textit{closeness} of $b$ to $b_0\pm\eta$ in the definition of $\mathcal{T}_3(b)$ is tending to zero. At this point, the restriction to $\mathcal{T}_3(b)$ is crucial.


%Replacing $b$ by $b_0\pm\eta$ within the additive correction $C(\cdot)$ entails a difference of at most $4\sqrt{A\eta/\sigma^2}$, because on the null, $\|b-b_0\|_{[-A,A]}\leq \eta$, see Remark \ref{remark_correction}. Thereafter, the particular construction of $\mathcal{T}_3(b)$ comes into play. It entails that $|Z_b(y,h)|/\sigma_b(y,h)$ can be approximated by either $|Z_{b_0+\eta}(y,h)|/\sigma_{b_0+\eta}(y,h)$ or $|Z_{b_0-\eta}(y,h)|/\sigma_{b_0-\eta}(y,h)$ up to an approximation error that is controlled uniformly over $b$. Indeed, this approximation error is driven by a hyperparameter $\epsilon>0$ that specifies \textit{closeness} of $b$ to $b_0\pm\eta$ in the definition of $\mathcal{T}_3(b)=\mathcal{T}_3(b,\epsilon)$: $\sup_{(y,h)\in\mathcal{T}_3(b,\epsilon)} \||b-b_0|-\eta\|_{[y-h,y+h]} \to 0$ as $\epsilon\searrow 0$.  %In both cases, we loose dependence on $b$. The last dependence on $b$ within the probability in \eqref{eqp: 8.3} appears in $\mathcal{T}_3(b,\epsilon)$.
%Upper bounding finally the supremum over $\mathcal{T}_3(b,\epsilon)$ by the supremum over all of $\mathcal{T}$, the resulting random variable is independent of $b$. Letting first $\epsilon\searrow 0$ and then $\delta\searrow 0$, we conclude that \eqref{eqp: 8.3} is bounded from above by
%\[ \Pr\left( S_1\vee S_2 + 4\sqrt{A\eta/\sigma^2} \geq r\right). \]



%\textcolor{blue}{
%\begin{remark}\label{remark_correction}
%One may wonder why the term $4\sqrt{A\eta/\sigma^2}$ occurs in the formulation of Theorem \ref{worst_case_delta}. It accounts for the fact that $q_{b_0}$ and $q_{b_0\pm\eta}$ have different behaviour on the interval $[-A,A]$ and comes up when switching from $C(\textrm{Ratio}_{b_0})$ to $C(\textrm{Ratio}_{b_0\pm\eta})$. This difference can be controlled by some constant (even for all $b\in H_0(b_0,\eta)$ as their deviation from $b_0$ is at maximum $\eta$) that ultimately leeds to the correction $4\sqrt{A\eta/\sigma^2}$.
%\end{remark}
%}




\begin{remark}
In order to find bounds for an expression of the form \eqref{eqp: 8.2}, typical techniques are Gaussian approximations for suprema as in \cite{CCK} or the Hungarian construction that was first described in \cite{KKT}. However, for an application of the results in \cite{CCK}, we miss the structure of a classical empirical process, and to the best of our knowledge, there is no Gaussian coupling result available for $(\int_0^T K_{y,h}(X_s) dW_s)_{(y,h)\in\mathcal{T}}$.
\end{remark}







\subsection{Route of the proof of Theorem \ref{weak_conv}}\label{SubSec_weak}

The proof of Theorem \ref{weak_conv} is a delicate combination of sophisticated empirical process theory, stochastic analysis und the theory of weak convergence. Subsequently, we use the notation $\mathcal{T}_\delta :=\{(y,h)\in\mathcal{T}\mid h\geq \delta\}$ and
\[Z_T(y,h) := \frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s. \]
%and
%\[ Z_b(y,h) := \int_\R K_{y,h}(z) \sqrt{q_b(z)} dW_z.\]
Slightly simplified, the proof is split into the following three steps which will be explained right after:
\begin{enumerate}
\item[(i)] First, we prove that for any $\delta>0$, the processes $(Z_T(y,h))_{(y,h)\in\mathcal{T}_\delta}$ converge in distribution to $(Z_b(y,h))_{(y,h)\in\mathcal{T}_\delta}$, uniformly in $b$, i.e.
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} d_{BL}^b \left( (Z_T(y,h))_{(y,h)\in\mathcal{T}_\delta}, (Z_b(y,h))_{(y,h)\in\mathcal{T}_\delta}\right) \stackrel{T\to\infty}{\longrightarrow} 0.\]
\item[(ii)] Next, we establish for any $\delta>0$
\[ \sup_{b\in\Sigma(C,A,\gamma,\sigma)} d_{BL}^b\left( T_T(\delta,1), S_b(\delta,1)\right) \stackrel{T\to\infty}{\longrightarrow} 0 \]
for  
\begin{align*}
T_T(\delta, 1) := \sup_{(y,h)\in\mathcal{T}_\delta} \left(\frac{\left|\frac{1}{\sqrt{T}} \int_0^T K_{y,h}(X_s) dW_s\right|}{\hat\sigma_T(y,h)} - C\left( \frac{\hat\sigma_T(y,h)^2}{\hat\sigma_{T,\max}^2}\right) \right), 
\end{align*} 
where the definition of $\hat\sigma_T, \hat\sigma_{T,\max}$ can be found in Theorem \ref{Multiscale_Lemma}, and
\[ S_b(\delta, 1) := \sup_{(y,h)\in\mathcal{T}_\delta} \left(\frac{\left|\int_\R K_{y,h}(z) \sqrt{\rho_b(z)} dW_z\right|}{\sigma_b(y,h) } - C\left( \frac{\sigma_b(y,h)^2}{\sigma_{b,\max}^2}\right) \right).\]
\item[(iii)] Finally, we conclude with the extension to 
\[\sup_{b\in\Sigma(C,A,\gamma,\sigma)} d_{BL}^b\left( T_T(0,1), S_b(0,1)\right)\stackrel{T\to\infty}{\longrightarrow} 0.\]
Note that $S_b(0,1)=S_b$ and $T_T(0,1) = T_T^b(X)$ under $\Pr_b$.
\end{enumerate}




On a conceptual level, the proof of the step (i) is based on the following result that is of independent interest. Our proof of this result is given in Appendix \ref{SubSec_C1}. For any metric space $E$, $\mathcal{F}_{BL}(E)$ denotes the closed unit ball of bounded Lipschitz functions on $E$, see Appendix~\ref{SubSec_C1}. For any pseudometric space $(\mathcal{S},\rho)$ and any $u>0$, we write $N(u,\mathcal{S},\rho)$ for the covering number with closed balls at radius $u$, see its definition \eqref{eq: covering_number}. $l_\infty(\mathcal{S})$ denotes all functions $f:\mathcal{S}\rightarrow\R$ with $\|f\|_\mathcal{S} <\infty$.


\begin{proposition}\label{prop_unif_weak}
Let $\left(X_n(s)\right)_{s\in\mathcal{S}}$ and $\left(Y_n(s)\right)_{s\in\mathcal{S}}$ be two stochastic processes with values in $l_\infty(\mathcal{S})$, where $\mathcal{S}$ is equipped with a metric $\rho_\theta$ that depends on some parameter $\theta\in\Theta$. Suppose the following three conditions hold:
\begin{enumerate}
\item[(a)] For any integer $k>0$ we have
\[ \sup_{\substack{B\subset\mathcal{S}: \# B\leq k}}\ \sup_{\theta\in\Theta} \sup_{f\in\mathcal{F}_{BL}(\R^{\# B})} \hspace{-0.05cm}\big| \E_\theta\big[ f\big((X_{n}(s))_{s\in B}\big)\big] -\E_\theta\big[ f\big((Y_{n}(s))_{s\in B}\big)\big]\big| \hspace{-0.05cm}\to 0 \]
in the limit $n\to\infty$. Here, $\#B$ denotes the cardinality of $B$.
\item[(b)] For each $\epsilon>0$ we have for $Z_n = X_n, Y_n$,
\[ \lim_{\delta\searrow 0} \limsup_{n\to\infty} \sup_{\theta\in\Theta} \Pr_\theta\left( \sup_{\rho_\theta(s,s')\leq\delta} |Z_n(s) - Z_n(s')| >\epsilon \right) =0.\]
\item[(c)] For all $u>0$ we have $\sup_{\theta\in\Theta}N(u, \mathcal{S},\rho_\theta) <\infty$.
\end{enumerate} \pagebreak
Then we have
\[ \sup_{\theta\in\Theta} \sup_{f\in\mathcal{F}_{BL}(l_\infty(\mathcal{S}))} \left| \E_\theta\left[ f(X_n)\right] - \E_\theta\left[f(Y_n)\right]\right| \stackrel{n\to\infty}{\longrightarrow}\ 0.\]
\end{proposition}





For step (ii), we first show that the random denominators $\hat\sigma_T(y,h)$ for $(y,h)\in\mathcal{T}_\delta$ in $\tilde T_T(\delta,1)$ can be replaced by their deterministic limiting counterparts $\sigma_b(y,h)$, see Lemma \ref{lemma_weak_2}.
In order to continue with continuous mapping type arguments, we are facing the problem that 
\begin{align}\label{eq: map_l_infty}
(x(y,h))_{(y,h)\in\mathcal{T}} \mapsto \sup_{(y,h)\in\mathcal{T}} \left|\frac{x(y,h)}{\sigma_b(y,h)} - C\big(\sigma_b(y,h)^2/\sigma_{b,\max}^2\big)\right| 
\end{align} 
is not continuous on $l_\infty(\mathcal{T})$. This is the point where the restriction to $\mathcal{T}_\delta$ is necessary. Moreover, the uniformity over $b$ from step (i) is only transferred by the continuous mapping theorem if the latter is applied to a Lipschitz continuous function, see Lemma \ref{uniform_continuous_mapping}. Lemma \ref{sup_mapping_Lipschitz} establishes Lipschitz continuity of the mapping \eqref{eq: map_l_infty} restricted to $l_\infty(\mathcal{T}_\delta)$.

Step (iii) relies on results about empirical process theory that were developed in derivation of Theorem \ref{Multiscale_Lemma}.











